Should we necessarily treat masses as localized when analysing tests of quantum gravity?

Recently proposed ``table-top tests of quantum gravity'' involve creating, separating and recombining superpositions of masses at non-relativistic speeds. The general expectation is that these generate superpositions of gravitational fields via the Newtonian potential. Analyses suggest that negligible gravitational radiation is generated if the interference experiments involve sufficiently small accelerations. One way of thinking about this is that matter and the static gravitational field are temporarily entangled and then disentangled. Another is that the static gravitational field degrees of freedom are dependent on the matter and do not belong to a separate Hilbert space, and that there is always negligible entanglement between matter and dynamical gravitational degrees of freedom. In this last picture, localized masses effectively become infinitely extended objects, inseparable from their Newtonian potentials. While this picture seems hard to extend to a fully relativistic theory of non-quantum gravity, it has significant implications for analyses of how or whether BMV and other non-relativistic experiments might test the quantum nature of gravity. If the masses in a BMV experiment are regarded as occupying overlapping regions (or indeed all of space), explaining how they become entangled does not require that their gravitational interaction involves quantum information exchange. On this view, while the experiments test gravity in a regime where quantum theory describes all relevant matter degrees of freedom, they do not necessarily test its quantum nature. It might be argued that no plausible explanation other than quantum gravity could be consistent both with these experiments and with relativity. But this relies on further theoretical assumptions and is weaker than claiming direct evidence for quantum gravitational interactions from the experiments alone.

==> spare <==
%REFERENCES FROM PHD THESIS
%INTRO CHAPTER
@ARTICLE{S48,
   author       = "C. E. Shannon",
title = "A mathematical theory of communication",
   journal      = "The Bell System Technical Journal",
   volume       = "27(3-4)", 
   pages        = "379-423,623-656",
   year         = "1948",
url = "http://www3.alcatel-lucent.com/bstj/vol27-1948/bstj-vol27-issue03.html",
url2 = "http://www3.alcatel-lucent.com/bstj/vol27-1948/bstj-vol27-issue04.html",
}

@ARTICLE{T37,
   author       = "A. M. Turing",
title = "On computable numbers, with an application to the {E}ntscheidungsproblem",
   journal      = "Proceedings of the London Mathematical Society ",
   volume       = "s2-42(1)", 
   pages        = "230-265",
   year         = "1937",
url = "http://plms.oxfordjournals.org/content/s2-42/1/230.full.pdf+html"
}

@Book{vonNeumannbook,
 author    = "John {von Neumann}",
 title     = "Mathematical Foundations of Quantum Mechanics",
 publisher = "Princeton University Press",
address= "Princeton, New Jersey",
 year      =  1955,
}


@Book{Rovellibook,
 author    = "Carlo Rovelli",
 title     = "Quantum Gravity",
 publisher = "Cambridge University Press",
address= "Cambridge, UK",
 year      =  2004,
}

@Book{GreenSchwarzWittenbook,
 author    = "M. Green and J. Schwarz and E. Witten",
 title     = "Superstring Theory",
 publisher = "Cambridge University Press",
address= "Cambridge, UK",
 year      =  1987,
}



Green, M., Schwarz, J., and Witten, E. (1987). Superstring Theory. Cambridge University Press, Cambridge, UK.

@ARTICLE{SSW17,
   author       = "P. Senellart and G. Solomon and A. White",
title = "High{-}performance semiconductor quantum{-}dot single{-}photon sources",
   journal      = "Nature Nanotech.",
   volume       = "12", 
   pages        = "1026-1039",
   year         = "2017",
doi = "10.1038/nnano.2017.218"
}

@Book{Michlerbook,
 author    = "P. Michler",
 title     = "Single semiconductor quantum dots",
 publisher = "NanoScience and Technology, Springer Berlin",
 year      =  2009,
}

@Book{Bohmbook,
 author    = "D. Bohm",
 title     = "Quantum Theory",
 publisher = "Prentice-Hall",
address= "New York",
 year      =  1951,
}

@Book{Bohmbook2,
 author    = "D. Bohm",
 title     = "The Special Theory of Relativity",
 publisher = "W. A. Benjamin",
address= "New York",
 year      =  1965,
}

@Book{theprincipleofrelativitybook,
 author    = "W. Perrett and G. B. Jeffery,",
 title     = "The Principle of Relativity",
 publisher = "General Publishing Company",
address= "Toronto, Canada",
 year      =  1923,
}

@Book{Weizsackerbook,
 author    = "C. F. {von Weizs\"{a}cker}",
 title     = "The Structure of Physics",
 publisher = "Springer",
address= "Dordrecht",
 year      =  2006,
}

@ARTICLE{E05,
   author       = "Albert Einstein",
title = "Zur Elektrodynamik bewegter K{\"{o}}rper",
   journal      = "Annalen der Physik",
   volume       = "17", 
   pages        = "891",
   year         = "1905",
note = "On the Electrodynamics of Moving Bodies. English translation in W. Perrett and G. B. Jeffery, (ed.), \emph{The Principle of Relativity} (General Publishing Company, Toronto, Canada, 1923)",
}



@ARTICLE{B80,
   author       = "P. Benioff",
title = "The Computer as a physical system: A microscopic quantum mechanical {H}amiltonian model of computers as represented by {T}uring machines",
   journal      = "Journal of Statistical Physics",
   volume       = "22(5)", 
   pages        = "563-591",
   year         = "1980",
url = "http://link.springer.com/article/10.1007/BF01011339"
}

@ARTICLE{B82,
   author       = "P. Benioff",
title = "Quantum mechanical {H}amiltonian models of {T}uring machines",
   journal      = "Journal of Statistical Physics",
   volume       = "29(3)", 
   pages        = "515-546",
   year         = "1982",
url = "http://link.springer.com/article/10.1007/BF01342185"
}

@ARTICLE{B82.1,
   author       = "P. Benioff",
title = "Quantum mechanical models of {T}uring machines that dissipate no energy",
   journal      = "Physical Review Letters",
   volume       = "48(23)", 
   pages        = "1581-1585",
   year         = "1982",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.48.1581"
}

@ARTICLE{F82,
   author       = "R. P. Feynman",
title = "Simulating physics with computers",
   journal      = "International Journal of Theoretical Physics",
   volume       = "21(6-7)", 
   pages        = "467-488",
   year         = "1982",
url = "http://link.springer.com/article/10.1007/BF02650179"
}

@INPROCEEDINGS{BBBW82,
   author       = "C. H. Bennett and G. Brassard and S. Breidbart and S. Wiesner",
title = "Quantum cryptography, or unforgeable subway tokens",
   booktitle      = "Advances in cryptology: Proceedings of CRYPTO 82",
   pages       = "267--275", 
 publisher       = "Plenum Press",
address= "New York",
   year         = "1983",
url = ""
}

@ARTICLE{D85,
   author       = "D. Deutsch",
title = "Quantum theory, the {C}hurch-{T}uring principle and the universal quantum computer",
   journal      = "Proceedings of the Royal Society of London A",
   volume       = "400(1818)", 
   pages        = "97-117",
   year         = "1985",
url = "http://rspa.royalsocietypublishing.org/content/400/1818/97.abstract"
}

@ARTICLE{F86,
   author       = "R. P. Feynman",
title = "Quantum mechanical computers",
   journal      = "Foundations of Physics",
   volume       = "16(6)", 
   pages        = "507-531",
   year         = "1986",
Note = "Originally appeared in {\emph{Optics News}}, February 1985",
url = "http://link.springer.com/article/10.1007/BF01886518"
}

@article{J97,
  title={Entanglement and quantum computation},
  author={Jozsa, R},
  journal={Geometric Issues in the Foundations of Science},
note={Preprint arXiv quant-ph/9707034},
url={https://arxiv.org/abs/quant-ph/9707034},
  year={1997},
  publisher={Oxford University Press}
}

@ARTICLE{E91,
   author       = "A. K. Ekert",
title = "Quantum cryptography based on {B}ell's theorem",
   journal      = "Phys. Rev. Lett.",
   volume       = "67", 
   pages        = "661-663",
   year         = "1991",
url = "http://prl.aps.org/abstract/PRL/v67/i6/p661_1"
}

@ARTICLE{DJ92,
   author       = "D. Deutsch and R. Jozsa",
title = "Rapid solution of problems by quantum computation",
   journal      = "Proc. R. Soc. London A",
   volume       = "439", 
   issue = "1907", 
   pages        = "553-558",
   year         = "1992",
url = "http://rspa.royalsocietypublishing.org/content/439/1907/553#related-urls"
}

@INPROCEEDINGS{S94,
   author       = "P. W. Shor",
title = "Algorithms for quantum computation: Discrete logarithms and factoring",
   booktitle      = "Proceedings of the 35th Annual Symposium on Foundations of Computer Science",
   pages       = "124--134", 
 publisher       = "IEEE Computer Society Press",
address= "Los Alamitos, California",
   year         = "1994",
doi = "10.1109/SFCS.1994.365700 ",
}








@ARTICLE{S95,
   author       = "B. Schumacher",
title = "Quantum coding",
   journal      = "Physical Review A",
   volume       = "51(4)", 
   pages        = "2738-2747",
   year         = "1995",
url = "http://pra.aps.org/abstract/PRA/v51/i4/p2738_1"
}

@ARTICLE{BH96,
   author       = "V. Bu\v{z}ek and M. Hillery",
title = "Quantum copying: Beyond the no-cloning theorem",
   journal      = "Physical Review A",
   volume       = "54(3)", 
   pages        = "1844-1852",
   year         = "1996",
url = "http://link.aps.org/doi/10.1103/PhysRevA.54.1844"
}

@ARTICLE{BDEFMS98,
   author       = "D. Bru\ss and D. P. DiVincenzo and A. Ekert and C. A. Fuchs and C. Macchiavello and J. A. Smolin",
title = "Optimal universal and state-dependent quantum cloning",
   journal      = "Physical Review A",
   volume       = "57(4)", 
   pages        = "2368-2378 ",
   year         = "1998",
url = "http://link.aps.org/doi/10.1103/PhysRevA.57.2368"
}

@ARTICLE{GM97,
   author       = "N. Gisin and S. Massar",
title = "Optimal quantum cloning machines",
   journal      = "Physical Review Letters",
   volume       = "79(11)", 
   pages        = "2153-2156",
   year         = "1997",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.79.2153"
}

@ARTICLE{W98,
   author       = "R. F. Werner",
title = "Optimal cloning of pure states",
   journal      = "Physical Review A",
   volume       = "58(3)", 
   pages        = "1827-1832",
   year         = "1998",
url = "http://link.aps.org/doi/10.1103/PhysRevA.58.1827"
}

@ARTICLE{KW99,
   author       = "M. Keyl and R. F. Werner",
title = "Optimal cloning of pure states, testing single clones",
   journal      = "Journal of Mathematical Physics",
   volume       = "40(7)", 
   pages        = "3283",
   year         = "1999",
url = "http://dx.doi.org/10.1063/1.532887"
}

@ARTICLE{SIGA05,
   author       = "V. Scarani and S. Iblisdir and N. Gisin and A. Ac\'in",
title = "Quantum cloning",
   journal      = "Review of Modern Physics",
   volume       = "77(4)", 
   pages        = "1225-1256",
   year         = "2005",
url = "http://link.aps.org/doi/10.1103/RevModPhys.77.1225"
}

@article{W06,
  title = {Tsirelson bounds for generalized {C}lauser-{H}orne-{S}himony-{H}olt inequalities},
  author = {S. Wehner},
  journal = {Physical Review A},
  volume = {73(2)},
  issue = {2},
  pages = {022110},
  numpages = {5},
  year = {2006},
  doi = {10.1103/PhysRevA.73.022110},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.73.022110},
  publisher = {American Physical Society}
}


@ARTICLE{BC90,
   author       = "S. L. Braunstein and C. M. Caves",
title="Wringing out better {B}ell inequalities",
   journal      = "Annals of Physics",
   volume       = "202(1)",
   pages        = "22--56",
   year         = "1990",
url = "http://www.sciencedirect.com/science/article/pii/000349169090339P"
}

@article{AGR81,
  title = {Experimental Tests of Realistic Local Theories via {B}ell's Theorem},
  author = {A. Aspect and P. Grangier and G. Roger},
  journal = {Phys. Rev. Lett.},
  volume = {47},
  issue = {7},
  pages = {460--463},
  year = {1981},
  doi = {10.1103/PhysRevLett.47.460},
  publisher = {American Physical Society}
}

@article{AGR82,
  title = {Experimental Realization of {E}instein-{P}odolsky-{R}osen-{B}ohm         \textit{Gedankenexperiment}      : {A} New Violation of {B}ell's Inequalities},
  author = {A. Aspect and P. Grangier and G. Roger},
  journal = {Phys. Rev. Lett.},
  volume = {49},
  issue = {2},
  pages = {91--94},
  year = {1982},
  doi = {10.1103/PhysRevLett.49.91},
  publisher = {American Physical Society}
}

@article{ADR82,
  title = {Experimental Test of {B}ell's Inequalities Using Time- Varying Analyzers},
  author = {A. Aspect and J. Dalibard and G. Roger},
  journal = {Phys. Rev. Lett.},
  volume = {49},
  pages = {1804--1807},
  year = {1982},
  doi = {10.1103/PhysRevLett.49.1804},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.49.1804},
  publisher = {American Physical Society}
}

@article{WJSWZ98,
  title = {Violation of {B}ell's Inequality under Strict {E}instein Locality Conditions},
  author = {G. Weihs and T. Jennewein and C. Simon and H. Weinfurter and A. Zeilinger},
  journal = {Phys. Rev. Lett.},
  volume = {81},
  issue = {23},
  pages = {5039--5043},
  year = {1998},
  doi = {10.1103/PhysRevLett.81.5039},
  publisher = {American Physical Society}
}

@article{B81,
title={Bertlmann's socks and the nature of reality},
author={J. S. Bell},
journal={Journal de Physique},
volume={42(3)},
pages={C2 41-61},
year={1981},
note= {Reprinted in \cite{Bellbook}, pages 139--158}
}

@article{TBZG98,
  title = {Violation of {B}ell Inequalities by Photons More Than 10 km Apart},
  author = {W. Tittel and J. Brendel and H. Zbinden and N. Gisin},
  journal = {Physical Review Letters},
  volume = {81(17)},
  issue = {17},
  pages = {3563--3566},
  year = {1998},
  doi = {10.1103/PhysRevLett.81.3563},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.81.3563},
  publisher = {American Physical Society}
}

@article{GZ99,
title={Bell inequality and the locality loophole: {A}ctive versus passive switches},
author={N. Gisin and H. Zbinden},
journal = {Physics Letters A},
Volume={264(2-3)},
pages={103--107},
year={1999},
doi={10.1016/S0375-9601(99)00807-5},
url={http://dx.doi.org/10.1016/S0375-9601(99)00807-5},
}

@article{Sa95,
title={Constraints for the violation of the {B}ell inequality in {E}instein-{P}odolsky-{R}osen-{B}ohm experiments},
author={E. Santos},
journal = {Physics Letters A},
Volume={200(1)},
pages={1--6},
year={1995},
doi={10.1016/0375-9601(95)00097-M},
url={http://dx.doi.org/10.1016/0375-9601(95)00097-M},
}


@article{GM87,
  title = {Detector inefficiencies in the {E}instein-{P}odolsky-{R}osen experiment},
  author = {A. Garg and N. D. Mermin},
  journal = {Physical Review D},
  volume = {35(12)},
  issue = {12},
  pages = {3831--3835},
  year = {1987},
  doi = {10.1103/PhysRevD.35.3831},
  url = {http://link.aps.org/doi/10.1103/PhysRevD.35.3831},
  publisher = {American Physical Society}
}

@article{Eb93,
  title = {Background level and counter efficiencies required for a loophole-free {E}instein-{P}odolsky-{R}osen experiment},
  author = {P. H. Eberhard},
  journal = {Physical Review A},
  volume = {47(2)},
  issue = {2},
  pages = {R747--R750},
  year = {1993},
  doi = {10.1103/PhysRevA.47.R747},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.47.R747},
  publisher = {American Physical Society}
}

@article{SBHGZ08,
  title = {Spacelike Separation in a {B}ell Test Assuming Gravitationally Induced Collapses},
  author = {D. Salart and A. Baas and  J. A. W. van Houwelingen and N. Gisin and H. Zbinden},
  journal = {Phys. Rev. Lett.},
  volume = {100},
  issue = {22},
  pages = {220404},
  numpages = {4},
  year = {2008},
  doi = {10.1103/PhysRevLett.100.220404},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.100.220404},
  publisher = {American Physical Society}
}

@INPROCEEDINGS{Bell71,
   author       = "J. S. Bell",
title = "Introduction to the hidden-variable question",
   booktitle      = "Foundations of Quantum Mechanics. Proceedings of the International School of Physics `Enrico Fermi', course IL",
   pages       = "171--181", 
 publisher       = "Academic",
address= "New York",
   year         = "1971",
Note="Reprinted in \cite{Bellbook}, pages 29--39",
url = ""
}

@book{Bellbook,
   author       = "J. S. Bell",
title = "Speakable and unspeakable in quantum mechanics",
   year         = "1987",
publisher = "Cambridge University Press",
address="Cambridge",
}

@unpublished{Kentnotes,
author="A. Kent",
title="Quantum Foundations",
note="Lecture notes for part III course of the Mathematical Tripos, University of Cambridge",
year="2011",
}

@article{K13,
author = "A. Kent",
title = "A no-summoning theorem in relativistic quantum theory",
journal="Quantum Information Processing",
volume="12(2)",
pages="1023--1032",
url="http://link.springer.com/article/10.1007%2Fs11128-012-0431-6",
year = "2013",
note = "E-print arXiv:1101.4612",
}

@article{K11.2,
author = "A. Kent",
title = "Unconditionally secure bit commitment with flying qudits ",
journal="New Journal of Physics",
volume="13",
pages="113015",
url="http://iopscience.iop.org/1367-2630/13/11/113015",
year = "2011",
}

@article{K11.3,
  title = {Location-oblivious data transfer with flying entangled qudits},
  author = {A. Kent},
  journal = {Physical Review A},
  volume = {84(1)},
  issue = {1},
  pages = {012328},
  numpages = {4},
  year = {2011},
  doi = {10.1103/PhysRevA.84.012328},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.84.012328},
  publisher = {American Physical Society}
}

@article{GMRWKBLCGNUZ13,
  title = {Bell violation using entangled photons without the fair-sampling assumption},
  author = {M. Giustina and A. Mech and S. Ramelow and B. Wittmann and J. Kofler and J. Beyer and A. Lita and B. Calkins and T. Gerrits and S. W. Nam and R. Ursin and A. Zeilinger},
  journal = {Nature},
  volume = {497},
  pages = {227--230},
  year = {2013},
  doi = {10.1038/nature12012 },
  url = {http://www.nature.com/nature/journal/v497/n7448/full/nature12012.html},
}

@unpublished{CMACGLMSZNBLGK13,
  title = {Detection-loophole-free test of quantum nonlocality, and applications},
  author = {B. G. Christensen and  K. T. McCusker and J. B. Altepeter and B. Calkins and T. Gerrits and A. E. Lita and A. Miller and L.
K. Shalm and Y. Zhang and S. W. Nam and N. Brunner and C. C. W. Lim and N. Gisin and P. G. Kwiat},
Note = "E-print arXiv:1306.5772",
year="2013",
eprint = "1306.5772",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1306.5772;%%",
url= "http://arxiv.org/abs/1306.5772",
}

@article{FC72,
  title = {Experimental Test of Local Hidden-Variable Theories},
  author = {S. J. Freedman and J. F. Clauser},
  journal = {Phys. Rev. Lett.},
  volume = {28},
  issue = {14},
  pages = {938--941},
  year = {1972},
  doi = {10.1103/PhysRevLett.28.938},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.28.938},
  publisher = {American Physical Society}
}

@unpublished{K13.2,
  title = {Quantum nonlocal correlations are not dominated},
  author = {A. Kent},
year="2013",
eprint = "1308.5009",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1308.5009;%%",
}







%LHV CHAPTER

@article{bukh,
  title={Measurable sets with excluded distances},
  author={B. Bukh},
  journal={Geometric and Functional Analysis},
  volume={18},
  number={3},
  pages={668--697},
  year={2008},
  publisher={Springer},
url={http://link.springer.com/article/10.1007/s00039-008-0673-8}
}

@article{de2008fourier,
  title={Fourier analysis, linear programming, and densities of distance
avoiding sets in $\mathbb{R}^n$},
  author={F. M. de Oliveira Filho and F. Vallentin},
  journal={Journal of the European Mathematical Society},
  volume={12(6)},
  pages={1417--1428},
  year={2010},
url={http://www.ems-ph.org/journals/show_abstract.php?issn=1435-9855&vol=12&iss=6&rank=5}
}

@article{AMRSV13,
author= "N. Aharon and S. Machnes and B. Reznik and J. Silman and L. Vaidman",
title= "Continuous input nonlocal games",
journal = "Natural Computing",
volume = "12(1)",
pages = "5--8",
year = "2013",
url = "http://link.springer.com/article/10.1007%2Fs11047-012-9354-5"
}

@article{W89,
  title = {Quantum states with {E}instein-{P}odolsky-{R}osen correlations admitting a hidden-variable model},
  author = {R. F. Werner},
  journal = {Phys. Rev. A},
  volume = {40},
  issue = {8},
  pages = {4277--4281},
  year = {1989},
  doi = {10.1103/PhysRevA.40.4277},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.40.4277},
  publisher = {American Physical Society}
}

@Unpublished{KPG13,
author = "A. Kent and D. Pital\'ua-Garc\'ia",
title = "Sphere colourings and {B}ell inequalities",
Note = "E-print arXiv:1307.6839",
year = "2013",
eprint = "1307.6839",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1307.6839;%%",
url = "http://arxiv.org/abs/1307.6839",
}

@misc{computerprogram,
author = "A. Kent and D. Pital\'ua-Garc\'ia",
title = "Sphere colourings and {B}ell inequalities: {S}upplemental material",
year= "2013",
note = "Computer program coded in Mathematica, which will be available as supplemental material in \cite{KPG13}",
}




%QIC CHAPTER


@ARTICLE{QIC,
   author       = "D. Pital\'ua{-}Garc\'ia",
title = "Quantum information causality",
   journal      = "Phys. Rev. Lett.",
   volume       = "110", 
   pages        = "210402",
   year         = "2013",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.110.210402"
}

@Book{NielsenandChuangbook,
 author    = "M. A. Nielsen and I. L. Chuang",
 title     = "Quantum Computation and Quantum Information",
 publisher = "Cambridge University Press",
address= "Cambridge, UK",
 year      =  2000,
}

@ARTICLE{WZ82,
   author       = "W. K. Wootters and W. H. Zurek",
 title = "A single quantum cannot be cloned",
   journal      = "Nature (London)",
   volume       = "299", 
   pages        = "802-803",
   year         = "1982",
url = "http://www.nature.com/nature/journal/v299/n5886/abs/299802a0.html"
}

@ARTICLE{D82,
   author       = "D. Dieks",
title = "Communication by {EPR} devices",
   journal      = "Physics Letters A",
   volume       = "92(6)", 
   pages        = "271-272",
   year         = "1982",
url = "http://dx.doi.org/10.1016/0375-9601(82)90084-6"
}

@ARTICLE{teleportation,
   author       = "C. H. Bennett and G. Brassard and C. Cr\'epeau and R. Jozsa and A. Peres and W. K. Wootters",
 title = "Teleporting an unknown quantum state via dual classical and {E}instein-{P}odolsky-{R}osen channels",
   journal      = "Phys. Rev. Lett.",
   volume       = "70", 
   pages        = "1895-1899",
   year         = "1993",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.70.1895"
}

@ARTICLE{sdc,
   author       = "C. H. Bennett  and S. J. Wiesner",
title = "Communication via one- and two-particle operators on {E}instein-{P}odolsky-{R}osen states",
   journal      = "Phys. Rev. Lett.",
   volume       = "69", 
   pages        = "2881-2884",
   year         = "1992",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.69.2881"
}

@INPROCEEDINGS{BB84,
   author       = "C. H. Bennett and G. Brassard",
title = "Quantum cryptography: {P}ublic key distribution and coin tossing",
booktitle      = "Proceedings of IEEE International Conference on Computers, Systems, and Signal Processing, Bangalore, India",
   pages        = "175--179",
   publisher       = "IEEE",
address= "New York",
   year         = "1984",
}


@ARTICLE{BHK05,
   author       = "J. Barrett and L. Hardy and A. Kent",
title = "No signaling and quantum key distribution",
   journal      = "Physical Review Letters",
   volume       = "95(1)", 
   pages        = "010503",
   year         = "2005",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.95.010503"
}

@ARTICLE{EPR35,
   author       = "A. Einstein and B. Podolsky and N. Rosen",
title = "Can quantum-mechanical description of physical reality be considered complete?",
   journal      = "Physical Review",
   volume       = "47(10)", 
   pages        = "777-780",
   year         = "1935",
url = "http://link.aps.org/doi/10.1103/PhysRev.47.777"
}

@ARTICLE{Bell,
   author       = "J. S. Bell",
title = "On the {E}instein-{P}odolsky-{R}osen paradox",
   journal      = "Physics",
   volume       = "1", 
   pages        = "195-200",
   year         = "1964",
note="Reprinted in \cite{Bellbook}, pages 14--21",
url = "",
}

@incollection{GRW85,
  title={A model for a unified quantum description of macroscopic and microscopic systems},
  author={Ghirardi, Gian Carlo and Rimini, Alberto and Weber, Tullio},
  booktitle={Quantum Probability and Applications II},
  pages={223--232},
  year={1985},
  publisher={Springer}
}

@article{GRW86,
  title = {Unified dynamics for microscopic and macroscopic systems},
  author = {Ghirardi, G. C. and Rimini, A. and Weber, T.},
  journal = {Phys. Rev. D},
  volume = {34},
  issue = {2},
  pages = {470--491},
  numpages = {0},
  year = {1986},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.34.470},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.34.470}
}

@article{G89,
  title={Stochastic quantum dynamics and relativity},
  author={Gisin, Nicolas},
  journal={Helv. Phys. Acta},
  volume={62},
  number={4},
  pages={363--371},
  year={1989}
}

@article{D88,
	doi = {10.1088/0305-4470/21/13/013},
	url = {https://doi.org/10.1088/0305-4470/21/13/013},
	year = 1988,
	month = {jul},
	publisher = {{IOP} Publishing},
	volume = {21},
	number = {13},
	pages = {2885--2898},
	author = {L Diosi},
	title = {Quantum stochastic processes as models for state vector reduction},
	journal = {J. Phys. A: Math. Gen.},
	abstract = {An elementary introduction of quantum-state-valued Markovian stochastic processes (QSP) for N-state quantum systems is given. It is pointed out that a so-called master constraint must be fulfilled. For a given master equation a continuous and, as a new alternative possibility, a discontinuous QSP are derived. Both are discussed as possible models for state reduction during measurement.}
}

@article{GPR90,
  title = {{M}arkov processes in {H}ilbert space and continuous spontaneous localization of systems of identical particles},
  author = {Ghirardi, Gian Carlo and Pearle, Philip and Rimini, Alberto},
  journal = {Phys. Rev. A},
  volume = {42},
  issue = {1},
  pages = {78--89},
  numpages = {0},
  year = {1990},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.42.78},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.42.78}
}


@article{G84,
  title = {Quantum Measurements and Stochastic Processes},
  author = {Gisin, N.},
  journal = {Phys. Rev. Lett.},
  volume = {52},
  issue = {19},
  pages = {1657--1660},
  numpages = {0},
  year = {1984},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.52.1657},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.52.1657}
}

 
@article{P76,
  title = {Reduction of the state vector by a nonlinear {S}chr\"odinger equation},
  author = {Pearle, Philip},
  journal = {Phys. Rev. D},
  volume = {13},
  issue = {4},
  pages = {857--868},
  numpages = {0},
  year = {1976},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.13.857},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.13.857}
}


@ARTICLE{GRW80,
   author       = "G. C. Ghirardi and A. Rimini and T. Weber",
title = "A general argument against superluminal transmission through the quantum mechanical measurement process",
   journal      = "Lettere al Nuovo Cimento",
   volume       = "27(10)", 
   pages        = "293-298",
   year         = "1980",
url = "http://www.springerlink.com/content/t5h287h1r26j25j4/"
}

@ARTICLE{K73,
   author       = "A. S. Kholevo",
   title = "Bounds for the quantity of information transmitted by a quantum communication channel",
   journal      = "Problems of Information Transmission",
   volume       = "9", 
   pages        = "177-183",
   year         = "1973",
note= "Translated from \emph{Problemy Peredachi Informatsii}, 9(3):3--11,1973.",
}

@ARTICLE{ic,
   author       = {M. Paw{\l}owski and T. Paterek and D. Kaszlikowski and V. Scarani and A. Winter and M. {\.{Z}}ukowski},
title = {Information causality as a physical principle.},
   journal      = {Nature (London)},
   volume       = {461}, 
   pages        = {1101-1104},
   year         = {2009},
url = {http://www.nature.com/nature/journal/v461/n7267/full/nature08400.html},
doi={10.1038/nature08400}
}


@ARTICLE{ABPS09,
   author       = "J. Allcock and N. Brunner and M. Paw{\l}owski and V. Scarani",
title = "Recovering part of the boundary between quantum and nonquantum correlations from information causality",
   journal      = "Physical Review A",
   volume       = "80(4)", 
   pages        = "040103(R)",
   year         = "2009",
url = "http://link.aps.org/doi/10.1103/PhysRevA.80.040103" 
}

@ARTICLE{CSS10,
   author       = "D. Cavalcanti and A. Salles and V. Scarani",
title = "Macroscopically local correlations can violate information causality",
   journal      = "Nature Communications",
   volume       = "1", 
   pages        = "136",
   year         = "2010",
url = "http://www.nature.com/ncomms/journal/v1/n9/full/ncomms1138.html"
}

@ARTICLE{GWAN11,
   author       = "R. Gallego and L. E. W{\"{u}}rflinger and A. Ac\'in and M. Navascu\'es",
title = "Quantum correlations require multipartite information principles",
   journal      = "Physical Review Letters",
   volume       = "107(21)", 
   pages        = "210403",
   year         = "2011",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.107.210403"
}

@ARTICLE{YCATS12,
   author       = "T. H. Yang and D. Cavalcanti and M. L. Almeida and C. Teo and V. Scarani",
title = "Information-causality and extremal tripartite correlations",
   journal      = "New Journal of Physics",
   volume       = "14", 
   pages        = "013061",
   year         = "2012",
url = "http://iopscience.iop.org/1367-2630/14/1/013061"
}

@ARTICLE{C80,
   author       = "B. S. Cirel'son",
title = "Quantum generalizations of {B}ell's inequality",
   journal      = "Lett. Math. Phys.",
   volume       = "4", 
   pages        = "93-100",
   year         = "1980",
   doi = "10.1007/BF00417500",
url = "https://doi.org/10.1007/BF00417500",
}



@article{GMCD10,
  title = {All Reversible Dynamics in Maximally Nonlocal Theories are Trivial},
  author = {Gross, David and M\"uller, Markus and Colbeck, Roger and Dahlsten, Oscar C. O.},
  journal = {Phys. Rev. Lett.},
  volume = {104},
  issue = {8},
  pages = {080402},
  numpages = {4},
  year = {2010},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.104.080402},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.104.080402}
}


@article{AS14,
	doi = {10.1088/1751-8113/47/32/325303},
	url = {https://doi.org/10.1088/1751-8113/47/32/325303},
	year = 2014,
	month = {jul},
	publisher = {{IOP} Publishing},
	volume = {47},
	number = {32},
	pages = {325303},
	author = {Sabri W Al-Safi and Anthony J Short},
	title = {Reversible dynamics in strongly non-local Boxworld systems},
	journal = {J. Phys. A: Math. Theor.},
	abstract = {In order to better understand the structure of quantum theory, or speculate about theories that may supersede it, it can be helpful to consider alternative physical theories. ‘Boxworld’ describes one such theory, in which all non-signaling correlations are achievable. In a limited class of multipartite Boxworld systems—wherein all subsystems are identical and all measurements have the same number of outcomes—it has been demonstrated that the set of reversible dynamics is ‘trivial’, generated solely by local relabellings of measurement choices and outcomes, and permutations of subsystems. We develop the convex formalism of Boxworld to give an alternative proof of this result, then extend this proof to all multipartite Boxworld systems, and discuss the potential relevance to other theories. These results lend further support to the idea that the rich reversible dynamics in quantum theory may be the key to understanding its structure and its informational capabilities.}
}

@ARTICLE{LR68,
   author       = "O. E. Lanford and D. W. Robinson",
title = "Mean entropy of states in quantum-statistical mechanics",
   journal      = "Journal of Mathematical Physics",
   volume       = "9(7)", 
   pages        = "1120-1125",
   year         = "1968",
url = "http://jmp.aip.org/resource/1/jmapaq/v9/i7/p1120_s1"
}

@ARTICLE{AL70,
   author       = "H. Araki and E. H. Lieb",
title = "Entropy inequalities",
   journal      = "Communications in Mathematical Physics",
   volume       = "18(2)", 
   pages        = "160-170",
   year         = "1970",
url = "http://www.springerlink.com/content/wk224145h1441527/"
}

@Unpublished{H01,
author = "L. Hardy",
title = "Quantum theory from five reasonable axioms",
year = "2001",
eprint = "quant-ph/0101012",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=quant-ph/0101012;%%",
}

@Unpublished{vD05,
author = "W. van Dam",
title = "Implausible Consequences of Superstrong Nonlocality",
year = "2005",
eprint = "quant-ph/0501159",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=quant-ph/0101012;%%",
}

@ARTICLE{B07,
   author       = "J. Barrett",
title = "Information processing in generalized probabilistic theories",
   journal      = "Phys. Rev. A",
   volume       = "75",
issue = "3",
   pages        = "032304",
   year         = "2007",
url = "http://link.aps.org/doi/10.1103/PhysRevA.75.032304"
}

@ARTICLE{BBLW07,
   author       = "H. Barnum and J. Barrett and M. Leifer and A. Wilce",
title = "Generalized no-broadcasting theorem",
   journal      = "Phys. Rev. Lett.",
   volume       = "99", 
issue="24",
   pages        = "240501",
   year         = "2007",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.99.240501"
}

@ARTICLE{SW10,
   author       = "A. J. Short and S. Wehner",
title = "Entropy in general physical theories",
   journal      = "New J. Phys.",
   volume       = "12", 
   pages        = "033023",
   year         = "2010",
url = "http://iopscience.iop.org/1367-2630/12/3/033023"
}

@ARTICLE{BBCLSSWW10,
   author       = "H. Barnum and J. Barrett and L. O. Clark and M. Leifer and R. Spekkens and N. Stepanik and A. Wilce and R. Wilke",
title = "Entropy and information causality in general probabilistic theories",
   journal      = "New J. Phys.",
   volume       = "12", 
   pages        = "033024",
   year         = "2010",
url = "http://iopscience.iop.org/1367-2630/12/3/033024"
}

@ARTICLE{AS11,
   author       = "S. W. Al-Safi and A. J. Short",
title = "Information causality from an entropic and a probabilistic perspective",
   journal      = "Physical Review A",
   volume       = "84(4)", 
   pages        = "042323",
   year         = "2011",
   url = "http://link.aps.org/doi/10.1103/PhysRevA.84.042323"
}

@Unpublished{MMAP12,
author = "L. Masanes and M. P. Mueller and R. Augusiak and D. Perez-Garcia",
title = "A digital approach to quantum theory",
year = "2012",
Note = "E-print arXiv:1208.0493",
eprint = "1208.0493",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1208.0493;%%",
url = "http://arxiv.org/abs/1208.0493",
}

@ARTICLE{W83,
   author       = "S. Wiesner",
title = "Conjugate coding",
   journal      = "SIGACT News",
   volume       = "15", 
   pages        = "78-88",
   year         = "1983",
url = "http://dl.acm.org/citation.cfm?doid=1008908.1008920"
}

@ARTICLE{ANTV02,
   author       = "A. Ambainis and A. Nayak and A. Ta-Shma and U. Vazirani",
title = "Dense quantum coding and quantum finite automata",
   journal      = "Journal of the ACM",
   volume       = "49(4)", 
   pages        = "496-511",
   year         = "2002",
url = "http://dl.acm.org/citation.cfm?doid=581771.581773"
}

@ARTICLE{PZ10,
   author       = "M. Paw{\l}owski and M. {\.{Z}}ukowski",
title = "Entanglement-assisted random access codes",
   journal      = "Physical Review A",
   volume       = "81(4)", 
   pages        = "042326",
   year         = "2010",
url = "http://link.aps.org/doi/10.1103/PhysRevA.81.042326"
}

@ARTICLE{T87,
   author       = "B. S. Tsirel'son",
   title = "Quantum analogues of the {B}ell inequalities. {T}he case of two spatially separated domains.",
   journal      = "J. Sov. Math.",
   volume       = "36", 
   pages        = "557-570",
   year         = "1987",
doi="10.1007/BF01663472"
}

@ARTICLE{DLR12,
   author       = "O. C. O. Dahlsten and D. Lercher and R. Renner",
title = "Tsirelson's bound from a generalized data processing inequality",
   journal      = "New Journal of Physics",
   volume       = "14", 
   pages        = "063024",
   year         = "2012",
url = "http://iopscience.iop.org/1367-2630/14/6/063024/"
}

@ARTICLE{HV01,
   author       = "L. Henderson and V. Vedral",
title = "Classical, quantum and total correlations",
   journal      = "Journal of Physics A: Mathematical and General",
   volume       = "34(35)", 
   pages        = "6899",
   year         = "2001",
url = "http://iopscience.iop.org/0305-4470/34/35/315/"
}

@ARTICLE{OZ01,
   author       = "H. Ollivier and W. H. Zurek",
title = "Quantum discord: A measure of the quantumness of correlations",
   journal      = "Physical Review Letters",
   volume       = "88(1)", 
   pages        = "017901",
   year         = "2001",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.88.017901"
}

@ARTICLE{GPW05,
   author       = "B. Groisman and S. Popescu and A. Winter",
title = "Quantum, classical, and total amount of correlations in a quantum state",
   journal      = "Physical Review A",
   volume       = "72(3)", 
   pages        = "032317",
   year         = "2005",
url = "http://link.aps.org/doi/10.1103/PhysRevA.72.032317"
}

@Unpublished{ALMO09,
author = "A. Ambainis and D. Leung and L. Mancinska and M. Ozols",
title = "Quantum random access codes with shared randomness",
note = "E-print arXiv:0810.2937",
eprint = "0810.2937",
archivePrefix = "arXiv",
year = "2009",
SLACcitation = "%%CITATION=arXiv:0810.2937;%%",
url = "http://arxiv.org/abs/0810.2937",
}

@Unpublished{PS11,
author = "M. Paw{\l}owski and V. Scarani",
title = "Information Causality",
note = "E-print arXiv:1112.1142",
eprint = "1112.1142",
archivePrefix = "arXiv",
year = "2011",
SLACcitation = "%%CITATION=arXiv:1112.1142;%%",
url = "http://arxiv.org/abs/1112.1142",
}

@ARTICLE{CHSH69,
   author       = "J. F. Clauser and M. A. Horne and A. Shimony and R. A. Holt",
title = "Proposed experiment to test local hidden-variable theories",
   journal      = "Phys. Rev. Lett.",
   volume       = "23", 
   pages        = "880-884",
   year         = "1969",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.23.880"
}

@article{CH74,
  title = {Experimental consequences of objective local theories},
  author = {J. F. Clauser and M. A. Horne},
  journal = {Physical Review D},
  volume = {10(2)},
  issue = {2},
  pages = {526--535},
  year = {1974},
  doi = {10.1103/PhysRevD.10.526},
  url = {http://link.aps.org/doi/10.1103/PhysRevD.10.526},
  publisher = {American Physical Society}
}

@article{D87,
author={L. Di\'{o}si},
title={A universal master equation for the gravitational violation of quantum mechanics},
journal={Phys. Lett. A},
volume={120},
pages={377--381},
year={1987},
doi={10.1016/0375-9601(87)90681-5}
}

@article{D89,
  title = {Models for universal reduction of macroscopic quantum fluctuations},
  author = {L. Di\'osi},
  journal = {Phys. Rev. A},
  volume = {40},
  issue = {3},
  pages = {1165--1174},
  year = {1989},
  doi = {10.1103/PhysRevA.40.1165},
  publisher = {American Physical Society}
}

@article{P14,
  title={On the gravitization of quantum mechanics 1: Quantum state reduction},
  author={Penrose, Roger},
  journal={Found. Phys.},
  volume={44},
  number={5},
  pages={557--575},
  year={2014},
doi={10.1007/s10701-013-9770-0},
  publisher={Springer}
}

@article{P96,
author={R. Penrose},
title={On Gravity's role in Quantum State Reduction},
journal={Gen. Relat. Gravit.},
volume={28},
pages={581--600},
year={1996},
doi={10.1007/BF02105068},
}

@article{HPF19,
	doi = {10.1088/1367-2630/ab104a},
	year = 2019,
	month = {apr},
	publisher = {{IOP} Publishing},
	volume = {21},
	number = {4},
	pages = {043047},
	author = {Richard Howl and Roger Penrose and Ivette Fuentes},
	title = {Exploring the unification of quantum theory and general relativity with a {B}ose{\textendash}{E}instein condensate},
	journal = {New J. Phys.},
	abstract = {Despite almost a century’s worth of study, it is still unclear how general relativity (GR) and quantum theory (QT) should be unified into a consistent theory. The conventional approach is to retain the foundational principles of QT, such as the superposition principle, and modify GR. This is referred to as ‘quantizing gravity’, resulting in a theory of ‘quantum gravity’. The opposite approach is ‘gravitizing QT’ where we attempt to keep the principles of GR, such as the equivalence principle, and consider how this leads to modifications of QT. What we are most lacking in understanding which route to take, if either, is experimental guidance. Here we consider using a Bose–Einstein condensate (BEC) to search for clues. In particular, we study how a single BEC in a superposition of two locations could test a gravitizing QT proposal where wavefunction collapse emerges from a unified theory as an objective process, resolving the measurement problem of QT. Such a modification to QT due to general relativistic principles is testable near the Planck mass scale, which is much closer to experiments than the Planck length scale where quantum, general relativistic effects are traditionally anticipated in quantum gravity theories. Furthermore, experimental tests of this proposal should be simpler to perform than recently suggested experiments that would test the quantizing gravity approach in the Newtonian gravity limit by searching for entanglement between two massive systems that are both in a superposition of two locations.}
}


@incollection{K09,
author={A. Kent},
title={A Proposed Test of the Local Causality of Spacetime},
booktitle={Quantum Reality, Relativistic Causality, and Closing the Epistemic Circle: Essays in Honour of Abner Shimony},
Publisher={Springer},
pages={369--378},
year={2009},
note="E-print arXiv:gr-qc/0507045",
url={http://arxiv.org/abs/gr-qc/0507045},
}

@article{MBCPV12,
  title = {The classical-quantum boundary for correlations: {D}iscord and related measures},
  author = {K. Modi, and A. Brodutch, and H. Cable, and T. Paterek, and V. Vedral},
  journal = {Reviews of Modern Physics},
  volume = {84(4)},
  issue = {4},
  pages = {1655--1707},
  year = {2012},
  doi = {10.1103/RevModPhys.84.1655},
  url = {http://link.aps.org/doi/10.1103/RevModPhys.84.1655},
  publisher = {American Physical Society}
}


















K. Modi, A. Brodutch, H. Cable, T. Paterek, and ::: and V. Vedral, Rev. Mod. Phys. 84, 1655 (2012).





%PBT CHAPTER







@ARTICLE{BH96,
   author       = "V. Bu{\v{z}}ek and M. Hillery",
title = "Quantum copying: Beyonf the no-cloning theorem",
   journal      = "Physical Review A",
   volume       = "54(3)", 
   pages        = "1844-1852",
   year         = "1996",
url = "http://link.aps.org/doi/10.1103/PhysRevA.54.1844"
}

@ARTICLE{IH08,
   author       = "S. Ishizaka and T. Hiroshima",
title = "Asymptotic teleportation scheme as a universal programmable quantum processor",
   journal      = "Physical Review Letters",
   volume       = "101(24)", 
   pages        = "240501",
   year         = "2008",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.101.240501"
}

@ARTICLE{IH09,
   author       = "S. Ishizaka and T. Hiroshima",
title = "Quantum teleportation scheme by selecting one of multiple output ports",
   journal      = "Physical Review A",
   volume       = "79(4)", 
   pages        = "042306",
   year         = "2009",
url = "http://link.aps.org/doi/10.1103/PhysRevA.79.042306"
}

@ARTICLE{G98,
   author       = "N. Gisin",
title = "Quantum cloning without signaling",
   journal      = "Physics Letters A",
   volume       = "242(1-2)", 
   pages        = "1-3",
   year         = "1998",
url = "http://dx.doi.org/10.1016/S0375-9601(98)00170-4"
}


@article{DamianPBT,
  title = {Deduction of an upper bound on the success probability of port-based teleportation from the no-cloning theorem and the no-signaling principle},
  author = {D. Pital\'ua-Garc\'ia},
  journal = {Physical Review A},
  volume = {87(4)},
  issue = {4},
  pages = {040303(R)},
  numpages = {5},
  year = {2013},
  doi = {10.1103/PhysRevA.87.040303},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.87.040303},
  publisher = {American Physical Society}
}




@UNPUBLISHED{DPG1,
   author = "D. Pital\'ua-Garc\'ia",
   note = "to be published",
}

@UNPUBLISHED{DPG2,
   author = "D. Pital\'ua-Garc\'ia",
   note = "to be published",
}













@ARTICLE{LP31,
   author       = "L. Landau and R. Peierls",
   journal      = "Zeitschrift fur Physik",
   volume       = "69(1-2)", 
   pages        = "56--69",
   year         = "1931",
url = "http://www.springerlink.com/content/r4035w7577745427/"
}

@ARTICLE{AA80,
   author       = "Y. Aharonov and D. Z. Albert",
title = "States and observables in relativistic quantum field theories",
   journal      = "Physical Review D",
   volume       = "21(12)", 
   pages        = "3316-3324",
   year         = "1980",
url = "http://link.aps.org/doi/10.1103/PhysRevD.21.3316"
}

@ARTICLE{AA81,
   author       = "Y. Aharonov and D. Z. Albert",
title = "Can we make sense out of the measurement process in relativistic quantum mechanics?",
   journal      = "Physical Review D",
   volume       = "24(2)", 
   pages        = "359-370",
   year         = "1981",
url = "http://link.aps.org/doi/10.1103/PhysRevD.24.359"
}

@ARTICLE{AA84.1,
   author       = "Y. Aharonov and D. Z. Albert",
title = "Is the usual notion of time evolution adequate for quantum-mechanical systems? {I}",
   journal      = "Physical Review D",
   volume       = "29(2)", 
   pages        = "223-227",
   year         = "1984",
url = "http://prd.aps.org/abstract/PRD/v29/i2/p223_1"

}

@ARTICLE{AA84.2,
   author       = "Y. Aharonov and D. Z. Albert",
title = "Is the usual notion of time evolution adequate for quantum-mechanical systems? {II}. {R}elativistic considerations",
   journal      = "Physical Review D",
   volume       = "29(2)", 
   pages        = "228-234",
   year         = "1984",
url = "http://link.aps.org/doi/10.1103/PhysRevD.29.228"
}

@ARTICLE{AAV86,
   author       = "Y. Aharonov and D. Z. Albert and L. Vaidman",
title = "Measurement process in relativistic quantum theory",
   journal      = "Physical Review D",
   volume       = "34(6)", 
   pages        = "1805-1813",
   year         = "1986",
url = "http://link.aps.org/doi/10.1103/PhysRevD.34.1805"
}

@ARTICLE{PV94,
   author       = "S. Popescu and L. Vaidman",
title = "Causality constraints on nonlocal quantum measurements",
   journal      = "Physical Review A",
   volume       = "49(6)", 
   pages        = "4331-4338",
   year         = "1994",
url = "http://link.aps.org/doi/10.1103/PhysRevA.49.4331"
}

@ARTICLE{BGNP01,
   author       = "D. Beckman and D. Gottesman and M. A. Nielsen and J. Preskill",
title = "Causal and localizable quantum operations",
   journal      = "Physical Review A",
   volume       = "64(5)", 
   pages        = "052309",
   year         = "2001",
url = "http://link.aps.org/doi/10.1103/PhysRevA.64.052309"
}

@ARTICLE{V03,
   author       = "L. Vaidman",
title = "Instantaneous measurement of nonlocal variables",
   journal      = "Physical Review Letters",
   volume       = "90(1)", 
   pages        = "010402",
   year         = "2003",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.90.010402"
}

@MISC{KBMS06, 

   author       = "A. P. Kent and W. J. Munro and T. P. Spiller and R. G. Beausoleil",
title = "Tagging systems",
   howpublished = "{US Patent No. }7,075,438", 
   year         =  "2006", 
url = "http://patft.uspto.gov/netacgi/nph-Parser?Sect1=PTO1&Sect2=HITOFF&d=PALL&p=1&u=%2Fnetahtml%2FPTO%2Fsrchnum.htm&r=1&f=G&l=50&s1=7,075,438.PN.&OS=PN/7,075,438&RS=PN/7,075,438",
}

@ARTICLE{M10.1,
   author       = "R. A. Malaney",
title = "Location-dependent communications using quantum entanglement",
   journal      = "Physical Review A",
   volume       = "81(4)", 
   pages        = "042319",
   year         = "2010",
url = "http://link.aps.org/doi/10.1103/PhysRevA.81.042319"
}

@Unpublished{M10.2,
author = "R. A. Malaney",
title= "Quantum location verification in noisy channels",
year = "2010",
note = "E-print arXiv:1004.4689",
eprint = "1004.4689",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1004.4689;%%",
url = "http://arxiv.org/abs/1004.4689",
}

@ARTICLE{KMS11,
   author       = "A. Kent and W. J. Munro and T. P. Spiller",
title = "Quantum tagging: Authenticating location via quantum information and relativistic signaling constraints",
   journal      = "Physical Review A",
   volume       = "84(1)", 
   pages        = "012326",
   year         = "2011",
url = "http://link.aps.org/doi/10.1103/PhysRevA.84.012326"
}

@ARTICLE{K11.1,
   author       = "A. Kent",
title = "Quantum tagging for tags containing secret classical data",
   journal      = "Physical Review A",
   volume       = "84(2)", 
   pages        = "022335",
   year         = "2011",
url ="http://link.aps.org/doi/10.1103/PhysRevA.84.022335"
}

@Unpublished{pbqc,
author = "H. Buhrman and N. Chandran and S. Fehr and R. Gelles and V. Goyal and R. Ostrovsky and C. Schaffner",
title = "Position-based quantum cryptography: Impossibility and constructions",
year = "2011",
note = "E-print arXiv:1009.2490",
eprint = "1009.2490",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1009.2490;%%",
url = "http://arxiv.org/abs/1009.2490",
}

@ARTICLE{LL11,
   author       = "H.-K. Lau and H.-K. Lo",
title = "Insecurity of position-based quantum-cryptography protocols against entanglement attacks",
   journal      = "Physical Review A",
   volume       = "83(1)", 
   pages        = "012322",
   year         = "2011",
url = "http://link.aps.org/doi/10.1103/PhysRevA.83.012322"
}

@ARTICLE{BHH11,
   author       = "J. Bae and W.-Y. Hwang and Y.-D. Han",
title = "No-signaling principle can determine optimal quantum state discrimination",
   journal      = "Physical Review Letters",
   volume       = "107(17)", 
   pages        = "170403",
   year         = "2011",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.107.170403"
}

@ARTICLE{BK11,
   author       = "S. Beigi and R. K{\"{o}}nig",
title = "Simplified instantaneous non-local quantum computation with applications to position-based cryptography",
   journal      = "New Journal of Physics",
   volume       = "13", 
   pages        = "093036",
   year         = "2011",
url ="http://iopscience.iop.org/1367-2630/13/9/093036/"
}

@Unpublished{J02,
author = "R. Jozsa",
title = " A stronger no-cloning theorem",
note = "E-print arXiv:quant-ph/0204153",
year = "2002",
eprint = "quant-ph/0204153v2",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:quant-ph/0204153v2;%%",
url = "http://arxiv.org/abs/quant-ph/0204153",
}

@Unpublished{J03,
author = "R. Jozsa",
title = "Illustrating the concept of quantum information",
note = "E-print arXiv:quant-ph/0305114",
year = "2003",
eprint = "quant-ph/0305114v1",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:0305114;%%",
url = "http://arxiv.org/abs/quant-ph/0305114",
}

@ARTICLE{B07,
   author       = "J. Barrett",
title = "Information processing in generalized probabilistic theories",
   journal      = "Physical Review A",
   volume       = "75(3)", 
   pages        = "032304",
   year         = "2007",
url = "http://link.aps.org/doi/10.1103/PhysRevA.75.032304"
}

@ARTICLE{NC97,
   author       = "M. A. Nielsen and I. L. Chuang",
   journal      = "Physical Review Letters",
title = "Programmable quantum gate arrays",
   volume       = "79(2)", 
   pages        = "321-324",
   year         = "1997",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.79.321"
}

@INPROCEEDINGS{BFSS11,
   author       = "H. Buhrman and S. Fehr and C. Schaffner and F. Speelman",
title = "The garden-hose model",
booktitle      = "Proceedings of the 4th conference on Innovations in Theoretical Computer Science",
   pages        = "145-158",
   publisher       = "ACM",
address= "New York",
   year         = "2013",
url = "http://dl.acm.org/citation.cfm?doid=2422436.2422455",
}

@Unpublished{BFSS11,
author = "H. Buhrman and S. Fehr and C. Schaffner and F. Speelman",
title = "The garden-hose model",
year = "2011",
eprint = "1109.2563",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1109.2563;%%"
}

@ARTICLE{GR02,
   author       = "B. Groisman and B. Reznik",
title = "Measurements of semilocal and nonmaximally entangled states",
   journal      = "Physical Review A",
   volume       = "66(2)", 
   pages        = "022110",
   year         = "2002",
url = "http://link.aps.org/doi/10.1103/PhysRevA.66.022110"
}

@ARTICLE{GRV03,
   author       = "B. Groisman and B. Reznik and L. Vaidman",
title = "Instantaneous measurements of nonlocal variables",
   journal      = "Journal of Modern Optics",
   volume       = "50(6-7)", 
   pages        = "943-949",
   year         = "2003",
url = "http://www.tandfonline.com/doi/abs/10.1080/09500340308234543"
}

@ARTICLE{CCJP10,
   author       = "S. R. Clark and A. J. Connor and D. Jaksch and S. Popescu",
title = "Entanglement consumption of instantaneous nonlocal quantum measurements",
   journal      = "New Journal of Physics",
   volume       = "12", 
   pages        = "083034",
   year         = "2010",
url = "http://iopscience.iop.org/1367-2630/12/8/083034"
}



@article{SHO13,
  title = {Generalized teleportation and entanglement recycling},
  author = {S. Strelchuk and M. Horodecki and J. Oppenheim},
  journal = {Physical Review Letters},
  volume = {110(1)},
  issue = {1},
  pages = {010505},
  numpages = {5},
  year = {2013},
  doi = {10.1103/PhysRevLett.110.010505},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.110.010505},
  publisher = {American Physical Society}
}












%OTHERS (TO BE VERIFIED and ARRANGED)





@ARTICLE{E57,
   author       = "H. Everett",
title= {Relative State Formulation of Quantum Mechanics},
   journal      = "Rev. Mod. Phys.",
   volume       = "29", 
   pages        = "454",
   year         = "1957",
note={reprinted in Ref. \cite{DeWittbook}, pp. 141-149}
}

@book{DeWittbook,
  title={The many{-}worlds interpretation of quantum mechanics},
  author={DeWitt, Bryce Seligman and Graham, Neill},
  volume={63},
  year={2015},
  publisher={Princeton University Press}
}




@ARTICLE{MVBS04,
   author       = "M. M{\"{o}}tt{\"{o}}nen and J. J. Vartiainen and V. Bergholm and M. M. Salomaa",
   journal      = "Physical Review Letters",
   volume       = "93", 
   pages        = "130502",
   year         = "2004",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.93.130502"
}

@article{PPM13,
  title = {No-Go Theorems for $\ensuremath{\psi}$-Epistemic Models Based on a Continuity Assumption},
  author = {Patra, M. K. and Pironio, S. and Massar, S.},
  journal = {Phys. Rev. Lett.},
  volume = {111},
  issue = {9},
  pages = {090402},
  numpages = {4},
  year = {2013},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.111.090402},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.111.090402}
}


@article{SJGBLM21,
author = {Sidhu, Jasminder S. and Joshi, Siddarth K. and Gündoğan, Mustafa and Brougham, Thomas and Lowndes, David and Mazzarella, Luca and Krutzik, Markus and Mohapatra, Sonali and Dequal, Daniele and Vallone, Giuseppe and Villoresi, Paolo and Ling, Alexander and Jennewein, Thomas and Mohageg, Makan and Rarity, John G. and Fuentes, Ivette and Pirandola, Stefano and Oi, Daniel K. L.},
title = {Advances in space quantum communications},
journal = {IET Quantum Communication},
volume = {n/a},
number = {n/a},
pages = {},
year = {2021},
doi = {https://doi.org/10.1049/qtc2.12015},
abstract = {Abstract Concerted efforts are underway to establish an infrastructure for a global quantum Internet to realise a spectrum of quantum technologies. This will enable more precise sensors, secure communications, and faster data processing. Quantum communications are a front-runner with quantum networks already implemented in several metropolitan areas. A number of recent proposals have modelled the use of space segments to overcome range limitations of purely terrestrial networks. Rapid progress in the design of quantum devices have enabled their deployment in space for in-orbit demonstrations. We review developments in this emerging area of space-based quantum technologies and provide a roadmap of key milestones towards a complete, global quantum networked landscape. Small satellites hold increasing promise to provide a cost effective coverage required to realise the quantum Internet. The state of art in small satellite missions is reviewed and the most current in-field demonstrations of quantum cryptography are collated. The important challenges in space quantum technologies that must be overcome and recent efforts to mitigate their effects are summarised. A perspective on future developments that would improve the performance of space quantum communications is included. The authors conclude with a discussion on fundamental physics experiments that could take advantage of a global, space-based quantum network.}
}



@article{KABBBDMOPR21,
  title={Quantum technologies in space},
  author={Kaltenbaek, Rainer and Acin, Antonio and Bacsardi, Laszlo and Bianco, Paolo and Bouyer, Philippe and Diamanti, Eleni and Marquardt, Christoph and Omar, Yasser and Pruneri, Valerio and Rasel, Ernst and Sang, Bernhard and Seidel, Stephan and Ulbricht, Hendrik and Ursin, Rupert and Villoresi, Paolo and van den Bossche, Mathias and von Klitzing, Wolf
and Zbinden, Hugo and Paternostro, Mauro and Bassi, Angelo},
  journal={Exp. Astron.},
  pages={1--18},
  year={2021},
  publisher={Springer},
doi={10.1007/s10686-021-09731-x}
}

@ARTICLE{Pearle70,
   author       = "P. M. Pearle",
title= "Hidden{-}Variable Example Based upon Data Rejection",
   journal      = "Phys. Rev. D",
   volume       = "2", 
   pages        = "1418--1425",
   year         = "1970",
doi="10.1103/PhysRevD.2.1418"
}

@ARTICLE{ADR82,
   author       = "A. Aspect and J. Dalibard and G. Roger",
   journal      = "Physical Review Letters",
   volume       = "49", 
   pages        = "1804",
   year         = "1982",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.49.1804"
}

@ARTICLE{WJSWZ98,
   author       = "G. Weihs and T. Jennewein and C. Simon and H. Weinfurter and A. Zeilinger",
   journal      = "Physical Review Letters",
   volume       = "81", 
   pages        = "5039",
   year         = "1998",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.81.5039"
}

@ARTICLE{RKMSIMW01,
   author       = "M. A. Rowe and D. Kielpinski and V. Meyer and C. A. Sackett and W. M. Itano and C. Monroe and D. J. Wineland",
title= "Experimental violation of a {B}ell's inequality with efficient detection",
   journal      = "Nature ",
   volume       = "409", 
   pages        = "791--794",
   year         = "2001",
url = "http://www.nature.com/nature/journal/v409/n6822/full/409791a0.html"
}

@ARTICLE{MMMOM08,
   author       = "D. N. Matsukevich and P. Maunz and D. L. Moehring and S. Olmschenk and C. Monroe",
title= "Bell inequality violation with two remote atomic qubits",
   journal      = "Phys. Rev. Lett.",
   volume       = "100", 
   pages        = "150404",
   year         = "2008", 
doi = {10.1103/PhysRevLett.100.150404}
}
















MISC{PBTSM,
note = "See Supplemental Material at [URL will be inserted by AIP] for the
proof of the Theorem and details about the primed PBT protocol."
}

@ARTICLE{Bell,
   author       = "J. S. Bell",
title = "On the {E}instein-{P}odolsky-{R}osen paradox",
   journal      = "Physics",
   volume       = "1", 
   pages        = "195-200",
   year         = "1964",
note="Reprinted in \cite{Bellbook}, pages 14--21",
}

@ARTICLE{teleportation,
   author       = "C. H. Bennett and G. Brassard and C. Cr\'epeau and R. Jozsa
and A. Peres and W. K. Wootters",
   journal      = "Phys. Rev. Lett.",
   volume       = "70",
   pages        = "1895",
   year         = "1993",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.70.1895"
}


@ARTICLE{BH96,
   author       = "V. Bu{\v{z}}ek and M. Hillery",
   journal      = "Phys. Rev. A",
   volume       = "54",
   pages        = "1844",
   year         = "1996",
url = "http://link.aps.org/doi/10.1103/PhysRevA.54.1844"
}

@ARTICLE{IH08,
   author       = "S. Ishizaka and T. Hiroshima",
   journal      = "Phys. Rev.  Lett.",
   volume       = "101",
   pages        = "240501",
   year         = "2008",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.101.240501"
}

@ARTICLE{IH09,
   author       = "S. Ishizaka and T. Hiroshima",
   journal      = "Phys. Rev. A",
   volume       = "79",
   pages        = "042306",
   year         = "2009",
url = "http://link.aps.org/doi/10.1103/PhysRevA.79.042306"
}

@ARTICLE{G98,
   author       = "N. Gisin",
   journal      = "Phys. Lett. A",
   volume       = "242",
   pages        = "1",
   year         = "1998",
url = "http://dx.doi.org/10.1016/S0375-9601(98)00170-4"
}


@UNPUBLISHED{DPG1,
   author = "D. Pital\'ua-Garc\'ia",
   note = "to be published",
}

@UNPUBLISHED{DPG2,
   author = "D. Pital\'ua-Garc\'ia",
   note = "to be published",
}

@ARTICLE{WZ82,
   author       = "W. K. Wootters and W. H. Zurek",
   journal      = "Nature (London)",
   volume       = "299",
   pages        = "802",
   year         = "1982",
url = "http://www.nature.com/nature/journal/v299/n5886/abs/299802a0.html"
}

@ARTICLE{D82,
   author       = "D. Dieks",
   journal      = "Phys. Lett. A",
   volume       = "92",
   pages        = "271",
   year         = "1982",
url = "http://dx.doi.org/10.1016/0375-9601(82)90084-6"
}

@Unpublished{K11.2,
author = "Kent, A.",
year = "2011",
eprint = "1101.4612",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1101.4612v3;%%"
}


@ARTICLE{LP31,
   author       = "L. Landau and R. Peierls",
   journal      = "Z. Phys.",
   volume       = "69",
   pages        = "56",
   year         = "1931",
url = "http://www.springerlink.com/content/r4035w7577745427/"
}

@ARTICLE{AA80,
   author       = "Y. Aharonov and D. Z. Albert",
   journal      = "Phys. Rev. D",
   volume       = "21",
   pages        = "3316",
   year         = "1980",
url = "http://link.aps.org/doi/10.1103/PhysRevD.21.3316"
}

@ARTICLE{AA81,
   author       = "Y. Aharonov and D. Z. Albert",
   journal      = "Phys. Rev. D",
   volume       = "24",
   pages        = "359",
   year         = "1981",
url = "http://link.aps.org/doi/10.1103/PhysRevD.24.359"
}

@ARTICLE{AA84.1,
   author       = "Y. Aharonov and D. Z. Albert",
   journal      = "Phys. Rev. D",
   volume       = "29",
   pages        = "223",
   year         = "1984",
url = "http://link.aps.org/doi/10.1103/PhysRevD.29.223"

}

@ARTICLE{AA84.2,
   author       = "Y. Aharonov and D. Z. Albert",
   journal      = "Phys. Rev. D",
   volume       = "29",
   pages        = "228",
   year         = "1984",
url = "http://link.aps.org/doi/10.1103/PhysRevD.29.228"
}

@ARTICLE{AAV86,
   author       = "Y. Aharonov and D. Z. Albert and L. Vaidman",
   journal      = "Phys. Rev. D",
   volume       = "34",
   pages        = "1805",
   year         = "1986",
url = "http://link.aps.org/doi/10.1103/PhysRevD.34.1805"
}

@ARTICLE{PV94,
   author       = "S. Popescu and L. Vaidman",
   journal      = "Phys. Rev. A",
   volume       = "49",
   pages        = "4331",
   year         = "1994",
url = "http://link.aps.org/doi/10.1103/PhysRevA.49.4331"
}

@ARTICLE{BGNP01,
   author       = "D. Beckman and D. Gottesman and M. A. Nielsen and J.
Preskill",
   journal      = "Phys. Rev. A",
   volume       = "64",
   pages        = "052309",
   year         = "2001",
url = "http://link.aps.org/doi/10.1103/PhysRevA.64.052309"
}

@ARTICLE{V03,
   author       = "L. Vaidman",
   journal      = "Phys. Rev. Lett.",
   volume       = "90",
   pages        = "010402",
   year         = "2003",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.90.010402"
}

@MISC{KBMS06,

   author       = "A. Kent and R. Beausoleil and W. Munro and T. Spiller",
   howpublished = "{US Patent No.}  US20067075438",
   year         =  "2006",
}

@ARTICLE{M10.1,
   author       = "R. A. Malaney",
   journal      = "Phys. Rev. A",
   volume       = "81",
   pages        = "042319",
   year         = "2010",
url = "http://link.aps.org/doi/10.1103/PhysRevA.81.042319"
}

@Unpublished{M10.2,
author = "Malaney, R. A.",
year = "2010",
eprint = "1004.4689",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1004.4689;%%"
}

@ARTICLE{KMS11,
   author       = "A. Kent and W. J. Munro and T. P. Spiller",
   journal      = "Phys. Rev. A",
   volume       = "84",
   pages        = "012326",
   year         = "2011",
url = "http://link.aps.org/doi/10.1103/PhysRevA.84.012326"
}

@ARTICLE{K11.1,
   author       = "A. Kent",
   journal      = "Phys. Rev. A",
   volume       = "84",
   pages        = "022335",
   year         = "2011",
url ="http://link.aps.org/doi/10.1103/PhysRevA.84.022335"
}

@Unpublished{pbqc,
author = "H. Buhrman and N. Chandran and S. Fehr and R. Gelles and V. Goyal and
R. Ostrovsky and C. Schaffner",
year = "2010",
eprint = "1009.2490",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1009.2490;%%"
}

@ARTICLE{LL11,
   author       = "H. K. Lau and H. K. Lo",
   journal      = "Phys. Rev. A",
   volume       = "83",
   pages        = "012322",
   year         = "2011",
url = "http://link.aps.org/doi/10.1103/PhysRevA.83.012322"
}

@Unpublished{BFSS11,
author = "H. Buhrman and S. Fehr and C. Schaffner and F. Speelman",
year = "2011",
eprint = "1109.2563",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1109.2563;%%"
}

@ARTICLE{GR02,
   author       = "B. Groisman and B. Reznik",
   journal      = "Phys. Rev. A",
   volume       = "66",
   pages        = "022110",
   year         = "2002",
url = "http://link.aps.org/doi/10.1103/PhysRevA.66.022110"
}

@ARTICLE{GRV03,
   author       = "B. Groisman and B. Reznik and L. Vaidman",
   journal      = "J. Mod. Opt.",
   volume       = "50",
   pages        = "943",
   year         = "2003",
url = "http://www.tandfonline.com/doi/abs/10.1080/09500340308234543"
}

@ARTICLE{CCJP10,
   author       = "S. R. Clark and A. J. Connor and D. Jaksch and S. Popescu",
   journal      = "New J. Phys.",
   volume       = "12",
   pages        = "083034",
   year         = "2010",
url = "http://iopscience.iop.org/1367-2630/12/8/083034"
}

@ARTICLE{BK11,
   author       = "S. Beigi and R. K{\"{o}}nig",
   journal      = "New J. Phys.",
   volume       = "13",
   pages        = "093036",
   year         = "2011",
url ="http://iopscience.iop.org/1367-2630/13/9/093036/"
}

@ARTICLE{MVBS04,
   author       = "M. M{\"{o}}tt{\"{o}}nen and J. J. Vartiainen and V. Bergholm
and M. M. Salomaa",
   journal      = "Phys. Rev. Lett.",
   volume       = "93",
   pages        = "130502",
   year         = "2004",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.93.130502"
}

@Unpublished{J02,
author = "R. Jozsa",
year = "2002",
eprint = "quant-ph/0204153v2",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:quant-ph/0204153v2;%%"
}

@Unpublished{J03,
author = "R. Jozsa",
year = "2003",
eprint = "quant-ph/0305114v1",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:0305114;%%"
}


@ARTICLE{BHK05,
   author       = "J. Barrett and L. Hardy and A. Kent",
   journal      = "Phys. Rev. Lett.",
   volume       = "95",
   pages        = "010503",
   year         = "2005",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.95.010503"
}

@ARTICLE{ic,
   author       = "M. Paw{\l}owski and T. Paterek and D. Kaszlikowski and V.
Scarani and A. Winter and M. {\.{Z}}ukowski",
   journal      = "Nature (London)",
   volume       = "461",
   pages        = "1101",
   year         = "2009",
url = "http://www.nature.com/nature/journal/v461/n7267/full/nature08400.html"
}

@ARTICLE{NC97,
   author       = "M. A. Nielsen and I. L. Chuang",
   journal      = "Phys. Rev. Lett.",
   volume       = "79",
   pages        = "321",
   year         = "1997",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.79.321"
}

@ARTICLE{Pearle70,
   author       = "P. M. Pearle",
   journal      = "Phys Rev. D.",
   volume       = "2",
   pages        = "1418",
   year         = "1970",
url = "http://link.aps.org/doi/10.1103/PhysRevD.2.1418"
}

@ARTICLE{ADR82,
   author       = "A. Aspect and J. Dalibard and G. Roger",
   journal      = "Phys. Rev. Lett.",
   volume       = "49",
   pages        = "1804",
   year         = "1982",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.49.1804"
}

@ARTICLE{WJSWZ81,
   author       = "G. Weihs and T. Jennewein and C. Simon and H. Weinfurter and
A. Zeilinger",
   journal      = "Phys. Rev. Lett.",
   volume       = "81",
   pages        = "5039",
   year         = "1998",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.81.5039"
}

@ARTICLE{RKMSIMW01,
   author       = "M. A. Rowe and D. Kielpinski and V. Meyer and C. A. Sackett
and W. M. Itano and C. Monroe and D. J. Wineland",
   journal      = "Nature",
   volume       = "409",
   pages        = "791",
   year         = "2001",
url = "http://www.nature.com/nature/journal/v409/n6822/full/409791a0.html"
}

@ARTICLE{MMMOM08,
   author       = "D. N. Matsukevich and P. Maunz and D. L. Moehring and S.
Olmschenk and C. Monroe",
   journal      = "Phys. Rev. Lett.",
   volume       = "100",
   pages        = "150404",
   year         = "2008",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.100.150404"
}
















@Book{Bohmbook,
 author    = "David Bohm",
 title     = "Quantum Theory",
 publisher = "Prentice-Hall",
 year      =  1951,
}

@Book{NielsenandChuangbook,
 author    = "M. A. Nielsen and I. L. Chuang",
 title     = "Quantum Computation and Quantum Information",
 publisher = "Cambridge University Press",
 year      =  2000,
}

@Unpublished{J02,
author = "R. Jozsa",
title = "A stronger no-cloning theorem",
year = "2002",
Note = "E-print arXiv:quant-ph/0204153",
}

@Unpublished{J03,
author = "R. Jozsa",
title = "Illustrating the concept of quantum information",
year = "2003",
Note = "E-print arXiv:quant-ph/0305114",
}

@ARTICLE{LP31,
   author       = "L. Landau and R. Peierls",
   journal      = "Z. Phys.",
   volume       = "69",
   pages        = "56",
   year         = "1931",
url = "http://www.springerlink.com/content/r4035w7577745427/"
}

@ARTICLE{EPR35,
   author       = "A. Einstein and B. Podolsky and N. Rosen",
title = "Can quantum-mechanical description of physical reality be considered
complete?",
   journal      = "Phys. Rev.",
   volume       = "47",
   pages        = "777-780",
   year         = "1935",
url = "http://link.aps.org/doi/10.1103/PhysRev.47.777"
}

@ARTICLE{Bell,
   author       = "J. S. Bell",
title = "On the {E}instein {P}odolsky {R}osen paradox",
   year         = "1964",
   journal      = "Physics",
   volume       = "1",
   pages        = "195-200",
}

@ARTICLE{LR68,
   author       = "O. E. Lanford and D. W. Robinson",
title = "Mean entropy of states in quantum-statistical mechanics",
   journal      = "J. Math. Phys.",
   volume       = "9",
   pages        = "1120-1125",
   year         = "1968",
url = "http://jmp.aip.org/resource/1/jmapaq/v9/i7/p1120_s1"
}



@ARTICLE{AL70,
   author       = "H. Araki and E. H. Lieb",
title = "Entropy inequalities",
   journal      = "Commun. Math. Phys.",
   volume       = "18",
   pages        = "160-170",
   year         = "1970",
url = "http://www.springerlink.com/content/wk224145h1441527/"
}

@ARTICLE{Pearle70,
   author       = "P. M. Pearle",
   journal      = "Phys Rev. D.",
   volume       = "2",
   pages        = "1418",
   year         = "1970",
url = "http://link.aps.org/doi/10.1103/PhysRevD.2.1418"
}

@ARTICLE{K73,
   author       = "A. S. Kholevo",
   title = "Bounds for the quantity of information transmitted by a quantum
communication channel",
   journal      = "Probl. Inf. Transm.",
   volume       = "9",
   pages        = "177-183",
   year         = "1973",
}

@ARTICLE{AA80,
   author       = "Y. Aharonov and D. Z. Albert",
   journal      = "Phys. Rev. D",
   volume       = "21",
   pages        = "3316",
   year         = "1980",
url = "http://link.aps.org/doi/10.1103/PhysRevD.21.3316"
}

@ARTICLE{C80,
   author       = "B. S. Cirel'son",
title = "Quantum generalizations of {B}ell's inequality",
   journal      = "Lett. Math. Phys.",
   volume       = "4",
   pages        = "93-100",
   year         = "1980",
url = "http://www.springerlink.com/content/l57053g573430450/"
}

@ARTICLE{GRW80,
   author       = "G. C. Ghirardi and A. Rimini and T. Weber",
title = "A general argument against superluminal transmission through the
quantum mechanical measurement process",
   journal      = "Lett. Nuov. Cim.",
   volume       = "27",
   pages        = "293-298",
   year         = "1980",
url = "http://www.springerlink.com/content/t5h287h1r26j25j4/"
}

@ARTICLE{AA81,
   author       = "Y. Aharonov and D. Z. Albert",
   journal      = "Phys. Rev. D",
   volume       = "24",
   pages        = "359",
   year         = "1981",
url = "http://link.aps.org/doi/10.1103/PhysRevD.24.359"
}

@ARTICLE{WZ82,
   author       = "W. K. Wootters and W. H. Zurek",
title = "A single quantum cannot be cloned",
   journal      = "Nature (London)",
   volume       = "299",
   pages        = "802-803",
   year         = "1982",
url = "http://www.nature.com/nature/journal/v299/n5886/abs/299802a0.html"
}

@ARTICLE{D82,
   author       = "D. Dieks",
   title = "Communication by {EPR} devices",
   journal      = "Phys. Lett. A",
   volume       = "92",
   pages        = "271-272",
   year         = "1982",
url = "http://dx.doi.org/10.1016/0375-9601(82)90084-6"
}

@ARTICLE{ADR82,
   author       = "A. Aspect and J. Dalibard and G. Roger",
   journal      = "Phys. Rev. Lett.",
   volume       = "49",
   pages        = "1804",
   year         = "1982",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.49.1804"
}

@ARTICLE{W83,
   author       = "S. Wiesner",
title = "Conjugate coding",
   journal      = "SIGACT News",
   volume       = "15",
   pages        = "78-88",
   year         = "1983",
url = "http://dl.acm.org/citation.cfm?doid=1008908.1008920"
}

@ARTICLE{AA84.1,
   author       = "Y. Aharonov and D. Z. Albert",
   journal      = "Phys. Rev. D",
   volume       = "29",
   pages        = "223",
   year         = "1984",
url = "http://link.aps.org/doi/10.1103/PhysRevD.29.223"
}

@ARTICLE{AA84.2,
   author       = "Y. Aharonov and D. Z. Albert",
   journal      = "Phys. Rev. D",
   volume       = "29",
   pages        = "228",
   year         = "1984",
url = "http://link.aps.org/doi/10.1103/PhysRevD.29.228"
}

@INPROCEEDINGS{BB84,
   author       = "C. H. Bennett and G. Brassard",
   booktitle      = "Proceedings IEEE Int. Conf. on Computers, Systems and
Signal Processing, Bangalore, India",
   pages        = "175-179",
   publisher       = "IEEE",
   year         = "1984",
}

@ARTICLE{AAV86,
   author       = "Y. Aharonov and D. Z. Albert and L. Vaidman",
   journal      = "Phys. Rev. D",
   volume       = "34",
   pages        = "1805",
   year         = "1986",
url = "http://link.aps.org/doi/10.1103/PhysRevD.34.1805"
}

@ARTICLE{BC90,
   author       = "S. L. Braunstein and C. M. Caves",
   journal      = "Ann. Phys.",
   volume       = "202",
   pages        = "22",
   year         = "1990",
url = "http://www.sciencedirect.com/science/article/pii/000349169090339P"
}



@ARTICLE{teleportation,
   author       = "C. H. Bennett and G. Brassard and C. Cr\'epeau and R. Jozsa
and A. Peres and W. K. Wootters",
   title = "Teleporting an unknown quantum state via dual classical and
{E}instein-{P}odolsky-{R}osen channels",
   journal      = "Phys. Rev. Lett.",
   volume       = "70",
   pages        = "1895-1899",
   year         = "1993",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.70.1895"
}

@ARTICLE{PV94,
   author       = "S. Popescu and L. Vaidman",
   journal      = "Phys. Rev. A",
   volume       = "49",
   pages        = "4331",
   year         = "1994",
url = "http://link.aps.org/doi/10.1103/PhysRevA.49.4331"
}

@ARTICLE{PR94,
   author       = "S. Popescu and D. Rohrlich",
title = "Quantum nonlocality as an axiom",
   journal      = "Found. Phys.",
   volume       = "24",
   pages        = "379-385",
   year         = "1994",
url = "http://www.springerlink.com/content/j842v3324u512nx0/"
}

@ARTICLE{BH96,
   author       = "V. Bu{\v{z}}ek and M. Hillery",
   journal      = "Phys. Rev. A",
   volume       = "54",
   pages        = "1844",
   year         = "1996",
url = "http://link.aps.org/doi/10.1103/PhysRevA.54.1844"
}

@ARTICLE{NC97,
   author       = "M. A. Nielsen and I. L. Chuang",
title = "Programmable Quantum Gate Arrays",
   journal      = "Phys. Rev. Lett.",
   volume       = "79",
   pages        = "321-324",
   year         = "1997",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.79.321"
}

@ARTICLE{G98,
   author       = "N. Gisin",
title = "Quantum cloning without signaling",
   journal      = "Phys. Lett. A",
   volume       = "242",
   pages        = "1-3",
   year         = "1998",
url = "http://dx.doi.org/10.1016/S0375-9601(98)00170-4"
}

@ARTICLE{WJSWZ81,
   author       = "G. Weihs and T. Jennewein and C. Simon and H. Weinfurter and
A. Zeilinger",
   journal      = "Phys. Rev. Lett.",
   volume       = "81",
   pages        = "5039",
   year         = "1998",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.81.5039"
}

@ARTICLE{BGNP01,
   author       = "D. Beckman and D. Gottesman and M. A. Nielsen and J.
Preskill",
   journal      = "Phys. Rev. A",
   volume       = "64",
   pages        = "052309",
   year         = "2001",
url = "http://link.aps.org/doi/10.1103/PhysRevA.64.052309"
}

@ARTICLE{RKMSIMW01,
   author       = "M. A. Rowe and D. Kielpinski and V. Meyer and C. A. Sackett
and W. M. Itano and C. Monroe and D. J. Wineland",
   journal      = "Nature",
   volume       = "409",
   pages        = "791",
   year         = "2001",
url = "http://www.nature.com/nature/journal/v409/n6822/full/409791a0.html"
}

@ARTICLE{GR02,
   author       = "B. Groisman and B. Reznik",
title = "Measurements of semilocal and nonmaximally entangled states",
   journal      = "Phys. Rev. A",
   volume       = "66",
   pages        = "022110",
   year         = "2002",
url = "http://link.aps.org/doi/10.1103/PhysRevA.66.022110"
}


@ARTICLE{ANTV02,
   author       = "A. Ambainis and A. Nayak and A. Ta-Shma and U. Vazirani",
title = "Dense quantum coding and quantum finite automata",
   journal      = "J. ACM",
   volume       = "49",
   pages        = "496-511",
   year         = "2002",
url = "http://dl.acm.org/citation.cfm?doid=581771.581773"
}


@ARTICLE{V03,
   author       = "L. Vaidman",
title = "Instantaneous Measurement of Nonlocal Variables",
   journal      = "Phys. Rev. Lett.",
   volume       = "90",
   pages        = "010402",
   year         = "2003",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.90.010402"
}

@ARTICLE{GRV03,
   author       = "B. Groisman and B. Reznik and L. Vaidman",
title = "Instantaneous measurements of nonlocal variables",
   journal      = "J. Mod. Opt.",
   volume       = "50",
   pages        = "943-949",
   year         = "2003",
url = "http://www.tandfonline.com/doi/abs/10.1080/09500340308234543"
}

@ARTICLE{MVBS04,
   author       = "M. M{\"{o}}tt{\"{o}}nen and J. J. Vartiainen and V. Bergholm
and M. M. Salomaa",
   journal      = "Phys. Rev. Lett.",
   volume       = "93",
   pages        = "130502",
   year         = "2004",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.93.130502"
}

@ARTICLE{BHK05,
   author       = "J. Barrett and L. Hardy and A. Kent",
title = "No signaling and quantum key distribution",
   journal      = "Phys. Rev. Lett.",
   volume       = "95",
   pages        = "010503",
   year         = "2005",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.95.010503"
}

@MISC{KBMS06,
   author       = "A. Kent and R. Beausoleil and W. Munro and T. Spiller",
   howpublished = "{US Patent No.}  US20067075438",
   year         =  "2006",
}

@ARTICLE{B07,
   author       = "J. Barrett",
title = "Information processing in generalized probabilistic theories",
   journal      = "Phys. Rev. A",
   volume       = "75",
   pages        = "032304",
   year         = "2007",
url = "http://link.aps.org/doi/10.1103/PhysRevA.75.032304"
}

@ARTICLE{BBLW07,
   author       = "H. Barnum and J. Barrett and M. Leifer and A. Wilce",
title = "Generalized no-broadcasting theorem",
   journal      = "Phys. Rev. Lett.",
   volume       = "99",
   pages        = "240501",
   year         = "2007",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.99.240501"
}

@ARTICLE{IH08,
   author       = "S. Ishizaka and T. Hiroshima",
title = "Asymptotic Teleportation Scheme as a Universal Programmable Quantum
Processor",
   journal      = "Phys. Rev.  Lett.",
   volume       = "101",
   pages        = "240501",
   year         = "2008",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.101.240501"
}

@ARTICLE{MMMOM08,
   author       = "D. N. Matsukevich and P. Maunz and D. L. Moehring and S.
Olmschenk and C. Monroe",
   journal      = "Phys. Rev. Lett.",
   volume       = "100",
   pages        = "150404",
   year         = "2008",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.100.150404"
}

@ARTICLE{IH09,
   author       = "S. Ishizaka and T. Hiroshima",
title = "Quantum teleportation scheme by selecting one of multiple output
ports",
   journal      = "Phys. Rev. A",
   volume       = "79",
   pages        = "042306",
   year         = "2009",
url = "http://link.aps.org/doi/10.1103/PhysRevA.79.042306"
}

@ARTICLE{ic,
   author       = "M. Paw{\l}owski and T. Paterek and D. Kaszlikowski and V.
Scarani and A. Winter and M. {\.{Z}}ukowski",
title = "Information causality as a physical principle",
   journal      = "Nature (London)",
   volume       = "461",
   pages        = "1101-1104",
   year         = "2009",
url = "http://www.nature.com/nature/journal/v461/n7267/full/nature08400.html"
}

@ARTICLE{ABPS09,
   author       = "J. Allcock and N. Brunner and M. Paw{\l}owski and V.
Scarani",
title = "Recovering part of the boundary between quantum and nonquantum
correlations from information causality",
   journal      = "Phys. Rev. A",
   volume       = "80",
   pages        = "040103",
   year         = "2009",
url = "http://link.aps.org/doi/10.1103/PhysRevA.80.040103"
}

@ARTICLE{M10.1,
   author       = "R. A. Malaney",
title = "Location-dependent communications using quantum entanglement",
   journal      = "Phys. Rev. A",
   volume       = "81",
   pages        = "042319",
   year         = "2010",
url = "http://link.aps.org/doi/10.1103/PhysRevA.81.042319"
}

@Unpublished{M10.2,
author = "R. A. Malaney",
title = " Quantum Location Verification in Noisy Channels",
year = "2010",
Note = "E-print arXiv:1004.4689",
url = "http://arxiv.org/abs/1004.4689"
}

@ARTICLE{CCJP10,
   author       = "S. R. Clark and A. J. Connor and D. Jaksch and S. Popescu",
title = "Entanglement consumption of instantaneous nonlocal quantum
measurements",
   journal      = "New J. Phys.",
   volume       = "12",
   pages        = "083034",
   year         = "2010",
url = "http://iopscience.iop.org/1367-2630/12/8/083034"
}

@Unpublished{pbqc,
author = "H. Buhrman and N. Chandran and S. Fehr and R. Gelles and V. Goyal and
R. Ostrovsky and C. Schaffner",
title = "Position-Based Quantum Cryptography: Impossibility and Constructions",
year = "2010",
Note = "E-print arXiv:1009.2490",
}

@ARTICLE{CSS10,
   author       = "D. Cavalcanti and A. Salles and V. Scarani",
title = "Macroscopically local correlations can violate information causality",
   journal      = "Nat. Commun.",
   volume       = "1",
   pages        = "136",
   year         = "2010",
url = "http://www.nature.com/ncomms/journal/v1/n9/full/ncomms1138.html"
}

@ARTICLE{SW10,
   author       = "A. J. Short and S. Wehner",
title = "Entropy in general physical theories",
   journal      = "New J. Phys.",
   volume       = "12",
   pages        = "033023",
   year         = "2010",
url = "http://iopscience.iop.org/1367-2630/12/3/033023"
}

@article{SS18,
  title = {Simple proof of the impossibility of bit commitment in generalized probabilistic theories using cone programming},
  author = {Sikora, Jamie and Selby, John},
  journal = {Phys. Rev. A},
  volume = {97},
  issue = {4},
  pages = {042302},
  numpages = {5},
  year = {2018},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.97.042302},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.97.042302}
}

@article{SS18.2,
  doi = {10.22331/q-2018-11-02-103},
  url = {https://doi.org/10.22331/q-2018-11-02-103},
  title = {How to make unforgeable money in generalised probabilistic theories},
  author = {Selby, John H. and Sikora, Jamie},
  journal = {{Quantum}},
  issn = {2521-327X},
  publisher = {{Verein zur F{\"{o}}rderung des Open Access Publizierens in den Quantenwissenschaften}},
  volume = {2},
  pages = {103},
  month = nov,
  year = {2018}
}

@article{LPW18,
  doi = {10.1007/s00220-018-3154-4},
  url = {https://doi.org/10.1007/s00220-018-3154-4},
  title = {Ultimate Data Hiding in Quantum Mechanics and Beyond},
  author = {L. Lami and C. Palazuelos and A. Winter },
  journal = {Commun. Math. Phys.},
  volume = {361},
  pages = {661--708},
  year = {2018}
}




@ARTICLE{BBCLSSWW10,
   author       = "H. Barnum and J. Barrett and L. O. Clark and M. Leifer and
R. Spekkens and N. Stepanik and A. Wilce and R. Wilke",
title = "Entropy and information causality in general probabilistic theories",
   journal      = "New J. Phys.",
   volume       = "12",
   pages        = "033024",
   year         = "2010",
url = "http://iopscience.iop.org/1367-2630/12/3/033024"
}

@ARTICLE{PZ10,
   author       = "M. Paw{\l}owski and M. {\.{Z}}ukowski",
title = "Entanglement-assisted random access codes",
   journal      = "Phys. Rev. A",
   volume       = "81",
   pages        = "042326",
   year         = "2010",
url = "http://link.aps.org/doi/10.1103/PhysRevA.81.042326"
}

@ARTICLE{KMS11,
   author       = "A. Kent and W. J. Munro and T. P. Spiller",
title = "Quantum tagging: Authenticating location via quantum information and
relativistic signaling constraints",
   journal      = "Phys. Rev. A",
   volume       = "84",
   pages        = "012326",
   year         = "2011",
url = "http://link.aps.org/doi/10.1103/PhysRevA.84.012326"
}

@ARTICLE{K11.1,
   author       = "A. Kent",
title = "Quantum tagging for tags containing secret classical data",
   journal      = "Phys. Rev. A",
   volume       = "84",
   pages        = "022335",
   year         = "2011",
url ="http://link.aps.org/doi/10.1103/PhysRevA.84.022335"
}

@Unpublished{K11.2,
author = "Kent, A.",
year = "2011",
eprint = "1101.4612",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1101.4612v3;%%"
}

@ARTICLE{LL11,
   author       = "H. K. Lau and H. K. Lo",
title = "Insecurity of position-based quantum-cryptography protocols against
entanglement attacks",
   journal      = "Phys. Rev. A",
   volume       = "83",
   pages        = "012322",
   year         = "2011",
url = "http://link.aps.org/doi/10.1103/PhysRevA.83.012322"
}

@Unpublished{BFSS11,
author = "H. Buhrman and S. Fehr and C. Schaffner and F. Speelman",
title = " The Garden-Hose Game: A New Model of Computation, and Application to
Position-Based Quantum Cryptography",
year = "2011",
Note = "E-print arXiv:1109.2563",
}

@ARTICLE{BK11,
   author       = "S. Beigi and R. K{\"{o}}nig",
title ="Simplified instantaneous non-local quantum computation with
applications to position-based cryptography",
   journal      = "New J. Phys.",
   volume       = "13",
   pages        = "093036",
   year         = "2011",
url ="http://iopscience.iop.org/1367-2630/13/9/093036/"
}

@ARTICLE{AS11,
   author       = "S. W. Al-Safi and A. J. Short",
title = "Information causality from an entropic and probabilistic
perspective.",
   journal      = "Phys. Rev. A",
   volume       = "84",
   pages        = "042323",
   year         = "2011",
url = "http://link.aps.org/doi/10.1103/PhysRevA.84.042323"
}

@ARTICLE{GWAN11,
   author       = "R. Gallego and L. E. W{\"{u}}rflinger and A. Ac\'in and M.
Navascu\'es",
title = "Quantum correlations require multipartite information principles",
   journal      = "Phys. Rev. Lett.",
   volume       = "107",
   pages        = "210403",
   year         = "2011",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.107.210403"
}

@ARTICLE{YCATS12,
   author       = "T. H. Yang and D. Cavalcanti and M. L. Almeida and C. Teo
and V. Scarani",
title = "Information-causality and extremal tripartite correlations",
   journal      = "New J. Phys.",
   volume       = "14",
   pages        = "013061",
   year         = "2012",
url = "http://iopscience.iop.org/1367-2630/14/1/013061"
}

@UNPUBLISHED{DPG1,
   author = "D. Pital\'ua-Garc\'ia",
   note = "to be published",
}

@UNPUBLISHED{DPG2,
   author = "D. Pital\'ua-Garc\'ia",
   note = "to be published",
}

@Book{NielsenandChuangbook,
 author    = "M. A. Nielsen and I. L. Chuang",
 title     = "Quantum Computation and Quantum Information",
 publisher = "Cambridge University Press",
address= "Cambridge, UK",
 year      =  2000,
}

@ARTICLE{WZ82,
   author       = "W. K. Wootters and W. H. Zurek",
 title = "A single quantum cannot be cloned",
   journal      = "Nature (London)",
   volume       = "299",
   pages        = "802",
   year         = "1982",
url = "http://www.nature.com/nature/journal/v299/n5886/abs/299802a0.html"
}

@ARTICLE{D82,
   author       = "D. Dieks",
title = "Communication by {EPR} devices",
   journal      = "Phys. Lett. A",
   volume       = "92",
   pages        = "271",
   year         = "1982",
url = "http://dx.doi.org/10.1016/0375-9601(82)90084-6"
}

@ARTICLE{teleportation,
   author       = "C. H. Bennett and G. Brassard and C. Cr\'epeau and R. Jozsa
and A. Peres and W. K. Wootters",
 title = "Teleporting an unknown quantum state via dual classical and
{E}instein-{P}odolsky-{R}osen channels",
   journal      = "Phys. Rev. Lett.",
   volume       = "70",
   pages        = "1895",
   year         = "1993",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.70.1895"
}



@INPROCEEDINGS{BB84,
   author       = "C. H. Bennett and G. Brassard",
booktitle      = "Proceedings of IEEE International Conference on Computers,
Systems, and Signal Processing, Bangalore, India",
   pages        = "175",
   publisher       = "IEEE",
address= "New York",
   year         = "1984",
}


@ARTICLE{BHK05,
   author       = "J. Barrett and L. Hardy and A. Kent",
title = "No signaling and quantum key distribution",
   journal      = "Phys. Rev. Lett.",
   volume       = "95",
   pages        = "010503",
   year         = "2005",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.95.010503"
}

@ARTICLE{EPR35,
   author       = "A. Einstein and B. Podolsky and N. Rosen",
title = "Can quantum-mechanical description of physical reality be considered
complete?",
   journal      = "Phys. Rev.",
   volume       = "47",
   pages        = "777",
   year         = "1935",
url = "http://link.aps.org/doi/10.1103/PhysRev.47.777"
}

@ARTICLE{Bell,
   author       = "J. S. Bell",
title = "On the {E}instein {P}odolsky {R}osen paradox",
   year         = "1964",
   journal      = "Physics",
   volume       = "1",
   pages        = "195-200",
}

@ARTICLE{GRW80,
   author       = "G. C. Ghirardi and A. Rimini and T. Weber",
title = "A general argument against superluminal transmission through the
quantum mechanical measurement process",
   journal      = "Lett. Nuov. Cim.",
   volume       = "27",
   pages        = "293",
   year         = "1980",
url = "http://www.springerlink.com/content/t5h287h1r26j25j4/"
}

@ARTICLE{K73,
   author       = "A. S. Kholevo",
   title = "Bounds for the quantity of information transmitted by a quantum
communication channel",
   journal      = "Probl. Inf. Transm.",
   volume       = "9",
   pages        = "177",
   year         = "1973",
}

@ARTICLE{ic,
   author       = "M. Paw{\l}owski and T. Paterek and D. Kaszlikowski and V.
Scarani and A. Winter and M. {\.{Z}}ukowski",
title = "Information causality as a physical principle.",
   journal      = "Nature (London)",
   volume       = "461",
   pages        = "1101",
   year         = "2009",
url = "http://www.nature.com/nature/journal/v461/n7267/full/nature08400.html"
}


@ARTICLE{ABPS09,
   author       = "J. Allcock and N. Brunner and M. Paw{\l}owski and V.
Scarani",
title = "Recovering part of the boundary between quantum and nonquantum
correlations from information causality",
   journal      = "Phys. Rev. A",
   volume       = "80",
   pages        = "040103",
   year         = "2009",
url = "http://link.aps.org/doi/10.1103/PhysRevA.80.040103"
}

@ARTICLE{CSS10,
   author       = "D. Cavalcanti and A. Salles and V. Scarani",
title = "Macroscopically local correlations can violate information causality",
   journal      = "Nat. Commun.",
   volume       = "1",
   pages        = "136",
   year         = "2010",
url = "http://www.nature.com/ncomms/journal/v1/n9/full/ncomms1138.html"
}

@ARTICLE{GWAN11,
   author       = "R. Gallego and L. E. W{\"{u}}rflinger and A. Ac\'in and M.
Navascu\'es",
title = "Quantum correlations require multipartite information principles",
   journal      = "Phys. Rev. Lett.",
   volume       = "107",
   pages        = "210403",
   year         = "2011",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.107.210403"
}

@ARTICLE{YCATS12,
   author       = "T. H. Yang and D. Cavalcanti and M. L. Almeida and C. Teo
and V. Scarani",
title = "Information-causality and extremal tripartite correlations",
   journal      = "New J. Phys.",
   volume       = "14",
   pages        = "013061",
   year         = "2012",
url = "http://iopscience.iop.org/1367-2630/14/1/013061"
}

@ARTICLE{C80,
   author       = "B. S. Cirel'son",
title = "Quantum generalizations of {B}ell's inequality",
   journal      = "Lett. Math. Phys.",
   volume       = "4",
   pages        = "93",
   year         = "1980",
url = "http://www.springerlink.com/content/l57053g573430450/"
}

@ARTICLE{PR94,
   author       = "S. Popescu and D. Rohrlich",
title = "Quantum nonlocality as an axiom",
   journal      = "Found. Phys.",
   volume       = "24",
   pages        = "379",
   year         = "1994",
url = "http://www.springerlink.com/content/j842v3324u512nx0/"
}

@ARTICLE{LR68,
   author       = "O. E. Lanford and D. W. Robinson",
title = "Mean entropy of states in quantum-statistical mechanics",
   journal      = "J. Math. Phys.",
   volume       = "9",
   pages        = "1120",
   year         = "1968",
url = "http://jmp.aip.org/resource/1/jmapaq/v9/i7/p1120_s1"
}

@ARTICLE{AL70,
   author       = "H. Araki and E. H. Lieb",
title = "Entropy inequalities",
   journal      = "Commun. Math. Phys.",
   volume       = "18",
   pages        = "160",
   year         = "1970",
url = "http://www.springerlink.com/content/wk224145h1441527/"
}

@Unpublished{H01,
author = "L. Hardy",
title ="Quantum Theory From Five Reasonable Axioms",
year = "2001",
note = "E-print arXiv:quant-ph/0101012v4",
}

@ARTICLE{B07,
   author       = "J. Barrett",
title = "Information processing in generalized probabilistic theories",
   journal      = "Phys. Rev. A",
   volume       = "75",
   pages        = "032304",
   year         = "2007",
url = "http://link.aps.org/doi/10.1103/PhysRevA.75.032304"
}

@ARTICLE{BBLW07,
   author       = "H. Barnum and J. Barrett and M. Leifer and A. Wilce",
title = "Generalized no-broadcasting theorem",
   journal      = "Phys. Rev. Lett.",
   volume       = "99",
   pages        = "240501",
   year         = "2007",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.99.240501"
}

@ARTICLE{SW10,
   author       = "A. J. Short and S. Wehner",
title = "Entropy in general physical theories",
   journal      = "New J. Phys.",
   volume       = "12",
   pages        = "033023",
   year         = "2010",
url = "http://iopscience.iop.org/1367-2630/12/3/033023"
}

@ARTICLE{BBCLSSWW10,
   author       = "H. Barnum and J. Barrett and L. O. Clark and M. Leifer and
R. Spekkens and N. Stepanik and A. Wilce and R. Wilke",
title = "Entropy and information causality in general probabilistic theories",
   journal      = "New J. Phys.",
   volume       = "12",
   pages        = "033024",
   year         = "2010",
url = "http://iopscience.iop.org/1367-2630/12/3/033024"
}

@ARTICLE{AS11,
   author       = "S. W. Al-Safi and A. J. Short",
title = "Information causality from an entropic and a probabilistic
perspective",
   journal      = "Phys. Rev. A",
   volume       = "84",
   pages        = "042323",
   year         = "2011",
   url = "http://link.aps.org/doi/10.1103/PhysRevA.84.042323"
}

@ARTICLE{W83,
   author       = "S. Wiesner",
title = "Conjugate coding",
   journal      = "SIGACT News",
   volume       = "15",
   pages        = "78",
   year         = "1983",
url = "http://dl.acm.org/citation.cfm?doid=1008908.1008920"
}

@ARTICLE{ANTV02,
   author       = "A. Ambainis and A. Nayak and A. Ta-Shma and U. Vazirani",
title = "Dense quantum coding and quantum finite automata",
   journal      = "J. ACM",
   volume       = "49",
   pages        = "496",
   year         = "2002",
url = "http://dl.acm.org/citation.cfm?doid=581771.581773"
}

@ARTICLE{PZ10,
   author       = "M. Paw{\l}owski and M. {\.{Z}}ukowski",
title = "Entanglement-assisted random access codes",
   journal      = "Phys. Rev. A",
   volume       = "81",
   pages        = "042326",
   year         = "2010",
url = "http://link.aps.org/doi/10.1103/PhysRevA.81.042326"
}




@ARTICLE{MMAP13,
author = {Masanes, Lluis and M\"{u}ller, Markus P. and Augusiak, Remigiusz and P\'{e}rez-Garc\'{i}a, David}, 
title = {Existence of an information unit as a postulate of quantum theory},
volume = {110}, 
number = {41}, 
pages = {16373-16377}, 
year = {2013}, 
doi = {10.1073/pnas.1304884110}, 
abstract ={Does information play a significant role in the foundations of physics? Information is the abstraction that allows us to refer to the states of systems when we choose to ignore the systems themselves. This is only possible in very particular frameworks, like in classical or quantum theory, or more generally, whenever there exists an information unit such that the state of any system can be reversibly encoded in a sufficient number of such units. In this work, we show how the abstract formalism of quantum theory can be deduced solely from the existence of an information unit with suitable properties, together with two further natural assumptions: the continuity and reversibility of dynamics, and the possibility of characterizing the state of a composite system by local measurements. This constitutes a set of postulates for quantum theory with a simple and direct physical meaning, like the ones of special relativity or thermodynamics, and it articulates a strong connection between physics and information.}, 
URL = {http://www.pnas.org/content/110/41/16373.abstract}, 
journal = {Proc. Natl. Acad. Sci. USA} 
}

@ARTICLE{KM19,
author = {M. Krumm and M. P. M\"{u}ller}, 
title = {Quantum computation is the unique reversible circuit model for which bits are balls},
volume = {5}, 
pages = {7}, 
year = {2019}, 
doi = {10.1038/s41534-018-0123-x}, 
URL = {https://doi.org/10.1038/s41534-018-0123-x}, 
journal = {npj Quantum Inf.} 
}

@ARTICLE{BLS18,
author = {H. Barnum and C.M. Lee and J.H. Selby}, 
title = {Oracles and Query Lower Bounds in Generalised Probabilistic Theories},
volume = {48}, 
pages = {954--981}, 
year = {2018}, 
doi = {10.1007/s10701-018-0198-4}, 
URL = {https://doi.org/10.1007/s10701-018-0198-4}, 
journal = {Found. Phys.} 
}

@ARTICLE{G18,
author = {A.J.P Garner}, 
title = {Interferometric Computation Beyond Quantum Theory},
volume = {48}, 
pages = {886--909}, 
year = {2018}, 
doi = {10.1007/s10701-018-0142-7}, 
URL = {https://doi.org/10.1007/s10701-018-0142-7}, 
journal = {Found. Phys.} 
}

@ARTICLE{BBHL19,
author = {J. Barrett and N. de Beaudrap and M. J. Hoban and C. M. Lee}, 
title = {The computational landscape of general physical theories},
volume = {5}, 
pages = {41}, 
year = {2019}, 
doi = {10.1038/s41534-019-0156-9}, 
URL = {https://doi.org/10.1038/s41534-019-0156-9}, 
journal = {npj Quantum Inf.} 
}

@article{LS16.2,
	doi = {10.1088/1367-2630/18/9/093047},
	url = {https://doi.org/10.1088/1367-2630/18/9/093047},
	year = 2016,
	month = {sep},
	publisher = {{IOP} Publishing},
	volume = {18},
	number = {9},
	pages = {093047},
	author = {Ciar{\'{a}}n M Lee and John H Selby},
	title = {Deriving {G}rover{\textquotesingle}s lower bound from simple physical principles},
	journal = {New J. Phys.},
	abstract = {Grover's algorithm constitutes the optimal quantum solution to the search problem and provides a quadratic speed-up over all possible classical search algorithms. Quantum interference between computational paths has been posited as a key resource behind this computational speed-up. However there is a limit to this interference, at most pairs of paths can ever interact in a fundamental way. Could more interference imply more computational power? Sorkin has defined a hierarchy of possible interference behaviours—currently under experimental investigation—where classical theory is at the first level of the hierarchy and quantum theory belongs to the second. Informally, the order in the hierarchy corresponds to the number of paths that have an irreducible interaction in a multi-slit experiment. In this work, we consider how Grover's speed-up depends on the order of interference in a theory. Surprisingly, we show that the quadratic lower bound holds regardless of the order of interference. Thus, at least from the point of view of the search problem, post-quantum interference does not imply a computational speed-up over quantum theory.}
}

@ARTICLE{LH16,
author = {C. M. Lee and M. J. Hoban}, 
title = {Bounds on the power of proofs and advice in general physical theories},
volume = {5}, 
pages = {47220160076}, 
year = {2016}, 
doi = {10.1098/rspa.2016.0076}, 
URL = {https://doi.org/10.1098/rspa.2016.0076}, 
journal = {Proc. R. Soc. A.} 
}

@article{LS16,
	doi = {10.1088/1367-2630/18/3/033023},
	url = {https://doi.org/10.1088/1367-2630/18/3/033023},
	year = 2016,
	month = {mar},
	publisher = {{IOP} Publishing},
	volume = {18},
	number = {3},
	pages = {033023},
	author = {Ciar{\'{a}}n M Lee and John H Selby},
	title = {Generalised phase kick-back: the structure of computational algorithms from physical principles},
	journal = {New J. Phys.},
	abstract = {The advent of quantum computing has challenged classical conceptions of which problems are efficiently solvable in our physical world. This motivates the general study of how physical principles bound computational power. In this paper we show that some of the essential machinery of quantum computation—namely reversible controlled transformations and the phase kick-back mechanism—exist in any operational-defined theory with a consistent notion of information. These results provide the tools for an exploration of the physics underpinning the structure of computational algorithms. We investigate the relationship between interference behaviour and computational power, demonstrating that non-trivial interference behaviour is a general resource for post-classical computation. In proving the above, we connect higher-order interference to the existence of post-quantum particle types, potentially providing a novel experimental test for higher-order interference. Finally, we conjecture that theories with post-quantum interference—the higher-order interference of Sorkin—can solve problems intractable even on a quantum computer.}
}


@article{bukh,
  title={Measurable sets with excluded distances},
  author={Bukh, Boris},
  journal={Geometric and Functional Analysis},
  volume={18},
  number={3},
  pages={668--697},
  year={2008},
  publisher={Springer},
url={http://link.springer.com/article/10.1007/s00039-008-0673-8}
}

@article{de2008fourier,
  title={Fourier analysis, linear programming, and densities of distance
avoiding sets in Rn},
  author={de Oliveira Filho, Fernando M{\'a}rio and Vallentin, Frank},
  journal={J. Eur. Math. Soc.},
  volume={12},
  pages={ 1417-1428},
  year={2010},
url={http://www.ems-ph.org/journals/show_abstract.php?issn=1435-9855&vol=12&iss=6&rank=5}
}

@article{W06,
  title = {Tsirelson bounds for generalized Clauser-Horne-Shimony-Holt inequalities},
  author = {Wehner, Stephanie},
  journal = {Phys. Rev. A},
  volume = {73},
  issue = {2},
  pages = {022110},
  numpages = {5},
  year = {2006},
  month = {Feb},
  doi = {10.1103/PhysRevA.73.022110},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.73.022110},
  publisher = {American Physical Society}
}


@Book{Mackeybook,
 author    = "G. W. Mackey",
 title     = "The Mathematical Foundations of Quantum Mechanics",
 publisher = "W. A. Benjamin Inc",
address= "New York",
 year      =  "1963",
}

@article{DL70,
  title = {An operational approach to quantum probability},
  author = {E. B. Davies and J. T. Lewis},
  journal = {Commun. Math. Phys.},
  volume = {17},
number={3},
doi={10.1007/BF01647093},
url={http://dx.doi.org/10.1007/BF01647093},
publisher={Springer-Verlag},
pages={239-260},
year= {1970}
}

@article{E70,
  title = {The operational approach to quantum probability {I}},
  author = {C. M. Edwards},
  journal = {Commun. Math. Phys.},
  volume = {16},
  pages = {207--230},
number={3},
doi={10.1007/BF01646788},
url={http://dx.doi.org/10.1007/BF01646788},
  year = {1970}
}

@INPROCEEDINGS{Foulis81,
   author       = "D. J. Foulis and C. H. Randall",
title = "Empirical logic and tensor products",
   booktitle      = "H. Neumann, (ed.), Interpretations and Foundations of Quantum Theory, Bibliographisches Institut, Wissenschaftsverlag, Mannheim",
      year         = "1981",
}

@Book{Ludwig85,
 author    = "G. Ludwig",
 title     = "An Axiomatic Basis of Quantum Mechanics 1, 2",
 publisher = "Springer--Verlag",
 year      =  "1985, 1987"
}





@article{Chiribella11,
  title = {Informational derivation of quantum theory},
  author = {Chiribella, Giulio and D'Ariano, Giacomo Mauro and Perinotti, Paolo},
  journal = {Phys. Rev. A},
  volume = {84},
  issue = {1},
  pages = {012311},
  numpages = {39},
  year = {2011},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.84.012311},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.84.012311}
}

@article{BPALSNG12,
  title = {Quantum non{-}locality based on finite{-}speed causal influences leads to superluminal signalling},
  author = {J{-}D. Bancal and S. Pironio and A. Ac{\i}n and Y{-}C. Liang and V. Scarani and N. Gisin},
  journal = {Nature Phys.},
  volume = {8},
  pages = {867–870},
  year = {2012},
  doi = {10.1038/nphys2460},
  url = {http://www.nature.com/nphys/journal/v8/n12/full/nphys2460.html}
}




@article{CDP11,
  title = {Informational derivation of quantum theory},
  author = {Chiribella, Giulio and D'Ariano, Giacomo Mauro and Perinotti, Paolo},
  journal = {Phys. Rev. A},
  volume = {84},
  issue = {1},
  pages = {012311},
  numpages = {39},
  year = {2011},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.84.012311},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.84.012311}
}

@article{CBH03,
  title = {Characterizing Quantum Theory in Terms of Information-Theoretic Constraints},
  author = {R. Clifton and J. Bub and H. Halvorson},
  journal = {Found. Phys.},
  volume = {33},
  pages = {1561--1591},
  year = {2003},
  doi = {10.1023/A:1026056716397},
  url = {https://doi.org/10.1023/A:1026056716397}
}

@article{F12,
  title = {Derivation of the Rules of Quantum Mechanics from Information-Theoretic Axioms},
  author = {D.I. Fivel},
  journal = {Found. Phys.},
  volume = {42},
  pages = {291--318},
  year = {2012},
  doi = {10.1007/s10701-011-9603-y},
  url = {https://doi.org/10.1007/s10701-011-9603-y}
}

@article{G08,
  title = {Information-geometric reconstruction of quantum theory},
  author = {Goyal, Philip},
  journal = {Phys. Rev. A},
  volume = {78},
  issue = {5},
  pages = {052120},
  numpages = {17},
  year = {2008},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.78.052120},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.78.052120}
}


@article{FS11,
  title = {A Quantum-Bayesian Route to Quantum-State Space},
  author = {C.A. Fuchs and R. Schack},
  journal = {Found. Phys.},
  volume = {41},
  pages = {345--356},
  year = {2011},
  doi = {10.1007/s10701-009-9404-8},
  url = {https://doi.org/10.1007/s10701-009-9404-8}
}









@article{MM11,
  author={Lluís Masanes and Markus P M\"{u}ller},
  title={A derivation of quantum theory from physical requirements},
  journal={New J. Phys.},
  volume={13},
  number={6},
  pages={063001},
  year={2011},
  abstract={Quantum theory (QT) is usually formulated in terms of abstract mathematical postulates involving Hilbert spaces, state vectors and unitary operators. In this paper, we show that the full formalism of QT can instead be derived from five simple physical requirements, based on elementary assumptions regarding preparations, transformations and measurements. This is very similar to the usual formulation of special relativity, where two simple physical requirements—the principles of relativity and light speed invariance—are used to derive the mathematical structure of Minkowski space–time. Our derivation provides insights into the physical origin of the structure of quantum state spaces (including a group-theoretic explanation of the Bloch ball and its three dimensionality) and suggests several natural possibilities to construct consistent modifications of QT.},
  doi={10.1088/1367-2630/13/6/063001}
}

@Unpublished{MM13,
author = "L. Masanes and M. P. M{\"{u}}ller",
title="Information-theoretic postulates for quantum theory",
year="2013",
eprint = "1203.4516v2",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=1203.4516v2;%%"
}

@Unpublished{FMPT13,
author = "S. Fiorini and S. Massar and M. K. Patra and H. R. Tiwary",
title="Generalised probabilistic theories and conic extensions of polytopes",
year="2013",
eprint = "1310.4125",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=1310.4125;%%"
}

@Unpublished{BKLS14,
author = "N. Brunner and M. Kaplan and A. Leverrier and P. Skrzypczyky",
title="Dimension of physical systems, information processing, and thermodynamics",
year="2014",
eprint = "1401.4488",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=1401.4488;%%"
}

@article{MP14,
  title = {Information and communication in polygon theories},
  author = {Massar, Serge and Patra, Manas K.},
  journal = {Phys. Rev. A},
  volume = {89},
  issue = {5},
  pages = {052124},
  numpages = {8},
  year = {2014},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.89.052124},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.89.052124}
}


@Unpublished{CHHH14,
author = "L. Czekaj and M. Horodecki and P. Horodecki and R. Horodecki",
title="Information Content of Elementary Systems as a Physical Principle",
year="2014",
eprint = "1403.4643",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=1403.4643;%%"
}

@article{H09,
  title = {Superadditivity of communication capacity using entangled inputs},
  author = {M.B. Hastings},
  journal = {Nature Physics},
  volume = {5},
  pages = {255--257},
  year = {2009},
doi={10.1038/nphys1224}
}

@INPROCEEDINGS{BW13,
title ="Post-Classical Probability Theory",
   author       = "H. Barnum and A. Wilce",
booktitle      = "G. Chiribella and R.W. Spekkens, (ed.), Quantum Theory: Informational Foundations and Foils, Springer",
year = "2014",
Note = "{P}ost-Classical Probability Theory. E-print arXiv:1205.3833 (2013).",
url = "http://arxiv.org/abs/1205.3833",
}

@ARTICLE{PDB10,
	author = { T. Paterek and B. Daki\'c and \v{C}. Brukner},
	title = { Theories of systems with limited information content },
	journal = {New J. Phys.},
	year = { 2010 },
	pages = { 053037 },
	volume = { 12 },
doi={10.1088/1367-2630/12/5/053037}
}


@article{PW12,
  title = {``Hyperbits'': The information quasiparticles},
  author = {Paw\l{}owski, Marcin and Winter, Andreas},
  journal = {Phys. Rev. A},
  volume = {85},
  issue = {2},
  pages = {022331},
  numpages = {6},
  year = {2012},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.85.022331},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.85.022331}
}


@article{Z08,
  author={Karol \.{Z}yczkowski},
  title={Quartic quantum theory: an extension of the standard quantum mechanics},
  journal={J. Phys. A: Math. Theor.},
  volume={41},
  number={35},
  pages={355302},
  url={http://stacks.iop.org/1751-8121/41/i=35/a=355302},
  year={2008},
  abstract={We propose an extended quantum theory, in which the number K of parameters necessary to characterize a quantum state behaves as fourth power of the number N of distinguishable states. As the simplex of classical N -point probability distributions can be embedded inside a higher-dimensional convex body ##IMG## [http://ej.iop.org/images/1751-8121/41/35/355302/jpa278068ieqn1.gif] {{\cal M}_N^Q} of mixed quantum states, one can further increase the dimensionality constructing the set of extended quantum states. The embedding proposed corresponds to an assumption that the physical system described in the N -dimensional Hilbert space is coupled with an auxiliary subsystem of the same dimensionality. The extended theory works for simple quantum systems and is shown to be a non-trivial generalization of the standard quantum theory for which K = N 2 . Imposing certain restrictions on initial conditions and dynamics allowed in the quartic theory one obtains quadratic theory as a special case. By imposing even stronger constraints one arrives at the classical theory, for which K = N .}
}
	
@article{U96,
author={A. Uhlmann},
title={Spheres and hemispheres as quantum state spaces},
journal={J. Geom. Phys.},
volume={18},
pages={76-92},
url = {http://www.sciencedirect.com/science/article/pii/0393044095000046},
year={1996}
}


@INPROCEEDINGS{DB09,
   author       = "B. Daki\'c and \v{C}. Brukner",
title = "Quantum Theory and Beyond: Is Entanglement Special?",
   booktitle      = "H. Halvorson, (ed.), Deep Beauty: Understanding the Quantum World through Mathematical Innovation, Cambridge University Press",
      year         = "2011",
pages= "365--392",
Note= "E-print arXiv:0911.0695 (2009).",
url = "http://arxiv.org/abs/0911.0695"
}




@INPROCEEDINGS{BBLW08,
   author = "H. Barnum and J. Barrett and M. Leifer and A. Wilce",
title = "Teleportation in General Probabilistic Theories",
year = "2012",
   booktitle      = "Proceedings of Symposia in Applied Mathematics",
      volume = "71",
pages= "25--48",
Note= "E-print arXiv:0805.3553.",
url = "http://arxiv.org/abs/0805.3553"
}

@Book{CTbook,
 author    = "T. M. Cover and J. A. Thomas",
 title     = "Elements of Information Theory",
 publisher = "John Wiley & Sons",
address= "New Jersey",
 year      =  2006,
}

@article{JL13,
  title = {Generalized probabilistic theories without the no-restriction hypothesis},
  author = {Janotta, Peter and Lal, Raymond},
  journal = {Phys. Rev. A},
  volume = {87},
  issue = {5},
  pages = {052131},
  numpages = {14},
  year = {2013},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.87.052131},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.87.052131}
}

@article{BDFMRSSW99,
  title = {Quantum nonlocality without entanglement},
  author = {Bennett, Charles H. and DiVincenzo, David P. and Fuchs, Christopher A. and Mor, Tal and Rains, Eric and Shor, Peter W. and Smolin, John A. and Wootters, William K.},
  journal = {Phys. Rev. A},
  volume = {59},
  issue = {2},
  pages = {1070--1091},
  numpages = {0},
  year = {1999},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.59.1070},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.59.1070}
}

	
@article{SB10,
  author={Anthony J Short and Jonathan Barrett},
  title={Strong nonlocality: a trade-off between states and measurements},
  journal={New J. Phys.},
  volume={12},
  number={3},
  pages={033034},
  url={http://stacks.iop.org/1367-2630/12/i=3/a=033034},
  year={2010},
  abstract={Measurements on entangled quantum states can produce outcomes that are nonlocally correlated. But according to Tsirelson's theorem, there is a quantitative limit on quantum nonlocality. It is interesting to explore what would happen if Tsirelson's bound were violated. To this end, we consider a model that allows arbitrary nonlocal correlations, colloquially referred to as 'box world'. We show that while box world allows more highly entangled states than quantum theory, measurements in box world are rather limited. As a consequence there is no entanglement swapping, teleportation or dense coding.}
}
@article{KBBM17,
	doi = {10.1088/1367-2630/aa68ef},
	url = {https://doi.org/10.1088/1367-2630/aa68ef},
	year = 2017,
	month = {apr},
	publisher = {{IOP} Publishing},
	volume = {19},
	number = {4},
	pages = {043025},
	author = {Marius Krumm and Howard Barnum and Jonathan Barrett and Markus P Müller},
	title = {Thermodynamics and the structure of quantum theory},
	journal = {New J. Phys.},
	abstract = {Despite its enormous empirical success, the formalism of quantum theory still raises fundamental questions: why is nature described in terms of complex Hilbert spaces, and what modifications of it could we reasonably expect to find in some regimes of physics? Here we address these questions by studying how compatibility with thermodynamics constrains the structure of quantum theory. We employ two postulates that any probabilistic theory with reasonable thermodynamic behaviour should arguably satisfy. In the framework of generalised probabilistic theories, we show that these postulates already imply important aspects of quantum theory, like self-duality and analogues of projective measurements, subspaces and eigenvalues. However, they may still admit a class of theories beyond quantum mechanics. Using a thought experiment by von Neumann, we show that these theories admit a consistent thermodynamic notion of entropy, and prove that the second law holds for projective measurements and mixing procedures. Furthermore, we study additional entropy-like quantities based on measurement probabilities and convex decomposition probabilities, and uncover a relation between one of these quantities and Sorkin’s notion of higher-order interference.}
}

@article{SS20,
  title = {Impossibility of coin flipping in generalized probabilistic theories via discretizations of semi-infinite programs},
  author = {Sikora, Jamie and Selby, John H.},
  journal = {Phys. Rev. Research},
  volume = {2},
  issue = {4},
  pages = {043128},
  numpages = {7},
  year = {2020},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevResearch.2.043128},
  url = {https://link.aps.org/doi/10.1103/PhysRevResearch.2.043128}
}


@article{SY08,
  author={Graeme Smith and Jon Yard},
  title={Quantum Communication with Zero-Capacity Channels},
  journal={Science},
  volume={321},
  number={5897},
  pages={1812-1815},
doi={10.1126/science.1162242},
  url={http://www.sciencemag.org/content/321/5897/1812},
  year={2008}
}



@article{ZZHE93,
  title = {``Event-ready-detectors'' Bell experiment via entanglement swapping},
  author = {\ifmmode \dot{Z}\else \.{Z}\fi{}ukowski, M. and Zeilinger, A. and Horne, M. A. and Ekert, A. K.},
  journal = {Phys. Rev. Lett.},
  volume = {71},
  issue = {26},
  pages = {4287--4290},
  numpages = {0},
  year = {1993},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.71.4287},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.71.4287}
}

@article{JGBB11,
  author={Peter Janotta and Christian Gogolin and Jonathan Barrett and Nicolas Brunner},
  title={Limits on nonlocal correlations from the structure of the local state space},
  journal={New J. Phys.},
  volume={13},
  number={6},
  pages={063024},
  url={http://stacks.iop.org/1367-2630/13/i=6/a=063024},
  year={2011},
  abstract={The outcomes of measurements on entangled quantum systems can be nonlocally correlated. However, while it is easy to write down toy theories allowing arbitrary nonlocal correlations, those allowed in quantum mechanics are limited. Quantum correlations cannot, for example, violate a principle known as macroscopic locality, which implies that they cannot violate Tsirelson's bound. This paper shows that there is a connection between the strength of nonlocal correlations in a physical theory and the structure of the state spaces of individual systems. This is illustrated by a family of models in which local state spaces are regular polygons, where a natural analogue of a maximally entangled state of two systems exists. We characterize the nonlocal correlations obtainable from such states. The family allows us to study the transition between classical, quantum and super-quantum correlations by varying only the local state space. We show that the strength of nonlocal correlations—in particular whether the maximally entangled state violates Tsirelson's bound or not—depends crucially on a simple geometric property of the local state space, known as strong self-duality. This result is seen to be a special case of a general theorem, which states that a broad class of entangled states in probabilistic theories—including, by extension, all bipartite classical and quantum states—cannot violate macroscopic locality. Finally, our results show that models exist that are locally almost indistinguishable from quantum mechanics, but can nevertheless generate maximally nonlocal correlations.}
}



@article{BLMPPR05,
  title = {Nonlocal correlations as an information-theoretic resource},
  author = {Barrett, Jonathan and Linden, Noah and Massar, Serge and Pironio, Stefano and Popescu, Sandu and Roberts, David},
  journal = {Phys. Rev. A},
  volume = {71},
  issue = {2},
  pages = {022101},
  numpages = {11},
  year = {2005},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.71.022101},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.71.022101}
}


@article{AACHKLMP10,
  title = {Unified Framework for Correlations in Terms of Local Quantum Observables},
  author = {Ac\'in, A. and Augusiak, R. and Cavalcanti, D. and Hadley, C. and Korbicz, J. K. and Lewenstein, M. and Masanes, Ll. and Piani, M.},
  journal = {Phys. Rev. Lett.},
  volume = {104},
  issue = {14},
  pages = {140404},
  numpages = {4},
  year = {2010},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.104.140404},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.104.140404}
}

@article{TMSM12,
  title = {Deriving Quantum Theory from Its Local Structure and Reversibility},
  author = {de la Torre, Gonzalo and Masanes, Llu\'\is and Short, Anthony J. and M{\"{u}}ller, Markus P.},
  journal = {Phys. Rev. Lett.},
  volume = {109},
  issue = {9},
  pages = {090403},
  numpages = {5},
  year = {2012},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.109.090403},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.109.090403}
}

@Book{StoneGoldbartbook,
 author    = "M. Stone and P. Goldbart",
 title     = "Mathematics for Physics",
 publisher = "Cambridge University Press",
address= " Cambridge",
 year      =  2009,
}

@Book{WeinbergQMbook,
 author    = "S. Weinberg",
 title     = "Lectures on Quantum Mechanics",
 publisher = "Cambridge University Press",
address= " Cambridge",
 year      =  "2013",
}

@Book{Weinbergbook,
 author    = "S. Weinberg",
 title     = "The Quantum Theory of Fields",
volume="I",
 publisher = "Cambridge University Press",
address= " Cambridge",
 year      =  1995,
}

@article{W39,
  title = {On Unitary Representations of the Inhomogeneous Lorentz Group},
  author = {E. Wigner},
  journal = {Ann. Math.},
  volume = {40},
  issue = {1},
  pages = {149-204},
  year = {1939},
}

@Book{Naimarkbook,
 author    = "M. A. Naimark",
 title     = "Linear representations of the Lorentz group",
 publisher = "Pergamon Press",
address= " Oxford",
 year      =  1964,
Note= "Translated from Russian by A. Swinfen and O. J. Marstrand. Translation edited by H. K. Farahat",
}

@article{BBBEW10,
  title = {Local Quantum Measurement and No-Signaling Imply Quantum Correlations},
  author = {Barnum, H. and Beigi, S. and Boixo, S. and Elliott, M. B. and Wehner, S.},
  journal = {Phys. Rev. Lett.},
  volume = {104},
  issue = {14},
  pages = {140401},
  numpages = {4},
  year = {2010},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.104.140401},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.104.140401}
}

@Article{H17.2,
AUTHOR = {H\"{o}hn, Philipp Andres},
TITLE = {Quantum Theory from Rules on Information Acquisition},
JOURNAL = {Entropy},
VOLUME = {19},
YEAR = {2017},
NUMBER = {3},
ARTICLE-NUMBER = {98},
URL = {https://www.mdpi.com/1099-4300/19/3/98},
ISSN = {1099-4300},
ABSTRACT = {We summarize a recent reconstruction of the quantum theory of qubits from rules constraining an observer’s acquisition of information about physical systems. This review is accessible and fairly self-contained, focusing on the main ideas and results and not the technical details. The reconstruction offers an informational explanation for the architecture of the theory and speciﬁcally for its correlation structure. In particular, it explains entanglement, monogamy and non-locality compellingly from limited accessible information and complementarity. As a by-product, it also unravels new ‘conserved informational charges’ from complementarity relations that characterize the unitary group and the set of pure states.},
DOI = {10.3390/e19030098}
}

@article{HW17,
  title = {Quantum theory from questions},
  author = {H\"ohn, Philipp Andres and Wever, Christopher S. P.},
  journal = {Phys. Rev. A},
  volume = {95},
  issue = {1},
  pages = {012102},
  numpages = {38},
  year = {2017},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.95.012102},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.95.012102}
}

@article{N20,
  title = {Derivation of quantum theory with superselection rules},
  author = {Nakahira, Kenji},
  journal = {Phys. Rev. A},
  volume = {101},
  issue = {2},
  pages = {022104},
  numpages = {27},
  year = {2020},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.101.022104},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.101.022104}
}


@article{R09,
title = "On quantum vs. classical probability",
journal = "Ann. Phys.",
volume = "324",
number = "12",
pages = "2622 - 2637",
year = "2009",
issn = "0003-4916",
doi = "https://doi.org/10.1016/j.aop.2009.09.013",
url = "http://www.sciencedirect.com/science/article/pii/S0003491609001882",
author = "Jochen Rau",
keywords = "Foundations of quantum theory, Probability theory, Reconstruction",
abstract = "Quantum theory shares with classical probability theory many important properties. I show that this common core regards at least the following six areas, and I provide details on each of these: the logic of propositions, symmetry, probabilities, composition of systems, state preparation and reductionism. The essential distinction between classical and quantum theory, on the other hand, is shown to be joint decidability versus smoothness; for the latter in particular I supply ample explanation and motivation. Finally, I argue that beyond quantum theory there are no other generalisations of classical probability theory that are relevant to physics."
}

@article{H17,
  doi = {10.22331/q-2017-12-14-38},
  url = {https://doi.org/10.22331/q-2017-12-14-38},
  title = {Toolbox for reconstructing quantum theory from rules on information  acquisition},
  author = {H{\"{o}}hn, Philipp Andres},
  journal = {{Quantum}},
  issn = {2521-327X},
  publisher = {{Verein zur F{\"{o}}rderung des Open Access Publizierens in den Quantenwissenschaften}},
  volume = {1},
  pages = {38},
  month = dec,
  year = {2017}
}




@article{R11,
  doi = {10.1007/s10701-010-9427-1},
  url = {https://doi.org/10.1007/s10701-010-9427-1},
  title = {Measurement-Based Quantum Foundations},
  author = {J. Rau},
  journal = {Found. Phys.},
  volume = {41},
  pages = {380--388},
  year = {2011}
}


@Unpublished{H13,
author = "L. Hardy",
title = "Reconstructing quantum theory",
year = "2013",
eprint = "1303.1538",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=1303.1538;%%",
}

@Unpublished{SSC18,
author = "J. H. Selby and C. M. Scandolo and B. Coecke",
title = "Reconstructing quantum theory from diagrammatic postulates",
year = "2018",
eprint = "1802.00367 ",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=1802.00367 ;%%",
}

@article{T20,
  TITLE = {A Categorical Reconstruction of Quantum Theory},
  AUTHOR = {Tull, Sean},
  URL = {https://lmcs.episciences.org/6035},
    DOI = {10.23638/LMCS-16(1:4)2020},
  JOURNAL = {Logical Methods in Computer Science},
  VOLUME = {16},
  YEAR = {2020},
  MONTH = {Jan},
  KEYWORDS = {Quantum Physics ; Computer Science - Logic in Computer Science ; Mathematics - Category Theory},
}

  
  
  
@article{vdW19,
  doi = {10.32408/compositionality-1-1},
  url = {https://doi.org/10.32408/compositionality-1-1},
  title = {An effect-theoretic reconstruction of quantum theory},
  author = {Wetering, John van de},
  journal = {{Compositionality}},
  issn = {2631-4444},
  publisher = {{Compositionality}},
  volume = {1},
  issue = {1},
  month = dec,
  year = {2019}
}

@article{W19,
  doi = {10.22331/q-2019-07-08-158},
  url = {https://doi.org/10.22331/q-2019-07-08-158},
  title = {Conjugates, {F}ilters and {Q}uantum {M}echanics},
  author = {Wilce, Alexander},
  journal = {{Quantum}},
  issn = {2521-327X},
  publisher = {{Verein zur F{\"{o}}rderung des Open Access Publizierens in den Quantenwissenschaften}},
  volume = {3},
  pages = {158},
  month = jul,
  year = {2019}
}

@Unpublished{H11,
author = "L. Hardy",
title = "Reformulating and Reconstructing Quantum Theory",
year = "2011",
eprint = "1104.2066",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=1104.2066;%%",
}

@article{BN36,
  title = {The Logic of Quantum Mechanics},
  author = {G. Birkhoff and J. {von Neumann}},
  journal = {Ann. Math.},
  volume = {37},
  pages = {823},
  year = {1936},
}

@article{JP63,
  title = {Can hidden variables be excluded in quantum mechanics?},
  author = {J. M. Jauch and C. Piron},
  journal = { Helv. Phys. Acta},
  volume = {36},
  pages = {827},
  year = {1963},
}



  	
@article{MM13.1,
  author={M. P. M\"{u}ller and L. Masanes},
  title={Three-dimensionality of space and the quantum bit: an information-theoretic approach},
  journal={New J. Phys.},
  volume={15},
  number={5},
  pages={053040},
  url={http://stacks.iop.org/1367-2630/15/i=5/a=053040},
  year={2013},
  abstract={It is sometimes pointed out as a curiosity that the state space of quantum two-level systems, i.e. the qubit, and actual physical space are both three-dimensional and Euclidean. In this paper, we suggest an information-theoretic analysis of this relationship, by proving a particular mathematical result: suppose that physics takes place in d spatial dimensions, and that some events happen probabilistically (not assuming quantum theory in any way). Furthermore, suppose there are systems that carry ‘minimal amounts of direction information’, interacting via some continuous reversible time evolution. We prove that this uniquely determines spatial dimension d = 3 and quantum theory on two qubits (including entanglement and unitary time evolution), and that it allows observers to infer local spatial geometry from probability measurements.}
}
	



@article{HM14,
author = "Philipp A. Hoehn and Markus P. Mueller",
title = "An operational approach to spacetime symmetries: Lorentz transformations from quantum communication",
year = "2016",
journal = "New J. Phys.",
volume = "18",
pages = " 063026",
doi = "10.1088/1367-2630/18/6/063026"
}

@Unpublished{GMD14,
author = "Andrew J. P. Garner and Markus P. Mueller and Oscar C. O. Dahlsten",
title = "The quantum bit from relativity of simultaneity on an interferometer",
year = "2014",
eprint = "1412.7112",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=1412.7112;%%",
}

@article{LB15,
	doi = {10.1088/1367-2630/17/8/083001},
	url = {https://doi.org/10.1088/1367-2630/17/8/083001},
	year = 2015,
	month = {aug},
	publisher = {{IOP} Publishing},
	volume = {17},
	number = {8},
	pages = {083001},
	author = {Ciar{\'{a}}n M Lee and Jonathan Barrett},
	title = {Computation in generalised probabilisitic theories},
	journal = {New J. Phys.},
	abstract = {From the general difficulty of simulating quantum systems using classical systems, and in particular the existence of an efficient quantum algorithm for factoring, it is likely that quantum computation is intrinsically more powerful than classical computation. At present, the best upper bound known for the power of quantum computation is that , where is a classical complexity class (known to be included in , hence ). This work investigates limits on computational power that are imposed by simple physical, or information theoretic, principles. To this end, we define a circuit-based model of computation in a class of operationally-defined theories more general than quantum theory, and ask: what is the minimal set of physical assumptions under which the above inclusions still hold? We show that given only an assumption of tomographic locality (roughly, that multipartite states and transformations can be characterized by local measurements), efficient computations are contained in . This inclusion still holds even without assuming a basic notion of causality (where the notion is, roughly, that probabilities for outcomes cannot depend on future measurement choices). Following Aaronson, we extend the computational model by allowing post-selection on measurement outcomes. Aaronson showed that the corresponding quantum complexity class, , is equal to . Given only the assumption of tomographic locality, the inclusion in still holds for post-selected computation in general theories. Hence in a world with post-selection, quantum theory is optimal for computation in the space of all operational theories. We then consider whether one can obtain relativized complexity results for general theories. It is not obvious how to define a sensible notion of a computational oracle in the general framework that reduces to the standard notion in the quantum case. Nevertheless, it is possible to define computation relative to a ‘classical oracle’. Then, we show there exists a classical oracle relative to which efficient computation in any theory satisfying the causality assumption does not include .}
}

@article{GMD17,
author = {Andrew J. P. Garner and Markus P. M\"{u}ller and Oscar C. O. Dahlsten},
title = {The complex and quaternionic quantum bit from relativity of simultaneity on an interferometer},
year = {2017},
journal = {Proc. R. Soc. A},
  volume = {473},
doi={10.1098/rspa.2017.0596},
pages={20170596}
}

@article{DL70,
  title = {An operational approach to quantum probability},
  author = {E. B. Davies and J. T. Lewis},
  journal = {Commun. Math. Phys.},
  volume = {17},
number={3},
doi={10.1007/BF01647093},
url={http://dx.doi.org/10.1007/BF01647093},
publisher={Springer-Verlag},
pages={239-260},
year= {1970}
}




@book{CDW75,
   author = "L. Castell and M. Drieschner and {C. F. von }Weizs{\"{a}}cker",
   title = "Quantum Theory and the Structures of Time and Space: Papers Presented at a Conference Held in Feldafing, July 1974",
   year = "1975",
   publisher = "{C}. {H}anser"
}

@book{Hartlebook,
   author = "James B. Hartle",
   title = "Gravity: An Introduction to Einstein's General Relativity",
   year = "2003",
   publisher = "Addison-Wesley"
}


@article{H07,
  author={Lucien Hardy},
  title={Towards quantum gravity: a framework for probabilistic theories with non-fixed causal structure},
  journal={J. Phys. A},
  volume={40},
  number={12},
  pages={3081},
  url={http://stacks.iop.org/1751-8121/40/i=12/a=S12},
  year={2007},
  abstract={General relativity is a deterministic theory with non-fixed causal structure. Quantum theory is a probabilistic theory with fixed causal structure. In this paper, we build a framework for probabilistic theories with non-fixed causal structure. This combines the radical elements of general relativity and quantum theory. We adopt an operational methodology for the purposes of theory construction (though without committing to operationalism as a fundamental philosophy). The key idea in the construction is physical compression . A physical theory relates quantities. Thus, if we specify a sufficiently large set of quantities (this is the compressed set), we can calculate all the others. We apply three levels of physical compression. First, we apply it locally to quantities (actually probabilities) that might be measured in a particular region of spacetime. Then we consider composite regions. We find that there is a second level of physical compression for a composite region over and above the first level physical compression for the component regions. Each application of first and second level physical compression is quantified by a matrix. We find that these matrices themselves are related by the physical theory and can therefore be subject to compression. This is the third level of physical compression. The third level of physical compression gives rise to a new mathematical object which we call the causaloid. From the causaloid for a particular physical theory we can calculate everything the physical theory can calculate. This approach allows us to set up a framework for calculating probabilistic correlations in data without imposing a fixed causal structure (such as a background time). We show how to put quantum theory in this framework (thus providing a new formulation of this theory). We indicate how general relativity might be put into this framework and how the framework might be used to construct a theory of quantum gravity.}
}


@article{BMU14,
  author={Howard Barnum and Markus P M\"{u}ller and Cozmin Ududec},
  title={Higher-order interference and single-system postulates characterizing quantum theory},
  journal={New J. Phys.},
  volume={16},
  number={12},
  pages={123029},
  url={http://stacks.iop.org/1367-2630/16/i=12/a=123029},
  year={2014},
  abstract={We present a new characterization of quantum theory in terms of simple physical principles that is different from previous ones in two important respects: first, it only refers to properties of single systems without any assumptions on the composition of many systems; and second, it is closer to experiment by having absence of higher-order interference as a postulate, which is currently the subject of experimental investigation. We give three postulates—no higher-order interference, classical decomposability of states, and strong symmetry—and prove that the only non-classical operational probabilistic theories satisfying them are real, complex, and quaternionic quantum theory, together with three-level octonionic quantum theory and ball state spaces of arbitrary dimension. Then we show that adding observability of energy as a fourth postulate yields complex quantum theory as the unique solution, relating the emergence of the complex numbers to the possibility of Hamiltonian dynamics. We also show that there may be interesting non-quantum theories satisfying only the first two of our postulates, which would allow for higher-order interference in experiments while still respecting the contextuality analogue of the local orthogonality principle.}
}




@Unpublished{H16,
author = "L. Hardy",
title = "Operational General Relativity: Possibilistic, Probabilistic, and Quantum",
year = "2016",
eprint = "1608.06940",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1608.06940;%%",
}

@Unpublished{Z12,
author = "M. Zaopo",
title = "Information Theoretic Axioms for Quantum Theory",
year = "2012",
eprint = "1205.2306",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1205.2306;%%",
}


@Book{LandauLifshitzbook,
 author    = "L. D. Landau and E. M. Lifshitz",
 title     = "The Classical Theory of Fields",
 publisher = "Pergamon Press",
address= "Oxford, UK",
 year      =  1971,
 pages = {1 -- 5},
 edition = {Third Revised English} 
}



@Book{WeinbergGravitationandCosmologybook,
 author    = "S. Weinberg",
 title     = "Gravitation and Cosmology: Principles
and Applications of the General Theory of Relativity",
 publisher = "John Wiley and Sons",
address= "New York, USA",
 year      =  1972,
 pages = {25 -- 28},
}

@article{MPP15,
  author={Serge Massar and Stefano Pironio and Dami\'an Pital\'ua{-}Garc\'ia},
  title={Hyperdense coding and superadditivity of classical capacities in hypersphere theories},
  journal={New J. Phys.},
  volume={17},
  number={11},
  pages={113002},
  url={http://stacks.iop.org/1367-2630/17/i=11/a=113002},
  year={2015}
}













%References from PhD thesis
%INTRO CHAPTER
@ARTICLE{S48,
   author       = "C. E. Shannon",
title = "A mathematical theory of communication",
   journal      = "The Bell System Technical Journal",
   volume       = "27(3-4)", 
   pages        = "379-423,623-656",
   year         = "1948",
url = "http://www3.alcatel-lucent.com/bstj/vol27-1948/bstj-vol27-issue03.html",
url2 = "http://www3.alcatel-lucent.com/bstj/vol27-1948/bstj-vol27-issue04.html",
}

@ARTICLE{T37,
   author       = "A. M. Turing",
title = "On computable numbers, with an application to the {E}ntscheidungsproblem",
   journal      = "Proceedings of the London Mathematical Society ",
   volume       = "s2-42(1)", 
   pages        = "230-265",
   year         = "1937",
url = "http://plms.oxfordjournals.org/content/s2-42/1/230.full.pdf+html"
}

@phdthesis{DPGthesis,
author={Pital\'ua{-}Garc\'ia, Dami\'an},
title={Quantum Information, Bell Inequalities and the No{-}Signalling Principle},
school={University of Cambridge},
year={2014},
url={https://www.repository.cam.ac.uk/handle/1810/245205}
}

@phdthesis{DLthesis,
author={D. L. D. Lowndes},
title={Low Cost, Short Range Free Space Quantum Cryptography for Consumer Applications: Pocket Size for Pocket Change},
school={University of Bristol},
year={2014},
url={http://hdl.handle.net/1983/bf48d846-d4c2-4838-92b3-5fb75bfd1cae}
}

@article{MSDS10,
title = {Coherence characteristics of light-emitting diodes},
journal = {J. Lumin.},
volume = {130},
number = {1},
pages = {96-102},
year = {2010},
issn = {0022-2313},
doi = {https://doi.org/10.1016/j.jlumin.2009.07.027},
url = {https://www.sciencedirect.com/science/article/pii/S0022231309003871},
author = {Dalip Singh Mehta and Kanchan Saxena and Satish Kumar Dubey and Chandra Shakher},
keywords = {Light-emitting diodes, Optical coherence},
abstract = {We report the measurement of coherence characteristics of light-emitting diodes (LEDs). Experiments were performed using red and green color LEDs directly illuminating the Young's double slit kept in the far-zone. Fourier transform fringe analysis technique was used for the measurement of the visibility of interference fringes from which the modulus of degree of spectral coherence was determined. Low degree of spectral coherence, typically 0.4 for red and 0.2 for green LED with double-slit separation of 400μm was observed. A variable slit was then kept in front of the LEDs and the double slit was illuminated with the light coming out of the slit. Experiments were performed with various slit sizes and the visibility of the interference fringes was observed. It was found that visibility of the interference fringes changes drastically in presence of variable slit kept in front of LEDs and a high degree of spectral coherence, typically 0.85 for red and 0.8 for green LED with double-slit separation of 400μm and rectangular slit opening of 500μm was observed. The experimental results are compared with the theoretical counterparts. Coherence lengths of both the LEDs were also determined and it was obtained 5.8±2 and 24±4μm for green and red LEDs, respectively.}
}

@INPROCEEDINGS{NDR11,
  author={R. {Nock} and N. {Dahnoun} and J. {Rarity}},
  booktitle={2011 IEEE International Instrumentation and Measurement Technology Conference}, 
  title={Low cost timing interval analyzers for quantum key distribution}, 
  year={2011},
  volume={},
  number={},
  pages={1-5},
  doi={10.1109/IMTC.2011.5944324}}

@inproceedings{MVRCCOW16,
author = {Gwenaelle M\'{e}len and Tobias Vogl and Markus Rau and Giacomo Corrielli and Andrea Crespi and Roberto Osellame and Harald Weinfurter},
title = {{Integrated quantum key distribution sender unit for daily-life implementations}},
volume = {9762},
booktitle = {Advances in Photonics of Quantum Computing, Memory, and Communication IX},
editor = {Zameer Ul Hasan and Philip R. Hemmer and Hwang Lee and Alan L. Migdall},
organization = {International Society for Optics and Photonics},
publisher = {SPIE},
pages = {31 -- 36},
keywords = {Quantum Key Distribution, Handheld devices, Smartphone, Integrated optics,  Vertical cavity surface emitting lasers, Optical transmitters, Vertical-cavity surface-emitting lasers},
year = {2016},
doi = {10.1117/12.2208643},
URL = {https://doi.org/10.1117/12.2208643}
}

@inproceedings{MFLVRSRW17,
author = {Gwenaelle M\'{e}len and Peter Freiwang and Jannik Luhn and Tobias Vogl and Markus Rau and Clemens Sonnleitner and Wenjamin Rosenfeld and Harald Weinfurter},
booktitle = {Quantum Information and Measurement (QIM) 2017},
journal = {Quantum Information and Measurement (QIM) 2017},
keywords = {Coupling efficiency; Laser beams; Optical systems; Quantum key distribution; Spatial filtering; Wire grid polarizers},
pages = {QT6A.57},
publisher = {Optical Society of America},
title = {Handheld Quantum Key Distribution},
year = {2017},
url = {http://www.osapublishing.org/abstract.cfm?URI=QIM-2017-QT6A.57},
doi = {10.1364/QIM.2017.QT6A.57},
abstract = {We present Quantum Key Distribution in handheld operation over short distances between a mobile integrated sender unit and a tracking receiver, achieving, with a QBER below 2\%, a secure bit rate of several 10 kBit/s.},
}

@article{HPLG07,
title = {On the Poisson approximation to photon distribution for faint lasers},
journal = {Phys. Lett. A},
volume = {367},
number = {3},
pages = {173-176},
year = {2007},
issn = {0375-9601},
doi = {https://doi.org/10.1016/j.physleta.2007.03.004},
url = {https://www.sciencedirect.com/science/article/pii/S0375960107003660},
author = {Yucheng Hu and Xiang Peng and Tiejun Li and Hong Guo},
abstract = {The photon number statistics for attenuated faint laser pulses is quantitatively studied. It confirms that, even for a non-Poissonian laser source, after being attenuated into faint laser with ultra-low mean photon number, the photon number distribution would approximately be a Poisson distribution. The error of such an approximation is estimated, and numerical tests verify our theoretical analysis. This work lays a sound mathematical foundation for the well-known intuitive idea which has been widely used in quantum cryptography.}
}


@article{CCFCBGCNWOB17,
author = {Hyunchae Chun and Iris Choi and Grahame Faulkner and Larry Clarke and Bryan Barber and Glenn George and Colin Capon and Antti Niskanen and Joachim Wabnig and Dominic O'Brien and David Bitauld},
journal = {Opt. Express},
keywords = {Quantum communications ; Quantum cryptography ; High throughput optics; Narrow band filters; Photon polarization; Position sensing; Pulse generation; Quantum key distribution},
number = {6},
pages = {6784--6795},
publisher = {OSA},
title = {Handheld free space quantum key distribution with dynamic motion compensation},
volume = {25},
month = {Mar},
year = {2017},
url = {http://www.opticsexpress.org/abstract.cfm?URI=oe-25-6-6784},
doi = {10.1364/OE.25.006784},
abstract = {Mobile devices have become an inseparable part of our everyday life. They are used to transmit an ever-increasing amount of sensitive health, financial and personal information. This exposes us to the growing scale and sophistication of cyber-attacks. Quantum Key Distribution (QKD) can provide unconditional and future-proof data security but implementing it for handheld mobile devices comes with specific challenges. To establish security, secret keys of sufficient length need to be transmitted during the time of a handheld transaction (~1s) despite device misalignment, ambient light and user\&\#x2019;s inevitable hand movements. Transmitters and receivers should ideally be compact and low-cost, while avoiding security loopholes. Here we demonstrate the first QKD transmission from a handheld transmitter with a key-rate large enough to overcome finite key effects. Using dynamic beam-steering, reference-frame-independent encoding and fast indistinguishable pulse generation, we obtain a secret key rate above 30kb/s over a distance of 0.5m.},
}




@Book{Bohmbook,
 author    = "D. Bohm",
 title     = "Quantum Theory",
 publisher = "Prentice-Hall",
address= "New York",
 year      =  1951,
}

@Book{Waldbook,
 author    = "R. M. Wald",
 title     = "General Relativity",
 publisher = "The University of Chicago Press",
address= "Chicago",
 year      =  1984,
}

@Book{Schutzbook,
 author    = "B. Schutz",
 title     = "A first course in general relativity",
 publisher = "Cambridge University Press",
address= "Cambridge",
 year      =  2009,
}




@Book{Bohmbook2,
 author    = "D. Bohm",
 title     = "The Special Theory of Relativity",
 publisher = "W. A. Benjamin",
address= "New York",
 year      =  1965,
}

@ARTICLE{B80,
   author       = "P. Benioff",
title = "The Computer as a physical system: A microscopic quantum mechanical {H}amiltonian model of computers as represented by {T}uring machines",
   journal      = "Journal of Statistical Physics",
   volume       = "22(5)", 
   pages        = "563-591",
   year         = "1980",
url = "http://link.springer.com/article/10.1007/BF01011339"
}

@ARTICLE{B82,
   author       = "P. Benioff",
title = "Quantum mechanical {H}amiltonian models of {T}uring machines",
   journal      = "Journal of Statistical Physics",
   volume       = "29(3)", 
   pages        = "515-546",
   year         = "1982",
url = "http://link.springer.com/article/10.1007/BF01342185"
}

@ARTICLE{B82.1,
   author       = "P. Benioff",
title = "Quantum mechanical models of {T}uring machines that dissipate no energy",
   journal      = "Physical Review Letters",
   volume       = "48(23)", 
   pages        = "1581-1585",
   year         = "1982",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.48.1581"
}

@ARTICLE{F82,
   author       = "R. P. Feynman",
title = "Simulating physics with computers",
   journal      = "International Journal of Theoretical Physics",
   volume       = "21(6-7)", 
   pages        = "467-488",
   year         = "1982",
url = "http://link.springer.com/article/10.1007/BF02650179"
}

@INPROCEEDINGS{BBBW82,
   author       = "C. H. Bennett and G. Brassard and S. Breidbart and S. Wiesner",
title = "Quantum cryptography, or unforgeable subway tokens",
   booktitle      = "Advances in cryptology: Proceedings of CRYPTO 82",
   pages       = "267--275", 
 publisher       = "Plenum Press",
address= "New York",
   year         = "1983",
url = "https://doi.org/10.1007/978-1-4757-0602-4_26"
}

@ARTICLE{D85,
   author       = "D. Deutsch",
title = "Quantum theory, the {C}hurch-{T}uring principle and the universal quantum computer",
   journal      = "Proceedings of the Royal Society of London A",
   volume       = "400(1818)", 
   pages        = "97-117",
   year         = "1985",
url = "http://rspa.royalsocietypublishing.org/content/400/1818/97.abstract"
}

@ARTICLE{F86,
   author       = "R. P. Feynman",
title = "Quantum mechanical computers",
   journal      = "Foundations of Physics",
   volume       = "16(6)", 
   pages        = "507-531",
   year         = "1986",
Note = "Originally appeared in {\emph{Optics News}}, February 1985",
url = "http://link.springer.com/article/10.1007/BF01886518"
}



@ARTICLE{DJ92,
   author       = "D. Deutsch and R. Jozsa",
title = "Rapid solution of problems by quantum computation",
   journal      = "Proceedings of the Royal Society of London A",
   volume       = "439(1907)", 
   pages        = "553-558",
   year         = "1992",
url = "http://rspa.royalsocietypublishing.org/content/439/1907/553#related-urls"
}

@INPROCEEDINGS{S94,
   author       = "P. W. Shor",
title = "Algorithms for quantum computation: Discrete logarithms and factoring",
   booktitle      = "Proceedings of the 35th Annual Symposium on Foundations of Computer Science",
   pages       = "124--134", 
 publisher       = "IEEE Computer Society Press",
address= "Los Alamitos, California",
   year         = "1994",
doi = "10.1109/SFCS.1994.365700 ",
}

@INPROCEEDINGS{ATVY00,
   author       = "D. Aharonov and A. Ta-Shma and U. Vazirani and A.Yao",
title = "Quantum bit escrow",
   booktitle      = "Proceedings of the 32nd ACM Symposium on Theory of Computing",
   pages       = "705--714", 
 publisher       = "ACM",
address= "New York, USA",
   year         = "2000",
doi = "10.1145/335305.335404",
}

@article{SR02,
  title = {Quantum Protocol for Cheat-Sensitive Weak Coin Flipping},
  author = {Spekkens, R. W. and Rudolph, Terry},
  journal = {Phys. Rev. Lett.},
  volume = {89},
  issue = {22},
  pages = {227901},
  numpages = {4},
  year = {2002},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.89.227901},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.89.227901}
}

@article{SR01,
  title = {Degrees of concealment and bindingness in quantum bit commitment protocols},
  author = {Spekkens, R. W. and Rudolph, T.},
  journal = {Phys. Rev. A},
  volume = {65},
  issue = {1},
  pages = {012310},
  numpages = {10},
  year = {2001},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.65.012310},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.65.012310}
}

@article{KN04,
title = "Weak coin flipping with small bias",
journal = "Inf. Process. Lett.",
volume = "89",
number = "3",
pages = "131 - 135",
year = "2004",
issn = "0020-0190",
doi = "https://doi.org/10.1016/j.ipl.2003.07.007",
url = "http://www.sciencedirect.com/science/article/pii/S0020019003004915",
author = "I. Kerenidis and A. Nayak",
keywords = "Quantum computation, Coin flipping, Cryptography, Algorithms, Quantum communication",
abstract = "This paper presents a quantum protocol that demonstrates that weak coin flipping with bias ≈0.239, less than 1/4, is possible. A bias of 1/4 was the smallest known, and followed from the strong coin flipping protocol of Ambainis in [33rd STOC, 2001] (also proposed by Spekkens and Rudolph [Phys. Rev. A 65 (2002) 012310]). Protocols with yet smaller bias ≈0.207 have independently been discovered by Ambainis (2001) and Spekkens and Rudolph [Phys. Rev. Lett. 89 (2002) 227901]. We also present an alternative strong coin flipping protocol with bias 1/4 with analysis simpler than that of Ambainis [33rd STOC, 2001]."
}

@ARTICLE{S95,
   author       = "B. Schumacher",
title = "Quantum coding",
   journal      = "Physical Review A",
   volume       = "51(4)", 
   pages        = "2738-2747",
   year         = "1995",
url = "http://pra.aps.org/abstract/PRA/v51/i4/p2738_1"
}

@ARTICLE{BH96,
   author       = "V. Bu\v{z}ek and M. Hillery",
title = "Quantum copying: Beyond the no-cloning theorem",
   journal      = "Physical Review A",
   volume       = "54(3)", 
   pages        = "1844-1852",
   year         = "1996",
url = "http://link.aps.org/doi/10.1103/PhysRevA.54.1844"
}

@ARTICLE{BDEFMS98,
   author       = "D. Bru\ss and D. P. DiVincenzo and A. Ekert and C. A. Fuchs and C. Macchiavello and J. A. Smolin",
title = "Optimal universal and state-dependent quantum cloning",
   journal      = "Physical Review A",
   volume       = "57(4)", 
   pages        = "2368-2378 ",
   year         = "1998",
url = "http://link.aps.org/doi/10.1103/PhysRevA.57.2368"
}

@ARTICLE{GM97,
   author       = "N. Gisin and S. Massar",
title = "Optimal quantum cloning machines",
   journal      = "Physical Review Letters",
   volume       = "79(11)", 
   pages        = "2153-2156",
   year         = "1997",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.79.2153"
}

@article{BM04,
  title = {Quantum coin tossing and bit-string generation in the presence of noise},
  author = {Barrett, Jonathan and Massar, Serge},
  journal = {Phys. Rev. A},
  volume = {69},
  issue = {2},
  pages = {022322},
  numpages = {6},
  year = {2004},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.69.022322},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.69.022322}
}

@article{BM04.2,
  title = {Security of quantum bit-string generation},
  author = {Barrett, Jonathan and Massar, Serge},
  journal = {Phys. Rev. A},
  volume = {70},
  issue = {5},
  pages = {052310},
  numpages = {11},
  year = {2004},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.70.052310},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.70.052310}
}


@article{LBABM05,
  title = {Provably Secure Experimental Quantum Bit-String Generation},
  author = {Lamoureux, L. P. and Brainis, E. and Amans, D. and Barrett, J. and Massar, S.},
  journal = {Phys. Rev. Lett.},
  volume = {94},
  issue = {5},
  pages = {050503},
  numpages = {4},
  year = {2005},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.94.050503},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.94.050503}
}



@ARTICLE{KW99,
   author       = "M. Keyl and R. F. Werner",
title = "Optimal cloning of pure states, testing single clones",
   journal      = "Journal of Mathematical Physics",
   volume       = "40(7)", 
   pages        = "3283",
   year         = "1999",
url = "http://dx.doi.org/10.1063/1.532887"
}

@ARTICLE{SIGA05,
   author       = "V. Scarani and S. Iblisdir and N. Gisin and A. Ac\'in",
title = "Quantum cloning",
   journal      = "Rev. Mod. Phys.",
   volume       = "77", 
   pages        = "1225-1256",
   year         = "2005",
url = "http://link.aps.org/doi/10.1103/RevModPhys.77.1225"
}

@article{W06,
  title = {Tsirelson bounds for generalized {C}lauser-{H}orne-{S}himony-{H}olt inequalities},
  author = {S. Wehner},
  journal = {Physical Review A},
  volume = {73(2)},
  issue = {2},
  pages = {022110},
  numpages = {5},
  year = {2006},
  doi = {10.1103/PhysRevA.73.022110},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.73.022110},
  publisher = {American Physical Society}
}


@ARTICLE{BC90,
   author       = "S. L. Braunstein and C. M. Caves",
title="Wringing out better {B}ell inequalities",
   journal      = "Annals of Physics",
   volume       = "202(1)",
   pages        = "22--56",
   year         = "1990",
url = "http://www.sciencedirect.com/science/article/pii/000349169090339P"
}


@article{LWHJCYLZLZGBH11,
  title = {Attacking a practical quantum-key-distribution system with wavelength-dependent beam-splitter and multiwavelength sources},
  author = {Li, Hong-Wei and Wang, Shuang and Huang, Jing-Zheng and Chen, Wei and Yin, Zhen-Qiang and Li, Fang-Yi and Zhou, Zheng and Liu, Dong and Zhang, Yang and Guo, Guang-Can and Bao, Wan-Su and Han, Zheng-Fu},
  journal = {Phys. Rev. A},
  volume = {84},
  issue = {6},
  pages = {062308},
  numpages = {5},
  year = {2011},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.84.062308},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.84.062308}
}

@article{QHWCYGH19,
author = {Yong-Jun Qian and De-Yong He and Shuang Wang and Wei Chen and Zhen-Qiang Yin and Guang-Can Guo and Zheng-Fu Han},
journal = {Optica},
keywords = {Laser damage; Laser sources; Numerical simulation; Quantum information; Quantum key distribution; Single photon detectors},
number = {9},
pages = {1178--1184},
publisher = {OSA},
title = {Robust countermeasure against detector control attack in a practical quantum key distribution system},
volume = {6},
month = {Sep},
year = {2019},
url = {http://www.osapublishing.org/optica/abstract.cfm?URI=optica-6-9-1178},
doi = {10.1364/OPTICA.6.001178},
abstract = {In real-life implementations of quantum key distribution (QKD), the physical systems with unwanted imperfections would be exploited by an eavesdropper. Based on imperfections in the detectors, detector-control attacks have been successfully launched on several QKD systems and attracted widespread concerns. Here, we propose a robust countermeasure against these attacks just by introducing a variable attenuator in front of the detector. This countermeasure is not only effective against attacks with blinding light, but it is also robust against attacks without blinding light, which are more concealed and threatening. Different from previous technical improvements, the single-photon detector in our countermeasure model is treated as a black box, and the eavesdropper can be detected by statistics of the detection and error rates of the QKD system. Besides theoretical proof, the countermeasure is also supported by an experimental demonstration. Our countermeasure is general in the sense that it is independent of the technical details of the detector, and can be easily applied to existing QKD systems.},
}

@article{HQWCYGH20,
author = {De-Yong He and Yong-Jun Qian and Shuang Wang and Wei Chen and Zhen-Qiang Yin and Guang-Can Guo and Zheng-Fu Han},
journal = {Optica},
keywords = {Attenuation; Illumination; Quantum key distribution; Single photon detectors; Switching},
number = {10},
pages = {1415--1416},
publisher = {OSA},
title = {Robust countermeasure against detector control attack in a practical quantum key distribution system: reply},
volume = {7},
month = {Oct},
year = {2020},
url = {http://www.osapublishing.org/optica/abstract.cfm?URI=optica-7-10-1415},
doi = {10.1364/OPTICA.403917},
abstract = {We reply to the comment on our robust countermeasure against the detector control attack \[Optica6, 1178 (2019)OPTIC82334-253610.1364/OPTICA.6.001178\] and explain that the concerns arising from an over-interpretation of our countermeasure are one-sided and untenable.},
}

@article{ZCWLL21,
  title = {Security proof of practical quantum key distribution with detection-efficiency mismatch},
  author = {Zhang, Yanbao and Coles, Patrick J. and Winick, Adam and Lin, Jie and L\"utkenhaus, Norbert},
  journal = {Phys. Rev. Research},
  volume = {3},
  issue = {1},
  pages = {013076},
  numpages = {13},
  year = {2021},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevResearch.3.013076},
  url = {https://link.aps.org/doi/10.1103/PhysRevResearch.3.013076}
}

@Unpublished{T20,
author = "Anton Trushechkin",
title = "Security of quantum key distribution with detection{-}efficiency mismatch in the multiphoton case",
year = "2020",
eprint = "2004.07809",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:2004.07809;%%",
url = "https://arxiv.org/abs/2004.07809",
}

@Unpublished{KST20,
author = "Srijita Kundu and Jamie Sikora and Ernest Y.-Z. Tan",
title = "A device{-}independent protocol for XOR oblivious transfer",
year = "2020",
eprint = "2006.06671",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:2006.066719;%%",
url = "https://arxiv.org/abs/2006.06671",
}

@Unpublished{O18,
author = "Jonathan Oppenheim",
title = "A post-quantum theory of classical gravity?",
year = "2018",
eprint = "1811.03116",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:2006.066719;%%",
url = "https://arxiv.org/abs/1811.03116",
}

@Unpublished{OSSW20,
author = "Jonathan Oppenheim, Carlo Sparaciari, Barbara Šoda, Zachary Weller-Davies",
title = "Objective trajectories in hybrid classical-quantum dynamics",
year = "2020",
eprint = "2011.06009",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:2006.066719;%%",
url = "https://arxiv.org/abs/2011.06009",
}







%ERIKA'S PAPER TO ADD IN MULTI-PHOTON ATTACK PAPER

@article{HBAM18,
	doi = {10.1088/1367-2630/aade06},
	url = {https://doi.org/10.1088/1367-2630/aade06},
	year = 2018,
	month = {oct},
	publisher = {{IOP} Publishing},
	volume = {20},
	number = {10},
	pages = {103016},
	author = {Anqi Huang and Stefanie Barz and Erika Andersson and Vadim Makarov},
	title = {Implementation vulnerabilities in general quantum cryptography},
	journal = {New J. Phys.},
	abstract = {Quantum cryptography is information-theoretically secure owing to its solid basis in quantum mechanics. However, generally, initial implementations with practical imperfections might open loopholes, allowing an eavesdropper to compromise the security of a quantum cryptographic system. This has been shown to happen for quantum key distribution (QKD). Here we apply experience from implementation security of QKD to several other quantum cryptographic primitives. We survey quantum digital signatures, quantum secret sharing, source-independent quantum random number generation, quantum secure direct communication, and blind quantum computing. We propose how the eavesdropper could in principle exploit the loopholes to violate assumptions in these protocols, breaking their security properties. Applicable countermeasures are also discussed. It is important to consider potential implementation security issues early in protocol design, to shorten the path to future applications.}
}


@article{QHWCYGH18,
  title = {Hacking the Quantum Key Distribution System by Exploiting the Avalanche-Transition Region of Single-Photon Detectors},
  author = {Qian, Yong-Jun and He, De-Yong and Wang, Shuang and Chen, Wei and Yin, Zhen-Qiang and Guo, Guang-Can and Han, Zheng-Fu},
  journal = {Phys. Rev. Applied},
  volume = {10},
  issue = {6},
  pages = {064062},
  numpages = {8},
  year = {2018},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevApplied.10.064062},
  url = {https://link.aps.org/doi/10.1103/PhysRevApplied.10.064062}
}






@article {SUKRMHRFLJZ10,
	author = {Scheidl, Thomas and Ursin, Rupert and Kofler, Johannes and Ramelow, Sven and Ma, Xiao-Song and Herbst, Thomas and Ratschbacher, Lothar and Fedrizzi, Alessandro and Langford, Nathan K. and Jennewein, Thomas and Zeilinger, Anton},
	title = {Violation of local realism with freedom of choice},
	volume = {107},
	number = {46},
	pages = {19708--19713},
	year = {2010},
	doi = {10.1073/pnas.1002780107},
	publisher = {National Academy of Sciences},
	abstract = {Bell{\textquoteright}s theorem shows that local realistic theories place strong restrictions on observable correlations between different systems, giving rise to Bell{\textquoteright}s inequality which can be violated in experiments using entangled quantum states. Bell{\textquoteright}s theorem is based on the assumptions of realism, locality, and the freedom to choose between measurement settings. In experimental tests, {\textquotedblleft}loopholes{\textquotedblright} arise which allow observed violations to still be explained by local realistic theories. Violating Bell{\textquoteright}s inequality while simultaneously closing all such loopholes is one of the most significant still open challenges in fundamental physics today. In this paper, we present an experiment that violates Bell{\textquoteright}s inequality while simultaneously closing the locality loophole and addressing the freedom-of-choice loophole, also closing the latter within a reasonable set of assumptions. We also explain that the locality and freedom-of-choice loopholes can be closed only within nondeterminism, i.e., in the context of stochastic local realism.},
	issn = {0027-8424},
	journal = {Proc. Natl. Acad. Sci. U.S.A.}
}

@article{B81,
title={Bertlmann's socks and the nature of reality},
author={J. S. Bell},
journal={Journal de Physique},
volume={42(3)},
pages={C2 41-61},
year={1981},
note= {Reprinted in \cite{Bellbook}, pages 139--158}
}

@article{TBZG98,
  title = {Violation of {B}ell Inequalities by Photons More Than 10 km Apart},
  author = {W. Tittel and J. Brendel and H. Zbinden and N. Gisin},
  journal = {Physical Review Letters},
  volume = {81(17)},
  issue = {17},
  pages = {3563--3566},
  year = {1998},
  doi = {10.1103/PhysRevLett.81.3563},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.81.3563},
  publisher = {American Physical Society}
}

@article{GZ99,
title={Bell inequality and the locality loophole: {A}ctive versus passive switches},
author={N. Gisin and H. Zbinden},
journal = {Physics Letters A},
Volume={264(2-3)},
pages={103--107},
year={1999},
doi={10.1016/S0375-9601(99)00807-5},
url={http://dx.doi.org/10.1016/S0375-9601(99)00807-5},
}

@article{Sa95,
title={Constraints for the violation of the {B}ell inequality in {E}instein-{P}odolsky-{R}osen-{B}ohm experiments},
author={E. Santos},
journal = {Physics Letters A},
Volume={200(1)},
pages={1--6},
year={1995},
doi={10.1016/0375-9601(95)00097-M},
url={http://dx.doi.org/10.1016/0375-9601(95)00097-M},
}

@book{Heisenbergbook,
  title={The Physical Principles of the Quantum Theory},
  author={Heisenberg, Werner},
note={Translated by C. Eckart and F. C. Hoyt},
  pages={16--21},
  year={1930},
adress={Chicago},
  publisher={University of Chicago Press}
}

@article{K20,
  title = {Stronger tests of the collapse{-}locality loophole in {B}ell experiments},
  author = {Kent, Adrian},
  journal = {Phys. Rev. A},
  volume = {101},
  issue = {1},
  pages = {012102},
  numpages = {8},
  year = {2020},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.101.012102},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.101.012102}
}

@article{K18.2.1,
  title = {Testing causal quantum theory},
  author = {A. Kent},
  journal = {Proc. R. Soc. A.},
  volume = {474},
  pages = {20180501},
  year = {2018},
  doi = {10.1098/rspa.2018.0501}
}



@article{EH77,
  title = {The necessity of quantizing the gravitational field},
  author = {Kenneth Eppley and Eric Hannah },
  journal = {Found. Phys.},
  volume = {7},
  pages = {51-68},
  year = {1977},
  doi = {10.1007/BF00715241}
}

@article{K18,
	doi = {10.1088/1361-6382/aaea20},
	url = {https://doi.org/10.1088/1361-6382/aaea20},
	year = 2018,
	month = {nov},
	publisher = {{IOP} Publishing},
	volume = {35},
	number = {24},
	pages = {245008},
	author = {Adrian Kent},
	title = {Simple refutation of the {E}ppley{\textendash}{H}annah argument},
	journal = {Class. Quantum Grav.},
	abstract = {In an influential paper, Eppley and Hannah argued that gravity must necessarily be quantized, by proposing a thought experiment involving classical gravitational waves interacting with quantum matter. They argue the interaction must either violate the uncertainty principle or allow superluminal signalling. The feasibility of implementing their experiment in our universe has been challenged by Mattingly, and other limitations of the argument have been noted by Huggett and Callender and by Albers et al. However, these critiques do not directly refute the claim that coupling quantum theories with a Copenhagen collapse postulate to unentanglable classical gravitational degrees of freedom leads to contradiction. I note here that if the gravitational field interacts with matter via the local quantum state, the Eppley–Hannah argument evidently fails. This seems a plausibly natural feature of a hybrid theory, whereas the alternative considered by Eppley–Hannah is evidently inconsistent with relativity.}
}

@article{M06,
  title = {Why {E}ppley and {H}annah's thought experiment fails},
  author = {Mattingly, James},
  journal = {Phys. Rev. D},
  volume = {73},
  issue = {6},
  pages = {064025},
  numpages = {8},
  year = {2006},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.73.064025},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.73.064025}
}


@article{W05,
author = {Wüthrich, Christian},
title = {To Quantize or Not to Quantize: Fact and Folklore in Quantum Gravity},
journal = {Philosophy of Science},
volume = {72},
number = {5},
pages = {777-788},
year = {2005},
doi = {10.1086/508946}
}


@incollection{M05,
  title={Is quantum gravity necessary?},
  author={Mattingly, James},
  booktitle={The universe of general relativity},
  pages={327--338},
  year={2005},
  publisher={Springer}
}

@article{MOS20,
title = {On the status of conservation laws in physics: Implications for semiclassical gravity},
journal = {Stud. Hist. Philos. Sci. B},
volume = {69},
pages = {67-81},
year = {2020},
issn = {1355-2198},
doi = {https://doi.org/10.1016/j.shpsb.2019.10.004},
author = {Tim Maudlin and Elias Okon and Daniel Sudarsky},
abstract = {We start by surveying the history of the idea of a fundamental conservation law and briefly examine the role conservation laws play in different classical contexts. In such contexts we find conservation laws to be useful, but often not essential. Next we consider the quantum setting, where the conceptual problems of the standard formalism obstruct a rigorous analysis of the issue. We then analyze the fate of energy conservation within the various viable paths to address such conceptual problems; in all cases we find no satisfactory way to define a (useful) notion of energy that is generically conserved. Finally, we focus on the implications of this for the semiclassical gravity program and conclude that Einstein's equations cannot be said to always hold.}
}

@article{HC01,
author = {Huggett, Nick and Callender, Craig},
title = {Why Quantize Gravity (Or Any Other Field for That Matter)?},
journal = {Philosophy of Science},
volume = {68},
number = {S3},
pages = {S382-S394},
year = {2001},
doi = {10.1086/392923}
}





@article{K05,
  title = {Causal quantum theory and the collapse locality loophole},
  author = {A. Kent},
  journal = {Phys. Rev. A},
  volume = {72},
  pages = {012107},
  numpages = {7},
  year = {2005},
  doi = {10.1103/PhysRevA.72.012107},
  publisher = {American Physical Society}
}


@article{K05.2,
  title = {Secure classical bit commitment using fixed capacity communication channels},
  author = {A. Kent},
  journal = {J. Cryptology},
  volume = {18},
  pages = {313--335},
  year = {2005},
  url = {http://link.springer.com/article/10.1007/s00145-005-0905-8}
}

@article{GM87,
  title = {Detector inefficiencies in the {E}instein-{P}odolsky-{R}osen experiment},
  author = {A. Garg and N. D. Mermin},
  journal = {Physical Review D},
  volume = {35(12)},
  issue = {12},
  pages = {3831--3835},
  year = {1987},
  doi = {10.1103/PhysRevD.35.3831},
  url = {http://link.aps.org/doi/10.1103/PhysRevD.35.3831},
  publisher = {American Physical Society}
}

@article{Eb93,
  title = {Background level and counter efficiencies required for a loophole-free {E}instein-{P}odolsky-{R}osen experiment},
  author = {P. H. Eberhard},
  journal = {Physical Review A},
  volume = {47(2)},
  issue = {2},
  pages = {R747--R750},
  year = {1993},
  doi = {10.1103/PhysRevA.47.R747},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.47.R747},
  publisher = {American Physical Society}
}

@INPROCEEDINGS{Bell71,
   author       = "J. S. Bell",
title = "Introduction to the hidden-variable question",
   booktitle      = "Foundations of Quantum Mechanics. Proceedings of the International School of Physics `Enrico Fermi', course IL",
   pages       = "171--181", 
 publisher       = "Academic",
address= "New York",
   year         = "1971",
Note="Reprinted in \cite{Bellbook}, pages 29--39",
url = ""
}

@book{Bellbook,
   author       = "J. S. Bell",
title = "Speakable and unspeakable in quantum mechanics",
   year         = "1987",
publisher = "Cambridge University Press",
address="Cambridge",
}

@unpublished{Kentnotes,
author="A. Kent",
title="Quantum Foundations",
note="Lecture notes for part III course of the Mathematical Tripos, University of Cambridge",
year="2011",
}

@article{K13,
author = "A. Kent",
title = "A no-summoning theorem in relativistic quantum theory",
journal="Quantum Inf. Process.",
volume="12",
pages="1023--1032",
url="http://link.springer.com/article/10.1007%2Fs11128-012-0431-6",
year = "2013"
}

@article{K11.2,
author = "A. Kent",
title = "Unconditionally secure bit commitment with flying qudits ",
journal="New J. Phys.",
volume="13",
pages="113015",
url="http://iopscience.iop.org/1367-2630/13/11/113015",
year = "2011",
}

@article{K11.3,
  title = {Location-oblivious data transfer with flying entangled qudits},
  author = {A. Kent},
  journal = {Phys. Rev. A},
  volume = {84},
  issue = {1},
  pages = {012328},
  numpages = {4},
  year = {2011},
  doi = {10.1103/PhysRevA.84.012328},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.84.012328},
  publisher = {American Physical Society}
}

@article{YCZLO12,
  title = {All Entangled Pure States Violate a Single {B}ell's Inequality},
  author = {Yu, Sixia and Chen, Qing and Zhang, Chengjie and Lai, C. H. and Oh, C. H.},
  journal = {Phys. Rev. Lett.},
  volume = {109},
  issue = {12},
  pages = {120402},
  numpages = {5},
  year = {2012},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.109.120402},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.109.120402}
}

@article{GVMWHHPSKLAAPMBGLSNSUWZ15,
  title = {Significant-Loophole-Free Test of {B}ell's Theorem with Entangled Photons},
  author = {Giustina, Marissa and Versteegh, Marijn A. M. and Wengerowsky, S\"oren and Handsteiner, Johannes and Hochrainer, Armin and Phelan, Kevin and Steinlechner, Fabian and Kofler, Johannes and Larsson, Jan-\AA{}ke and Abell\'an, Carlos and Amaya, Waldimar and Pruneri, Valerio and Mitchell, Morgan W. and Beyer, J\"orn and Gerrits, Thomas and Lita, Adriana E. and Shalm, Lynden K. and Nam, Sae Woo and Scheidl, Thomas and Ursin, Rupert and Wittmann, Bernhard and Zeilinger, Anton},
  journal = {Phys. Rev. Lett.},
  volume = {115},
  issue = {25},
  pages = {250401},
  numpages = {7},
  year = {2015},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.115.250401},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.115.250401}
}

@article{PBR12,
  title={On the reality of the quantum state},
  author={Pusey, Matthew F and Barrett, Jonathan and Rudolph, Terry},
  journal={Nat. Phys.},
  volume={8},
doi={10.1038/nphys2309},
  number={6},
  pages={475--478},
  year={2012},
  publisher={Nature Publishing Group}
}

@article{L14,
  title={Is the Quantum State Real? {A}n Extended Review of $\psi$-ontology Theorems},
  author={Leifer, Matthew Saul},
  journal={Quanta},
  volume={3},
  number={1},
  pages={67--155},
  year={2014},
doi={10.12743/quanta.v3i1.22}
}



@article{BCLM14,
  title = {No $\ensuremath{\psi}$-Epistemic Model Can Fully Explain the Indistinguishability of Quantum States},
  author = {Barrett, Jonathan and Cavalcanti, Eric G. and Lal, Raymond and Maroney, Owen J. E.},
  journal = {Phys. Rev. Lett.},
  volume = {112},
  issue = {25},
  pages = {250403},
  numpages = {6},
  year = {2014},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.112.250403},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.112.250403}
}


@article{L13,
author = {Hardy, Lucien},
title = {ARE QUANTUM STATES REAL?},
journal = {Int. J. Mod. Phys. B},
volume = {27},
number = {01n03},
pages = {1345012},
year = {2013},
doi = {10.1142/S0217979213450124},
    abstract = { In this paper we consider theories in which reality is described by some underlying variables, λ. Each value these variables can take represents an ontic state (a particular state of reality). The preparation of a quantum state corresponds to a distribution over the ontic states, λ. If we make three basic assumptions, we can show that the distributions over ontic states corresponding to distinct pure states are nonoverlapping. This means that we can deduce the quantum state from a knowledge of the ontic state. Hence, if these assumptions are correct, we can claim that the quantum state is a real thing (it is written into the underlying variables that describe reality). The key assumption we use in this proof is ontic indifference — that quantum transformations that do not affect a given pure quantum state can be implemented in such a way that they do not affect the ontic states in the support of that state. In fact this assumption is violated in the Spekkens toy model (which captures many aspects of quantum theory and in which different pure states of the model have overlapping distributions over ontic states). This paper proves that ontic indifference must be violated in any model reproducing quantum theory in which the quantum state is not a real thing. The argument presented in this paper is different from that given in a recent paper by Pusey, Barrett and Rudolph. It uses a different key assumption and it pertains to a single copy of the system in question. }
}



@article{B70,
  title = {The Statistical Interpretation of Quantum Mechanics},
  author = {Ballentine, L. E.},
  journal = {Rev. Mod. Phys.},
  volume = {42},
  issue = {4},
  pages = {358--381},
  numpages = {0},
  year = {1970},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.42.358},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.42.358}
}


@article{CFS02,
  title = {Quantum probabilities as {B}ayesian probabilities},
  author = {Caves, Carlton M. and Fuchs, Christopher A. and Schack, R\"udiger},
  journal = {Phys. Rev. A},
  volume = {65},
  issue = {2},
  pages = {022305},
  numpages = {6},
  year = {2002},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.65.022305}
}


@article{FS14,
	doi = {10.1088/0031-8949/90/1/015104},
	url = {https://doi.org/10.1088/0031-8949/90/1/015104},
	year = 2014,
	month = {dec},
	publisher = {{IOP} Publishing},
	volume = {90},
	number = {1},
	pages = {015104},
	author = {Christopher A Fuchs and Rüdiger Schack},
	title = {{QBism} and the {G}reeks: why a quantum state does not represent an element of physical reality},
	journal = {Phys. Scr.},
	abstract = {In QBism (or quantum Bayesianism) a quantum state does not represent an element of physical reality but an agentʼs personal probability assignments, reflecting his subjective degrees of belief about the future content of his experience. In this paper, we contrast QBism with hidden-variable accounts of quantum mechanics and show the sense in which QBism explains quantum correlations. QBismʼs agent-centered worldview can be seen as a development of ideas expressed in Schrödingerʼs essay ‘Nature and the Greeks’.}
}

@article{HS10,
  title={Einstein, incompleteness, and the epistemic view of quantum states},
  author={Harrigan, Nicholas and Spekkens, Robert W},
  journal={Found. Phys.},
  volume={40},
  number={2},
  pages={125--157},
  year={2010},
doi={10.1007/s10701-009-9347-0},
  publisher={Springer}
}

@article{S07,
  title = {Evidence for the epistemic view of quantum states: A toy theory},
  author = {Spekkens, Robert W.},
  journal = {Phys. Rev. A},
  volume = {75},
  issue = {3},
  pages = {032110},
  numpages = {30},
  year = {2007},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.75.032110},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.75.032110}
}

@article{HBDRKBRVSAAPMMTEWTH15,
  title = {Loophole-free {B}ell inequality violation using electron spins separated by 1.3 kilometres},
  author = {B. Hensen and H. Bernien and A. E. Dr\'eau and A. Reiserer and N. Kalb and M. S. Blok and J. Ruitenberg and R. F. L. Vermeulen and R. N. Schouten and C. Abell\'an and W. Amaya and V. Pruneri and M. W. Mitchell and M. Markham and D. J. Twitchen and D. Elkouss and S. Wehner and T. H. Taminiau and R. Hanson},
  journal = {Nature},
  volume = {526},
  pages = {682--686},
  year = {2015},
  doi = {10.1038/nature15759},
}



@article{RUV13,
  title = {Classical command of quantum systems},
  author = {B. W. Reichardt and F. Unger and U. Vazirani},
  journal = {Nature},
  volume = {496},
  pages = {456--460},
  year = {2013},
  doi = {10.1038/nature12035},
  url = {http://www.nature.com/nature/journal/v496/n7446/abs/nature12035.html},
}


@article{L14,
	doi = {10.1088/1751-8113/47/42/424003},
	url = {https://doi.org/10.1088/1751-8113/47/42/424003},
	year = 2014,
	month = {oct},
	publisher = {{IOP} Publishing},
	volume = {47},
	number = {42},
	pages = {424003},
	author = {Jan-{\AA}ke Larsson},
	title = {Loopholes in {B}ell inequality tests of local realism},
	journal = {Journal of Physics A: Mathematical and Theoretical},
	abstract = {Bell inequalities are intended to show that local realist theories cannot describe the world. A local realist theory is one where physical properties are defined prior to and independent of measurement, and no physical influence can propagate faster than the speed of light. Quantum-mechanical predictions for certain experiments violate the Bell inequality while a local realist theory cannot, and this shows that a local realist theory cannot give those quantum-mechanical predictions. However, because of unexpected circumstances or ‘loopholes’ in available experiment tests, local realist theories can reproduce the data from these experiments. This paper reviews such loopholes, what effect they have on Bell inequality tests, and how to avoid them in experiment. Avoiding all these simultaneously in one experiment, usually called a ‘loophole-free’ or ‘definitive’ Bell test, remains an open task, but is very important for technological tasks such as device-independent security of quantum cryptography, and ultimately for our understanding of the world.

This article is part of a special issue of Journal of Physics A: Mathematical and Theoretical devoted to ‘50 years of Bell’s theorem’.}
}

@article{SMCBWSGGHACDHLVLTMZSAAPJMKBMKN15,
  title = {Strong Loophole-Free Test of Local Realism},
  author = {Shalm, Lynden K. and Meyer-Scott, Evan and Christensen, Bradley G. and Bierhorst, Peter and Wayne, Michael A. and Stevens, Martin J. and Gerrits, Thomas and Glancy, Scott and Hamel, Deny R. and Allman, Michael S. and Coakley, Kevin J. and Dyer, Shellee D. and Hodge, Carson and Lita, Adriana E. and Verma, Varun B. and Lambrocco, Camilla and Tortorici, Edward and Migdall, Alan L. and Zhang, Yanbao and Kumor, Daniel R. and Farr, William H. and Marsili, Francesco and Shaw, Matthew D. and Stern, Jeffrey A. and Abell\'an, Carlos and Amaya, Waldimar and Pruneri, Valerio and Jennewein, Thomas and Mitchell, Morgan W. and Kwiat, Paul G. and Bienfang, Joshua C. and Mirin, Richard P. and Knill, Emanuel and Nam, Sae Woo},
  journal = {Phys. Rev. Lett.},
  volume = {115},
  issue = {25},
  pages = {250402},
  numpages = {10},
  year = {2015},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.115.250402},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.115.250402}
}


@unpublished{CMACGLMSZNBLGK13,
  title = {Detection-loophole-free test of quantum nonlocality, and applications},
  author = {B. G. Christensen and  K. T. McCusker and J. B. Altepeter and B. Calkins and T. Gerrits and A. E. Lita and A. Miller and L.
K. Shalm and Y. Zhang and S. W. Nam and N. Brunner and C. C. W. Lim and N. Gisin and P. G. Kwiat},
Note = "E-print arXiv:1306.5772",
year="2013",
eprint = "1306.5772",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1306.5772;%%",
url= "http://arxiv.org/abs/1306.5772",
}


@article{Keifer13,
  title={Conceptual problems in quantum gravity and quantum cosmology},
  author={Kiefer, Claus},
  journal={International Scholarly Research Notices},
  volume={2013},
  year={2013},
doi={10.1155/2013/509316},
  publisher={Hindawi}
}



@unpublished{K13.2,
  title = {Quantum nonlocal correlations are not dominated},
  author = {A. Kent},
year="2013",
eprint = "1308.5009",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1308.5009;%%",
}

@unpublished{ABCDHSZ21,
  title = {Experimental relativistic zero-knowledge proofs},
  author = {P. Alikhani and N. Brunner and C. Cr\'epeau and S. Designolle and R. Houlmann and W. Shi and H. Zbinden},
year="2021",
eprint = "2012.10452",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1308.5009;%%",
}



@unpublished{LP05,
  title = {Phase randomization improves the security of quantum key distribution},
  author = {Hoi-Kwong Lo and John Preskill},
year="2005",
eprint = "quant-ph/0504209",
archivePrefix = "arXiv",
}




@unpublished{Kitaev02,
  title = {Quantum coin-flipping},
  author = {A. Y. Kitaev},
year="2002",
Note="Talk at QIP 2003 (unpublished); proof reproduced in \cite{ABDR04}",
url = "www.msri.org/realvideo/ln/msri/2002/qip/kitaev/1/index.html",
}

@article{NPCT21,
  title = {Practical Quantum Key Distribution That is Secure Against Side Channels},
  author = {Navarrete, \'Alvaro and Pereira, Margarida and Curty, Marcos and Tamaki, Kiyoshi},
  journal = {Phys. Rev. Applied},
  volume = {15},
  issue = {3},
  pages = {034072},
  numpages = {12},
  year = {2021},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevApplied.15.034072},
  url = {https://link.aps.org/doi/10.1103/PhysRevApplied.15.034072}
}





@misc{FF15,
    author = {Serge Fehr and Max Fillinger},
    title = {On the Composition of Two-Prover Commitments, and Applications to Multi-Round Relativistic Commitments},
    howpublished = {Cryptology ePrint Archive, Report 2016/113},
    year = {2016},
    note = {\url{http://eprint.iacr.org/2016/113}},
}


@article{CCL15,
  title = {Arbitrarily Long Relativistic Bit Commitment},
  author = {Chakraborty, Kaushik and Chailloux, Andr\'e and Leverrier, Anthony},
  journal = {Phys. Rev. Lett.},
  volume = {115},
  issue = {25},
  pages = {250501},
  numpages = {4},
  year = {2015},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.115.250501},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.115.250501}
}

@InProceedings{CL17,
author="Chailloux, Andr{\'e}
and Leverrier, Anthony",
editor="Coron, Jean-S{\'e}bastien
and Nielsen, Jesper Buus",
title="Relativistic (or 2-Prover 1-Round) Zero-Knowledge Protocol for                                                                           {\$}{\$}{\backslash}mathsf {\{}NP{\}}{\$}{\$}                 Secure Against Quantum Adversaries",
booktitle="Advances in Cryptology -- EUROCRYPT 2017",
year="2017",
publisher="Springer International Publishing",
address="Cham",
pages="369--396",
abstract="In this paper, we show that the zero-knowledge construction for Hamiltonian Cycle remains secure against quantum adversaries in the relativistic setting. Our main technical contribution is a tool for studying the action of consecutive measurements on a quantum state which in turn gives upper bounds on the value of some entangled games. This allows us to prove the security of our protocol against quantum adversaries. We also prove security bounds for the (single-round) relativistic string commitment and bit commitment in parallel against quantum adversaries. As an additional consequence of our result, we answer an open question from [Unr12] and show tight bounds on the quantum knowledge error of some                                                                                   {\$}{\$}{\backslash}varSigma {\$}{\$}                  -protocols.",
isbn="978-3-319-56617-7"
}




%LHV CHAPTER

@article{bukh,
  title={Measurable sets with excluded distances},
  author={B. Bukh},
  journal={Geometric and Functional Analysis},
  volume={18},
  number={3},
  pages={668--697},
  year={2008},
  publisher={Springer},
url={http://link.springer.com/article/10.1007/s00039-008-0673-8}
}

@article{de2008fourier,
  title={Fourier analysis, linear programming, and densities of distance
avoiding sets in $\mathbb{R}^n$},
  author={F. M. de Oliveira Filho and F. Vallentin},
  journal={Journal of the European Mathematical Society},
  volume={12(6)},
  pages={1417--1428},
  year={2010},
url={http://www.ems-ph.org/journals/show_abstract.php?issn=1435-9855&vol=12&iss=6&rank=5}
}

@article{AMRSV13,
author= "N. Aharon and S. Machnes and B. Reznik and J. Silman and L. Vaidman",
title= "Continuous input nonlocal games",
journal = "Natural Computing",
volume = "12(1)",
pages = "5--8",
year = "2013",
url = "http://link.springer.com/article/10.1007%2Fs11047-012-9354-5"
}


@Unpublished{KPG13,
author = "A. Kent and D. Pital\'ua-Garc\'ia",
title = "Sphere colourings and {B}ell inequalities",
Note = "E-print arXiv:1307.6839",
year = "2013",
eprint = "1307.6839",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1307.6839;%%",
url = "http://arxiv.org/abs/1307.6839",
}

@Unpublished{C10,
author = "A. Chailloux",
title = "Improved Loss-Tolerant Quantum Coin Flipping",
year = "2010",
eprint = "1009.0044",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1009.0044;%%"
}


@article{AMS10,
  title = {Family of loss-tolerant quantum coin-flipping protocols},
  author = {Aharon, N. and Massar, S. and Silman, J.},
  journal = {Phys. Rev. A},
  volume = {82},
  issue = {5},
  pages = {052307},
  numpages = {7},
  year = {2010},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.82.052307},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.82.052307}
}


@article{DWTSTLPYDCTEGWP19,
  title = {Cambridge quantum network},
  author = {J. F. Dynes and A. Wonfor and W. W. -S. Tam and A. W. Sharpe and R. Takahashi and M. Lucamarini and A. Plews and Z. L. Yuan and A. R. Dixon and J. Cho and Y. Tanizawa and J. -P. Elbers and H. Grei{\ss}er and I. H. White and R. V. Penty and A. J. Shields },
  journal = {npj Quantum Inf.},
  volume = {5},
  pages = {101},
  year = {2019},
  doi = {10.1038/s41534-019-0221-4},
  url = {https://www.nature.com/articles/s41534-019-0221-4}
}

@article{K08,
  title = {The quantum internet},
  author = {H. J. Kimble},
  journal = {Nature},
  volume = {453},
  pages = {1023--1030},
  year = {2008},
  doi = {10.1038/nature07127},
  url = {https://www.nature.com/articles/nature07127}
}

@article{Liaoetal17,
  title = {Satellite-to-ground quantum key distribution},
  author = {Sheng-Kai Liao and Wen-Qi Cai and Wei-Yue Liu and Liang Zhang and Yang Li and Ji-Gang Ren and Juan Yin and Qi Shen and Yuan Cao and Zheng-Ping Li and Feng-Zhi and Xia-Wei Chen and Li-Hua Sun and Jian-Jun Jia and Jin-Cai Wu and Xiao-Jun Jiang and Jian-Feng Wang and Yong-Mei Huang and Qiang Wang and Yi-Lin Zhou and Lei Deng and Tao Xi and Lu Ma and Tai Hu and Qiang Zhang and Yu-Ao Chen and Nai-Le Liu and Xiang-Bin Wang and Zhen-Cai Zhu and Chao-Yang Lu and Rong Shu and Cheng-Zhi Peng and Jian-Yu Wang and Jian-Wei Pan},
  journal = {Nature},
  volume = {549},
  pages = {43--47},
  year = {2017},
  doi = {10.1038/nature23655},
  url = {https://www.nature.com/articles/nature23655/}
}


@article{CR19,
title = {On the possibility of laboratory evidence for quantum superposition of geometries},
journal = {Phys. Lett. B},
volume = {792},
pages = {64-68},
year = {2019},
issn = {0370-2693},
doi = {10.1016/j.physletb.2019.03.015},
url = {https://www.sciencedirect.com/science/article/pii/S0370269319301698},
author = {Marios Christodoulou and Carlo Rovelli},
abstract = {We analyse the recent proposal of measuring a quantum gravity phenomenon in the lab by entangling two mesoscopic particles gravitationally. We give a generally covariant description of this phenomenon, where the relevant effect turns out to be a quantum superposition of proper times. We point out that if General Relativity is assumed to hold for masses at this scale, measurement of this effect would count as evidence for quantum superposition of spacetime geometries. This interpretation addresses objections appeared in the literature. We observe that the effect sheds light on the Planck mass, and argue that it is very plausibly a real effect.}
}



@article {Yinetal17,
	author = {Yin, Juan and Cao, Yuan and Li, Yu-Huai and Liao, Sheng-Kai and Zhang, Liang and Ren, Ji-Gang and Cai, Wen-Qi and Liu, Wei-Yue and Li, Bo and Dai, Hui and Li, Guang-Bing and Lu, Qi-Ming and Gong, Yun-Hong and Xu, Yu and Li, Shuang-Lin and Li, Feng-Zhi and Yin, Ya-Yun and Jiang, Zi-Qing and Li, Ming and Jia, Jian-Jun and Ren, Ge and He, Dong and Zhou, Yi-Lin and Zhang, Xiao-Xiang and Wang, Na and Chang, Xiang and Zhu, Zhen-Cai and Liu, Nai-Le and Chen, Yu-Ao and Lu, Chao-Yang and Shu, Rong and Peng, Cheng-Zhi and Wang, Jian-Yu and Pan, Jian-Wei},
	title = {Satellite{-}based entanglement distribution over 1200 kilometers},
	volume = {356},
	number = {6343},
	pages = {1140--1144},
	year = {2017},
	doi = {10.1126/science.aan3211},
	publisher = {American Association for the Advancement of Science},
	abstract = {A successful quantum communication network will rely on the ability to distribute entangled photons over large distances between receiver stations. So far, free-space demonstrations have been limited to line-of-sight links across cities or between mountaintops. Scattering and coherence decay have limited the link separations to around 100 km. Yin et al. used the Micius satellite, which was launched last year and is equipped with a specialized quantum optical payload. They successfully demonstrated the satellite-based entanglement distribution to receiver stations separated by more than 1200 km. The results illustrate the possibility of a future global quantum communication network.Science, this issue p. 1140Long-distance entanglement distribution is essential for both foundational tests of quantum physics and scalable quantum networks. Owing to channel loss, however, the previously achieved distance was limited to ~100 kilometers. Here we demonstrate satellite-based distribution of entangled photon pairs to two locations separated by 1203 kilometers on Earth, through two satellite-to-ground downlinks with a summed length varying from 1600 to 2400 kilometers. We observed a survival of two-photon entanglement and a violation of Bell inequality by 2.37 {\textpm} 0.09 under strict Einstein locality conditions. The obtained effective link efficiency is orders of magnitude higher than that of the direct bidirectional transmission of the two photons through telecommunication fibers.},
	issn = {0036-8075},
	URL = {https://science.sciencemag.org/content/356/6343/1140},
	journal = {Science}
}


@inproceedings{ECPPSY05,
author = {Chip Elliott and Alexander Colvin and David Pearson and Oleksiy Pikalo and John Schlafer and Henry Yeh},
title = {{Current status of the DARPA quantum network}},
volume = {5815},
booktitle = {Quantum Information and Computation III},
editor = {Eric J. Donkor and Andrew R. Pirich and Howard E. Brandt},
organization = {International Society for Optics and Photonics},
publisher = {SPIE},
pages = {138 -- 149},
keywords = {quantum cryptography, network security, information assurance},
year = {2005},
doi = {10.1117/12.606489},
URL = {https://doi.org/10.1117/12.606489}
}



@article{Liaoetal18,
  title = {Satellite{-}Relayed Intercontinental Quantum Network},
  author = {Liao, Sheng-Kai and Cai, Wen-Qi and Handsteiner, Johannes and Liu, Bo and Yin, Juan and Zhang, Liang and Rauch, Dominik and Fink, Matthias and Ren, Ji-Gang and Liu, Wei-Yue and Li, Yang and Shen, Qi and Cao, Yuan and Li, Feng-Zhi and Wang, Jian-Feng and Huang, Yong-Mei and Deng, Lei and Xi, Tao and Ma, Lu and Hu, Tai and Li, Li and Liu, Nai-Le and Koidl, Franz and Wang, Peiyuan and Chen, Yu-Ao and Wang, Xiang-Bin and Steindorfer, Michael and Kirchner, Georg and Lu, Chao-Yang and Shu, Rong and Ursin, Rupert and Scheidl, Thomas and Peng, Cheng-Zhi and Wang, Jian-Yu and Zeilinger, Anton and Pan, Jian-Wei},
  journal = {Phys. Rev. Lett.},
  volume = {120},
  issue = {3},
  pages = {030501},
  numpages = {4},
  year = {2018},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.120.030501},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.120.030501}
}



@article{S17,
  title = {Towards a global quantum network},
  author = {C. Simon},
  journal = {Nat. Photon.},
  volume = {11},
  pages = {678--680},
  year = {2017},
  doi = {10.1038/s41566-017-0032-0},
  url = {https://www.nature.com/articles/s41566-017-0032-0}
}


@misc{computerprogram,
author = "A. Kent and D. Pital\'ua-Garc\'ia",
title = "Sphere colourings and {B}ell inequalities: {S}upplemental material",
year= "2013",
note = "Computer program coded in Mathematica, which will be available as supplemental material in \cite{KPG13}",
}




%QIC CHAPTER


@ARTICLE{QIC,
   author       = "D. Pital\'ua{-}Garc\'ia",
title = "Quantum information causality",
   journal      = "Phys. Rev. Lett.",
   volume       = "110", 
   pages        = "210402",
   year         = "2013",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.110.210402"
}

@Book{NielsenandChuangbook,
 author    = "M. A. Nielsen and I. L. Chuang",
 title     = "Quantum Computation and Quantum Information",
 publisher = "Cambridge University Press",
address= "Cambridge, UK",
 year      =  2000,
}

@Book{Mitzenmacherbook,
 author    = "M. Mitzenmacher and E. Upfal",
 title     = "Probability and Computing: Randomized Algorithms and Probabilistic Analysis",
 publisher = "Cambridge University Press",
address= "Cambridge, UK",
 year      =  2005,
}



@Book{Hartlebook,
 author    = "J. Hartle",
 title     = "Gravity: An Introduction to Einstein's General Relativity",
 publisher = "Addison-Wesley",
address= "San Francisco, CA",
 year      =  2003,
}

@ARTICLE{WZ82,
   author       = "W. K. Wootters and W. H. Zurek",
 title = "A single quantum cannot be cloned",
   journal      = "Nature",
   volume       = "299", 
   pages        = "802-803",
   year         = "1982",
url = "http://www.nature.com/nature/journal/v299/n5886/abs/299802a0.html"
}



@ARTICLE{teleportation,
   author       = "C. H. Bennett and G. Brassard and C. Cr\'epeau and R. Jozsa and A. Peres and W. K. Wootters",
 title = "Teleporting an unknown quantum state via dual classical and {E}instein-{P}odolsky-{R}osen channels",
   journal      = "Phys. Rev. Lett.",
   volume       = "70", 
   pages        = "1895-1899",
   year         = "1993",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.70.1895"
}

@ARTICLE{sdc,
   author       = "C. H. Bennett  and S. J. Wiesner",
title = "Communication via one- and two-particle operators on {E}instein-{P}odolsky-{R}osen states",
   journal      = "Phys. Rev. Lett.",
   volume       = "69", 
   pages        = "2881-2884",
   year         = "1992",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.69.2881"
}

@INPROCEEDINGS{BB84,
   author       = "C. H. Bennett and G. Brassard",
title = "Quantum cryptography: {P}ublic key distribution and coin tossing",
booktitle      = "Proceedings of IEEE International Conference on Computers, Systems, and Signal Processing, Bangalore, India",
   pages        = "175--179",
   publisher       = "IEEE",
address= "New York",
   year         = "1984",
}



@ARTICLE{BHK05,
   author       = "J. Barrett and L. Hardy and A. Kent",
title = "No signaling and quantum key distribution",
   journal      = "Phys. Rev. Lett.",
   volume       = "95", 
   pages        = "010503",
   year         = "2005",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.95.010503"
}

@ARTICLE{EPR35,
   author       = "A. Einstein and B. Podolsky and N. Rosen",
title = "Can quantum-mechanical description of physical reality be considered complete?",
   journal      = "Physical Review",
   volume       = "47(10)", 
   pages        = "777-780",
   year         = "1935",
url = "http://link.aps.org/doi/10.1103/PhysRev.47.777"
}

@ARTICLE{Bell,
   author       = "J. S. Bell",
title = "On the {E}instein-{P}odolsky-{R}osen paradox",
doi = {10.1103/PhysicsPhysiqueFizika.1.195},
   journal      = "Physics",
   volume       = "1", 
   pages        = "195-200",
   year         = "1964",
note="Reprinted in \cite{Bellbook}, pages 14--21",
}

@ARTICLE{GRW80,
   author       = "G. C. Ghirardi and A. Rimini and T. Weber",
title = "A general argument against superluminal transmission through the quantum mechanical measurement process",
   journal      = "Lettere al Nuovo Cimento",
   volume       = "27(10)", 
   pages        = "293-298",
   year         = "1980",
url = "http://www.springerlink.com/content/t5h287h1r26j25j4/"
}

@ARTICLE{K73,
   author       = "A. S. Kholevo",
   title = "Bounds for the quantity of information transmitted by a quantum communication channel",
   journal      = "Problems of Information Transmission",
   volume       = "9", 
   pages        = "177-183",
   year         = "1973",
note= "Translated from \emph{Problemy Peredachi Informatsii}, 9(3):3--11,1973.",
}

@ARTICLE{ic,
   author       = {M. Paw{\l}owski and T. Paterek and D. Kaszlikowski and V. Scarani and A. Winter and M. {\.{Z}}ukowski},
title = {Information causality as a physical principle.},
   journal      = {Nature (London)},
   volume       = {461}, 
   pages        = {1101-1104},
   year         = {2009},
url = {http://www.nature.com/nature/journal/v461/n7267/full/nature08400.html},
doi={10.1038/nature08400}
}


@ARTICLE{ABPS09,
   author       = "J. Allcock and N. Brunner and M. Paw{\l}owski and V. Scarani",
title = "Recovering part of the boundary between quantum and nonquantum correlations from information causality",
   journal      = "Physical Review A",
   volume       = "80(4)", 
   pages        = "040103(R)",
   year         = "2009",
url = "http://link.aps.org/doi/10.1103/PhysRevA.80.040103" 
}

@ARTICLE{CSS10,
   author       = "D. Cavalcanti and A. Salles and V. Scarani",
title = "Macroscopically local correlations can violate information causality",
   journal      = "Nature Communications",
   volume       = "1", 
   pages        = "136",
   year         = "2010",
url = "http://www.nature.com/ncomms/journal/v1/n9/full/ncomms1138.html"
}

@ARTICLE{BBBGST11,
   author       = "G. Berl\'{i}n and G. Brassard and F. Bussi\`{e}res and N. Godbout and J. A. Slater and W. Tittel ",
title = "Experimental loss{-}tolerant quantum coin flipping",
   journal      = "Nat. Commun.",
   volume       = "2", 
   pages        = "561",
   year         = "2011",
url = "https://www.nature.com/articles/ncomms1572"
}

@ARTICLE{GWAN11,
   author       = "R. Gallego and L. E. W{\"{u}}rflinger and A. Ac\'in and M. Navascu\'es",
title = "Quantum correlations require multipartite information principles",
   journal      = "Physical Review Letters",
   volume       = "107(21)", 
   pages        = "210403",
   year         = "2011",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.107.210403"
}

@ARTICLE{YCATS12,
   author       = "T. H. Yang and D. Cavalcanti and M. L. Almeida and C. Teo and V. Scarani",
title = "Information-causality and extremal tripartite correlations",
   journal      = "New Journal of Physics",
   volume       = "14", 
   pages        = "013061",
   year         = "2012",
url = "http://iopscience.iop.org/1367-2630/14/1/013061"
}

@ARTICLE{C80,
   author       = "B. S. Cirel'son",
title = "Quantum generalizations of {B}ell's inequality",
   journal      = "Letters in Mathematical Physics",
   volume       = "4(2)", 
   pages        = "93-100",
   year         = "1980",
url = "http://www.springerlink.com/content/l57053g573430450/"
}

@ARTICLE{PR94,
   author       = "S. Popescu and D. Rohrlich",
title = "Quantum nonlocality as an axiom",
   journal      = "Foundations of Physics",
   volume       = "24(3)", 
   pages        = "379-385",
   year         = "1994",
url = "http://www.springerlink.com/content/j842v3324u512nx0/"
}

@ARTICLE{LR68,
   author       = "O. E. Lanford and D. W. Robinson",
title = "Mean entropy of states in quantum-statistical mechanics",
   journal      = "Journal of Mathematical Physics",
   volume       = "9(7)", 
   pages        = "1120-1125",
   year         = "1968",
url = "http://jmp.aip.org/resource/1/jmapaq/v9/i7/p1120_s1"
}

@ARTICLE{AL70,
   author       = "H. Araki and E. H. Lieb",
title = "Entropy inequalities",
   journal      = "Communications in Mathematical Physics",
   volume       = "18(2)", 
   pages        = "160-170",
   year         = "1970",
url = "http://www.springerlink.com/content/wk224145h1441527/"
}

@Unpublished{H01,
author = "L. Hardy",
title = "Quantum theory from five reasonable axioms",
year = "2001",
eprint = "quant-ph/0101012",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=quant-ph/0101012;%%",
}

@Unpublished{PR14,
author = "C. Portmann and R. Renner",
title = "Cryptographic security of quantum key distribution",
year = "2014",
eprint = "1409.3525",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1409.3525;%%",
}





@ARTICLE{B07,
   author       = "J. Barrett",
title = "Information processing in generalized probabilistic theories",
   journal      = "Phys. Rev. A",
   volume       = "75",
issue = "3",
   pages        = "032304",
   year         = "2007",
url = "http://link.aps.org/doi/10.1103/PhysRevA.75.032304"
}

@ARTICLE{BBLW07,
   author       = "H. Barnum and J. Barrett and M. Leifer and A. Wilce",
title = "Generalized no-broadcasting theorem",
   journal      = "Phys. Rev. Lett.",
   volume       = "99", 
issue="24",
   pages        = "240501",
   year         = "2007",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.99.240501"
}

@article{CDP10,
  title = {Probabilistic theories with purification},
  author = {Chiribella, Giulio and D'Ariano, Giacomo Mauro and Perinotti, Paolo},
  journal = {Phys. Rev. A},
  volume = {81},
  issue = {6},
  pages = {062348},
  numpages = {40},
  year = {2010},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.81.062348},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.81.062348}
}



@ARTICLE{SW10,
   author       = "A. J. Short and S. Wehner",
title = "Entropy in general physical theories",
   journal      = "New J. Phys.",
   volume       = "12", 
   pages        = "033023",
   year         = "2010",
url = "http://iopscience.iop.org/1367-2630/12/3/033023"
}

@ARTICLE{BBCLSSWW10,
   author       = "H. Barnum and J. Barrett and L. O. Clark and M. Leifer and R. Spekkens and N. Stepanik and A. Wilce and R. Wilke",
title = "Entropy and information causality in general probabilistic theories",
   journal      = "New J. Phys.",
   volume       = "12", 
   pages        = "033024",
   year         = "2010",
url = "http://iopscience.iop.org/1367-2630/12/3/033024"
}

@ARTICLE{AS11,
   author       = "S. W. Al-Safi and A. J. Short",
title = "Information causality from an entropic and a probabilistic perspective",
   journal      = "Physical Review A",
   volume       = "84(4)", 
   pages        = "042323",
   year         = "2011",
   url = "http://link.aps.org/doi/10.1103/PhysRevA.84.042323"
}

@article{GMD17,
author = {Andrew J. P. Garner and Markus P. M\"{u}ller and Oscar C. O. Dahlsten},
title = {The complex and quaternionic quantum bit from relativity of simultaneity on an interferometer},
year = {2017},
journal = {Proc. R. Soc. A},
  volume = {473},
doi={10.1098/rspa.2017.0596},
pages={20170596}
}

@Unpublished{MMAP12,
author = "L. Masanes and M. P. Mueller and R. Augusiak and D. Perez-Garcia",
title = "A digital approach to quantum theory",
year = "2012",
Note = "E-print arXiv:1208.0493",
eprint = "1208.0493",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1208.0493;%%",
url = "http://arxiv.org/abs/1208.0493",
}

@ARTICLE{W83,
   author       = "S. Wiesner",
title = "Conjugate coding",
   journal      = "SIGACT News",
   volume       = "15", 
   pages        = "78-88",
   year         = "1983",
url = "http://dl.acm.org/citation.cfm?doid=1008908.1008920"
}

@ARTICLE{ANTV02,
   author       = "A. Ambainis and A. Nayak and A. Ta-Shma and U. Vazirani",
title = "Dense quantum coding and quantum finite automata",
   journal      = "Journal of the ACM",
   volume       = "49(4)", 
   pages        = "496-511",
   year         = "2002",
url = "http://dl.acm.org/citation.cfm?doid=581771.581773"
}



@ARTICLE{PZ10,
   author       = "M. Paw{\l}owski and M. {\.{Z}}ukowski",
title = "Entanglement-assisted random access codes",
   journal      = "Phys. Rev. A",
   volume       = "81", 
   pages        = "042326",
   year         = "2010",
url = "http://link.aps.org/doi/10.1103/PhysRevA.81.042326"
}


@ARTICLE{DLR12,
   author       = "O. C. O. Dahlsten and D. Lercher and R. Renner",
title = "Tsirelson's bound from a generalized data processing inequality",
   journal      = "New Journal of Physics",
   volume       = "14", 
   pages        = "063024",
   year         = "2012",
url = "http://iopscience.iop.org/1367-2630/14/6/063024/"
}

@ARTICLE{HV01,
   author       = "L. Henderson and V. Vedral",
title = "Classical, quantum and total correlations",
   journal      = "Journal of Physics A: Mathematical and General",
   volume       = "34(35)", 
   pages        = "6899",
   year         = "2001",
url = "http://iopscience.iop.org/0305-4470/34/35/315/"
}

@ARTICLE{OZ01,
   author       = "H. Ollivier and W. H. Zurek",
title = "Quantum discord: A measure of the quantumness of correlations",
   journal      = "Physical Review Letters",
   volume       = "88(1)", 
   pages        = "017901",
   year         = "2001",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.88.017901"
}

@ARTICLE{GPW05,
   author       = "B. Groisman and S. Popescu and A. Winter",
title = "Quantum, classical, and total amount of correlations in a quantum state",
   journal      = "Physical Review A",
   volume       = "72(3)", 
   pages        = "032317",
   year         = "2005",
url = "http://link.aps.org/doi/10.1103/PhysRevA.72.032317"
}

@Unpublished{ALMO09,
author = "A. Ambainis and D. Leung and L. Mancinska and M. Ozols",
title = "Quantum random access codes with shared randomness",
eprint = "0810.2937",
archivePrefix = "arXiv",
year = "2009",
SLACcitation = "%%CITATION=arXiv:0810.2937;%%",
url = "http://arxiv.org/abs/0810.2937",
}
%note = "E-print arXiv:0810.2937",

@Unpublished{PS11,
author = "M. Paw{\l}owski and V. Scarani",
title = "Information Causality",
note = "E-print arXiv:1112.1142",
eprint = "1112.1142",
archivePrefix = "arXiv",
year = "2011",
SLACcitation = "%%CITATION=arXiv:1112.1142;%%",
url = "http://arxiv.org/abs/1112.1142",
}

@ARTICLE{CHSH69,
   author       = "J. F. Clauser and M. A. Horne and A. Shimony and R. A. Holt",
title = "Proposed experiment to test local hidden-variable theories",
   journal      = "Physical Review Letters",
   volume       = "23(15)", 
   pages        = "880-884",
   year         = "1969",
url = "http://prl.aps.org/abstract/PRL/v23/i15/p880_1"
}

@article{CH74,
  title = {Experimental consequences of objective local theories},
  author = {J. F. Clauser and M. A. Horne},
  journal = {Physical Review D},
  volume = {10(2)},
  issue = {2},
  pages = {526--535},
  year = {1974},
  doi = {10.1103/PhysRevD.10.526},
  url = {http://link.aps.org/doi/10.1103/PhysRevD.10.526},
  publisher = {American Physical Society}
}




@article{K66,
  title = {Gravitation and quantum mechanics of macroscopic objects},
  author = {F. Karolyhazy},
  journal = {Nuovo Cimento A (1965-1970)},
  volume = {42},
  pages = {390--402},
  year = {1966},
  doi = {10.1007/BF02717926}
}

@unpublished{H18,
  title = {The construction interpretation: {C}onceptual roads to quantum gravity},
  author = {Hardy, Lucien},
year={2018},
eprint = {1807.10980},
archivePrefix = {arXiv},
SLACcitation = {%%CITATION=arXiv:1308.5009;%%},
}



@article{BGU17,
	doi = {10.1088/1361-6382/aa864f},
	url = {https://doi.org/10.1088/1361-6382/aa864f},
	year = 2017,
	month = {sep},
	publisher = {{IOP} Publishing},
	volume = {34},
	number = {19},
	pages = {193002},
	author = {Angelo Bassi and Andr{\'{e}} Gro{\ss}ardt and Hendrik Ulbricht},
	title = {Gravitational decoherence},
	journal = {Class. Quantum Grav.},
	abstract = {We discuss effects of loss of coherence in low energy quantum systems caused by or related to gravitation, referred to as gravitational decoherence. These effects, resulting from random metric fluctuations, for instance, promise to be accessible by relatively inexpensive table-top experiments, way before the scales where true quantum gravity effects become important. Therefore, they can provide a first experimental view on gravity in the quantum regime. We will survey models of decoherence induced both by classical and quantum gravitational fluctuations; it will be manifest that a clear understanding of gravitational decoherence is still lacking. Next we will review models where quantum theory is modified, under the assumption that gravity causes the collapse of the wave functions, when systems are large enough. These models challenge the quantum-gravity interplay, and can be tested experimentally. In the last part we have a look at the state of the art of experimental research. We will review efforts aiming at more and more accurate measurements of gravity (G and g) and ideas for measuring conventional and unconventional gravity effects on nonrelativistic quantum systems.}
}

@article{P05,
  title = {Quasirelativistic quasilocal finite wave-function collapse model},
  author = {Pearle, Philip},
  journal = {Phys. Rev. A},
  volume = {71},
  issue = {3},
  pages = {032101},
  numpages = {8},
  year = {2005},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.71.032101},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.71.032101}
}


@article{P99,
  title = {Relativistic collapse model with tachyonic features},
  author = {Pearle, Philip},
  journal = {Phys. Rev. A},
  volume = {59},
  issue = {1},
  pages = {80--101},
  numpages = {0},
  year = {1999},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.59.80},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.59.80}
}


@article{Tumulka06,
  title={A relativistic version of the {G}hirardi--{R}imini--{W}eber model},
  author={Tumulka, Roderich},
  journal={J. Stat. Phys.},
  volume={125},
  number={4},
  pages={821--840},
  year={2006},
doi={10.1007/s10955-006-9227-3},
  publisher={Springer}
}

@article{B11,
  title={Relativistic state reduction dynamics},
  author={Bedingham, Daniel J},
  journal={Found. Phys.},
  volume={41},
  number={4},
  pages={686--704},
  year={2011},
doi={10.1007/s10701-010-9510-7},
  publisher={Springer}
}

@article{BLSSU13,
  title = {Models of wave-function collapse, underlying theories, and experimental tests},
  author = {Bassi, Angelo and Lochan, Kinjalk and Satin, Seema and Singh, Tejinder P. and Ulbricht, Hendrik},
  journal = {Rev. Mod. Phys.},
  volume = {85},
  issue = {2},
  pages = {471--527},
  numpages = {0},
  year = {2013},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.85.471},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.85.471}
}


@article{GGR90,
  title = {Continuous-spontaneous-reduction model involving gravity},
  author = {Ghirardi, GianCarlo and Grassi, Renata and Rimini, Alberto},
  journal = {Phys. Rev. A},
  volume = {42},
  issue = {3},
  pages = {1057--1064},
  numpages = {0},
  year = {1990},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.42.1057},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.42.1057}
}





@incollection{K10,
author={A. Kent},
title={One world versus many: the inadequacy of {E}verettian accounts of evolution, probability, and scientific confirmation},
booktitle={Many Worlds? Everett, Quantum Theory and Reality},
Publisher={Oxford University Press},
editor={ S. Saunders and J. Barrett and A. Kent and D. Wallace},
pages={307--354},
year={2010},
note={E-print arXiv:0905.0624},
url={https://arxiv.org/abs/0905.0624},
}

@article{MBCPV12,
  title = {The classical-quantum boundary for correlations: {D}iscord and related measures},
  author = {K. Modi, and A. Brodutch, and H. Cable, and T. Paterek, and V. Vedral},
  journal = {Reviews of Modern Physics},
  volume = {84(4)},
  issue = {4},
  pages = {1655--1707},
  year = {2012},
  doi = {10.1103/RevModPhys.84.1655},
  url = {http://link.aps.org/doi/10.1103/RevModPhys.84.1655},
  publisher = {American Physical Society}
}



@article{MV17,
  title = {Gravitationally Induced Entanglement between Two Massive Particles is Sufficient Evidence of Quantum Effects in Gravity},
  author = {Marletto, C. and Vedral, V.},
  journal = {Phys. Rev. Lett.},
  volume = {119},
  issue = {24},
  pages = {240402},
  numpages = {5},
  year = {2017},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.119.240402},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.119.240402}
}

@article{MV17.2,
  title={Why we need to quantise everything, including gravity},
  author={Marletto, Chiara and Vedral, Vlatko},
  journal={npj Quantum Inf.},
  volume={3},
  number={1},
  pages={1--5},
  year={2017},
doi={10.1038/s41534-017-0028-0},
  publisher={Nature Publishing Group}
}

@inbook{DR11,
  title={The role of gravitation in physics: report from the 1957 {C}hapel {H}ill Conference},
  author={C{\'e}cile M. DeWitt and Dean Rickles},
  volume={5},
  year={2011},
chapter={23},
  publisher={epubli}
}

@InCollection{WR21,
	author       =	{Weinstein, Steven and Rickles, Dean},
	title        =	{{Quantum Gravity}},
	booktitle    =	{The {Stanford} Encyclopedia of Philosophy},
	editor       =	{Edward N. Zalta},
	howpublished =	{\url{https://plato.stanford.edu/archives/fall2021/entries/quantum-gravity/}},
	year         =	{2021},
	edition      =	{{F}all 2021},
	publisher    =	{Metaphysics Research Lab, Stanford University}
}


@article{T06,
  title={Inconsistency of quantum-Classical dynamics, and what it implies},
  author={Terno, Daniel R},
  journal={Found. Phys.},
  volume={36},
  number={1},
  pages={102--111},
  year={2006},
doi={10.1007/s10701-005-9007-y},
  publisher={Springer, Springer Nature}
}

@article{AKR08,
  title = {Measurement analysis and quantum gravity},
  author = {Albers, Mark and Kiefer, Claus and Reginatto, Marcel},
  journal = {Phys. Rev. D},
  volume = {78},
  issue = {6},
  pages = {064051},
  numpages = {17},
  year = {2008},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.78.064051},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.78.064051}
}


@article{MV20,
  title = {Witnessing nonclassicality beyond quantum theory},
  author = {Marletto, Chiara and Vedral, Vlatko},
  journal = {Phys. Rev. D},
  volume = {102},
  issue = {8},
  pages = {086012},
  numpages = {8},
  year = {2020},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.102.086012},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.102.086012}
}


@article{BMMUTPGBKM17,
  title = {Spin Entanglement Witness for Quantum Gravity},
  author = {Bose, Sougato and Mazumdar, Anupam and Morley, Gavin W. and Ulbricht, Hendrik and Toro\ifmmode \check{s}\else \v{s}\fi{}, Marko and Paternostro, Mauro and Geraci, Andrew A. and Barker, Peter F. and Kim, M. S. and Milburn, Gerard},
  journal = {Phys. Rev. Lett.},
  volume = {119},
  issue = {24},
  pages = {240401},
  numpages = {6},
  year = {2017},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.119.240401},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.119.240401}
}















K. Modi, A. Brodutch, H. Cable, T. Paterek, and ::: and V. Vedral, Rev. Mod. Phys. 84, 1655 (2012).





%PBT CHAPTER







@ARTICLE{BH96,
   author       = "V. Bu{\v{z}}ek and M. Hillery",
title = "Quantum copying: Beyonf the no-cloning theorem",
   journal      = "Physical Review A",
   volume       = "54(3)", 
   pages        = "1844-1852",
   year         = "1996",
url = "http://link.aps.org/doi/10.1103/PhysRevA.54.1844"
}

@ARTICLE{IH08,
   author       = "S. Ishizaka and T. Hiroshima",
title = "Asymptotic teleportation scheme as a universal programmable quantum processor",
   journal      = "Physical Review Letters",
   volume       = "101(24)", 
   pages        = "240501",
   year         = "2008",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.101.240501"
}

@ARTICLE{IH09,
   author       = "S. Ishizaka and T. Hiroshima",
title = "Quantum teleportation scheme by selecting one of multiple output ports",
   journal      = "Physical Review A",
   volume       = "79(4)", 
   pages        = "042306",
   year         = "2009",
url = "http://link.aps.org/doi/10.1103/PhysRevA.79.042306"
}

@ARTICLE{G98,
   author       = "N. Gisin",
title = "Quantum cloning without signaling",
   journal      = "Physics Letters A",
   volume       = "242(1-2)", 
   pages        = "1-3",
   year         = "1998",
url = "http://dx.doi.org/10.1016/S0375-9601(98)00170-4"
}


@article{DamianPBT,
  title = {Deduction of an upper bound on the success probability of port-based teleportation from the no-cloning theorem and the no-signaling principle},
  author = {D. Pital\'ua-Garc\'ia},
  journal = {Physical Review A},
  volume = {87(4)},
  issue = {4},
  pages = {040303(R)},
  numpages = {5},
  year = {2013},
  doi = {10.1103/PhysRevA.87.040303},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.87.040303},
  publisher = {American Physical Society}
}




@UNPUBLISHED{DPG1,
   author = "D. Pital\'ua-Garc\'ia",
   note = "to be published",
}

@UNPUBLISHED{DPG2,
   author = "D. Pital\'ua-Garc\'ia",
   note = "to be published",
}













@ARTICLE{LP31,
   author       = "L. Landau and R. Peierls",
   journal      = "Zeitschrift fur Physik",
   volume       = "69(1-2)", 
   pages        = "56--69",
   year         = "1931",
url = "http://www.springerlink.com/content/r4035w7577745427/"
}

@ARTICLE{AA80,
   author       = "Y. Aharonov and D. Z. Albert",
title = "States and observables in relativistic quantum field theories",
   journal      = "Physical Review D",
   volume       = "21(12)", 
   pages        = "3316-3324",
   year         = "1980",
url = "http://link.aps.org/doi/10.1103/PhysRevD.21.3316"
}

@ARTICLE{AA81,
   author       = "Y. Aharonov and D. Z. Albert",
title = "Can we make sense out of the measurement process in relativistic quantum mechanics?",
   journal      = "Physical Review D",
   volume       = "24(2)", 
   pages        = "359-370",
   year         = "1981",
url = "http://link.aps.org/doi/10.1103/PhysRevD.24.359"
}

@ARTICLE{AA84.1,
   author       = "Y. Aharonov and D. Z. Albert",
title = "Is the usual notion of time evolution adequate for quantum-mechanical systems? {I}",
   journal      = "Physical Review D",
   volume       = "29(2)", 
   pages        = "223-227",
   year         = "1984",
url = "http://prd.aps.org/abstract/PRD/v29/i2/p223_1"

}

@ARTICLE{AA84.2,
   author       = "Y. Aharonov and D. Z. Albert",
title = "Is the usual notion of time evolution adequate for quantum-mechanical systems? {II}. {R}elativistic considerations",
   journal      = "Physical Review D",
   volume       = "29(2)", 
   pages        = "228-234",
   year         = "1984",
url = "http://link.aps.org/doi/10.1103/PhysRevD.29.228"
}

@ARTICLE{AAV86,
   author       = "Y. Aharonov and D. Z. Albert and L. Vaidman",
title = "Measurement process in relativistic quantum theory",
   journal      = "Physical Review D",
   volume       = "34(6)", 
   pages        = "1805-1813",
   year         = "1986",
url = "http://link.aps.org/doi/10.1103/PhysRevD.34.1805"
}

@ARTICLE{PV94,
   author       = "S. Popescu and L. Vaidman",
title = "Causality constraints on nonlocal quantum measurements",
   journal      = "Physical Review A",
   volume       = "49(6)", 
   pages        = "4331-4338",
   year         = "1994",
url = "http://link.aps.org/doi/10.1103/PhysRevA.49.4331"
}

@ARTICLE{BGNP01,
   author       = "D. Beckman and D. Gottesman and M. A. Nielsen and J. Preskill",
title = "Causal and localizable quantum operations",
   journal      = "Physical Review A",
   volume       = "64(5)", 
   pages        = "052309",
   year         = "2001",
url = "http://link.aps.org/doi/10.1103/PhysRevA.64.052309"
}

@ARTICLE{V03,
   author       = "L. Vaidman",
title = "Instantaneous measurement of nonlocal variables",
   journal      = "Physical Review Letters",
   volume       = "90(1)", 
   pages        = "010402",
   year         = "2003",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.90.010402"
}

@MISC{KBMS06, 
   author       = "A. P. Kent and W. J. Munro and T. P. Spiller and R. G. Beausoleil",
title = "Tagging systems",
   howpublished = "{US Patent No. }7,075,438", 
   year         =  "2006", 
url = "http://patft.uspto.gov/netacgi/nph-Parser?Sect1=PTO1&Sect2=HITOFF&d=PALL&p=1&u=%2Fnetahtml%2FPTO%2Fsrchnum.htm&r=1&f=G&l=50&s1=7,075,438.PN.&OS=PN/7,075,438&RS=PN/7,075,438"
}

@MISC{M14, 
   author       = "R. Malaney",
title = "Location{-}enabled security services in wireless network",
   howpublished = "{US Patent No. }8,707,458", 
   year         =  "2014", 
url = "http://patft.uspto.gov/netacgi/nph-Parser?Sect1=PTO2&Sect2=HITOFF&p=1&u=%2Fnetahtml%2FPTO%2Fsearch-bool.html&r=8&f=G&l=50&co1=AND&d=PTXT&s1=8707458&OS=8707458&RS=8707458"
}

@MISC{PG17, 
   author       = "Pital\'ua{-}Garc\'ia, Dami\'an",
title = "Method and system for spacetime{-}constrained oblivious transfer",
   howpublished = "{US Non Provisional Patent Application No. }15844514. Patent pending.", 
   year         =  "December, 2017"
}

@misc{quantumtokenspat, 
   author       = "A. Kent",
title = "Quantum tokens",
   howpublished = "{US Patent No. }10,790,972", 
   year         =  2020
   } 
%url = "http://patft.uspto.gov/netacgi/nph-Parser?Sect1=PTO2&Sect2=HITOFF&u=%2Fnetahtml%2FPTO%2Fsearch-adv.htm&r=1&p=1&f=G&l=50&d=PTXT&S1=10,790,972&OS=10,790,972&RS=10,790,972"




@MISC{Kentfuturepositioncommitment, 
   author       = "Kent, Adrian",
title = "Future Position Commitment",
   howpublished = "{International Patent Application No. }WO2017001850A1. Patent pending.", 
   year         =  "2018"
}

@MISC{Kentmethodandsystem, 
   author       = "Kent, Adrian",
title = "Cryptographic method and system",
   howpublished = "{UK Patent Application No. }GB1719870.6. Patent pending.", 
}

@MISC{PGK18patent, 
   author       = "Pital\'ua{-}Garc\'ia, Dami\'an and Kerenidis Iordanis",
title = "Method for spacetime{-}constrained oblivious transfer",
   howpublished = "{US Provisional Patent Application No. }62650791", 
   year         =  "March, 2018"
}


@Unpublished{M10.2,
author = "R. A. Malaney",
title= "Quantum location verification in noisy channels",
year = "2010",
note = "E-print arXiv:1004.4689",
eprint = "1004.4689",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1004.4689;%%",
url = "http://arxiv.org/abs/1004.4689",
}

@ARTICLE{KMS11,
   author       = "A. Kent and W. J. Munro and T. P. Spiller",
title = "Quantum tagging: Authenticating location via quantum information and relativistic signaling constraints",
   journal      = "Phys. Rev. A",
   volume       = "84", 
   pages        = "012326",
   year         = "2011",
url = "http://link.aps.org/doi/10.1103/PhysRevA.84.012326"
}

@ARTICLE{K11.1,
   author       = "A. Kent",
title = "Quantum tagging for tags containing secret classical data",
   journal      = "Phys. Rev. A",
   volume       = "84", 
   pages        = "022335",
   year         = "2011",
url ="http://link.aps.org/doi/10.1103/PhysRevA.84.022335"
}

@article{pbqc,
author = "H. Buhrman and N. Chandran and S. Fehr and R. Gelles and V. Goyal and R. Ostrovsky and C. Schaffner",
title = "Position-based quantum cryptography: Impossibility and constructions",
journal="SIAM J. Comput.",
year = "2014",
volume="43",
pages="150",
url = "http://dx.doi.org/10.1137/130913687"
}


@ARTICLE{BHH11,
   author       = "J. Bae and W.-Y. Hwang and Y.-D. Han",
title = "No-signaling principle can determine optimal quantum state discrimination",
   journal      = "Physical Review Letters",
   volume       = "107(17)", 
   pages        = "170403",
   year         = "2011",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.107.170403"
}

@ARTICLE{BK11,
   author       = "S. Beigi and R. K{\"{o}}nig",
title = "Simplified instantaneous non-local quantum computation with applications to position-based cryptography",
   journal      = "New Journal of Physics",
   volume       = "13", 
   pages        = "093036",
   year         = "2011",
url ="http://iopscience.iop.org/1367-2630/13/9/093036/"
}

@Unpublished{J02,
author = "R. Jozsa",
title = " A stronger no-cloning theorem",
note = "E-print arXiv:quant-ph/0204153",
year = "2002",
eprint = "quant-ph/0204153v2",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:quant-ph/0204153v2;%%",
url = "http://arxiv.org/abs/quant-ph/0204153",
}

@Unpublished{J03,
author = "R. Jozsa",
title = "Illustrating the concept of quantum information",
note = "E-print arXiv:quant-ph/0305114",
year = "2003",
eprint = "quant-ph/0305114v1",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:0305114;%%",
url = "http://arxiv.org/abs/quant-ph/0305114",
}

@ARTICLE{B07,
   author       = "J. Barrett",
title = "Information processing in generalized probabilistic theories",
   journal      = "Physical Review A",
   volume       = "75(3)", 
   pages        = "032304",
   year         = "2007",
url = "http://link.aps.org/doi/10.1103/PhysRevA.75.032304"
}

@ARTICLE{NC97,
   author       = "M. A. Nielsen and I. L. Chuang",
   journal      = "Physical Review Letters",
title = "Programmable quantum gate arrays",
   volume       = "79(2)", 
   pages        = "321-324",
   year         = "1997",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.79.321"
}

@INPROCEEDINGS{BFSS11,
   author       = "H. Buhrman and S. Fehr and C. Schaffner and F. Speelman",
title = "The garden-hose model",
booktitle      = "Proceedings of the 4th conference on Innovations in Theoretical Computer Science",
   pages        = "145-158",
   publisher       = "ACM",
address= "New York",
   year         = "2013",
url = "http://dl.acm.org/citation.cfm?doid=2422436.2422455",
}

@Unpublished{BFSS11,
author = "H. Buhrman and S. Fehr and C. Schaffner and F. Speelman",
title = "The garden-hose model",
year = "2011",
eprint = "1109.2563",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1109.2563;%%"
}

@ARTICLE{GR02,
   author       = "B. Groisman and B. Reznik",
title = "Measurements of semilocal and nonmaximally entangled states",
   journal      = "Physical Review A",
   volume       = "66(2)", 
   pages        = "022110",
   year         = "2002",
url = "http://link.aps.org/doi/10.1103/PhysRevA.66.022110"
}

@ARTICLE{GRV03,
   author       = "B. Groisman and B. Reznik and L. Vaidman",
title = "Instantaneous measurements of nonlocal variables",
   journal      = "Journal of Modern Optics",
   volume       = "50(6-7)", 
   pages        = "943-949",
   year         = "2003",
url = "http://www.tandfonline.com/doi/abs/10.1080/09500340308234543"
}

@ARTICLE{CCJP10,
   author       = "S. R. Clark and A. J. Connor and D. Jaksch and S. Popescu",
title = "Entanglement consumption of instantaneous nonlocal quantum measurements",
   journal      = "New Journal of Physics",
   volume       = "12", 
   pages        = "083034",
   year         = "2010",
url = "http://iopscience.iop.org/1367-2630/12/8/083034"
}



@article{SHO13,
  title = {Generalized teleportation and entanglement recycling},
  author = {S. Strelchuk and M. Horodecki and J. Oppenheim},
  journal = {Physical Review Letters},
  volume = {110(1)},
  issue = {1},
  pages = {010505},
  numpages = {5},
  year = {2013},
  doi = {10.1103/PhysRevLett.110.010505},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.110.010505},
  publisher = {American Physical Society}
}












%OTHERS (TO BE VERIFIED and ARRANGED)






@ARTICLE{MVBS04,
   author       = "M. M{\"{o}}tt{\"{o}}nen and J. J. Vartiainen and V. Bergholm and M. M. Salomaa",
   journal      = "Physical Review Letters",
   volume       = "93", 
   pages        = "130502",
   year         = "2004",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.93.130502"
}



@ARTICLE{Pearle70,
   author       = "P. M. Pearle",
title= "Hidden-Variable Example Based upon Data Rejection",
   journal      = "Phys. Rev. D",
   volume       = "2", 
   pages        = "1418--1425",
   year         = "1970",
   doi = "10.1103/PhysRevD.2.1418",
   url = "http://link.aps.org/doi/10.1103/PhysRevD.2.1418"
}

@ARTICLE{ADR82,
   author       = "A. Aspect and J. Dalibard and G. Roger",
   journal      = "Physical Review Letters",
   volume       = "49", 
   pages        = "1804",
   year         = "1982",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.49.1804"
}

@ARTICLE{WJSWZ98,
   author       = "G. Weihs and T. Jennewein and C. Simon and H. Weinfurter and A. Zeilinger",
   journal      = "Physical Review Letters",
   volume       = "81", 
   pages        = "5039",
   year         = "1998",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.81.5039"
}







SC{PBTSM,
note = "See Supplemental Material at [URL will be inserted by AIP] for the
proof of the Theorem and details about the primed PBT protocol."
}

@ARTICLE{Bell,
   author       = "J. Bell",
   year         = "1964",
   journal      = "Physics",
   volume       = "1",
   pages        = "195",
}

@ARTICLE{teleportation,
   author       = "C. H. Bennett and G. Brassard and C. Cr\'epeau and R. Jozsa
and A. Peres and W. K. Wootters",
   journal      = "Phys. Rev. Lett.",
   volume       = "70",
   pages        = "1895",
   year         = "1993",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.70.1895"
}


@ARTICLE{BH96,
   author       = "V. Bu{\v{z}}ek and M. Hillery",
   journal      = "Phys. Rev. A",
   volume       = "54",
   pages        = "1844",
   year         = "1996",
url = "http://link.aps.org/doi/10.1103/PhysRevA.54.1844"
}

@ARTICLE{IH08,
   author       = "S. Ishizaka and T. Hiroshima",
   journal      = "Phys. Rev.  Lett.",
   volume       = "101",
   pages        = "240501",
   year         = "2008",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.101.240501"
}

@ARTICLE{IH09,
   author       = "S. Ishizaka and T. Hiroshima",
   journal      = "Phys. Rev. A",
   volume       = "79",
   pages        = "042306",
   year         = "2009",
url = "http://link.aps.org/doi/10.1103/PhysRevA.79.042306"
}

@ARTICLE{G98,
   author       = "N. Gisin",
   journal      = "Phys. Lett. A",
   volume       = "242",
   pages        = "1",
   year         = "1998",
url = "http://dx.doi.org/10.1016/S0375-9601(98)00170-4"
}


@UNPUBLISHED{DPG1,
   author = "D. Pital\'ua-Garc\'ia",
   note = "to be published",
}

@UNPUBLISHED{DPG2,
   author = "D. Pital\'ua-Garc\'ia",
   note = "to be published",
}




@article{D82,
title = {Communication by {EPR} devices},
journal = {Phys. Lett. A},
volume = {92},
number = {6},
pages = {271-272},
year = {1982},
issn = {0375-9601},
doi = {https://doi.org/10.1016/0375-9601(82)90084-6},
url = {https://www.sciencedirect.com/science/article/pii/0375960182900846},
author = {D. Dieks},
abstract = {A recent proposal to achieve faster-than-light communication by means of an EPR-type experimental set-up is examined. We demonstrate that such superluminal communication is not possible. The crucial role of the linearity of the quantum mechanical evolution laws in preventing causal anomalies is stressed.}
}

@Unpublished{K11.2,
author = "Kent, A.",
year = "2011",
eprint = "1101.4612",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1101.4612v3;%%"
}


@ARTICLE{LP31,
   author       = "L. Landau and R. Peierls",
   journal      = "Z. Phys.",
   volume       = "69",
   pages        = "56",
   year         = "1931",
url = "http://www.springerlink.com/content/r4035w7577745427/"
}

@ARTICLE{AA80,
   author       = "Y. Aharonov and D. Z. Albert",
   journal      = "Phys. Rev. D",
   volume       = "21",
   pages        = "3316",
   year         = "1980",
url = "http://link.aps.org/doi/10.1103/PhysRevD.21.3316"
}

@ARTICLE{AA81,
   author       = "Y. Aharonov and D. Z. Albert",
   journal      = "Phys. Rev. D",
   volume       = "24",
   pages        = "359",
   year         = "1981",
url = "http://link.aps.org/doi/10.1103/PhysRevD.24.359"
}

@ARTICLE{AA84.1,
   author       = "Y. Aharonov and D. Z. Albert",
   journal      = "Phys. Rev. D",
   volume       = "29",
   pages        = "223",
   year         = "1984",
url = "http://link.aps.org/doi/10.1103/PhysRevD.29.223"

}

@ARTICLE{AA84.2,
   author       = "Y. Aharonov and D. Z. Albert",
   journal      = "Phys. Rev. D",
   volume       = "29",
   pages        = "228",
   year         = "1984",
url = "http://link.aps.org/doi/10.1103/PhysRevD.29.228"
}

@ARTICLE{AAV86,
   author       = "Y. Aharonov and D. Z. Albert and L. Vaidman",
   journal      = "Phys. Rev. D",
   volume       = "34",
   pages        = "1805",
   year         = "1986",
url = "http://link.aps.org/doi/10.1103/PhysRevD.34.1805"
}

@ARTICLE{PV94,
   author       = "S. Popescu and L. Vaidman",
   journal      = "Phys. Rev. A",
   volume       = "49",
   pages        = "4331",
   year         = "1994",
url = "http://link.aps.org/doi/10.1103/PhysRevA.49.4331"
}

@ARTICLE{BGNP01,
   author       = "D. Beckman and D. Gottesman and M. A. Nielsen and J.
Preskill",
   journal      = "Phys. Rev. A",
   volume       = "64",
   pages        = "052309",
   year         = "2001",
url = "http://link.aps.org/doi/10.1103/PhysRevA.64.052309"
}

@ARTICLE{V03,
   author       = "L. Vaidman",
   journal      = "Phys. Rev. Lett.",
   volume       = "90",
   pages        = "010402",
   year         = "2003",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.90.010402"
}

@MISC{KBMS06,

   author       = "A. Kent and R. Beausoleil and W. Munro and T. Spiller",
   howpublished = "{US Patent No.}  US20067075438",
   year         =  "2006",
}

@ARTICLE{M10.1,
   author       = "R. A. Malaney",
   journal      = "Phys. Rev. A",
   volume       = "81",
   pages        = "042319",
   year         = "2010",
url = "http://link.aps.org/doi/10.1103/PhysRevA.81.042319"
}

@Unpublished{M10.2,
author = "Malaney, R. A.",
year = "2010",
eprint = "1004.4689",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1004.4689;%%"
}

@ARTICLE{KMS11,
   author       = "A. Kent and W. J. Munro and T. P. Spiller",
   journal      = "Phys. Rev. A",
   volume       = "84",
   pages        = "012326",
   year         = "2011",
url = "http://link.aps.org/doi/10.1103/PhysRevA.84.012326"
}

@ARTICLE{K11.1,
   author       = "A. Kent",
   journal      = "Phys. Rev. A",
   volume       = "84",
   pages        = "022335",
   year         = "2011",
url ="http://link.aps.org/doi/10.1103/PhysRevA.84.022335"
}


@ARTICLE{LL11,
   author       = "H. K. Lau and H. K. Lo",
   journal      = "Phys. Rev. A",
   volume       = "83",
   pages        = "012322",
   year         = "2011",
url = "http://link.aps.org/doi/10.1103/PhysRevA.83.012322"
}

@Unpublished{BFSS11,
author = "H. Buhrman and S. Fehr and C. Schaffner and F. Speelman",
year = "2011",
eprint = "1109.2563",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1109.2563;%%"
}

@ARTICLE{GR02,
   author       = "B. Groisman and B. Reznik",
   journal      = "Phys. Rev. A",
   volume       = "66",
   pages        = "022110",
   year         = "2002",
url = "http://link.aps.org/doi/10.1103/PhysRevA.66.022110"
}

@ARTICLE{GRV03,
   author       = "B. Groisman and B. Reznik and L. Vaidman",
   journal      = "J. Mod. Opt.",
   volume       = "50",
   pages        = "943",
   year         = "2003",
url = "http://www.tandfonline.com/doi/abs/10.1080/09500340308234543"
}

@ARTICLE{CCJP10,
   author       = "S. R. Clark and A. J. Connor and D. Jaksch and S. Popescu",
   journal      = "New J. Phys.",
   volume       = "12",
   pages        = "083034",
   year         = "2010",
url = "http://iopscience.iop.org/1367-2630/12/8/083034"
}

@ARTICLE{BK11,
   author       = "S. Beigi and R. K{\"{o}}nig",
   journal      = "New J. Phys.",
   volume       = "13",
   pages        = "093036",
   year         = "2011",
url ="http://iopscience.iop.org/1367-2630/13/9/093036/"
}

@ARTICLE{MVBS04,
   author       = "M. M{\"{o}}tt{\"{o}}nen and J. J. Vartiainen and V. Bergholm
and M. M. Salomaa",
   journal      = "Phys. Rev. Lett.",
   volume       = "93",
   pages        = "130502",
   year         = "2004",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.93.130502"
}

@Unpublished{J02,
author = "R. Jozsa",
year = "2002",
eprint = "quant-ph/0204153v2",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:quant-ph/0204153v2;%%"
}

@Unpublished{J03,
author = "R. Jozsa",
year = "2003",
eprint = "quant-ph/0305114v1",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:0305114;%%"
}


@ARTICLE{BHK05,
   author       = "J. Barrett and L. Hardy and A. Kent",
   journal      = "Phys. Rev. Lett.",
   volume       = "95",
   pages        = "010503",
   year         = "2005",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.95.010503"
}

@ARTICLE{ic,
   author       = "M. Paw{\l}owski and T. Paterek and D. Kaszlikowski and V.
Scarani and A. Winter and M. {\.{Z}}ukowski",
   journal      = "Nature (London)",
   volume       = "461",
   pages        = "1101",
   year         = "2009",
url = "http://www.nature.com/nature/journal/v461/n7267/full/nature08400.html"
}

@ARTICLE{NC97,
   author       = "M. A. Nielsen and I. L. Chuang",
   journal      = "Phys. Rev. Lett.",
   volume       = "79",
   pages        = "321",
   year         = "1997",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.79.321"
}



@ARTICLE{ADR82,
   author       = "A. Aspect and J. Dalibard and G. Roger",
   journal      = "Phys. Rev. Lett.",
   volume       = "49",
   pages        = "1804",
   year         = "1982",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.49.1804"
}

@ARTICLE{WJSWZ81,
   author       = "G. Weihs and T. Jennewein and C. Simon and H. Weinfurter and
A. Zeilinger",
   journal      = "Phys. Rev. Lett.",
   volume       = "81",
   pages        = "5039",
   year         = "1998",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.81.5039"
}

@ARTICLE{RKMSIMW01,
   author       = "M. A. Rowe and D. Kielpinski and V. Meyer and C. A. Sackett
and W. M. Itano and C. Monroe and D. J. Wineland",
   journal      = "Nature",
   volume       = "409",
   pages        = "791",
   year         = "2001",
url = "http://www.nature.com/nature/journal/v409/n6822/full/409791a0.html"
}

@ARTICLE{MMMOM08,
   author       = "D. N. Matsukevich and P. Maunz and D. L. Moehring and S.
Olmschenk and C. Monroe",
   journal      = "Phys. Rev. Lett.",
   volume       = "100",
   pages        = "150404",
   year         = "2008",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.100.150404"
}
















@Book{Bohmbook,
 author    = "David Bohm",
 title     = "Quantum Theory",
 publisher = "Prentice-Hall",
 year      =  1951,
}

@Book{NielsenandChuangbook,
 author    = "M. A. Nielsen and I. L. Chuang",
 title     = "Quantum Computation and Quantum Information",
 publisher = "Cambridge University Press",
 year      =  2000,
}

@Unpublished{J02,
author = "R. Jozsa",
title = "A stronger no-cloning theorem",
year = "2002",
Note = "E-print arXiv:quant-ph/0204153",
}

@Unpublished{J03,
author = "R. Jozsa",
title = "Illustrating the concept of quantum information",
year = "2003",
Note = "E-print arXiv:quant-ph/0305114",
}

@ARTICLE{LP31,
   author       = "L. Landau and R. Peierls",
   journal      = "Z. Phys.",
   volume       = "69",
   pages        = "56",
   year         = "1931",
url = "http://www.springerlink.com/content/r4035w7577745427/"
}

@ARTICLE{EPR35,
   author       = "A. Einstein and B. Podolsky and N. Rosen",
title = "Can quantum-mechanical description of physical reality be considered
complete?",
   journal      = "Phys. Rev.",
   volume       = "47",
   pages        = "777-780",
   year         = "1935",
url = "http://link.aps.org/doi/10.1103/PhysRev.47.777"
}

@ARTICLE{Bell,
   author       = "J. S. Bell",
title = "On the {E}instein {P}odolsky {R}osen paradox",
   year         = "1964",
   journal      = "Physics",
   volume       = "1",
   pages        = "195-200",
}

@ARTICLE{LR68,
   author       = "O. E. Lanford and D. W. Robinson",
title = "Mean entropy of states in quantum-statistical mechanics",
   journal      = "J. Math. Phys.",
   volume       = "9",
   pages        = "1120-1125",
   year         = "1968",
url = "http://jmp.aip.org/resource/1/jmapaq/v9/i7/p1120_s1"
}

@ARTICLE{CHSH69,
   author       = "J. F. Clauser and M. A. Horne and A. Shimony and R. A.
Holt",
   journal      = "Phys. Rev. Lett.",
   volume       = "23",
   pages        = "880",
   year         = "1969",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.23.880"
}

@ARTICLE{AL70,
   author       = "H. Araki and E. H. Lieb",
title = "Entropy inequalities",
   journal      = "Commun. Math. Phys.",
   volume       = "18",
   pages        = "160-170",
   year         = "1970",
url = "http://www.springerlink.com/content/wk224145h1441527/"
}



@ARTICLE{K73,
   author       = "A. S. Kholevo",
   title = "Bounds for the quantity of information transmitted by a quantum
communication channel",
   journal      = "Probl. Inf. Transm.",
   volume       = "9",
   pages        = "177-183",
   year         = "1973",
}

@ARTICLE{AA80,
   author       = "Y. Aharonov and D. Z. Albert",
   journal      = "Phys. Rev. D",
   volume       = "21",
   pages        = "3316",
   year         = "1980",
url = "http://link.aps.org/doi/10.1103/PhysRevD.21.3316"
}

@ARTICLE{C80,
   author       = "B. S. Cirel'son",
title = "Quantum generalizations of {B}ell's inequality",
   journal      = "Lett. Math. Phys.",
   volume       = "4",
   pages        = "93-100",
   year         = "1980",
url = "http://www.springerlink.com/content/l57053g573430450/"
}

@ARTICLE{GRW80,
   author       = "G. C. Ghirardi and A. Rimini and T. Weber",
title = "A general argument against superluminal transmission through the
quantum mechanical measurement process",
   journal      = "Lett. Nuov. Cim.",
   volume       = "27",
   pages        = "293-298",
   year         = "1980",
url = "http://www.springerlink.com/content/t5h287h1r26j25j4/"
}

@ARTICLE{AA81,
   author       = "Y. Aharonov and D. Z. Albert",
   journal      = "Phys. Rev. D",
   volume       = "24",
   pages        = "359",
   year         = "1981",
url = "http://link.aps.org/doi/10.1103/PhysRevD.24.359"
}



@ARTICLE{ADR82,
   author       = "A. Aspect and J. Dalibard and G. Roger",
   journal      = "Phys. Rev. Lett.",
   volume       = "49",
   pages        = "1804",
   year         = "1982",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.49.1804"
}

@ARTICLE{W83,
   author       = "S. Wiesner",
title = "Conjugate coding",
   journal      = "SIGACT News",
   volume       = "15",
   pages        = "78-88",
   year         = "1983",
url = "http://dl.acm.org/citation.cfm?doid=1008908.1008920"
}

@ARTICLE{AA84.1,
   author       = "Y. Aharonov and D. Z. Albert",
   journal      = "Phys. Rev. D",
   volume       = "29",
   pages        = "223",
   year         = "1984",
url = "http://link.aps.org/doi/10.1103/PhysRevD.29.223"
}

@ARTICLE{AA84.2,
   author       = "Y. Aharonov and D. Z. Albert",
   journal      = "Phys. Rev. D",
   volume       = "29",
   pages        = "228",
   year         = "1984",
url = "http://link.aps.org/doi/10.1103/PhysRevD.29.228"
}

@INPROCEEDINGS{BB84,
   author       = "C. H. Bennett and G. Brassard",
   booktitle      = "Proceedings IEEE Int. Conf. on Computers, Systems and
Signal Processing, Bangalore, India",
   pages        = "175-179",
   publisher       = "IEEE",
   year         = "1984",
}

@ARTICLE{AAV86,
   author       = "Y. Aharonov and D. Z. Albert and L. Vaidman",
   journal      = "Phys. Rev. D",
   volume       = "34",
   pages        = "1805",
   year         = "1986",
url = "http://link.aps.org/doi/10.1103/PhysRevD.34.1805"
}



@ARTICLE{BC90,
   author       = "S. L. Braunstein and C. M. Caves",
   journal      = "Ann. Phys.",
   volume       = "202",
   pages        = "22",
   year         = "1990",
url = "http://www.sciencedirect.com/science/article/pii/000349169090339P"
}




@ARTICLE{teleportation,
   author       = "C. H. Bennett and G. Brassard and C. Cr\'epeau and R. Jozsa
and A. Peres and W. K. Wootters",
   title = "Teleporting an unknown quantum state via dual classical and
{E}instein-{P}odolsky-{R}osen channels",
   journal      = "Phys. Rev. Lett.",
   volume       = "70",
   pages        = "1895-1899",
   year         = "1993",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.70.1895"
}

@ARTICLE{PV94,
   author       = "S. Popescu and L. Vaidman",
   journal      = "Phys. Rev. A",
   volume       = "49",
   pages        = "4331",
   year         = "1994",
url = "http://link.aps.org/doi/10.1103/PhysRevA.49.4331"
}

@ARTICLE{PR94,
   author       = "S. Popescu and D. Rohrlich",
title = "Quantum nonlocality as an axiom",
   journal      = "Found. Phys.",
   volume       = "24",
   pages        = "379-385",
   year         = "1994",
url = "http://www.springerlink.com/content/j842v3324u512nx0/"
}

@ARTICLE{BH96,
   author       = "V. Bu{\v{z}}ek and M. Hillery",
   journal      = "Phys. Rev. A",
   volume       = "54",
   pages        = "1844",
   year         = "1996",
url = "http://link.aps.org/doi/10.1103/PhysRevA.54.1844"
}

@ARTICLE{NC97,
   author       = "M. A. Nielsen and I. L. Chuang",
title = "Programmable Quantum Gate Arrays",
   journal      = "Phys. Rev. Lett.",
   volume       = "79",
   pages        = "321-324",
   year         = "1997",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.79.321"
}

@ARTICLE{G98,
   author       = "N. Gisin",
title = "Quantum cloning without signaling",
   journal      = "Phys. Lett. A",
   volume       = "242",
   pages        = "1-3",
   year         = "1998",
url = "http://dx.doi.org/10.1016/S0375-9601(98)00170-4"
}

@ARTICLE{WJSWZ81,
   author       = "G. Weihs and T. Jennewein and C. Simon and H. Weinfurter and
A. Zeilinger",
   journal      = "Phys. Rev. Lett.",
   volume       = "81",
   pages        = "5039",
   year         = "1998",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.81.5039"
}

@ARTICLE{BGNP01,
   author       = "D. Beckman and D. Gottesman and M. A. Nielsen and J.
Preskill",
   journal      = "Phys. Rev. A",
   volume       = "64",
   pages        = "052309",
   year         = "2001",
url = "http://link.aps.org/doi/10.1103/PhysRevA.64.052309"
}

@ARTICLE{RKMSIMW01,
   author       = "M. A. Rowe and D. Kielpinski and V. Meyer and C. A. Sackett
and W. M. Itano and C. Monroe and D. J. Wineland",
   journal      = "Nature",
   volume       = "409",
   pages        = "791",
   year         = "2001",
url = "http://www.nature.com/nature/journal/v409/n6822/full/409791a0.html"
}

@ARTICLE{GR02,
   author       = "B. Groisman and B. Reznik",
title = "Measurements of semilocal and nonmaximally entangled states",
   journal      = "Phys. Rev. A",
   volume       = "66",
   pages        = "022110",
   year         = "2002",
url = "http://link.aps.org/doi/10.1103/PhysRevA.66.022110"
}


@ARTICLE{ANTV02,
   author       = "A. Ambainis and A. Nayak and A. Ta-Shma and U. Vazirani",
title = "Dense quantum coding and quantum finite automata",
   journal      = "J. ACM",
   volume       = "49",
   pages        = "496-511",
   year         = "2002",
url = "http://dl.acm.org/citation.cfm?doid=581771.581773"
}


@ARTICLE{V03,
   author       = "L. Vaidman",
title = "Instantaneous Measurement of Nonlocal Variables",
   journal      = "Phys. Rev. Lett.",
   volume       = "90",
   pages        = "010402",
   year         = "2003",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.90.010402"
}

@ARTICLE{GRV03,
   author       = "B. Groisman and B. Reznik and L. Vaidman",
title = "Instantaneous measurements of nonlocal variables",
   journal      = "J. Mod. Opt.",
   volume       = "50",
   pages        = "943-949",
   year         = "2003",
url = "http://www.tandfonline.com/doi/abs/10.1080/09500340308234543"
}

@ARTICLE{MVBS04,
   author       = "M. M{\"{o}}tt{\"{o}}nen and J. J. Vartiainen and V. Bergholm
and M. M. Salomaa",
   journal      = "Phys. Rev. Lett.",
   volume       = "93",
   pages        = "130502",
   year         = "2004",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.93.130502"
}

@ARTICLE{BHK05,
   author       = "J. Barrett and L. Hardy and A. Kent",
title = "No signaling and quantum key distribution",
   journal      = "Phys. Rev. Lett.",
   volume       = "95",
   pages        = "010503",
   year         = "2005",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.95.010503"
}



@MISC{KBMS06,
   author       = "A. Kent and R. Beausoleil and W. Munro and T. Spiller",
   howpublished = "{US Patent No.}  US20067075438",
   year         =  "2006",
}

@ARTICLE{B07,
   author       = "J. Barrett",
title = "Information processing in generalized probabilistic theories",
   journal      = "Phys. Rev. A",
   volume       = "75",
   pages        = "032304",
   year         = "2007",
url = "http://link.aps.org/doi/10.1103/PhysRevA.75.032304"
}

@ARTICLE{BBLW07,
   author       = "H. Barnum and J. Barrett and M. Leifer and A. Wilce",
title = "Generalized no-broadcasting theorem",
   journal      = "Phys. Rev. Lett.",
   volume       = "99",
   pages        = "240501",
   year         = "2007",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.99.240501"
}

@ARTICLE{IH08,
   author       = "S. Ishizaka and T. Hiroshima",
title = "Asymptotic Teleportation Scheme as a Universal Programmable Quantum
Processor",
   journal      = "Phys. Rev.  Lett.",
   volume       = "101",
   pages        = "240501",
   year         = "2008",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.101.240501"
}

@ARTICLE{MMMOM08,
   author       = "D. N. Matsukevich and P. Maunz and D. L. Moehring and S.
Olmschenk and C. Monroe",
   journal      = "Phys. Rev. Lett.",
   volume       = "100",
   pages        = "150404",
   year         = "2008",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.100.150404"
}

@ARTICLE{IH09,
   author       = "S. Ishizaka and T. Hiroshima",
title = "Quantum teleportation scheme by selecting one of multiple output
ports",
   journal      = "Phys. Rev. A",
   volume       = "79",
   pages        = "042306",
   year         = "2009",
url = "http://link.aps.org/doi/10.1103/PhysRevA.79.042306"
}

@ARTICLE{ic,
   author       = "M. Paw{\l}owski and T. Paterek and D. Kaszlikowski and V.
Scarani and A. Winter and M. {\.{Z}}ukowski",
title = "Information causality as a physical principle",
   journal      = "Nature (London)",
   volume       = "461",
   pages        = "1101-1104",
   year         = "2009",
url = "http://www.nature.com/nature/journal/v461/n7267/full/nature08400.html"
}

@ARTICLE{ABPS09,
   author       = "J. Allcock and N. Brunner and M. Paw{\l}owski and V.
Scarani",
title = "Recovering part of the boundary between quantum and nonquantum
correlations from information causality",
   journal      = "Phys. Rev. A",
   volume       = "80",
   pages        = "040103",
   year         = "2009",
url = "http://link.aps.org/doi/10.1103/PhysRevA.80.040103"
}

@ARTICLE{M10.1,
   author       = "R. A. Malaney",
title = "Location-dependent communications using quantum entanglement",
   journal      = "Phys. Rev. A",
   volume       = "81",
   pages        = "042319",
   year         = "2010",
url = "http://link.aps.org/doi/10.1103/PhysRevA.81.042319"
}

@Unpublished{M10.2,
author = "R. A. Malaney",
title = " Quantum Location Verification in Noisy Channels",
year = "2010",
Note = "E-print arXiv:1004.4689",
url = "http://arxiv.org/abs/1004.4689"
}

@ARTICLE{CCJP10,
   author       = "S. R. Clark and A. J. Connor and D. Jaksch and S. Popescu",
title = "Entanglement consumption of instantaneous nonlocal quantum
measurements",
   journal      = "New J. Phys.",
   volume       = "12",
   pages        = "083034",
   year         = "2010",
url = "http://iopscience.iop.org/1367-2630/12/8/083034"
}


@ARTICLE{CSS10,
   author       = "D. Cavalcanti and A. Salles and V. Scarani",
title = "Macroscopically local correlations can violate information causality",
   journal      = "Nat. Commun.",
   volume       = "1",
   pages        = "136",
   year         = "2010",
url = "http://www.nature.com/ncomms/journal/v1/n9/full/ncomms1138.html"
}

@ARTICLE{SW10,
   author       = "A. J. Short and S. Wehner",
title = "Entropy in general physical theories",
   journal      = "New J. Phys.",
   volume       = "12",
   pages        = "033023",
   year         = "2010",
url = "http://iopscience.iop.org/1367-2630/12/3/033023"
}

@ARTICLE{BBCLSSWW10,
   author       = "H. Barnum and J. Barrett and L. O. Clark and M. Leifer and
R. Spekkens and N. Stepanik and A. Wilce and R. Wilke",
title = "Entropy and information causality in general probabilistic theories",
   journal      = "New J. Phys.",
   volume       = "12",
   pages        = "033024",
   year         = "2010",
url = "http://iopscience.iop.org/1367-2630/12/3/033024"
}

@ARTICLE{PZ10,
   author       = "M. Paw{\l}owski and M. {\.{Z}}ukowski",
title = "Entanglement-assisted random access codes",
   journal      = "Phys. Rev. A",
   volume       = "81",
   pages        = "042326",
   year         = "2010",
url = "http://link.aps.org/doi/10.1103/PhysRevA.81.042326"
}

@ARTICLE{KMS11,
   author       = "A. Kent and W. J. Munro and T. P. Spiller",
title = "Quantum tagging: Authenticating location via quantum information and
relativistic signaling constraints",
   journal      = "Phys. Rev. A",
   volume       = "84",
   pages        = "012326",
   year         = "2011",
url = "http://link.aps.org/doi/10.1103/PhysRevA.84.012326"
}

@ARTICLE{K11.1,
   author       = "A. Kent",
title = "Quantum tagging for tags containing secret classical data",
   journal      = "Phys. Rev. A",
   volume       = "84",
   pages        = "022335",
   year         = "2011",
url ="http://link.aps.org/doi/10.1103/PhysRevA.84.022335"
}

@Unpublished{K11.2,
author = "Kent, A.",
year = "2011",
eprint = "1101.4612",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1101.4612v3;%%"
}

@ARTICLE{LL11,
   author       = "H. K. Lau and H. K. Lo",
title = "Insecurity of position-based quantum-cryptography protocols against
entanglement attacks",
   journal      = "Phys. Rev. A",
   volume       = "83",
   pages        = "012322",
   year         = "2011",
url = "http://link.aps.org/doi/10.1103/PhysRevA.83.012322"
}

@Unpublished{BFSS11,
author = "H. Buhrman and S. Fehr and C. Schaffner and F. Speelman",
title = " The Garden-Hose Game: A New Model of Computation, and Application to
Position-Based Quantum Cryptography",
year = "2011",
Note = "E-print arXiv:1109.2563",
}

@ARTICLE{BK11,
   author       = "S. Beigi and R. K{\"{o}}nig",
title ="Simplified instantaneous non-local quantum computation with
applications to position-based cryptography",
   journal      = "New J. Phys.",
   volume       = "13",
   pages        = "093036",
   year         = "2011",
url ="http://iopscience.iop.org/1367-2630/13/9/093036/"
}

@ARTICLE{AS11,
   author       = "S. W. Al-Safi and A. J. Short",
title = "Information causality from an entropic and probabilistic
perspective.",
   journal      = "Phys. Rev. A",
   volume       = "84",
   pages        = "042323",
   year         = "2011",
url = "http://link.aps.org/doi/10.1103/PhysRevA.84.042323"
}

@ARTICLE{GWAN11,
   author       = "R. Gallego and L. E. W{\"{u}}rflinger and A. Ac\'in and M.
Navascu\'es",
title = "Quantum correlations require multipartite information principles",
   journal      = "Phys. Rev. Lett.",
   volume       = "107",
   pages        = "210403",
   year         = "2011",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.107.210403"
}

@ARTICLE{YCATS12,
   author       = "T. H. Yang and D. Cavalcanti and M. L. Almeida and C. Teo
and V. Scarani",
title = "Information-causality and extremal tripartite correlations",
   journal      = "New J. Phys.",
   volume       = "14",
   pages        = "013061",
   year         = "2012",
url = "http://iopscience.iop.org/1367-2630/14/1/013061"
}

@UNPUBLISHED{DPG1,
   author = "D. Pital\'ua-Garc\'ia",
   note = "to be published",
}

@UNPUBLISHED{DPG2,
   author = "D. Pital\'ua-Garc\'ia",
   note = "to be published",
}

@Book{NielsenandChuangbook,
 author    = "M. A. Nielsen and I. L. Chuang",
 title     = "Quantum Computation and Quantum Information",
 publisher = "Cambridge University Press",
address= "Cambridge, UK",
 year      =  2000,
}




@ARTICLE{teleportation,
   author       = "C. H. Bennett and G. Brassard and C. Cr\'epeau and R. Jozsa
and A. Peres and W. K. Wootters",
 title = "Teleporting an unknown quantum state via dual classical and
{E}instein-{P}odolsky-{R}osen channels",
   journal      = "Phys. Rev. Lett.",
   volume       = "70",
   pages        = "1895",
   year         = "1993",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.70.1895"
}



@incollection{BBCS92,
year={1992},
isbn={978-3-540-55188-1},
booktitle={Advances in Cryptology — CRYPTO ’91},
volume={576},
series={Lecture Notes in Computer Science},
editor={Feigenbaum, Joan},
doi={10.1007/3-540-46766-1_29},
title={Practical Quantum Oblivious Transfer},
url={http://dx.doi.org/10.1007/3-540-46766-1_29},
publisher={Springer Berlin Heidelberg},
author={Bennett, CharlesH. and Brassard, Gilles and Cr\'epeau, Claude and Skubiszewska, Marie-Hélène},
pages={351-366},
language={English}
}



, “Practical quantum
oblivious transfer,” in Advances in Cryptology: Proceedings of Crypto ’91, Lecture Notes
in Computer Science, Vol. 576, p. 351-366. Springer-Verlag, 1992.



@INPROCEEDINGS{BB84,
   author       = "C. H. Bennett and G. Brassard",
booktitle      = "Proceedings of IEEE International Conference on Computers,
Systems, and Signal Processing, Bangalore, India",
   pages        = "175",
   publisher       = "IEEE",
address= "New York",
   year         = "1984",
}


@ARTICLE{BHK05,
   author       = "J. Barrett and L. Hardy and A. Kent",
title = "No signaling and quantum key distribution",
   journal      = "Phys. Rev. Lett.",
   volume       = "95",
   pages        = "010503",
   year         = "2005",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.95.010503"
}

@ARTICLE{EPR35,
   author       = "A. Einstein and B. Podolsky and N. Rosen",
title = "Can quantum-mechanical description of physical reality be considered
complete?",
   journal      = "Phys. Rev.",
   volume       = "47",
   pages        = "777",
   year         = "1935",
url = "http://link.aps.org/doi/10.1103/PhysRev.47.777"
}

@ARTICLE{Bell,
   author       = "J. S. Bell",
title = "On the {E}instein {P}odolsky {R}osen paradox",
   year         = "1964",
   journal      = "Physics",
   volume       = "1",
   pages        = "195-200",
}

@ARTICLE{GRW80,
   author       = "G. C. Ghirardi and A. Rimini and T. Weber",
title = "A general argument against superluminal transmission through the
quantum mechanical measurement process",
   journal      = "Lett. Nuov. Cim.",
   volume       = "27",
   pages        = "293",
   year         = "1980",
url = "http://www.springerlink.com/content/t5h287h1r26j25j4/"
}

@ARTICLE{K73,
   author       = "A. S. Kholevo",
   title = "Bounds for the quantity of information transmitted by a quantum
communication channel",
   journal      = "Probl. Inf. Transm.",
   volume       = "9",
   pages        = "177",
   year         = "1973",
}

@ARTICLE{ic,
   author       = "M. Paw{\l}owski and T. Paterek and D. Kaszlikowski and V.
Scarani and A. Winter and M. {\.{Z}}ukowski",
title = "Information causality as a physical principle.",
   journal      = "Nature (London)",
   volume       = "461",
   pages        = "1101",
   year         = "2009",
url = "http://www.nature.com/nature/journal/v461/n7267/full/nature08400.html"
}


@ARTICLE{ABPS09,
   author       = "J. Allcock and N. Brunner and M. Paw{\l}owski and V.
Scarani",
title = "Recovering part of the boundary between quantum and nonquantum
correlations from information causality",
   journal      = "Phys. Rev. A",
   volume       = "80",
   pages        = "040103",
   year         = "2009",
url = "http://link.aps.org/doi/10.1103/PhysRevA.80.040103"
}

@ARTICLE{CSS10,
   author       = "D. Cavalcanti and A. Salles and V. Scarani",
title = "Macroscopically local correlations can violate information causality",
   journal      = "Nat. Commun.",
   volume       = "1",
   pages        = "136",
   year         = "2010",
url = "http://www.nature.com/ncomms/journal/v1/n9/full/ncomms1138.html"
}

@ARTICLE{GWAN11,
   author       = "R. Gallego and L. E. W{\"{u}}rflinger and A. Ac\'in and M.
Navascu\'es",
title = "Quantum correlations require multipartite information principles",
   journal      = "Phys. Rev. Lett.",
   volume       = "107",
   pages        = "210403",
   year         = "2011",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.107.210403"
}

@ARTICLE{YCATS12,
   author       = "T. H. Yang and D. Cavalcanti and M. L. Almeida and C. Teo
and V. Scarani",
title = "Information-causality and extremal tripartite correlations",
   journal      = "New J. Phys.",
   volume       = "14",
   pages        = "013061",
   year         = "2012",
url = "http://iopscience.iop.org/1367-2630/14/1/013061"
}

@ARTICLE{C80,
   author       = "B. S. Cirel'son",
title = "Quantum generalizations of {B}ell's inequality",
   journal      = "Lett. Math. Phys.",
   volume       = "4",
   pages        = "93",
   year         = "1980",
url = "http://www.springerlink.com/content/l57053g573430450/"
}

@ARTICLE{PR94,
   author       = "S. Popescu and D. Rohrlich",
title = "Quantum nonlocality as an axiom",
   journal      = "Found. Phys.",
   volume       = "24",
   pages        = "379",
   year         = "1994",
url = "http://www.springerlink.com/content/j842v3324u512nx0/"
}

@ARTICLE{LR68,
   author       = "O. E. Lanford and D. W. Robinson",
title = "Mean entropy of states in quantum-statistical mechanics",
   journal      = "J. Math. Phys.",
   volume       = "9",
   pages        = "1120",
   year         = "1968",
url = "http://jmp.aip.org/resource/1/jmapaq/v9/i7/p1120_s1"
}

@ARTICLE{AL70,
   author       = "H. Araki and E. H. Lieb",
title = "Entropy inequalities",
   journal      = "Commun. Math. Phys.",
   volume       = "18",
   pages        = "160",
   year         = "1970",
url = "http://www.springerlink.com/content/wk224145h1441527/"
}

@Unpublished{H01,
author = "L. Hardy",
title ="Quantum Theory From Five Reasonable Axioms",
year = "2001",
note = "E-print arXiv:quant-ph/0101012v4",
}

@ARTICLE{B07,
   author       = "J. Barrett",
title = "Information processing in generalized probabilistic theories",
   journal      = "Phys. Rev. A",
   volume       = "75",
   pages        = "032304",
   year         = "2007",
url = "http://link.aps.org/doi/10.1103/PhysRevA.75.032304"
}

@ARTICLE{BBLW07,
   author       = "H. Barnum and J. Barrett and M. Leifer and A. Wilce",
title = "Generalized no-broadcasting theorem",
   journal      = "Phys. Rev. Lett.",
   volume       = "99",
   pages        = "240501",
   year         = "2007",
url = "http://link.aps.org/doi/10.1103/PhysRevLett.99.240501"
}

@ARTICLE{SW10,
   author       = "A. J. Short and S. Wehner",
title = "Entropy in general physical theories",
   journal      = "New J. Phys.",
   volume       = "12",
   pages        = "033023",
   year         = "2010",
url = "http://iopscience.iop.org/1367-2630/12/3/033023"
}

@ARTICLE{BBCLSSWW10,
   author       = "H. Barnum and J. Barrett and L. O. Clark and M. Leifer and
R. Spekkens and N. Stepanik and A. Wilce and R. Wilke",
title = "Entropy and information causality in general probabilistic theories",
   journal      = "New J. Phys.",
   volume       = "12",
   pages        = "033024",
   year         = "2010",
url = "http://iopscience.iop.org/1367-2630/12/3/033024"
}

@ARTICLE{AS11,
   author       = "S. W. Al-Safi and A. J. Short",
title = "Information causality from an entropic and a probabilistic
perspective",
   journal      = "Phys. Rev. A",
   volume       = "84",
   pages        = "042323",
   year         = "2011",
   url = "http://link.aps.org/doi/10.1103/PhysRevA.84.042323"
}

@ARTICLE{W83,
   author       = "S. Wiesner",
title = "Conjugate coding",
   journal      = "SIGACT News",
   volume       = "15",
   pages        = "78",
   year         = "1983",
url = "http://dl.acm.org/citation.cfm?doid=1008908.1008920"
}

@ARTICLE{ANTV02,
   author       = "A. Ambainis and A. Nayak and A. Ta-Shma and U. Vazirani",
title = "Dense quantum coding and quantum finite automata",
   journal      = "J. ACM",
   volume       = "49",
   pages        = "496",
   year         = "2002",
url = "http://dl.acm.org/citation.cfm?doid=581771.581773"
}

@ARTICLE{PZ10,
   author       = "M. Paw{\l}owski and M. {\.{Z}}ukowski",
title = "Entanglement-assisted random access codes",
   journal      = "Phys. Rev. A",
   volume       = "81",
   pages        = "042326",
   year         = "2010",
url = "http://link.aps.org/doi/10.1103/PhysRevA.81.042326"
}

@article{G91,
title = {Bell's inequality holds for all non-product states},
journal = {Phys. Lett. A},
volume = {154},
number = {5},
pages = {201-202},
year = {1991},
issn = {0375-9601},
doi = {https://doi.org/10.1016/0375-9601(91)90805-I},
url = {https://www.sciencedirect.com/science/article/pii/037596019190805I},
author = {N. Gisin},
abstract = {We prove that any non-product state of two-particle systems violates a Bell inequality.}
}






@article{bukh,
  title={Measurable sets with excluded distances},
  author={Bukh, Boris},
  journal={Geometric and Functional Analysis},
  volume={18},
  number={3},
  pages={668--697},
  year={2008},
  publisher={Springer},
url={http://link.springer.com/article/10.1007/s00039-008-0673-8}
}

@article{de2008fourier,
  title={Fourier analysis, linear programming, and densities of distance
avoiding sets in Rn},
  author={de Oliveira Filho, Fernando M{\'a}rio and Vallentin, Frank},
  journal={J. Eur. Math. Soc.},
  volume={12},
  pages={ 1417-1428},
  year={2010},
url={http://www.ems-ph.org/journals/show_abstract.php?issn=1435-9855&vol=12&iss=6&rank=5}
}

@article{W06,
  title = {Tsirelson bounds for generalized Clauser-Horne-Shimony-Holt inequalities},
  author = {Wehner, Stephanie},
  journal = {Phys. Rev. A},
  volume = {73},
  issue = {2},
  pages = {022110},
  numpages = {5},
  year = {2006},
  month = {Feb},
  doi = {10.1103/PhysRevA.73.022110},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.73.022110},
  publisher = {American Physical Society}
}


@Book{Mackey63,
 author    = "G. Mackey",
 title     = "Mathematical Foundations of Quantum Mechanics",
 publisher = "Benjamin",
 year      =  1963
}

@article{DL70,
  title = {An operational approach to quantum probability},
  author = {E. B. Davies and J. T. Lewis},
  journal = {Commun. Math. Phys.},
  volume = {17},
number={3},
doi={10.1007/BF01647093},
url={http://dx.doi.org/10.1007/BF01647093},
publisher={Springer-Verlag},
pages={239-260},
year= {1970}
}



@INPROCEEDINGS{Foulis81,
   author       = "D. J. Foulis and C. H. Randall",
title = "Empirical logic and tensor products",
   booktitle      = "H. Neumann, (ed.), Interpretations and Foundations of Quantum Theory, Bibliographisches Institut, Wissenschaftsverlag, Mannheim",
      year         = "1981",
}

@Book{Ludwig85,
 author    = "G. Ludwig",
 title     = "An Axiomatic Basis of Quantum Mechanics 1, 2",
 publisher = "Springer--Verlag",
 year      =  "1985, 1987"
}

@article{Chiribella10,
  title = {Probabilistic theories with purification},
  author = {Chiribella, Giulio and D'Ariano, Giacomo Mauro and Perinotti, Paolo},
  journal = {Phys. Rev. A},
  volume = {81},
  issue = {6},
  pages = {062348},
  numpages = {40},
  year = {2010},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.81.062348},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.81.062348}
}

@article{Chiribella11,
  title = {Informational derivation of quantum theory},
  author = {Chiribella, Giulio and D'Ariano, Giacomo Mauro and Perinotti, Paolo},
  journal = {Phys. Rev. A},
  volume = {84},
  issue = {1},
  pages = {012311},
  numpages = {39},
  year = {2011},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.84.012311},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.84.012311}
}

@article{BPALSNG12,
  title = {Quantum non{-}locality based on finite{-}speed causal influences leads to superluminal signalling},
  author = {J{-}D. Bancal and S. Pironio and A. Ac{\i}n and Y{-}C. Liang and V. Scarani and N. Gisin},
  journal = {Nature Phys.},
  volume = {8},
  pages = {867–870},
  year = {2012},
  doi = {10.1038/nphys2460},
  url = {http://www.nature.com/nphys/journal/v8/n12/full/nphys2460.html}
}




@article{CDP11,
  title = {Informational derivation of quantum theory},
  author = {Chiribella, Giulio and D'Ariano, Giacomo Mauro and Perinotti, Paolo},
  journal = {Phys. Rev. A},
  volume = {84},
  issue = {1},
  pages = {012311},
  numpages = {39},
  year = {2011},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.84.012311},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.84.012311}
}



@Unpublished{MM13,
author = "L. Masanes and M. P. M{\"{u}}ller",
title="Information-theoretic postulates for quantum theory",
year="2013",
eprint = "1203.4516v2",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=1203.4516v2;%%"
}

@article{FMPT13,
  author={Samuel Fiorini and Serge Massar and Manas K Patra and Hans Raj Tiwary},
  title={Generalized probabilistic theories and conic extensions of polytopes},
  journal={J. Phys. A: Math. Theor.},
  volume={48},
  number={2},
  pages={025302},
  url={http://stacks.iop.org/1751-8121/48/i=2/a=025302},
  year={2015},
  abstract={Generalized probabilistic theories (GPT) provide a general framework that includes classical and quantum theories. It is described by a cone C and its dual C *. We show that whether some one-way communication complexity problems can be solved within a GPT is equivalent to the recently introduced cone factorization of the corresponding communication matrix M . We also prove an analogue of Holevoʼs theorem: when the cone C is contained in ##IMG## [http://ej.iop.org/images/1751-8121/48/2/025302/jpa505184ieqn1.gif] {${{\mathbb{R}}^{n}}$} , the classical capacity of the channel realized by sending GPT states and measuring them is bounded by ##IMG## [http://ej.iop.org/images/1751-8121/48/2/025302/jpa505184ieqn2.gif] {${\rm log} n$} . Polytopes and optimising functions over polytopes arise in many areas of discrete mathematics. A conic extension of a polytope is the intersection of a cone C with an affine subspace whose projection onto the original space yields the desired polytope. Extensions of polytopes can sometimes be much simpler geometric objects than the polytope itself. The existence of a conic extension of a polytope is equivalent to that of a cone factorization of the slack matrix of the polytope, on the same cone. We show that all ##IMG## [http://ej.iop.org/images/1751-8121/48/2/025302/jpa505184ieqn3.gif] {$0/1$} polytopes whose vertices can be recognized by a polynomial size circuit, which includes as a special case the travelling salesman polytope and many other polytopes from combinatorial optimization, have small conic extension complexity when the cone is the completely positive cone. Using recent exponential lower bounds on the linear extension complexity of polytopes, this provides an exponential gap between the communication complexity of GPT based on the completely positive cone and classical communication complexity, and a conjectured exponential gap with quantum communication complexity. Our work thus relates the communication complexity of generalizations of quantum theory to questions of mainstream interest in the area of combinatorial optimization.}
}
	
  	
@article{BKLS14,
  author={Nicolas Brunner and Marc Kaplan and Anthony Leverrier and Paul Skrzypczyk},
  title={Dimension of physical systems, information processing, and thermodynamics},
  journal={New J. Phys.},
  volume={16},
  number={12},
  pages={123050},
  url={http://stacks.iop.org/1367-2630/16/i=12/a=123050},
  year={2014},
  abstract={We ask how quantum theory compares to more general physical theories from the point of view of dimension. To do so, we first give two model-independent definitions of the dimension of physical systems, based on measurements and the capacity of storing information. While both definitions are equivalent in classical and quantum mechanics, they are different in generalized probabilistic theories. We discuss in detail the case of a theory known as ‘boxworld’, and show that such a theory features systems with dimension mismatch. This dimension mismatch can be made arbitrarily large using an amplification procedure. Furthermore, we show that the dimension mismatch of boxworld has strong consequences on its power for performing information-theoretic tasks, leading to the collapse of communication complexity and to the violation of information causality. Finally, we discuss the consequences of a dimension mismatch from the perspective of thermodynamics, and ask whether this effect could break Landauerʼs erasure principle and thus the second law.}
}
	
@article{MP14,
  title = {Information and communication in polygon theories},
  author = {Massar, Serge and Patra, Manas K.},
  journal = {Phys. Rev. A},
  volume = {89},
  issue = {5},
  pages = {052124},
  numpages = {8},
  year = {2014},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.89.052124},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.89.052124}
}


@Unpublished{CHHH14,
author = "L. Czekaj and M. Horodecki and P. Horodecki and R. Horodecki",
title="Information Content of Elementary Systems as a Physical Principle",
year="2014",
eprint = "1403.4643",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=1403.4643;%%"
}

@article{H09,
  title = {Superadditivity of communication capacity using entangled inputs},
  author = {M.B. Hastings},
  journal = {Nature Physics},
  volume = {5},
  pages = {255--257},
  year = {2009},
doi={10.1038/nphys1224}
}

@INPROCEEDINGS{BW13,
title ="Post-Classical Probability Theory",
   author       = "H. Barnum and A. Wilce",
booktitle      = "G. Chiribella and R.W. Spekkens, (ed.), Quantum Theory: Informational Foundations and Foils, Springer",
year = "2014",
Note = "{P}ost-Classical Probability Theory. E-print arXiv:1205.3833 (2013).",
url = "http://arxiv.org/abs/1205.3833",
}

@ARTICLE{PDB10,
	author = { T. Paterek and B. Daki\'c and \v{C}. Brukner},
	title = { Theories of systems with limited information content },
	journal = {New J. Phys.},
	year = { 2010 },
	pages = { 053037 },
	volume = { 12 },
doi={10.1088/1367-2630/12/5/053037}
}


@article{PW12,
  title = {``Hyperbits'': The information quasiparticles},
  author = {Paw\l{}owski, Marcin and Winter, Andreas},
  journal = {Phys. Rev. A},
  volume = {85},
  issue = {2},
  pages = {022331},
  numpages = {6},
  year = {2012},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.85.022331},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.85.022331}
}


@article{Z08,
  author={Karol \.{Z}yczkowski},
  title={Quartic quantum theory: an extension of the standard quantum mechanics},
  journal={J. Phys. A: Math. Theor.},
  volume={41},
  number={35},
  pages={355302},
  url={http://stacks.iop.org/1751-8121/41/i=35/a=355302},
  year={2008},
  abstract={We propose an extended quantum theory, in which the number K of parameters necessary to characterize a quantum state behaves as fourth power of the number N of distinguishable states. As the simplex of classical N -point probability distributions can be embedded inside a higher-dimensional convex body ##IMG## [http://ej.iop.org/images/1751-8121/41/35/355302/jpa278068ieqn1.gif] {{\cal M}_N^Q} of mixed quantum states, one can further increase the dimensionality constructing the set of extended quantum states. The embedding proposed corresponds to an assumption that the physical system described in the N -dimensional Hilbert space is coupled with an auxiliary subsystem of the same dimensionality. The extended theory works for simple quantum systems and is shown to be a non-trivial generalization of the standard quantum theory for which K = N 2 . Imposing certain restrictions on initial conditions and dynamics allowed in the quartic theory one obtains quadratic theory as a special case. By imposing even stronger constraints one arrives at the classical theory, for which K = N .}
}
	
@article{U96,
author={A. Uhlmann},
title={Spheres and hemispheres as quantum state spaces},
journal={J. Geom. Phys.},
volume={18},
pages={76-92},
url = {http://www.sciencedirect.com/science/article/pii/0393044095000046},
year={1996}
}


@INPROCEEDINGS{DB09,
   author       = "B. Daki\'c and \v{C}. Brukner",
title = "Quantum Theory and Beyond: Is Entanglement Special?",
   booktitle      = "H. Halvorson, (ed.), Deep Beauty: Understanding the Quantum World through Mathematical Innovation, Cambridge University Press",
      year         = "2011",
pages= "365--392",
Note= "E-print arXiv:0911.0695 (2009).",
url = "http://arxiv.org/abs/0911.0695"
}

@Unpublished{BBLW08,
author = "H. Barnum and J. Barrett and M. Leifer and A. Wilce",
title = "Teleportation in General Probabilistic Theories",
year = "2008",
eprint = "0805.3553",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=0805.3553;%%",
}

@Book{CTbook,
 author    = "T. M. Cover and J. A. Thomas",
 title     = "Elements of Information Theory",
 publisher = "John Wiley & Sons",
address= "New Jersey",
 year      =  2006,
}

@article{JL13,
  title = {Generalized probabilistic theories without the no-restriction hypothesis},
  author = {Janotta, Peter and Lal, Raymond},
  journal = {Phys. Rev. A},
  volume = {87},
  issue = {5},
  pages = {052131},
  numpages = {14},
  year = {2013},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.87.052131},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.87.052131}
}

@article{BDFMRSSW99,
  title = {Quantum nonlocality without entanglement},
  author = {Bennett, Charles H. and DiVincenzo, David P. and Fuchs, Christopher A. and Mor, Tal and Rains, Eric and Shor, Peter W. and Smolin, John A. and Wootters, William K.},
  journal = {Phys. Rev. A},
  volume = {59},
  issue = {2},
  pages = {1070--1091},
  numpages = {0},
  year = {1999},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.59.1070},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.59.1070}
}

	
@article{SB12,
  author={Anthony J Short and Jonathan Barrett},
  title={Strong nonlocality: a trade-off between states and measurements},
  journal={New J. Phys.},
  volume={12},
  number={3},
  pages={033034},
  url={http://stacks.iop.org/1367-2630/12/i=3/a=033034},
  year={2010},
  abstract={Measurements on entangled quantum states can produce outcomes that are nonlocally correlated. But according to Tsirelson's theorem, there is a quantitative limit on quantum nonlocality. It is interesting to explore what would happen if Tsirelson's bound were violated. To this end, we consider a model that allows arbitrary nonlocal correlations, colloquially referred to as 'box world'. We show that while box world allows more highly entangled states than quantum theory, measurements in box world are rather limited. As a consequence there is no entanglement swapping, teleportation or dense coding.}
}

@article{SY08,
  author={Graeme Smith and Jon Yard},
  title={Quantum Communication with Zero-Capacity Channels},
  journal={Science},
  volume={321},
  number={5897},
  pages={1812-1815},
doi={10.1126/science.1162242},
  url={http://www.sciencemag.org/content/321/5897/1812},
  year={2008}
}



@article{ZZHE93,
  title = {``Event-ready-detectors'' Bell experiment via entanglement swapping},
  author = {\ifmmode \dot{Z}\else \.{Z}\fi{}ukowski, M. and Zeilinger, A. and Horne, M. A. and Ekert, A. K.},
  journal = {Phys. Rev. Lett.},
  volume = {71},
  issue = {26},
  pages = {4287--4290},
  numpages = {0},
  year = {1993},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.71.4287},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.71.4287}
}

@article{JGBB11,
  author={Peter Janotta and Christian Gogolin and Jonathan Barrett and Nicolas Brunner},
  title={Limits on nonlocal correlations from the structure of the local state space},
  journal={New Journal of Physics},
  volume={13},
  number={6},
  pages={063024},
  url={http://stacks.iop.org/1367-2630/13/i=6/a=063024},
  year={2011},
  abstract={The outcomes of measurements on entangled quantum systems can be nonlocally correlated. However, while it is easy to write down toy theories allowing arbitrary nonlocal correlations, those allowed in quantum mechanics are limited. Quantum correlations cannot, for example, violate a principle known as macroscopic locality, which implies that they cannot violate Tsirelson's bound. This paper shows that there is a connection between the strength of nonlocal correlations in a physical theory and the structure of the state spaces of individual systems. This is illustrated by a family of models in which local state spaces are regular polygons, where a natural analogue of a maximally entangled state of two systems exists. We characterize the nonlocal correlations obtainable from such states. The family allows us to study the transition between classical, quantum and super-quantum correlations by varying only the local state space. We show that the strength of nonlocal correlations—in particular whether the maximally entangled state violates Tsirelson's bound or not—depends crucially on a simple geometric property of the local state space, known as strong self-duality. This result is seen to be a special case of a general theorem, which states that a broad class of entangled states in probabilistic theories—including, by extension, all bipartite classical and quantum states—cannot violate macroscopic locality. Finally, our results show that models exist that are locally almost indistinguishable from quantum mechanics, but can nevertheless generate maximally nonlocal correlations.}
}



@article{AACHKLMP10,
  title = {Unified Framework for Correlations in Terms of Local Quantum Observables},
  author = {Ac\'in, A. and Augusiak, R. and Cavalcanti, D. and Hadley, C. and Korbicz, J. K. and Lewenstein, M. and Masanes, Ll. and Piani, M.},
  journal = {Phys. Rev. Lett.},
  volume = {104},
  issue = {14},
  pages = {140404},
  numpages = {4},
  year = {2010},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.104.140404},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.104.140404}
}

@article{TMSM12,
  title = {Deriving Quantum Theory from Its Local Structure and Reversibility},
  author = {de la Torre, Gonzalo and Masanes, Llu\'\is and Short, Anthony J. and M\"uller, Markus P.},
  journal = {Phys. Rev. Lett.},
  volume = {109},
  issue = {9},
  pages = {090403},
  numpages = {5},
  year = {2012},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.109.090403},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.109.090403}
}

@Book{StoneGoldbartbook,
 author    = "M. Stone and P. Goldbart",
 title     = "Mathematics for Physics",
 publisher = "Cambridge University Press",
address= " Cambridge",
 year      =  2009,
}

@Book{Weinbergbook,
 author    = "S. Weinberg",
 title     = "The Quantum Theory of Fields",
volume="I",
 publisher = "Cambridge University Press",
address= " Cambridge",
 year      =  1995,
}


@article{W39,
  title = {On Unitary Representations of the Inhomogeneous Lorentz Group},
  author = {E. Wigner},
  journal = {Ann. Math.},
  volume = {40},
  issue = {1},
  pages = {149-204},
  year = {1939},
}

@Book{Naimarkbook,
 author    = "M. A. Naimark",
 title     = "Linear representations of the Lorentz group",
 publisher = "Pergamon Press",
address= " Oxford",
 year      =  1964,
Note= "Translated from Russian by A. Swinfen and O. J. Marstrand. Translation edited by H. K. Farahat",
}

@article{BBBEW10,
  title = {Local Quantum Measurement and No-Signaling Imply Quantum Correlations},
  author = {Barnum, H. and Beigi, S. and Boixo, S. and Elliott, M. B. and Wehner, S.},
  journal = {Phys. Rev. Lett.},
  volume = {104},
  issue = {14},
  pages = {140401},
  numpages = {4},
  year = {2010},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.104.140401},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.104.140401}
}


@Unpublished{H13,
author = "L. Hardy",
title = "Reconstructing quantum theory",
year = "2013",
eprint = "1303.1538",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=1303.1538;%%",
}

@Unpublished{H11,
author = "L. Hardy",
title = "Reformulating and Reconstructing Quantum Theory",
year = "2011",
eprint = "1104.2066",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=1104.2066;%%",
}


@article{L97,
  title = {Insecurity of quantum secure computations},
  author = {Hoi-Kwong Lo},
  journal = {Phys. Rev. A},
  volume = {56},
  issue = {2},
  pages = {1154-1162},
  numpages = {9},
  year = {1997},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.56.1154}
}


@article{M97,
  title = {Unconditionally Secure Quantum Bit Commitment is Impossible},
  author = {D. Mayers},
  journal = {Phys. Rev. Lett.},
  volume = {78},
  issue = {17},
  pages = {3414},
  numpages = {4},
  year = {1997},
  doi = {10.1103/PhysRevLett.78.3414},
  publisher = {American Physical Society}
}

@article{LC97,
  title = {Is Quantum Bit Commitment Really Possible?},
  author = {Hoi-Kwong Lo and H. F. Chau},
  journal = {Phys. Rev. Lett.},
  volume = {78},
  issue = {17},
  pages = {3410-3413},
  numpages = {4},
  year = {1997},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.78.3410}
}

@article{C07,
  title = {Impossibility of secure two-party classical computation},
  author = {R. Colbeck},
  journal = {Phys. Rev. A},
  volume = {76},
  pages = {062308},
  numpages = {8},
  year = {2007},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.76.062308}
}

@article{HW06,
  title = {Oblivious transfer using quantum entanglement},
  author = {He, Guang Ping and Wang, Z. D.},
  journal = {Phys. Rev. A},
  volume = {73},
  issue = {1},
  pages = {012331},
  numpages = {9},
  year = {2006},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.73.012331},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.73.012331}
}




@article{BCS12,
  title = {Complete Insecurity of Quantum Protocols for Classical Two-Party Computation},
  author = {H. Buhrman and M. Christandl and C. Schaffner},
  journal = {Phys. Rev. Lett.},
  volume = {109},
  pages = {160501},
  numpages = {5},
  year = {2012},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.109.160501}
}

@article{K12,
  title = {Unconditionally Secure Bit Commitment by Transmitting Measurement Outcomes},
  author = {A. Kent},
  journal = {Phys. Rev. Lett.},
  volume = {109},
  pages = {130501},
  numpages = {4},
  year = {2012},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.109.130501}
}

@article{LKBHTKGWZ13,
  title = {Experimental Bit Commitment Based on Quantum Communication and Special Relativity},
  author = {T. Lunghi and J. Kaniewski and F. Bussi\`{e}res and R. Houlmann and M. Tomamichel and A. Kent and N. Gisin and S. Wehner and H. Zbinden},
  journal = {Phys. Rev. Lett.},
  volume = {111},
  pages = {180504},
  numpages = {5},
  year = {2013},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.111.180504}
}

@article{SRKBPMLM15,
  title = {Attacks exploiting deviation of mean photon number in quantum key distribution and coin tossing},
  author = {Sajeed, Shihan and Radchenko, Igor and Kaiser, Sarah and Bourgoin, Jean-Philippe and Pappa, Anna and Monat, Laurent and Legr\'e, Matthieu and Makarov, Vadim},
  journal = {Phys. Rev. A},
  volume = {91},
  issue = {3},
  pages = {032326},
  numpages = {13},
  year = {2015},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.91.032326},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.91.032326}
}

@manual{singlequantum,
title = {Single Quantum Eos},
organization = {Single Quantum},
note = {Datasheet},
 url = {www.singlequantum.com}
}

#




@article{LCCLWCLLSLZZCPZCP14,
  title = {Experimental Unconditionally Secure Bit Commitment},
  author = {Y. Liu and Y. Cao and M. Curty and S.-K. Liao and J. Wang and K. Cui and Y.-H. Li and Z.-H. Lin and Q.-C. Sun and D.-D. Li and H.-F. Zhang and Y. Zhao and T.-Y Chen and C.-Z. Peng and Q. Zhang and A. Cabello and J.-W. Pan},
  journal = {Phys. Rev. Lett.},
  volume = {112},
  pages = {010504},
  numpages = {5},
  year = {2014},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.112.010504}
}

@article{KMS14,
  title = {Secure and Robust Transmission and Verification of Unknown Quantum States in Minkowski Space},
  author = {A. Kent and S. Massar and J. Silman},
  journal = {Sci. Rep.},
  volume = {4},
  pages = {3901},
  numpages = {7},
  year = {2014},
  publisher = {American Physical Society},
  doi = {10.1038/srep03901}
}

@article{AK15.1,
author = {Adlam, Emily and Kent, Adrian},
title = {Deterministic relativistic quantum bit commitment},
journal = {Int. J. Quantum Inf.},
volume = {13},
number = {05},
pages = {1550029},
year = {2015},
doi = {10.1142/S021974991550029X},
URL = {http://www.worldscientific.com/doi/abs/10.1142/S021974991550029X}
}

@article{AK15.2,
  title = {Device-independent relativistic quantum bit commitment},
  author = {Adlam, Emily and Kent, Adrian},
  journal = {Phys. Rev. A},
  volume = {92},
  issue = {2},
  pages = {022315},
  numpages = {9},
  year = {2015},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.92.022315},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.92.022315}
}

@article{WF10,
  title = {Relativistic statistical arbitrage},
  author = {Wissner-Gross, A. D. and Freer, C. E.},
  journal = {Phys. Rev. E},
  volume = {82},
  issue = {5},
  pages = {056104},
  numpages = {7},
  year = {2010},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.82.056104},
  url = {http://link.aps.org/doi/10.1103/PhysRevE.82.056104}
}


@techreport{R81,
    author    = "M. O. Rabin",
    title     = "How To exchange Secrets with Oblivious Transfer",
    institution = "Aiken Computation Lab, Harvard University",
    year      = "1981",
url ="https://www.iacr.org/museum/rabin-obt/obtrans-eprint187.pdf"
}

@INPROCEEDINGS{BB84,
   author       = "C. H. Bennett and G. Brassard",
title = "Quantum cryptography: {P}ublic key distribution and coin tossing",
booktitle      = "Proceedings of IEEE International Conference on Computers, Systems, and Signal Processing, Bangalore, India",
   pages        = "175--179",
   publisher       = "IEEE",
address= "New York",
   year         = "1984",
}



@INPROCEEDINGS{K88,
author={J. Kilian},
title={Founding Crytpography on Oblivious Transfer},
booktitle={Proceedings of the Twentieth Annual ACM Symposium on Theory of Computing, STOC '88},
pages={20--31},
publisher={ACM},
address={New York},
year={1988},
} 
 %series = "STOC '88'',
%isbn = {0-89791-264-0},
 %location = {Chicago, Illinois, USA},
%numpages = {12},
%doi = {10.1145/62212.62215},
 %acmid = {62215},
% url = {http://doi.acm.org/10.1145/62212.62215},

@article{SIGA05,
  title = {Quantum cloning},
  author = {Scarani, Valerio and Iblisdir, Sofyan and Gisin, Nicolas and Ac\'{i}n, Antonio},
  journal = {Rev. Mod. Phys.},
  volume = {77},
  issue = {4},
  pages = {1225--1256},
  numpages = {0},
  year = {2005},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.77.1225},
  url = {http://link.aps.org/doi/10.1103/RevModPhys.77.1225}
}

@article{K99,
  title = {Unconditionally Secure Bit Commitment},
  author = {Kent, Adrian},
  journal = {Phys. Rev. Lett.},
  volume = {83},
  issue = {7},
  pages = {1447--1450},
  numpages = {0},
  year = {1999},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.83.1447},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.83.1447}
}

@article{CK12,
  title = {Security details for bit commitment by transmitting measurement outcomes},
  author = {Croke, Sarah and Kent, Adrian},
  journal = {Phys. Rev. A},
  volume = {86},
  issue = {5},
  pages = {052309},
  numpages = {3},
  year = {2012},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.86.052309},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.86.052309}
}


  	
@article{BC09,
  author={Stephen M Barnett and Sarah Croke},
  title={On the conditions for discrimination between quantum states with minimum error},
  journal={Journal of Physics A: Mathematical and Theoretical},
  volume={42},
  number={6},
  pages={062001},
  url={http://stacks.iop.org/1751-8121/42/i=6/a=062001},
  year={2009},
  abstract={We provide a simple proof for the necessity of conditions for discriminating with minimum error between a known set of quantum states.}
}
	

@ARTICLE{KTHW13, 
author={Kaniewski, J. and Tomamichel, M. and Hanggi, E. and Wehner, S.}, 
journal={Information Theory, IEEE Transactions on}, 
title={Secure Bit Commitment From Relativistic Constraints}, 
year={2013}, 
month={July}, 
volume={59}, 
number={7}, 
pages={4687-4699}, 
keywords={cryptographic protocols;quantum cryptography;quantum theory;Kent quantum protocol;Mayers-Lo-Chau no-go argument;quantum mechanics;relativistic constraints;secure bit commitment;special relativity;split models;two-party cryptographic protocols;Cryptography;Entropy;Mathematical model;Protocols;Registers;Uncertainty;Bit commitment;quantum theory;special relativity}, 
doi={10.1109/TIT.2013.2247463}, 
ISSN={0018-9448},}

@article{AK15.2,
  title = {Device-independent relativistic quantum bit commitment},
  author = {Adlam, Emily and Kent, Adrian},
  journal = {Phys. Rev. A},
  volume = {92},
  issue = {2},
  pages = {022315},
  numpages = {9},
  year = {2015},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.92.022315},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.92.022315}
}

@article{AK15.1,
  title = {Deterministic relativistic quantum bit commitment},
  author = {Adlam, Emily and Kent, Adrian},
  journal = {Int. J. Quantum Inf. },
  year = {2015},
  doi = {10.1142/S021974991550029X}
}


  	
@article{K12.1,
  author={Adrian Kent},
  title={Quantum tasks in {M}inkowski space},
  journal={Class. Quantum Grav.},
  volume={29},
  number={22},
  pages={224013},
  url={http://stacks.iop.org/0264-9381/29/i=22/a=224013},
  year={2012},
  abstract={The fundamental properties of quantum information and its applications to computing and cryptography have been greatly illuminated by considering information-theoretic tasks that are provably possible or impossible within non-relativistic quantum mechanics. I describe here a general framework for defining tasks within (special) relativistic quantum theory and illustrate it with examples from relativistic quantum cryptography and relativistic distributed quantum computation. The framework gives a unified description of all tasks previously considered and also defines a large class of new questions about the properties of quantum information in relation to Minkowski causality. It offers a way of exploring interesting new fundamental tasks and applications, and also highlights the scope for a more systematic understanding of the fundamental information-theoretic properties of relativistic quantum theory.}
}
	
@article{CK06,
  title = {Variable-bias coin tossing},
  author = {Colbeck, Roger and Kent, Adrian},
  journal = {Phys. Rev. A},
  volume = {73},
  issue = {3},
  pages = {032320},
  numpages = {11},
  year = {2006},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.73.032320},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.73.032320}
}

@article{DK02,
  title = {An introduction to quantum coin tossing},
  author = {C. D\"{o}scher and M. Keyl},
  journal = {Fluctuation and Noise Letters},
  volume = {02},
  issue = {04},
  pages = {R125--R137},
  year = {2002},
  doi = {10.1142/S0219477502000944},
  url = {https://www.worldscientific.com/doi/abs/10.1142/S0219477502000944}
}


@article{C07.2,
title = "An entanglement-based protocol for strong coin tossing with bias 1/4",
journal = "Phys. Lett. A",
volume = "362",
number = "5",
pages = "390 - 392",
year = "2007",
issn = "0375-9601",
doi = "https://doi.org/10.1016/j.physleta.2006.10.062",
url = "http://www.sciencedirect.com/science/article/pii/S0375960106016823",
author = "Roger Colbeck",
abstract = "In the literature, strong coin tossing protocols based on bit commitment have been proposed. Here we examine a protocol that instead tries to achieve the task by sharing entanglement securely. The protocol uses only qubits, and has bias 14. This is equal to the best known bias for bit commitment based schemes."
}

@phdthesis{C09,
author={Colbeck, Roger},
title={Quantum And Relativistic Protocols For Secure Multi-Party Computation},
school={University of Cambridge},
year={2006},
Note ={Eprint arXiv:0911.3814},
url={http://arxiv.org/abs/0911.3814}
}

@phdthesis{Rennerthesis,
author={Renner, Renato},
title={Security of Quantum Key Distribution},
school={Swiss Federal Institute of Technology},
year={2005},
Note ={Eprint arXiv:quant-ph/0512258},
url={https://arxiv.org/abs/quant-ph/0512258}
}



@phdthesis{K15,
author={Kaniewski, Jędrzej},
title={Relativistic quantum cryptography},
school={Centre for Quantum Technologies, National University of Singapore},
year={2015},
Note ={Eprint arXiv:1512.00602},
url={http://arxiv.org/abs/1512.00602}
}

@article{M10.1,
  title = {Location-dependent communications using quantum entanglement},
  author = {Malaney, Robert A.},
  journal = {Phys. Rev. A},
  volume = {81},
  issue = {4},
  pages = {042319},
  numpages = {4},
  year = {2010},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.81.042319},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.81.042319}
}

@Unpublished{HM12,
author = "Patrick Hayden and Alex May",
year = "2012",
eprint = "1210.0913",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1210.0913;%%",
url = "http://arxiv.org/abs/1210.0913",
}

@article{AK15.3,
  title = {Quantum paradox of choice: More freedom makes summoning a quantum state harder},
  author = {Adlam, Emily and Kent, Adrian},
  journal = {Phys. Rev. A},
  volume = {93},
  issue = {6},
  pages = {062327},
  numpages = {7},
  year = {2016},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.93.062327},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.93.062327}
}



@Unpublished{R02NATURE,
author ={Terry Rudolp},
title = {The Laws of Physics and Cryptographic Security},
year = "2002",
note = "Preprint at \url{http://arxiv.org/abs/quant-ph/0202143}",
url = "http://arxiv.org/abs/quant-ph/0202143",
}

@Unpublished{M07,
author = "Carlos Mochon",
title= "Quantum weak coin flipping with arbitrarily small bias",
year = "2007",
eprint = "0711.4114",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:0711.4114;%%"
}
%url = "http://arxiv.org/abs/0711.4114",


@Unpublished{G09,
author = "Maor Ganz",
title= "Quantum leader election",
year = "2009",
eprint = "0910.4952",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:0910.4952;%%"
}

@INPROCEEDINGS{BD84,  author={A. Z. {Broder} and D. {Dolev}},  booktitle={25th Annual Symposium on Foundations of Computer Science, 1984.},   title={Flipping Coins In Many Pockets (Byzantine Agreement On Uniformly Random Values)},   year={1984},  volume={},  number={},  pages={157-170},  doi={10.1109/SFCS.1984.715912}}


@unpublished{PG15.2,
  title = {Practical protocols for spacetime constrained oblivious transfer},
  author = {D. Pital\'ua{-}Garc\'ia},
year= {2015},
  note ={In preparation}
}

@unpublished{quantumtagginginvention,
  title = {Method for quantum tagging with stored secret classical data},
  author = {D. Pital\'ua{-}Garc\'ia},
year= {June, 2018},
  note ={In preparation}
}

@article{W98,
  title = {Optimal cloning of pure states},
  author = {Werner, R. F.},
  journal = {Phys. Rev. A},
  volume = {58},
  issue = {3},
  pages = {1827--1832},
  numpages = {0},
  year = {1998},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.58.1827},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.58.1827}
}

	
@article{H07,
  author={Lucien Hardy},
  title={Towards quantum gravity: a framework for probabilistic theories with non-fixed causal structure},
  journal={J. Phys. A},
  volume={40},
  number={12},
  pages={3081},
  url={http://stacks.iop.org/1751-8121/40/i=12/a=S12},
  year={2007},
  abstract={General relativity is a deterministic theory with non-fixed causal structure. Quantum theory is a probabilistic theory with fixed causal structure. In this paper, we build a framework for probabilistic theories with non-fixed causal structure. This combines the radical elements of general relativity and quantum theory. We adopt an operational methodology for the purposes of theory construction (though without committing to operationalism as a fundamental philosophy). The key idea in the construction is physical compression . A physical theory relates quantities. Thus, if we specify a sufficiently large set of quantities (this is the compressed set), we can calculate all the others. We apply three levels of physical compression. First, we apply it locally to quantities (actually probabilities) that might be measured in a particular region of spacetime. Then we consider composite regions. We find that there is a second level of physical compression for a composite region over and above the first level physical compression for the component regions. Each application of first and second level physical compression is quantified by a matrix. We find that these matrices themselves are related by the physical theory and can therefore be subject to compression. This is the third level of physical compression. The third level of physical compression gives rise to a new mathematical object which we call the causaloid. From the causaloid for a particular physical theory we can calculate everything the physical theory can calculate. This approach allows us to set up a framework for calculating probabilistic correlations in data without imposing a fixed causal structure (such as a background time). We show how to put quantum theory in this framework (thus providing a new formulation of this theory). We indicate how general relativity might be put into this framework and how the framework might be used to construct a theory of quantum gravity.}
}
	
@article{PG15.1,
  title = {Spacetime-constrained oblivious transfer},
  author = {Pital\'ua{-}Garc\'{\i}a, Dami\'an},
  journal = {Phys. Rev. A},
  volume = {93},
  issue = {6},
  pages = {062346},
  numpages = {8},
  year = {2016},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.93.062346},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.93.062346}
}


@Unpublished{H16,
author = "L. Hardy",
title = "Operational General Relativity: Possibilistic, Probabilistic, and Quantum",
year = "2016",
eprint = "1608.06940",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1608.06940;%%",
}


@unpublished{PGK16,
author = {D. Pital\'ua{-}Garc\'ia and Iordanis Kerenidis},
  title = {Practical and unconditionally secure spacetime constrained oblivious transfer},
note={To be submitted},
}

@unpublished{PGK17,
author = {D. Pital\'ua{-}Garc\'ia and Iordanis Kerenidis},
  title = {Security analysis of a proposed experimental demonstration of a practical and unconditionally secure protocol for spacetime constrained oblivious transfer},
note={In preparation},
}

@unpublished{PG16,
author = {D. Pital\'ua{-}Garc\'ia},
  title = {Multi-input spacetime constrained oblivious transfer},
year ={2016},
note ="in preparation",
}


@unpublished{PGMP17,
author = {D. Pital\'ua{-}Garc\'ia and S. Massar and S. Pironio},
  title = {Device-independent spacetime{-}constrained oblivious transfer},
note={In preparation},
}

@unpublished{BDKPG18,
author = {M. Bozzio and E. Diamanti and A. Kent and D. Pital\'ua{-}Garc\'ia},
  title = {A new loophole in photonic implementations of quantum cryptography},
note={In preparation},
year={2018},
}

@unpublished{PG17.2,
author = {D. Pital\'ua{-}Garc\'ia},
  title = {Experimental proposal to implement unconditionally secure multi{-}party coin tossing
with a practical classical and relativistic protocol},
note={In preparation},
}

@article {WER18,
	author = {Wehner, Stephanie and Elkouss, David and Hanson, Ronald},
	title = {Quantum internet: A vision for the road ahead},
	volume = {362},
	number = {6412},
	elocation-id = {eaam9288},
	year = {2018},
	publisher = {American Association for the Advancement of Science},
	abstract = {As indispensable as the internet has become in our daily lives, it still has many shortcomings, not least of which is that communication can be intercepted and information stolen. If, however, the internet attained the capability of transmitting quantum information{\textemdash}qubits{\textemdash}many of these security concerns would be addressed. Wehner et al. review what it will take to achieve this so-called quantum internet and propose stages of development that each correspond to increasingly powerful applications. Although a full-blown quantum internet, with functional quantum computers as nodes connected through quantum communication channels, is still some ways away, the first long-range quantum networks are already being planned.Science, this issue p. eaam9288BACKGROUNDThe internet has had a revolutionary impact on our world. The vision of a quantum internet is to provide fundamentally new internet technology by enabling quantum communication between any two points on Earth. Such a quantum internet will{\textemdash}in synergy with the {\textquotedblleft}classical{\textquotedblright} internet that we have today{\textemdash}connect quantum information processors in order to achieve unparalleled capabilities that are provably impossible by using only classical information.As with any radically new technology, it is hard to predict all uses of the future quantum internet. However, several major applications have already been identified, including secure communication, clock synchronization, extending the baseline of telescopes, secure identification, achieving efficient agreement on distributed data, exponential savings in communication, quantum sensor networks, as well as secure access to remote quantum computers in the cloud.Central to all these applications is the ability of a quantum internet to transmit quantum bits (qubits) that are fundamentally different than classical bits. Whereas classical bits can take only two values, 0 or 1, qubits can be in a superposition of being 0 and 1 at the same time. Moreover, qubits can be entangled with each other, leading to correlations over large distances that are much stronger than is possible with classical information. Qubits also cannot be copied, and any attempt to do so can be detected. This feature makes qubits well suited for security applications but at the same time makes the transmission of qubits require radically new concepts and technology. Rapid experimental progress in recent years has brought first rudimentary quantum networks within reach, highlighting the timeliness and need for a unified framework for quantum internet researchers.ADVANCESWe define different stages of development toward a full-blown quantum internet. We expect that this classification will be instrumental in guiding and assessing experimental progress as well as stimulating the development of new applications by providing a common language and reference frame for the different scientific and engineering disciplines involved.More advanced stages are distinguished by a larger amount of functionality, thus supporting ever more sophisticated application protocols. For each stage, we describe some of the application protocols that are already known and that can be realized with the functionality provided in that stage. It is conceivable that a simpler protocol, or better theoretical analysis, may be found in the future that solves the same task but is less demanding in terms of functionality. In parallel to the daunting experimental challenges in making quantum internet a reality, there is thus an opportunity for quantum software developers to design protocols that can realize a task in a stage that can be implemented more easily. We identify relevant parameters for each stage to establish a common language between hardware and software developers. Last, we review technological progress in experimental physics, engineering, and computer science that is required to attain such stages.OUTLOOKBuilding and scaling quantum networks is a formidable endeavor, requiring sustained and concerted efforts in physics, computer science, and engineering to succeed. The proposed stages of development will facilitate interdisciplinary communication by summarizing what we may actually want to achieve and providing guidelines both to protocol design and software development as well as hardware implementations through experimental physics and engineering. Although it is hard to predict what the exact components of a future quantum internet will be, it is likely that we will see the birth of the first multinode quantum networks in the next few years. This development brings the exciting opportunity to test all the ideas and functionalities that so far only exist on paper and may indeed be the dawn of a future large-scale quantum internet.Stages in the development of a quantum internet.Each stage is characterized by an increase in functionality at the expense of greater technological difficulty. This Review provides a clear definition of each stage, including benchmarks and examples of known applications, and provides an overview of the technological progress required to attain these stages.The internet{\textemdash}a vast network that enables simultaneous long-range classical communication{\textemdash}has had a revolutionary impact on our world. The vision of a quantum internet is to fundamentally enhance internet technology by enabling quantum communication between any two points on Earth. Such a quantum internet may operate in parallel to the internet that we have today and connect quantum processors in order to achieve capabilities that are provably impossible by using only classical means. Here, we propose stages of development toward a full-blown quantum internet and highlight experimental and theoretical progress needed to attain them.},
	issn = {0036-8075},
		URL = {https://science.sciencemag.org/content/362/6412/eaam9288},
	journal = {Science}
}

@article{BBBG09,
  title = {Fair loss-tolerant quantum coin flipping},
  author = {Berl\'{\i}n, Guido and Brassard, Gilles and Bussi\`eres, F\'elix and Godbout, Nicolas},
  journal = {Phys. Rev. A},
  volume = {80},
  issue = {6},
  pages = {062321},
  numpages = {11},
  year = {2009},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.80.062321},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.80.062321}
}


@article{LKBHTWZ15,
  title = {Practical Relativistic Bit Commitment},
  author = {Lunghi, T. and Kaniewski, J. and Bussi\`{e}res, F. and Houlmann, R. and Tomamichel, M. and Wehner, S. and Zbinden, H.},
  journal = {Phys. Rev. Lett.},
  volume = {115},
  issue = {3},
  pages = {030502},
  numpages = {5},
  year = {2015},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.115.030502},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.115.030502}
}

@article{K99.2,
  title = {Coin Tossing is Strictly Weaker than Bit Commitment},
  author = {Kent, Adrian},
  journal = {Phys. Rev. Lett.},
  volume = {83},
  issue = {25},
  pages = {5382--5384},
  numpages = {0},
  year = {1999},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.83.5382},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.83.5382}
}



@article{EGL85,
 author = {Even, Shimon and Goldreich, Oded and Lempel, Abraham},
 title = {A Randomized Protocol for Signing Contracts},
 journal = {Commun. ACM},
 issue_date = {June 1985},
 volume = {28},
 number = {6},
 month = jun,
 year = {1985},
 issn = {0001-0782},
 pages = {637--647},
 numpages = {11},
 url = {http://doi.acm.org/10.1145/3812.3818},
 doi = {10.1145/3812.3818},
 acmid = {3818},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@article{LC98,
title = "Why quantum bit commitment and ideal quantum coin tossing are impossible ",
journal = "Physica D: Nonlinear Phenomena ",
volume = "120",
number = "1–2",
pages = "177 - 187",
year = "1998",
note = "Proceedings of the Fourth Workshop on Physics and Consumption ",
issn = "0167-2789",
url = "http://www.sciencedirect.com/science/article/pii/S0167278998000530",
author = "Hoi-Kwong Lo and H.F. Chau",
abstract = "There had been well-known claims of unconditionally secure quantum protocols for bit commitment. However, we, and independently Mayers, showed that all proposed quantum bit commitment schemes are, in principle, insecure because the sender, Alice, can almost always cheat successfully by using an Einstein-Podolsky-Rosen (EPR) type of attack and delaying her measurements. One might wonder if secure quantum bit commitment protocols exist at all. We answer this question by showing that the same type of attack by Alice will, in principle, break any bit commitment scheme. The cheating strategy generally requires a quantum computer. We emphasize the generality of this “no-go theorem”: Unconditionally secure bit commitment schemes based on quantum mechanics-fully quantum, classical or quantum but with measurements-are all ruled out by this result. Since bit commitment is a useful primitive for building up more sophisticated protocols such as zero-knowledge proofs, our results cast very serious doubt on the security of quantum cryptography in the so-called “post-cold-war” applications. We also show that ideal quantum coin tossing is impossible because of the \{EPR\} attack. This no-go theorem for ideal quantum coin tossing may help to shed some lights on the possibility of non-ideal protocols. "
}

@INPROCEEDINGS{ABDR04,
   author       = "A. Ambainis and H. Buhrman and Y. Dodis and H. Rohrig",
title = "Multiparty Quantum Coin Flipping",
   booktitle      = "Proceedings of the 19th IEEE Annual Conference on Computational Complexity",
   pages       = "250--259", 
 publisher       = "IEEE Computer Society",
address= "",
   year         = "2004",
note = "quant-ph/0304112"
}
%url = "http://arxiv.org/abs/quant-ph/0304112"

@article{NS03,
  title = {Bit-commitment-based quantum coin flipping},
  author = {Nayak, Ashwin and Shor, Peter},
  journal = {Phys. Rev. A},
  volume = {67},
  issue = {1},
  pages = {012304},
  numpages = {11},
  year = {2003},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.67.012304},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.67.012304}
}
@article{A04,
title = "A new protocol and lower bounds for quantum coin flipping",
journal = "J. Comput. Syst. Sci.",
volume = "68",
number = "2",
pages = "398--416",
year = "2004",
note = "Special Issue on STOC 2001",
issn = "0022-0000",
doi = "https://doi.org/10.1016/j.jcss.2003.07.010",
url = "http://www.sciencedirect.com/science/article/pii/S0022000003001417",
author = "Andris Ambainis",
abstract = "We present a new protocol and two lower bounds for quantum coin flipping. In our protocol, no dishonest party can achieve one outcome with probability more than 0.75. Then we show that out protocol is optimal among 3-round protocols of a certain form. For arbitrary quantum protocols, we show that if a protocol achieves a bias of at most ε, it must use at least Ω(loglog1ε) rounds of communication. This implies that the parallel repetition fails for quantum coin flipping. (The bias of a protocol cannot be arbitrarily decreased by running several copies of it in parallel.)"
}


@article{LCQ12,
  title = {Measurement-Device-Independent Quantum Key Distribution},
  author = {Lo, Hoi-Kwong and Curty, Marcos and Qi, Bing},
  journal = {Phys. Rev. Lett.},
  volume = {108},
  issue = {13},
  pages = {130503},
  numpages = {5},
  year = {2012},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.108.130503},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.108.130503}
}


@INPROCEEDINGS{Y95,
   author       = "ACC Yao",
title = "Security of quantum protocols against coherent measurements",
   booktitle      = "Proceedings of the twenty-seventh annual ACM symposium on Theory of computing",
   pages       = "67--75", 
 publisher       = "ACM",
address= "New York, NY, USA",
   year         = "1995",
url = "http://dl.acm.org/citation.cfm?id=225085"
}



@INPROCEEDINGS{Y82, 
author={A. C. Yao},
title={Protocols for secure computations},
booktitle={23rd Annual Symposium on Foundations of Computer Science, 1982. SFCS '08}, 
pages={160-164},
publisher={IEEE},
address={Chicago, IL, USA},
year={1982}, 
 }
%keywords={Algorithm design and analysis;Cryptography;Databases;Privacy;Protocols;Security;Stochastic processes;Telephony;Voting}, 
%doi={10.1109/SFCS.1982.38}, 
%ISSN={0272-5428},
%month={Nov},

@article{RJADHAKLMMMMMSSST12,
  author={David Rideout and Thomas Jennewein and Giovanni Amelino-Camelia and Tommaso F Demarie and Brendon L Higgins and Achim
Kempf and Adrian Kent and Raymond Laflamme and Xian Ma and Robert B Mann and Eduardo Martín-Martínez and Nicolas C
Menicucci and John Moffat and Christoph Simon and Rafael Sorkin and Lee Smolin and Daniel R Terno},
  title={Fundamental quantum optics experiments conceivable with satellites—reaching relativistic distances and velocities},
  journal={Classical and Quantum Gravity},
  volume={29},
  number={22},
  pages={224011},
  url={http://stacks.iop.org/0264-9381/29/i=22/a=224011},
  year={2012},
  abstract={Physical theories are developed to describe phenomena in particular regimes, and generally are valid only within a limited range of scales. For example, general relativity provides an effective description of the Universe at large length scales, and has been tested from the cosmic scale down to distances as small as 10 m (Dimopoulos 2007 Phys. Rev. Lett. 98 111102; 2008 Phys. Rev. D 78 042003). In contrast, quantum theory provides an effective description of physics at small length scales. Direct tests of quantum theory have been performed at the smallest probeable scales at the Large Hadron Collider, ∼10 −20 m, up to that of hundreds of kilometres (Ursin et al 2007 Nature Phys. 3 481–6). Yet, such tests fall short of the scales required to investigate potentially significant physics that arises at the intersection of quantum and relativistic regimes. We propose to push direct tests of quantum theory to larger and larger length scales, approaching that of the radius of curvature of spacetime, where we begin to probe the interaction between gravity and quantum phenomena. In particular, we review a wide variety of potential tests of fundamental physics that are conceivable with artificial satellites in Earth orbit and elsewhere in the solar system, and attempt to sketch the magnitudes of potentially observable effects. The tests have the potential to determine the applicability of quantum theory at larger length scales, eliminate various alternative physical theories, and place bounds on phenomenological models motivated by ideas about spacetime microstructure from quantum gravity. From a more pragmatic perspective, as quantum communication technologies such as quantum key distribution advance into space towards large distances, some of the fundamental physical effects discussed here may need to be taken into account to make such schemes viable.}
}

@article{S10,
  title = {Simple protocols for oblivious transfer and secure identification in the noisy-quantum-storage model},
  author = {Schaffner, Christian},
  journal = {Phys. Rev. A},
  volume = {82},
  issue = {3},
  pages = {032308},
  numpages = {12},
  year = {2010},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.82.032308},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.82.032308}
}

@article{YPF14,
  title = {Limitations on information-theoretically-secure quantum homomorphic encryption},
  author = {Yu, Li and P\'erez-Delgado, Carlos A. and Fitzsimons, Joseph F.},
  journal = {Phys. Rev. A},
  volume = {90},
  issue = {5},
  pages = {050303},
  numpages = {5},
  year = {2014},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.90.050303},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.90.050303}
}

@INPROCEEDINGS{BFK09, 
author={A. Broadbent and J. Fitzsimons and E. Kashefi}, 
booktitle={Foundations of Computer Science, 2009. FOCS '09. 50th Annual IEEE Symposium on}, 
title={Universal Blind Quantum Computation}, 
year={2009}, 
pages={517-526}, 
keywords={cryptographic protocols;quantum cryptography;theorem proving;authentication protocol;blind quantum computation;cheating server detection;measurement-based quantum computing;noncommunicating entangled servers;purely classical client setting;single-qubit measurement;two-prover interactive proof;two-way classical communication;Authentication;Computer aided instruction;Computer science;Fault detection;Fault tolerance;Informatics;Privacy;Protocols;Quantum computing;Quantum entanglement;measurement-based quantum computing;quantum cryptography;quantum prover interactive proofs}, 
doi={10.1109/FOCS.2009.36}, 
ISSN={0272-5428}, 
month={Oct},}


@Unpublished{MF16,
author = "T. Morimae and J. Fitzsimons",
title= "Post hoc verification with a single prover",
year = "2016",
eprint = "1603.06046",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1603.06046;%%",
}


@article{MF13,
  title = {Blind quantum computation protocol in which Alice only makes measurements},
  author = {Morimae, Tomoyuki and Fujii, Keisuke},
  journal = {Phys. Rev. A},
  volume = {87},
  issue = {5},
  pages = {050301},
  numpages = {5},
  year = {2013},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.87.050301},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.87.050301}
}




@article{BMU14,
  author={Howard Barnum and Markus P M\"{u}ller and Cozmin Ududec},
  title={Higher-order interference and single-system postulates characterizing quantum theory},
  journal={New J. Phys.},
  volume={16},
  number={12},
  pages={123029},
  url={http://stacks.iop.org/1367-2630/16/i=12/a=123029},
  year={2014},
  abstract={We present a new characterization of quantum theory in terms of simple physical principles that is different from previous ones in two important respects: first, it only refers to properties of single systems without any assumptions on the composition of many systems; and second, it is closer to experiment by having absence of higher-order interference as a postulate, which is currently the subject of experimental investigation. We give three postulates—no higher-order interference, classical decomposability of states, and strong symmetry—and prove that the only non-classical operational probabilistic theories satisfying them are real, complex, and quaternionic quantum theory, together with three-level octonionic quantum theory and ball state spaces of arbitrary dimension. Then we show that adding observability of energy as a fourth postulate yields complex quantum theory as the unique solution, relating the emergence of the complex numbers to the possibility of Hamiltonian dynamics. We also show that there may be interesting non-quantum theories satisfying only the first two of our postulates, which would allow for higher-order interference in experiments while still respecting the contextuality analogue of the local orthogonality principle.}
}


@article{MPP15,
  author={Serge Massar and Stefano Pironio and Dami\'an Pital\'ua{-}Garc\'ia},
  title={Hyperdense coding and superadditivity of classical capacities in hypersphere theories},
  journal={New Journal of Physics},
  volume={17},
  number={11},
  pages={113002},
  url={http://stacks.iop.org/1367-2630/17/i=11/a=113002},
  year={2015}
}
  	
@article{TFKW13,
  author={Marco Tomamichel and Serge Fehr and Jędrzej Kaniewski and Stephanie Wehner},
  title={A monogamy-of-entanglement game with applications to device-independent quantum cryptography},
  journal={New J. Phys.},
  volume={15},
  number={10},
  pages={103002},
  url={http://stacks.iop.org/1367-2630/15/i=10/a=103002},
  year={2013},
  abstract={We consider a game in which two separate laboratories collaborate to prepare a quantum system and are then asked to guess the outcome of a measurement performed by a third party in a random basis on that system. Intuitively, by the uncertainty principle and the monogamy of entanglement, the probability that both players simultaneously succeed in guessing the outcome correctly is bounded. We are interested in the question of how the success probability scales when many such games are performed in parallel. We show that any strategy that maximizes the probability to win every game individually is also optimal for the parallel repetition of the game. Our result implies that the optimal guessing probability can be achieved without the use of entanglement. We explore several applications of this result. Firstly, we show that it implies security for standard BB84 quantum key distribution when the receiving party uses fully untrusted measurement devices , i.e. we show that BB84 is one-sided device independent. Secondly, we show how our result can be used to prove security of a one-round position-verification scheme. Finally, we generalize a well-known uncertainty relation for the guessing probability to quantum side information.}
}


@Unpublished{JMRW15,
author = "Nathaniel Johnston and Rajat Mittal and Vincent Russo and John Watrous",
title= "Extended nonlocal games and monogamy{-}of{-}entanglement games",
year = "2015",
eprint = "1510.02083",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1510.02083;%%",
url = "http://arxiv.org/abs/1510.02083",
}

@article{NPA07,
  title = {Bounding the Set of Quantum Correlations},
  author = {Navascu\'es, Miguel and Pironio, Stefano and Ac\'{\i}n, Antonio},
  journal = {Phys. Rev. Lett.},
  volume = {98},
  issue = {1},
  pages = {010401},
  numpages = {4},
  year = {2007},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.98.010401},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.98.010401}
}



@article{NPA08,
  author={Navascu\'es, Miguel and Pironio, Stefano and Ac\'{\i}n, Antonio},
  title={A convergent hierarchy of semidefinite programs characterizing the set of quantum correlations},
  journal={New Journal of Physics},
  volume={10},
  number={7},
  pages={073013},
  url={http://stacks.iop.org/1367-2630/10/i=7/a=073013},
  year={2008},
  abstract={We are interested in the problem of characterizing the correlations that arise when performing local measurements on separate quantum systems. In a previous work (Navascués et al 2007 Phys. Rev. Lett. 98 010401), we introduced an infinite hierarchy of conditions necessarily satisfied by any set of quantum correlations. Each of these conditions could be tested using semidefinite programming. We present here new results concerning this hierarchy. We prove in particular that it is complete, in the sense that any set of correlations satisfying every condition in the hierarchy has a quantum representation in terms of commuting measurements. Although our tests are conceived to rule out non-quantum correlations, and can in principle certify that a set of correlations is quantum only in the asymptotic limit where all tests are satisfied, we show that in some cases it is possible to conclude that a given set of correlations is quantum after performing only a finite number of tests. We provide a criterion to detect when such a situation arises, and we explain how to reconstruct the quantum states and measurement operators reproducing the given correlations. Finally, we present several applications of our approach. We use it in particular to bound the quantum violation of various Bell inequalities.}
}

@misc{BT08,
    author = {Anne Broadbent  and   Alain Tapp},
    title = {Information-Theoretically Secure Voting Without an Honest Majority},
    howpublished = {Cryptology ePrint Archive, Report 2008/266},
    year = {2008},
    note = {\url{http://eprint.iacr.org/}},
}


@article{T04,
  author={B Terhal},
  title={ Is entanglement monogamous?},
  journal={IBM J. Res. Dev.},
  volume={48},
  number={1},
  pages={71-78},
doi = {10.1147/rd.481.0071},
  url={http://ieeexplore.ieee.org/xpl/articleDetails.jsp?arnumber=5388928},
  year={2004},
}

@article{H21,
	doi = {10.1088/1367-2630/abd97d},
	year = 2021,
	month = {mar},
	publisher = {{IOP} Publishing},
	volume = {23},
	number = {3},
	pages = {033020},
	author = {Simon A Haine},
	title = {Searching for signatures of quantum gravity in quantum gases},
	journal = {New J. Phys.},
	abstract = {We explore the possibility of testing the quantum nature of the gravitational field with an ensemble of ultra-cold atoms. The use of many microscopic particles may circumvent some of the experimental obstacles encountered in recent proposals involving a pair of particles with mesoscopic mass. We employ multi-parameter estimation techniques, including the quantum and classical Fisher information to provide a criteria for the observability of the quantum effects, and compare to other recently proposed schemes. Crucially, we find that by preparing the appropriate initial state, interactions mediated via a quantum-valued gravitational field provide a signature that is distinct from classical gravitational interactions. We find that a definitive demonstration of the quantum gravitational interaction is not possible with current experimental capabilities, due to uncertainty in the residual electromagnetic interactions between the atoms. However, it may be possible with significant improvements to current experimental techniques.}
}



@article{S89,
  author={M. Saks},
  title={ A Robust Noncryptographic Protocol for Collective Coin Flipping},
  journal={SIAM J. Discrete Math.},
  volume={2},
  number={2},
  pages={240--244},
doi = {10.1137/0402020},
  url={https://epubs.siam.org/doi/abs/10.1137/0402020},
  year={1989},
}


@article{SCK14,
  title = {Strong connections between quantum encodings, nonlocality, and quantum cryptography},
  author = {Sikora, Jamie and Chailloux, Andr\'e and Kerenidis, Iordanis},
  journal = {Phys. Rev. A},
  volume = {89},
  issue = {2},
  pages = {022334},
  numpages = {8},
  year = {2014},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.89.022334},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.89.022334}
}


@article{CKS13,
  title = {Lower Bounds for Quantum Oblivious Transfer},
  author = {André Chailloux and Iordanis Kerenidis and Jamie Sikora},
  journal = {Quantum Information and Computation},
  volume = {13},
  issue = {1,2},
  pages = {158-177},
  year = {2013},
  note = {arXiv:1007.1875},
   url={https://arxiv.org/abs/1007.1875},
}

@article{ColbeckKent11,
  author={Roger Colbeck and Adrian Kent},
  title={Private randomness expansion with untrusted devices},
  journal={Journal of Physics A: Mathematical and Theoretical},
  volume={44},
  number={9},
  pages={095305},
    year={2011}
  }
  %url={http://stacks.iop.org/1751-8121/44/i=9/a=095305},

@article{PAMBMMOHLMM10,
  author={S. Pironio and A. Ac\'{\i}n and S. Massar and A. Boyer de la Giroday and D. N. Matsukevich and P. Maunz and S. Olmschenk and D. Hayes and L. Luo and T. A. Manning and C. Monroe},
  title={Random numbers certified by Bell’s theorem},
  journal={Nature},
  volume={464},
  pages={1021-1024},
doi={10.1038/nature09008},
  year={2010},
}

@article{SpaceQUEST,
  author={Josep Maria Perdigues Armengol and Bernhard Furcha and Clovis Jacinto de Matos and
Olivier Minster and Luigi Cacciapuoti and Martin Pfennigbauer and Markus Aspelmeyer and Thomas Jennewein and Rupert Ursin and Tobias Schmitt-Manderbach and Guy Baister and John Rarity and Walter Leeb and Cesare Barbieri and Harald Weinfurter and Anton Zeilinger},
  title={Quantum communications at ESA: towards a space experiment on the ISS},
  journal={Acta Astronaut.},
  volume={63},
  pages={165-178},
doi={10.1016/j.actaastro.2007.12.039},
  year={2007},
}

@article{VMHBBZ16,
  title = {24{-}Hour Relativistic Bit Commitment},
  author = {Verbanis, Ephanielle and Martin, Anthony and Houlmann, Rapha\"el and Boso, Gianluca and Bussi\`eres, F\'elix and Zbinden, Hugo},
  journal = {Phys. Rev. Lett.},
  volume = {117},
  issue = {14},
  pages = {140506},
  numpages = {5},
  year = {2016},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.117.140506},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.117.140506}
}

@article{JADW00,
  title = {Quantum Clock Synchronization Based on Shared Prior Entanglement},
  author = {Jozsa, Richard and Abrams, Daniel S. and Dowling, Jonathan P. and Williams, Colin P.},
  journal = {Phys. Rev. Lett.},
  volume = {85},
  issue = {9},
  pages = {2010--2013},
  numpages = {0},
  year = {2000},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.85.2010},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.85.2010}
}

@article{CMP07,
  title = {Secret Quantum Communication of a Reference Frame},
  author = {Chiribella, Giulio and Maccone, Lorenzo and Perinotti, Paolo},
  journal = {Phys. Rev. Lett.},
  volume = {98},
  issue = {12},
  pages = {120501},
  numpages = {4},
  year = {2007},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.98.120501},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.98.120501}
}

@article{FFQF08,
  title = {Consistency of shared reference frames should be reexamined},
  author = {Gao, Fei and Guo, Fen-Zhuo and Wen, Qiao-Yan and Zhu, Fu-Chen},
  journal = {Phys. Rev. A},
  volume = {77},
  issue = {1},
  pages = {014302},
  numpages = {3},
  year = {2008},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.77.014302},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.77.014302}
}


@article{SWFUTSPSKRZW07,
  title = {Experimental Demonstration of Free-Space Decoy-State Quantum Key Distribution over 144 km},
  author = {Schmitt-Manderbach, Tobias and Weier, Henning and F\"urst, Martin and Ursin, Rupert and Tiefenbacher, Felix and Scheidl, Thomas and Perdigues, Josep and Sodnik, Zoran and Kurtsiefer, Christian and Rarity, John G. and Zeilinger, Anton and Weinfurter, Harald},
  journal = {Phys. Rev. Lett.},
  volume = {98},
  issue = {1},
  pages = {010504},
  numpages = {4},
  year = {2007},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.98.010504},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.98.010504}
}


  	
@article{SWVTGZGTT09,
  author={D Stucki and N Walenta and F Vannel and R T Thew and N Gisin and H Zbinden and S Gray and C R Towery and S Ten},
  title={High rate, long-distance quantum key distribution over 250 km of ultra low loss fibres},
  journal={New Journal of Physics},
  volume={11},
  number={7},
  pages={075003},
  url={http://stacks.iop.org/1367-2630/11/i=7/a=075003},
  year={2009},
  abstract={We present a fully automated quantum key distribution prototype running at 625 MHz clock rate. Taking advantage of ultra low loss (ULL) fibres and low-noise superconducting detectors, we can distribute 6000 secret bits s −1 over 100 km and 15 bits s −1 over 250 km.}
}
	
@article{KLHGLNSTZ15,
  author={B Korzhand	C Lim and	R Houlmann and	Nicolas Gisin and	Ming Jun Li and	Daniel Nolan and	Bruno Sanguinetti and	Rob Thew	and Hugo Zbinden},
  title={Provably secure and practical quantum key distribution over 307 km of optical fibre},
  journal={Nat. Photon.},
  volume={9},
  pages={163--168},
  doi={10.1038/nphoton.2014.327},
  year={2015},
}


@Unpublished{CL16,
author = "Andre Chailloux ad Anthony Leverrier",
title= "Relativistic (or 2{-}prover 1{-}round) zero{-}knowledge protocol for NP secure against quantum adversaries",
year = "2016",
eprint = "1612.07627",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1612.07627;%%",
url = "http://arxiv.org/abs/1612.07627",
}

@article{CL15,
  title = {Practical position-based quantum cryptography},
  author = {Chakraborty, Kaushik and Leverrier, Anthony},
  journal = {Phys. Rev. A},
  volume = {92},
  issue = {5},
  pages = {052304},
  numpages = {10},
  year = {2015},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.92.052304},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.92.052304}
}

@misc{IBM16,
    title = {{IBM} Makes Quantum Computing Available on {IBM} Cloud to Accelerate Innovation},
    howpublished = {IBM Press release, May 2016},
    url = {https://www-03.ibm.com/press/us/en/pressrelease/49661.wss},
}


@Unpublished{chernoffboundnotes,
author = "Michel Goemans",
title= "Chernoff bounds, and some applications",
year = "2015",
Note= "{MIT L}ecture notes",
url = "http://math.mit.edu/~goemans/18310S15/chernoff-notes.pdf",
}


@article{BOVZKD18,
  title = {Experimental investigation of practical unforgeable quantum money},
  author = {M. Bozzio and  A. Orieux and L. T. Vidarte and I. Zaquine and I. Kerenidis and E. Diamanti},
journal = {npj Quantum Inf.},
volume = {4},
pages = {5},
year = {2018},
doi = {10.1038/s41534-018-0058-2},
}

@article{BML08,
  title = {Squashing Models for Optical Measurements in Quantum Communication},
  author = {Beaudry, Normand J. and Moroder, Tobias and L\"utkenhaus, Norbert},
  journal = {Phys. Rev. Lett.},
  volume = {101},
  issue = {9},
  pages = {093601},
  numpages = {4},
  year = {2008},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.101.093601},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.101.093601}
}


@article{JBCL19,
  title = {Experimentally attacking quantum money schemes based on quantum retrieval games},
  author = {K. Jir\'{a}kov\'{a} and K. Bartkiewicz and A. \v{C}ernoch and K. Lemr},
journal = {Sci. Rep.},
volume = {9},
pages = {16318},
year = {2019},
doi = {10.1038/s41598-019-51953-9},
url = {https://doi.org/10.1038/s41598-019-51953-9},
}

@article{BCGLMN17,
  title = {Experimental quantum forgery of quantum optical money},
  author = {K. Bartkiewicz and A. \v{C}ernoch and G. Chimczak and K. Lemr and A. Miranowicz and F. Nori},
journal = {npj Quantum Inf.},
volume = {3},
pages = {7},
year = {2017},
doi = {10.1038/s41534-017-0010-x},
url = {https://doi.org/10.1038/s41534-017-0010-x}
}

@article{GAAZLYWZP18,
  title = {Experimental preparation and verification of quantum money},
  author = {Guan, Jian-Yu and Arrazola, Juan Miguel and Amiri, Ryan and Zhang, Weijun and Li, Hao and You, Lixing and Wang, Zhen and Zhang, Qiang and Pan, Jian-Wei},
  journal = {Phys. Rev. A},
  volume = {97},
  issue = {3},
  pages = {032338},
  numpages = {6},
  year = {2018},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.97.032338},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.97.032338}
}


@inproceedings{GK15,
  title={New constructions for quantum money},
  author={Georgiou, Marios and Kerenidis, Iordanis},
  booktitle={LIPIcs-Leibniz International Proceedings in Informatics},
  volume={44},
  year={2015},
  organization={Schloss Dagstuhl-Leibniz-Zentrum fuer Informatik}
}

@article{APKA16,
  title = {Secure quantum signatures using insecure quantum channels},
  author = {Amiri, Ryan and Wallden, Petros and Kent, Adrian and Andersson, Erika},
  journal = {Phys. Rev. A},
  volume = {93},
  issue = {3},
  pages = {032325},
  numpages = {9},
  year = {2016},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.93.032325},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.93.032325}
}
@article{AWKA16,
  title = {Secure quantum signatures using insecure quantum channels},
  author = {Amiri, Ryan and Wallden, Petros and Kent, Adrian and Andersson, Erika},
  journal = {Phys. Rev. A},
  volume = {93},
  issue = {3},
  pages = {032325},
  numpages = {9},
  year = {2016},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.93.032325},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.93.032325}
}

@article{WDKA15,
  title = {Quantum digital signatures with quantum-key-distribution components},
  author = {Wallden, Petros and Dunjko, Vedran and Kent, Adrian and Andersson, Erika},
  journal = {Phys. Rev. A},
  volume = {91},
  issue = {4},
  pages = {042304},
  numpages = {10},
  year = {2015},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.91.042304},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.91.042304}
}


@Article{AA15,
AUTHOR = {Amiri, Ryan and Andersson, Erika},
TITLE = {Unconditionally Secure Quantum Signatures},
JOURNAL = {Entropy},
VOLUME = {17},
YEAR = {2015},
NUMBER = {8},
PAGES = {5635--5659},
URL = {http://www.mdpi.com/1099-4300/17/8/5635},
ISSN = {1099-4300},
ABSTRACT = {Signature schemes, proposed in 1976 by Diffie and Hellman, have become ubiquitous across modern communications. They allow for the exchange of messages from one sender to multiple recipients, with the guarantees that messages cannot be forged or tampered with and that messages also can be forwarded from one recipient to another without compromising their validity. Signatures are different from, but no less important than encryption, which ensures the privacy of a message. Commonly used signature protocols—signatures based on the Rivest–Adleman–Shamir (RSA) algorithm, the digital signature algorithm (DSA), and the elliptic curve digital signature algorithm (ECDSA)—are only computationally secure, similar to public key encryption methods. In fact, since these rely on the difficulty of finding discrete logarithms or factoring large primes, it is known that they will become completely insecure with the emergence of quantum computers. We may therefore see a shift towards signature protocols that will remain secure even in a post-quantum world. Ideally, such schemes would provide unconditional or information-theoretic security. In this paper, we aim to provide an accessible and comprehensive review of existing unconditionally securesecure signature schemes for signing classical messages, with a focus on unconditionally secure quantum signature schemes.},
DOI = {10.3390/e17085635}
}


@article{WC81,
title = "New hash functions and their use in authentication and set equality",
journal = "Journal of Computer and System Sciences",
volume = "22",
number = "3",
pages = "265 - 279",
year = "1981",
note = "",
issn = "0022-0000",
doi = "http://dx.doi.org/10.1016/0022-0000(81)90033-7",
url = "http://www.sciencedirect.com/science/article/pii/0022000081900337",
author = "Mark N. Wegman and J.Lawrence Carter",

}

@unpublished{K13.2,
  title = {Quantum nonlocal correlations are not dominated},
  author = {A. Kent},
year="2013",
eprint = "1308.5009",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1308.5009;%%",
}


@article{AWA15,
author = "J. M. Arrazola and P. Wallden and E. Andersson",
title = "Multiparty Quantum Signature Schemes",
journal = "Quantum Inf. Comput.",
volume = "6",
pages = "0435",
year = "2016",
url = "https://arxiv.org/abs/1505.07509",
}

@article{TR11,
  title = {Uncertainty Relation for Smooth Entropies},
  author = {Tomamichel, Marco and Renner, Renato},
  journal = {Phys. Rev. Lett.},
  volume = {106},
  issue = {11},
  pages = {110506},
  numpages = {4},
  year = {2011},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.106.110506},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.106.110506}
}


@Book{Lintbook,
 author    = "J. H. van Lint",
 title     = "Introduction to coding Theory",
 publisher = "Springer",
address= "Berlin",
 year      =  1999,
}

@ARTICLE{TCR10, 
author={M. Tomamichel and R. Colbeck and R. Renner}, 
journal={IEEE Transactions on Information Theory}, 
title={Duality Between Smooth Min- and Max-Entropies}, 
year={2010}, 
volume={56}, 
number={9}, 
pages={4674-4681}, 
keywords={entropy;quantum theory;cryptographic security proof;duality relation;entropy measure;quantum information theory;smooth max-entropy;smooth min-entropy;von Neumann entropy;Character generation;Cryptography;Data mining;Data processing;Data security;Entropy;Error correction;Hilbert space;Information theory;Optimization;Physics;Quantum mechanics;Smoothing methods;Conditional entropies;quantum information;smooth entropies}, 
doi={10.1109/TIT.2010.2054130}, 
ISSN={0018-9448}, 
month={Sept},}

@ARTICLE{KRS09, 
author={R. Konig and R. Renner and C. Schaffner}, 
journal={IEEE Transactions on Information Theory}, 
title={The Operational Meaning of Min- and Max-Entropy}, 
year={2009}, 
volume={55}, 
number={9}, 
pages={4337-4347}, 
keywords={information theory;maximum entropy methods;minimum entropy methods;information theory;max-entropy;min-entropy;Channel capacity;Communication channels;Entropy;Information security;Information theory;Merging;Quantum entanglement;Quantum mechanics;Random variables;Veins;Entropy measures;max-entropy;min-entropy;operational interpretations;quantum hypothesis testing;quantum information theory;single-shot information theory;singlet fraction}, 
doi={10.1109/TIT.2009.2025545}, 
ISSN={0018-9448}, 
month={Sept},}


@ARTICLE{TLGR12,
   author       = "M. Tomamichel and C. C. W. Lim and  N. Gisin and R. Renner",
 title = "Tight finite-key analysis for quantum cryptography",
   journal      = "Nat. Commun.",
   volume       = "3",
   pages        = "634",
   year         = "2012",
doi="10.1038/ncomms1631",
url = "https://www.ncbi.nlm.nih.gov/pmc/articles/PMC3274703/"
}

@Article{DBWR14,
author="Dupuis, Fr{\'e}d{\'e}ric
and Berta, Mario
and Wullschleger, J{\"u}rg
and Renner, Renato",
title="One-Shot Decoupling",
journal="Communications in Mathematical Physics",
year="2014",
month="May",
day="01",
volume="328",
number="1",
pages="251--284",
abstract="If a quantum system A, which is initially correlated to another system, E, undergoes an evolution separated from E, then the correlation to E generally decreases. Here, we study the conditions under which the correlation disappears (almost) completely, resulting in a decoupling of A from E. We give a criterion for decoupling in terms of two smooth entropies, one quantifying the amount of initial correlation between A and E, and the other characterizing the mapping that describes the evolution of A. The criterion applies to arbitrary such mappings in the general one-shot setting. Furthermore, the criterion is tight for mappings that satisfy certain natural conditions. One-shot decoupling has a number of applications both in physics and information theory, e.g., as a building block for quantum information processing protocols. As an example, we give a one-shot state merging protocol and show that it is essentially optimal in terms of its entanglement consumption/production.",
issn="1432-0916",
doi="10.1007/s00220-014-1990-4",
url="https://doi.org/10.1007/s00220-014-1990-4"
}

@ARTICLE{KRS09, 
author={R. Konig and R. Renner and C. Schaffner}, 
journal={IEEE Transactions on Information Theory}, 
title={The Operational Meaning of Min- and Max-Entropy}, 
year={2009}, 
volume={55}, 
number={9}, 
pages={4337-4347}, 
keywords={information theory;maximum entropy methods;minimum entropy methods;information theory;max-entropy;min-entropy;Channel capacity;Communication channels;Entropy;Information security;Information theory;Merging;Quantum entanglement;Quantum mechanics;Random variables;Veins;Entropy measures;max-entropy;min-entropy;operational interpretations;quantum hypothesis testing;quantum information theory;single-shot information theory;singlet fraction}, 
doi={10.1109/TIT.2009.2025545}, 
ISSN={0018-9448}, 
month={Sept},}



@ARTICLE{PJLCLTKD14,
   author       = "A. Pappa and P. Jouguet and T. Lawson and A. Chailloux and M. Legr\'e and P. Trinkler and I. Kerenidis and E. Diamanti",
title = "Experimental plug and play quantum coin flipping",
   journal      = "Nat. Commun.",
   volume       = "5", 
   pages        = "3717",
   year         = "2014",
url = "https://www.nature.com/articles/ncomms4717"
}

@article{NFHM08,
	doi = {10.1088/1367-2630/10/8/083037},
	url = {https://doi.org/10.1088/1367-2630/10/8/083037},
	year = 2008,
	month = {aug},
	publisher = {{IOP} Publishing},
	volume = {10},
	number = {8},
	pages = {083037},
	author = {A T Nguyen and J Frison and K Phan Huy and S Massar},
	title = {Experimental quantum tossing of a single coin},
	journal = {New J. Phys.},
	abstract = {The cryptographic protocol of coin tossing consists of two parties, Alice and Bob, who do not trust each other, but want to generate a random bit. If the parties use a classical communication channel and have unlimited computational resources, one of them can always cheat perfectly. If the parties use a quantum communication channel, there exist protocols such that neither party can cheat perfectly, although they may be able to significantly bias the coin. Here, we analyze in detail how the performance of a quantum coin tossing experiment should be compared to classical protocols, taking into account the inevitable experimental imperfections. We then report an all-optical fiber experiment in which a single coin is tossed whose randomness is higher than achievable by any classical protocol and present some easily realizable cheating strategies by Alice and Bob.}
}

@article{TVUZ05,
  title = {Experimental Quantum Coin Tossing},
  author = {Molina-Terriza, G. and Vaziri, A. and Ursin, R. and Zeilinger, A.},
  journal = {Phys. Rev. Lett.},
  volume = {94},
  issue = {4},
  pages = {040501},
  numpages = {4},
  year = {2005},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.94.040501},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.94.040501}
}


@ARTICLE{ENGLWW14,
   author       = "C. Erven and N. Ng and N. Gigov and R. Laflamme and S. Wehner and G. Weihs",
title = "An experimental implementation of oblivious transfer in the noisy storage mode",
   journal      = "Nat. Commun.",
   volume       = "5", 
   pages        = "3418",
   year         = "2014",
url = "https://doi.org/10.1038/ncomms4418"
}





@ARTICLE{KLHGLNSZ14,
   author       = "B. Korzh and C. Ci Wen Lim and R. Houlmann and N. Gisin and M. Jun Li and D. Nolan and	B. Sanguinetti and R. Thew and H. Zbinden",
title = "Provably secure and practical quantum key distribution over 307 km of optical fibre",
   journal      = "Nat. Photon.",
   volume       = "9", 
   pages        = "163",
   year         = "2014",
url = "https://www.nature.com/nphoton/journal/v9/n3/abs/nphoton.2014.327.html"
}

@article {ZKBRCMBCVSMSBF17,
	author = {Zhong, Tian and Kindem, Jonathan M. and Bartholomew, John G. and Rochman, Jake and Craiciu, Ioana and Miyazono, Evan and Bettinelli, Marco and Cavalli, Enrico and Verma, Varun and Nam, Sae Woo and Marsili, Francesco and Shaw, Matthew D. and Beyer, Andrew D. and Faraon, Andrei},
	title = {Nanophotonic rare-earth quantum memory with optically controlled retrieval},
	year = {2017},
	doi = {10.1126/science.aan5959},
	publisher = {American Association for the Advancement of Science},
	abstract = {Optical quantum memories are essential elements in quantum networks for long distance distribution of quantum entanglement. Scalable development of quantum network nodes requires on-chip qubit storage functionality with control of its readout time. We demonstrate a high-fidelity nanophotonic quantum memory based on a mesoscopic neodymium ensemble coupled to a photonic crystal cavity. The nanocavity enables \&gt;95\% spin polarization for efficient initialization of the atomic frequency comb memory, and time-bin-selective readout via enhanced optical Stark shift of the comb frequencies. Our solid-state memory is integrable with other chip-scale photon source and detector devices for multiplexed quantum and classical information processing at the network nodes.},
	issn = {0036-8075},
	URL = {http://science.sciencemag.org/content/early/2017/08/30/science.aan5959},
	journal = {Science}
}


@article{KNIDAAMKLAMT14,
title = "Polarization entangled photon-pair source based on quantum nonlinear photonics and interferometry",
journal = "Optics Communications",
volume = "327",
number = "Supplement C",
pages = "7 - 16",
year = "2014",
note = "Special Issue on Nonlinear Quantum Photonics",
issn = "0030-4018",
doi = "https://doi.org/10.1016/j.optcom.2014.03.056",
url = "http://www.sciencedirect.com/science/article/pii/S0030401814002879",
author = "F. Kaiser and L.A. Ngah and A. Issautier and T. Delord and D. Aktas and V. D׳Auria and M.P. De Micheli and A. Kastberg and L. Labonté and O. Alibart and A. Martin and S. Tanzilli",
keywords = "Quantum communication, Polarization entanglement, Nonlinear integrated photonics"
}

@inproceedings{TSMSYSHSFH17,
author = {Yoshiaki Tamura and Hirotaka Sakuma and Keisei Morita and Masato Suzuki and Yoshinori Yamamoto and Kensaku Shimada and Yuya Honma and Kazuyuki Sohma and Takashi Fujii and Takemi Hasegawa},
booktitle = {Optical Fiber Communication Conference Postdeadline Papers},
journal = {Optical Fiber Communication Conference Postdeadline Papers},
keywords = {Fiber design and fabrication; Fiber optics communications; Fibers, single-mode},
pages = {Th5D.1},
publisher = {Optical Society of America},
title = {Lowest-Ever 0.1419-dB/km Loss Optical Fiber},
year = {2017},
url = {http://www.osapublishing.org/abstract.cfm?URI=OFC-2017-Th5D.1},
doi = {10.1364/OFC.2017.Th5D.1},
abstract = {Lowest-ever 0.1419-dB/km loss at 1560-nm wavelength was realized in a silica-core fiber with 1290-{\textdegree}C low fictive temperature, 147-{\textmu}m2 large effective area and low microbending loss due to soft primary coating.},
}

@article{FLDCTPSYS17,
author = {Bernd Fr\"{o}hlich and Marco Lucamarini and James F. Dynes and Lucian C. Comandar and Winci W.-S. Tam and Alan Plews and Andrew W. Sharpe and Zhiliang Yuan and Andrew J. Shields},
journal = {Optica},
keywords = {Quantum communications ; Quantum cryptography ; Quantum information and processing},
number = {1},
pages = {163--167},
publisher = {OSA},
title = {Long-distance quantum key distribution secure against coherent attacks},
volume = {4},
month = {Jan},
year = {2017},
url = {http://www.osapublishing.org/optica/abstract.cfm?URI=optica-4-1-163},
doi = {10.1364/OPTICA.4.000163},
abstract = {Quantum key distribution (QKD) permits information-theoretically secure transmission of digital encryption keys, assuming that the behavior of the devices employed for the key exchange can be reliably modeled and predicted. Remarkably, no assumptions have to be made on the capabilities of an eavesdropper other than that she is bounded by the laws of nature, thus making the security of QKD ``unconditional.'' However, unconditional security is hard to achieve in practice. For example, any experimental realization can only collect finite data samples, leading to vulnerabilities against coherent attacks, the most general class of attacks, and for some protocols the theoretical proof of robustness against these attacks is still missing. For these reasons, in the past many QKD experiments have fallen short of implementing an unconditionally secure protocol and have instead considered limited attacking capabilities by the eavesdropper. Here, we explore the security of QKD against coherent attacks in the most challenging environment: the long-distance transmission of keys. We demonstrate that the BB84 protocol can provide positive key rates for distances up to 240 km without multiplexing of conventional signals, and up to 200 km with multiplexing. Useful key rates can be achieved even for the longest distances, using practical thermo-electrically cooled single-photon detectors.},
}

@article{RDZJJKK10,
  title = {A quantum memory with telecom{-}wavelength conversion},
  author = {A. G. Radnaev and	Y. O. Dudin and	R. Zhao and	H. H. Jen and S. D. Jenkins and	A. Kuzmich	and T. A. B. Kennedy},
  journal = {Nature Phys.},
  volume = {6},
  pages = {894–899},
  year = {2010},
  doi = {10.1038/nphys1773},
  url = {https://www.nature.com/nphys/journal/v6/n11/full/nphys1773.html}
}



@article{WST08,
  title = {Cryptography from Noisy Storage},
  author = {Wehner, Stephanie and Schaffner, Christian and Terhal, Barbara M.},
  journal = {Phys. Rev. Lett.},
  volume = {100},
  issue = {22},
  pages = {220502},
  numpages = {4},
  year = {2008},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.100.220502},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.100.220502}
}

@article{DFSS08,
author = "I. Damgard and S. Fehr and L. Salvail and C. Schaffner",
title = "Cryptography in the Bounded-Quantum-Storage Model",
journal="SIAM J. Comput.",
year = "2008",
volume="37",
pages="1865-1890",
url = "http://epubs.siam.org/doi/abs/10.1137/060651343"
}

@article{GFKZR06,
  title = {Trojan-horse attacks on quantum-key-distribution systems},
  author = {Gisin, N. and Fasel, S. and Kraus, B. and Zbinden, H. and Ribordy, G.},
  journal = {Phys. Rev. A},
  volume = {73},
  issue = {2},
  pages = {022320},
  numpages = {6},
  year = {2006},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.73.022320},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.73.022320}
}


@article{M09,
	doi = {10.1088/1367-2630/11/6/065003},
	url = {https://doi.org/10.1088%2F1367-2630%2F11%2F6%2F065003},
	year = 2009,
	month = {jun},
	publisher = {{IOP} Publishing},
	volume = {11},
	number = {6},
	pages = {065003},
	author = {Vadim Makarov},
	title = {Controlling passively quenched single photon detectors by bright light},
	journal = {New J. Phys.},
	abstract = {Single photon detectors (SPDs) based on passively quenched avalanche photodiodes can be temporarily blinded by relatively bright light, of intensity less than 1 nW. A bright-light regime suitable for attacking a quantum key distribution system containing such detectors is described in this paper. In this regime, all SPDs in the receiver Bob are uniformly blinded by continuous illumination coming from the eavesdropper Eve. When Eve needs a certain detector in Bob to produce a click, she modifies the polarization (or other parameters used to encode quantum states) of the light she sends to Bob such that the target detector stops receiving light, while the other detector(s) continue to be illuminated. The target detector regains single photon sensitivity and, when Eve modifies the polarization again, produces a single click. Thus, Eve has full control of Bob and can perform a successful intercept–resend attack. To check the feasibility of the attack, three different models of passively quenched detectors have been tested. In the experiment, I have simulated the intensity diagrams the detectors would receive in a real QKD system under attack. Control parameters and side effects are considered. It appears that the attack could be practically possible.}
}

@article{LWWESM10,
  title = {Hacking commercial quantum cryptography systems by tailored bright illumination},
  author = {L. Lydersen and C. Wiechers and C. Wittmann and D. Elser and J. Skaar and V. Makarov},
  journal = {Nature Photon.},
  volume = {4},
  pages = {686–689},
  year = {2010},
  doi = {10.1038/nphoton.2010.214},
  url = {https://www.nature.com/articles/nphoton.2010.214}
}

@article{MAS06,
  title = {Effects of detector efficiency mismatch on security of quantum cryptosystems},
  author = {Makarov, Vadim and Anisimov, Andrey and Skaar, Johannes},
  journal = {Phys. Rev. A},
  volume = {74},
  issue = {2},
  pages = {022313},
  numpages = {11},
  year = {2006},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.74.022313},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.74.022313}
}

@article{ZFQCL08,
  title = {Quantum hacking: Experimental demonstration of time-shift attack against practical quantum-key-distribution systems},
  author = {Zhao, Yi and Fung, Chi-Hang Fred and Qi, Bing and Chen, Christine and Lo, Hoi-Kwong},
  journal = {Phys. Rev. A},
  volume = {78},
  issue = {4},
  pages = {042333},
  numpages = {5},
  year = {2008},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.78.042333},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.78.042333}
}



@article{FTLM09,
  author    = {Chi{-}Hang Fred Fung and
               Kiyoshi Tamaki and
               Bing Qi and
               Hoi{-}Kwong Lo and
               Xiongfeng Ma},
  title     = {Security proof of quantum key distribution with detection efficiency
               mismatch},
  journal   = {Quantum Inf. Comput.},
  volume    = {9},
  number    = {1{\&}2},
  pages     = {131--165},
  year      = {2009},
  url       = {http://www.rintonpress.com/xxqic9/qic-9-12/0131-0165.pdf},
  timestamp = {Mon, 25 May 2020 09:12:17 +0200},
  biburl    = {https://dblp.org/rec/journals/qic/FungTQLM09.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@article{LJWMSMML11,
  title = {Superlinear threshold detectors in quantum cryptography},
  author = {Lydersen, Lars and Jain, Nitin and Wittmann, Christoffer and Mar\o{}y, \O{}ystein and Skaar, Johannes and Marquardt, Christoph and Makarov, Vadim and Leuchs, Gerd},
  journal = {Phys. Rev. A},
  volume = {84},
  issue = {3},
  pages = {032320},
  numpages = {7},
  year = {2011},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.84.032320},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.84.032320}
}

@ARTICLE{KYS08,
   author       = "B. E. Kardynał and Z. L. Yuan and A. J. Shields",
title = "An avalanche‐photodiode{-}based photon-number-resolving detector",
   journal      = "Nature Photon.",
   volume       = "2", 
   pages        = "425",
   year         = "2008",
url = "https://www.nature.com/articles/nphoton.2008.101"
}

@article{LMN08,
author = {Adriana E. Lita and Aaron J. Miller and Sae Woo Nam},
journal = {Opt. Express},
keywords = {Optical design and fabrication; Quantum detectors},
number = {5},
pages = {3032--3040},
publisher = {OSA},
title = {Counting near{-}infrared single{-}photons with 95\% efficiency},
volume = {16},
month = {Mar},
year = {2008},
url = {http://www.opticsexpress.org/abstract.cfm?URI=oe-16-5-3032},
doi = {10.1364/OE.16.003032},
abstract = {Single-photon detectors operating at visible and near-infrared wavelengths with high detection efficiency and low noise are a requirement for many quantum-information applications. Superconducting transition-edge sensors (TESs) are capable of detecting visible and near-infrared light at the single-photon level and are capable of discriminating between one-and two-photon absorption events; however these capabilities place stringent design requirements on the TES heat capacity, thermometry, and optical detection efficiency. We describe the fabrication and evaluation of a fiber-coupled, photon-number-resolving TES detector optimized for absorption at 1550 and 1310 nm wavelengths. The measured system detection efficiency at 1556 nm is 95 \%{\textpm}2 \%, which to our knowledge is the highest system detection efficiency reported for a near-infrared single-photon detector.Work of US government: not subject to US copyright},
}


  	
@article{ZQLQ10,
  author={Yi Zhao and Bing Qi and Hoi-Kwong Lo and Li Qian},
  title={Security analysis of an untrusted source for quantum key distribution: passive approach},
  journal={New Journal of Physics},
  volume={12},
  number={2},
  pages={023024},
  url={http://stacks.iop.org/1367-2630/12/i=2/a=023024},
  year={2010},
  abstract={We present a passive approach to the security analysis of quantum key distribution (QKD) with an untrusted source. A complete proof of its unconditional security is also presented. This scheme has significant advantages in real-life implementations as it does not require fast optical switching or a quantum random number generator. The essential idea is to use a beam splitter to split each input pulse. We show that we can characterize the source using a cross-estimate technique without active routing of each pulse. We have derived analytical expressions for the passive estimation scheme. Moreover, using simulations, we have considered four real-life imperfections: additional loss introduced by the 'plug&play' structure, inefficiency of the intensity monitor noise of the intensity monitor, and statistical fluctuation introduced by finite data size. Our simulation results show that the passive estimate of an untrusted source remains useful in practice, despite these four imperfections. Also, we have performed preliminary experiments, confirming the utility of our proposal in real-life applications. Our proposal makes it possible to implement the 'plug&play' QKD with the security guaranteed, while keeping the implementation practical.}
}

@article{ILM07,
  title = {Unconditional security of practical quantum key distribution},
  author = {H. Inamori and N. L\"utkenhaus and D. Mayers},
  journal = {Eur. Phys. J. D},
  volume = {41},
  issue = {},
  pages = {599},
  numpages = {},
  year = {2007},
  month = {},
  publisher = {},
  doi = {10.1140/epjd/e2007-00010-4},
  url = {}
}


@article{ZQL08,
  title = {Quantum key distribution with an unknown and untrusted source},
  author = {Zhao, Yi and Qi, Bing and Lo, Hoi-Kwong},
  journal = {Phys. Rev. A},
  volume = {77},
  issue = {5},
  pages = {052327},
  numpages = {14},
  year = {2008},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.77.052327},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.77.052327}
}

@article{DHL00,
  title = {Unambiguous state discrimination in quantum cryptography with weak coherent states},
  author = {Du\ifmmode \check{s}\else \v{s}\fi{}ek, Miloslav and Jahma, Mika and L\"utkenhaus, Norbert},
  journal = {Phys. Rev. A},
  volume = {62},
  issue = {2},
  pages = {022306},
  numpages = {9},
  year = {2000},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.62.022306},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.62.022306}
}



	

@Article{KW15,
author="Kamm, Liina
and Willemson, Jan",
title="Secure floating point arithmetic and private satellite collision analysis",
journal="International Journal of Information Security",
year="2015",
month="Nov",
day="01",
volume="14",
number="6",
pages="531--548",
abstract="In this paper, we show that it is possible and, indeed, feasible to use secure multiparty computation (SMC) for calculating the probability of a collision between two satellites. For this purpose, we first describe basic floating point arithmetic operators (addition and multiplication) for multiparty computations. The operators are implemented on the                                                                           {\$}{\$}{\{}{\backslash}textsc {\{}Sharemind{\}}{\}}{\$}{\$}                                                                                    S                                                  H                          A                          R                          E                          M                          I                          N                          D                                                                                                     SMC engine. We discuss the implementation details, provide methods for evaluating example elementary functions (inverse, square root, exponentiation of                                                                           {\$}{\$}e{\$}{\$}                                                            e                                                      , error function). Using these primitives, we implement a satellite conjunction analysis algorithm and give benchmark results for the primitives as well as the conjunction analysis itself.",
issn="1615-5270",
doi="10.1007/s10207-014-0271-8",
url="https://doi.org/10.1007/s10207-014-0271-8"
}

@INPROCEEDINGS{A09, 
author={S. Aaronson}, 
booktitle={2009 24th Annual IEEE Conference on Computational Complexity}, 
title={Quantum Copy-Protection and Quantum Money}, 
year={2009}, 
volume={}, 
number={}, 
pages={229-242}, 
keywords={computational complexity;copy protection;quantum computing;Grover search;Wiesner scheme;complexity-theoretic no-cloning theorem;computational complexity;publicly-verifiable quantum money;quantum copy-protection;quantum oracles;quantum states;quantum t-designs;random stabilizer states;security argument;Authentication;Computational complexity;Computer science;Counterfeiting;Cryptography;Information security;Physics computing;Quantum computing;Quantum entanglement;Quantum mechanics;copy-protection;electronic cash;no-cloning theorem;quantum computing;stabilizer states;t-designs}, 
doi={10.1109/CCC.2009.42}, 
ISSN={1093-0159}, 
month={July},}

@Article {PYLLC12,
	author = {Pastawski, Fernando and Yao, Norman Y. and Jiang, Liang and Lukin, Mikhail D. and Cirac, J. Ignacio},
	title = {Unforgeable noise{-}tolerant quantum tokens},
	volume = {109},
	number = {40},
	pages = {16079-16082},
	year = {2012},
	doi = {10.1073/pnas.1203552109},
	publisher = {National Academy of Sciences},
	issn = {0027-8424},
		journal = {Proc. Natl. Acad. Sci. USA},
}
%URL = {http://www.pnas.org/content/109/40/16079},
	%eprint = {http://www.pnas.org/content/109/40/16079.full.pdf},

@INPROCEEDINGS{G12, 
author={D. Gavinsky}, 
booktitle={2012 IEEE 27th Conference on Computational Complexity}, 
title={Quantum Money with Classical Verification}, 
year={2012}, 
volume={}, 
number={}, 
pages={42-52}, 
keywords={banking;quantum cryptography;classical communication;classical verification;coin verification;secure quantum money scheme;Communication channels;Databases;Protocols;Quantum mechanics;Registers;Resistance;Security}, 
doi={10.1109/CCC.2012.10}, 
ISSN={1093-0159}, 
month={June},}





@inproceedings{BBBW83,
author = {C.H. Bennett and G. Brassard and S. Breidbart and S. Wiesner},
title = {Quantum Cryptography, or Unforgeable Subway Tokens},
year = {1983},
editor = {D. Chaum and R.L. Rivest and A.T. Sherman},
publisher = {Springer},
address = {Boston, MA},
url = {https://doi.org/10.1007/978-1-4757-0602-4_26},
booktitle = {Advances in Cryptology},
location = {Boston, MA}
}



@inproceedings{AC12,
author = {Aaronson, Scott and Christiano, Paul},
title = {Quantum Money from Hidden Subspaces},
year = {2012},
isbn = {9781450312455},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2213977.2213983},
doi = {10.1145/2213977.2213983},
abstract = {Forty years ago, Wiesner pointed out that quantum mechanics raises the striking possibility of money that cannot be counterfeited according to the laws of physics. We propose the first quantum money scheme that is (1) public-key---meaning that anyone can verify a banknote as genuine, not only the bank that printed it, and (2) cryptographically secure, under a "classical" hardness assumption that has nothing to do with quantum money. Our scheme is based on hidden subspaces, encoded as the zero-sets of random multivariate polynomials. A main technical advance is to show that the "black-box" version of our scheme, where the polynomials are replaced by classical oracles, is unconditionally secure. Previously, such a result had only been known relative to a quantum oracle (and even there, the proof was never published).Even in Wiesner's original setting---quantum money that can only be verified by the bank---we are able to use our techniques to patch a major security hole in Wiesner's scheme. We give the first private-key quantum money scheme that allows unlimited verifications and that remains unconditionally secure, even if the counterfeiter can interact adaptively with the bank.Our money scheme is simpler than previous public-key quantum money schemes, including a knot-based scheme of Farhi et al. The verifier needs to perform only two tests, one in the standard basis and one in the Hadamard basis---matching the original intuition for quantum money, based on the existence of complementary observables.Our security proofs use a new variant of Ambainis's quantum adversary method, and several other tools that might be of independent interest.},
booktitle = {Proceedings of the Forty-Fourth Annual ACM Symposium on Theory of Computing},
pages = {41–60},
numpages = {20},
keywords = {no-cloning theorem, quantum cryptography, quantum money, multivariate polynomials, quantum computing},
location = {New York, New York, USA},
series = {STOC '12}
}





@MISC{PCJYL14, 
   author       = "Pastawski, Fernando and Yao, Norman Y. and Jiang, Liang and Lukin, Mikhail D. and Cirac, J. Ignacio",
title = "Unforgeable noise{-}tolerant quantum tokens",
   howpublished = "{US Patent No. }0358793", 
   year         =  "2014", 
}

@article{PGK18,
  title = {Practical and unconditionally secure spacetime-constrained oblivious transfer},
  author = {Pital\'ua-Garc\'{\i}a, Dami\'an and Kerenidis, Iordanis},
  journal = {Phys. Rev. A},
  volume = {98},
  issue = {3},
  pages = {032327},
  numpages = {9},
  year = {2018},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.98.032327},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.98.032327}
}

@article{PG19,
  title = {One-out-of-$m$ spacetime-constrained oblivious transfer},
  author = {Pital\'ua-Garc\'{\i}a, Dami\'an},
  journal = {Phys. Rev. A},
  volume = {100},
  issue = {1},
  pages = {012302},
  numpages = {20},
  year = {2019},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.100.012302},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.100.012302}
}




@article{SBKTP09,
  title = {Preparation Contextuality Powers Parity-Oblivious Multiplexing},
  author = {Spekkens, Robert W. and Buzacott, D. H. and Keehn, A. J. and Toner, Ben and Pryde, G. J.},
  journal = {Phys. Rev. Lett.},
  volume = {102},
  issue = {1},
  pages = {010401},
  numpages = {4},
  year = {2009},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.102.010401},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.102.010401}
}

@INPROCEEDINGS{ANTV99,
 author = {Ambainis, Andris and Nayak, Ashwin and Ta-Shma, Ammon and Vazirani, Umesh},
 title = {Dense Quantum Coding and a Lower Bound for 1-way Quantum Automata},
 booktitle = {Proceedings of the Thirty-first Annual ACM Symposium on Theory of Computing, STOC '99},
  pages = {376--383},
  publisher = {ACM},
 address = {New York, NY, USA},
  year = {1999},
  }
 
 %series = {STOC '99},
%isbn = {1-58113-067-8},
 %location = {Atlanta, Georgia, USA},
% numpages = {8},
 %url = {http://doi.acm.org/10.1145/301250.301347},
 %doi = {10.1145/301250.301347},
 %acmid = {301347},


@article{HINRY06,
  author={M Hayashi and K Iwama and H Nishimura and R Raymond and S Yamashita},
  title={(4,1)-Quantum random access coding does not exist—one qubit is not enough to recover one of four bits},
  journal={New J. Phys.},
  volume={8},
  number={8},
  pages={129},
  url={http://stacks.iop.org/1367-2630/8/i=8/a=129},
  year={2006},
  abstract={An ( n ,1, p )-quantum random access (QRA) coding, introduced by Ambainis et al (1999 ACM Symp. Theory of Computing p 376), is the following communication system: the sender which has n -bit information encodes his/her information into one qubit, which is sent to the receiver. The receiver can recover any one bit of the original n bits correctly with probability at least p , through a certain decoding process based on positive operator-valued measures. Actually, Ambainis et al shows the existence of a (2,1,0.85)-QRA coding and also proves the impossibility of its classical counterpart. Chuang immediately extends it to a (3,1,0.79)-QRA coding and whether or not a (4,1, p )-QRA coding such that p > 1/2 exists has been open since then. This paper gives a negative answer to this open question. Moreover, we generalize its negative answer for one-qubit encoding to the case of multiple-qubit encoding}
}


@article{L17,
  title = {Improved classical and quantum random access codes},
  author = {Liab\o{}tr\o{}, O.},
  journal = {Phys. Rev. A},
  volume = {95},
  issue = {5},
  pages = {052315},
  numpages = {13},
  year = {2017},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.95.052315},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.95.052315}
}

@INPROCEEDINGS{Y86, 
author={A. C. Yao}, 
booktitle={27th Annual Symposium on Foundations of Computer Science (sfcs 1986)}, 
title={How to generate and exchange secrets},
pages={162-167},
year={1986}, 
}
%keywords={Polynomials;Probability distribution;Turing machines;Privacy;Knowledge transfer;History;Computer science;Cryptographic protocols;Cryptography;Circuits}, 
%doi={10.1109/SFCS.1986.25}, 
%ISSN={0272-5428}, 
%month={Oct},}


@INPROCEEDINGS{AMTW00, 
author={A. Ambainis and M. Mosca and A. Tapp and R. De Wolf}, 
booktitle={Proceedings 41st Annual Symposium on Foundations of Computer Science}, 
title={Private quantum channels}, 
pages={547-553},
year={2000},
}
%keywords={quantum computing;cryptography;private quantum channels;classical private key;insecure one-way quantum channel;private communication;quantum information;qubits;one-time pad encryption scheme;Information security;Cryptography;Marine vehicles;Teleportation;Ice;Entropy}, 
%doi={10.1109/SFCS.2000.892142}, 
%ISSN={0272-5428}, 
%month={Nov},}

@article{PGK18.2,
  title = {Practical and unconditionally secure spacetime-constrained oblivious transfer},
  author = {Pital\'ua-Garc\'{\i}a, Dami\'an and Kerenidis, Iordanis},
  journal = {Phys. Rev. A},
  volume = {98},
  issue = {3},
  pages = {032327},
  numpages = {9},
  year = {2018},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.98.032327},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.98.032327}
}

@unpublished{K18,
  title = {Summonable {S}upermoney: virtual tokens for a relativistic economy},
  author = {A. Kent},
year="2018",
eprint = "1806.05884",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1806.05884;%%",
}

@unpublished{HM18,
  title = {Localizing and excluding quantum information; or, how to share a quantum secret in spacetime},
  author = {P. Hayden and A. May},
year="2018",
eprint = "1806.04154",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1806.04154;%%",
}



@unpublished{K18.2,
  title = {Unconstrained Summoning},
  author = {A. Kent},
year="2018",
eprint = "1806.01736",
archivePrefix = "arXiv",
SLACcitation = "%%CITATION=arXiv:1806.01736;%%",
}

@article{KSmoney,
author = {Adrian Kent },
title = {S-money: virtual tokens for a relativistic economy},
journal = {Proc. R. Soc. A},
volume = {475},
number = {2225},
pages = {20190170},
year = {2019},
doi = {10.1098/rspa.2019.0170},
URL = {https://royalsocietypublishing.org/doi/abs/10.1098/rspa.2019.0170},
}



@article {Pastawski16079,
	author = {Pastawski, Fernando and Yao, Norman Y. and Jiang, Liang and Lukin, Mikhail D. and Cirac, J. Ignacio},
	title = {Unforgeable noise-tolerant quantum tokens},
	volume = {109},
	number = {40},
	pages = {16079--16082},
	year = {2012},
	doi = {10.1073/pnas.1203552109},
	publisher = {National Academy of Sciences},
	abstract = {The realization of devices that harness the laws of quantum mechanics represents an exciting challenge at the interface of modern technology and fundamental science. An exemplary paragon of the power of such quantum primitives is the concept of {\textquotedblleft}quantum money{\textquotedblright} [Wiesner S (1983) ACM SIGACT News 15:78{\textendash}88]. A dishonest holder of a quantum bank note will invariably fail in any counterfeiting attempts; indeed, under assumptions of ideal measurements and decoherence-free memories such security is guaranteed by the no-cloning theorem. In any practical situation, however, noise, decoherence, and operational imperfections abound. Thus, the development of secure {\textquotedblleft}quantum money{\textquotedblright}-type primitives capable of tolerating realistic infidelities is of both practical and fundamental importance. Here, we propose a novel class of such protocols and demonstrate their tolerance to noise; moreover, we prove their rigorous security by determining tight fidelity thresholds. Our proposed protocols require only the ability to prepare, store, and measure single quantum bit memories, making their experimental realization accessible with current technologies.},
	issn = {0027-8424},
	URL = {https://www.pnas.org/content/109/40/16079},
	eprint = {https://www.pnas.org/content/109/40/16079.full.pdf},
	journal = {r, Proc. Natl. Acad. Sci. U.S.A.}
}




%% References below given by Adrian in relmoney.short.bib on 17 August 2019



@article{kaniewski2013secure,
  title={Secure bit commitment from relativistic constraints},
  author={Kaniewski, J{\k{e}}drzej and Tomamichel, Marco and H{\"a}nggi, Esther and Wehner, Stephanie},
  journal={IEEE Transactions on Information Theory},
  volume={59},
  number={7},
  pages={4687--4699},
  year={2013},
  publisher={IEEE}
}

@article{kent2019s,
  title={S-money: virtual tokens for a relativistic economy},
  author={Kent, Adrian},
  journal={Proc. R. Soc. A},
  volume={475},
  number={2225},
  pages={20190170},
  year={2019},
  publisher={The Royal Society Publishing}
}

@book{ferguson1999house,
  title={The House of Rothschild: Volume 1: Money's Prophets: 1798-1848},
  author={Ferguson, Niall},
  volume={1},
  year={1999},
  publisher={Penguin}
}

@article{lansky2018possible,
  title={Possible State Approaches to Cryptocurrencies},
  author={Lansky, Jan},
  journal={Journal of Systems Integration},
  volume={9},
  number={1},
  pages={19},
  year={2018},
  publisher={Journal of Systems Integration}
}

@article{krugman2010theory,
  title={The theory of interstellar trade},
  author={Krugman, Paul},
  journal={Economic Inquiry},
  volume={48},
  number={4},
  pages={1119--1123},
  year={2010},
  publisher={Wiley Online Library}
}

@misc{patents,
author={Adrian Kent}, 
title={{UK} patent application {GB}1511652.8, submitted 2.7.15;
further patent applications in process}}

@article{CK12,
  title={Security details for bit commitment by transmitting measurement outcomes},
  author={Croke, Sarah and Kent, Adrian},
  journal={Physical Review A},
  volume={86},
  number={5},
  pages={052309},
  year={2012},
  publisher={APS}
}

@article{wiesner1983conjugate,
  title={Conjugate coding},
  author={Wiesner, Stephen},
  journal={ACM Sigact News},
  volume={15},
  number={1},
  pages={78--88},
  year={1983},
  publisher={ACM}
}

@inproceedings{MVW12,
  title={Optimal Counterfeiting Attacks and Generalizations for {W}iesner's Quantum Money.},
  author={Molina, Abel and Vidick, Thomas and Watrous, John},
  booktitle={TQC},
  pages={45--64},
  year={2012},
  organization={Springer},
  url = {https://link.springer.com/chapter/10.1007/978-3-642-35656-8_4}
}





@article{pastawski2012unforgeable,
  title={Unforgeable noise-tolerant quantum tokens},
  author={Pastawski, Fernando and Yao, Norman Y and Jiang, Liang and Lukin, Mikhail D and Cirac, J Ignacio},
  journal={Proceedings of the National Academy of Sciences},
  volume={109},
  number={40},
  pages={16079--16082},
  year={2012},
  publisher={National Acad Sciences}
}

@inproceedings{gavinsky2012quantum,
  title={Quantum money with classical verification},
  author={Gavinsky, Dmitry},
  booktitle={Computational Complexity (CCC), 2012 IEEE 27th Annual Conference on},
  pages={42--52},
  year={2012},
  organization={IEEE},
  doi = {10.1109/CCC.2012.10}
}
@inproceedings{aaronson2012quantum,
  title={Quantum money from hidden subspaces},
  author={Aaronson, Scott and Christiano, Paul},
  booktitle={Proceedings of the forty-fourth annual ACM symposium on Theory of computing},
  pages={41--60},
  year={2012},
  organization={ACM}
}


@article{kent2013no,
  title={A no-summoning theorem in relativistic quantum theory},
  author={Kent, Adrian},
  journal={Quantum Information Processing},
  pages={1--10},
  year={2013},
  publisher={Springer}
}

@article{kent2012quantum,
  title={Quantum tasks in {M}inkowski space},
  author={Kent, Adrian},
  journal={Classical and Quantum Gravity},
  volume={29},
  number={22},
  pages={224013},
  year={2012},
  publisher={IOP Publishing}
}

@article{hayden2016summoning,
  title={Summoning information in spacetime, or where and when can a qubit be?},
  author={Hayden, Patrick and May, Alex},
  journal={J. Phys. A: Math. Theor.},
  volume={49},
  number={17},
  pages={175304},
  year={2016},
  publisher={IOP Publishing}
}

@article{HM16,
	doi = {10.1088/1751-8113/49/17/175304},
	url = {https://doi.org/10.1088/1751-8113/49/17/175304},
	year = 2016,
	month = {mar},
	publisher = {{IOP} Publishing},
	volume = {49},
	number = {17},
	pages = {175304},
	author = {Patrick Hayden and Alex May},
	title = {Summoning information in spacetime, or where and when can a qubit be?},
	journal = {J. Phys. A: Math. Theor.},
	abstract = {One of the most important properties of quantum information, and the one ultimately responsible for its cryptographic applications, is that it can not be copied. That statement, however, is not completely accurate. While the no-cloning theorem of quantum mechanics prevents quantum information from being copied in space, the reversibility of microscopic physics actually requires that the information be copied in time. In spacetime as a whole, therefore, quantum information is widely replicated but in a restricted fashion. We fully characterize which regions of spacetime can all hold the same quantum information. Because quantum information can be delocalized through quantum error correction and teleportation, it need not follow well-defined trajectories. Instead, replication of the information in any configuration of spacetime regions not leading to violations of causality or the no-cloning principle is allowed. To demonstrate this, we answer the operational question of exactly when the information can be summoned to a set of spacetime points, showing how to do so efficiently using a combination of teleportation and codeword-stabilized quantum codes. This provides a simple and complete description of where and when a qubit can be located in spacetime, revealing a remarkable variety of possibilities.}
}

@article{adlam2016quantum,
  title={Quantum paradox of choice: More freedom makes summoning a quantum state harder},
  author={Adlam, Emily and Kent, Adrian},
  journal={Physical Review A},
  volume={93},
  number={6},
  pages={062327},
  year={2016},
  publisher={APS}}


@article{vaidman2003instantaneous,
  title={Instantaneous measurement of nonlocal variables},
  author={Vaidman, Lev},
  journal={Physical Review Letters},
  volume={90},
  number={1},
  pages={010402},
  year={2003},
  publisher={APS}}


@article{buhrman2014position,
  title={Position-based quantum cryptography: Impossibility and constructions},
  author={Buhrman, Harry and Chandran, Nishanth and Fehr, Serge and Gelles, Ran and Goyal, Vipul and Ostrovsky, Rafail and Schaffner, Christian},
  journal={SIAM Journal on Computing},
  volume={43},
  number={1},
  pages={150--178},
  year={2014},
  publisher={SIAM}
}


@article{brassard1988minimum,
  title={Minimum disclosure proofs of knowledge},
  author={Brassard, Gilles and Chaum, David and Cr{\'e}peau, Claude},
  journal={Journal of Computer and System Sciences},
  volume={37},
  number={2},
  pages={156--189},
  year={1988},
  publisher={Elsevier}
}

@article{kentrel,
author={Adrian Kent}, 
title={Unconditionally secure bit commitment},
journal={Phys. Rev. Lett.},
volume= { 83},
pages={ 1447--1450},
year={1999}}

@article{kent2011unconditionally,
  title={Unconditionally secure bit commitment with flying qudits},
  author={Kent, Adrian},
  journal={New Journal of Physics},
  volume={13},
  number={11},
  pages={113015},
  year={2011},
  publisher={IOP Publishing}
}


@article{kent2012unconditionally,
  title={Unconditionally secure bit commitment by transmitting measurement outcomes},
  author={Kent, Adrian},
  journal={Physical Review Letters},
  volume={109},
  number={13},
  pages={130501},
  year={2012},
  publisher={APS}
}

@article{lunghi2013experimental,
  title={Experimental bit commitment based on quantum communication and special relativity},
  author={Lunghi, Tommaso and Kaniewski, J and Bussieres, F{\'e}lix and Houlmann, Rapha{\"e}l and Tomamichel, M and Kent, A and Gisin, Nicolas and Wehner, S and Zbinden, Hugo},
  journal={Physical Review Letters},
  volume={111},
  number={18},
  pages={180504},
  year={2013},
  publisher={APS}
}
	
@article{kent2014secure,
  title={Secure and Robust Transmission and Verification of Unknown Quantum States in {M}inkowski Space},
  author={Kent, Adrian and Massar, Serge and Silman, Jonathan},
  journal={Scientific Reports},
  volume={4},
  pages={3901},
  year={2014},
  publisher={Nature Publishing Group}
}

@inproceedings{pedersen1991non,
  title={Non-interactive and information-theoretic secure verifiable secret sharing},
  author={Pedersen, Torben Pryds},
  booktitle={Annual International Cryptology Conference},
  pages={129--140},
  year={1991},
  organization={Springer}
}

@inproceedings{chailloux2017relativistic,
  title={Relativistic (or 2-Prover 1-Round) Zero-Knowledge Protocol for {NP} Secure Against Quantum Adversaries},
  author={Chailloux, Andr{\'e} and Leverrier, Anthony},
  booktitle={Annual International Conference on the Theory and Applications of Cryptographic Techniques},
  pages={369--396},
  year={2017},
  organization={Springer}
}

@article{kent2018unconstrained,
title={Unconstrained Summoning},
author={Kent, Adrian},
journal={Phys. Rev. A},
volume={98},
page={062332},
year={2018}}

@inproceedings{chaum1983blind,
  title={Blind signatures for untraceable payments},
  author={Chaum, David},
  booktitle={Advances in cryptology},
  pages={199--203},
  year={1983},
  organization={Springer}
}

@inproceedings{chaum1988untraceable,
  title={Untraceable electronic cash},
  author={Chaum, David and Fiat, Amos and Naor, Moni},
  booktitle={Conference on the Theory and Application of Cryptography},
  pages={319--327},
  year={1988},
  organization={Springer}
}

@inproceedings{kumar2017traceability,
  title={A traceability analysis of Monero�s blockchain},
  author={Kumar, Amrit and Fischer, Cl{\'e}ment and Tople, Shruti and Saxena, Prateek},
  booktitle={European Symposium on Research in Computer Security},
  pages={153--173},
  year={2017},
  organization={Springer}
}

@inproceedings{aaronson2009quantum,
  title={Quantum copy-protection and quantum money},
  author={Aaronson, Scott},
  booktitle={Computational Complexity, 2009. CCC'09. 24th Annual IEEE Conference on},
  pages={229--242},
  year={2009},
  organization={IEEE}
}

@article{MS10,
  title={Quantum coins},
  author={Mosca, Michele and Stebila, Douglas},
  journal={Error-Correcting Codes, Finite Geometries and Cryptography},
  volume={523},
  pages={35--47},
  year={2010},
  publisher={American Mathematical Soc.}
}

@inproceedings{FGHLS12,
author = {Farhi, Edward and Gosset, David and Hassidim, Avinatan and Lutomirski, Andrew and Shor, Peter},
title = {Quantum Money from Knots},
year = {2012},
isbn = {9781450311151},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2090236.2090260},
doi = {10.1145/2090236.2090260},
abstract = {Quantum money is a cryptographic protocol in which a mint can produce a quantum state, no one else can copy the state, and anyone (with a quantum computer) can verify that the state came from the mint. We present a concrete quantum money scheme based on superpositions of diagrams that encode oriented links with the same Alexander polynomial. We expect our scheme to be secure against computationally bounded adversaries.},
booktitle = {Proceedings of the 3rd Innovations in Theoretical Computer Science Conference},
pages = {276–289},
numpages = {14},
location = {Cambridge, Massachusetts},
series = {ITCS '12}
}




@article{MP16,
  title={Quantum cheques},
  author={S. R. Moulick and P. K. Panigrahi},
  journal={Quantum Inf. Process.},
  volume={15},
  pages={2475–2486},
  year={2016},
  url = {https://doi.org/10.1007/s11128-016-1273-4},
}


@ARTICLE{NJMKW12,
   author={N. Ng and S. Joshi and C. {Chen Ming} and C. Kurtsiefer and S. Wehner},
title={Experimental implementation of bit commitment in the noisy-storage model},
   journal={Nat. Commun.},
   volume={3}, 
   pages={1326},
   year={2012},
doi={10.1038/ncomms2268},
url={https://doi.org/10.1038/ncomms2268}
}
















@article{kaniewski2013secure,
  title={Secure bit commitment from relativistic constraints},
  author={Kaniewski, J{\k{e}}drzej and Tomamichel, Marco and H{\"a}nggi, Esther and Wehner, Stephanie},
  journal={IEEE Transactions on Information Theory},
  volume={59},
  number={7},
  pages={4687--4699},
  year={2013},
  publisher={IEEE}
}

@article{kent2019s,
  title={S-money: virtual tokens for a relativistic economy},
  author={Kent, Adrian},
  journal={Proc. R. Soc. A},
  volume={475},
  number={2225},
  pages={20190170},
  year={2019},
  publisher={The Royal Society Publishing}
}

@book{ferguson1999house,
  title={The House of Rothschild: Volume 1: Money's Prophets: 1798-1848},
  author={Ferguson, Niall},
  volume={1},
  year={1999},
  publisher={Penguin}
}

@article{lansky2018possible,
  title={Possible State Approaches to Cryptocurrencies},
  author={Lansky, Jan},
  journal={Journal of Systems Integration},
  volume={9},
  number={1},
  pages={19},
  year={2018},
  publisher={Journal of Systems Integration}
}

@article{krugman2010theory,
  title={The theory of interstellar trade},
  author={Krugman, Paul},
  journal={Economic Inquiry},
  volume={48},
  number={4},
  pages={1119--1123},
  year={2010},
  publisher={Wiley Online Library}
}

@misc{patents,
author={Adrian Kent}, 
title={{UK} patent application {GB}1511652.8, submitted 2.7.15;
further patent applications in process}}

@article{croke2012security,
  title={Security details for bit commitment by transmitting measurement outcomes},
  author={Croke, Sarah and Kent, Adrian},
  journal={Physical Review A},
  volume={86},
  number={5},
  pages={052309},
  year={2012},
  publisher={APS}
}

@article{wiesner1983conjugate,
  title={Conjugate coding},
  author={Wiesner, Stephen},
  journal={ACM Sigact News},
  volume={15},
  number={1},
  pages={78--88},
  year={1983},
  publisher={ACM}
}
@inproceedings{molina2012optimal,
  title={Optimal Counterfeiting Attacks and Generalizations for {W}iesner's Quantum Money.},
  author={Molina, Abel and Vidick, Thomas and Watrous, John},
  booktitle={TQC},
  pages={45--64},
  year={2012},
  organization={Springer}
}
@article{pastawski2012unforgeable,
  title={Unforgeable noise-tolerant quantum tokens},
  author={Pastawski, Fernando and Yao, Norman Y and Jiang, Liang and Lukin, Mikhail D and Cirac, J Ignacio},
  journal={Proceedings of the National Academy of Sciences},
  volume={109},
  number={40},
  pages={16079--16082},
  year={2012},
  publisher={National Acad Sciences}
}

@article{ASSBW03,
author = {Daryl Achilles and Christine Silberhorn and Cezary \'{S}liwa and Konrad Banaszek and Ian A. Walmsley},
journal = {Opt. Lett.},
keywords = {Photon counting; Quantum detectors; Fiber optics sources and detectors; Photon statistics; Avalanche photodiodes; Coherent states; Diode lasers; Fiber optic components; Photon statistics; Quantum information processing},
number = {23},
pages = {2387--2389},
publisher = {OSA},
title = {Fiber-assisted detection with photon number resolution},
volume = {28},
month = {Dec},
year = {2003},
url = {http://ol.osa.org/abstract.cfm?URI=ol-28-23-2387},
doi = {10.1364/OL.28.002387},
abstract = {We report the development of a photon-number-resolving detector based on a fiber-optical setup and a pair of standard avalanche photodiodes. The detector is capable of resolving individual photon numbers and operates on the well-known principle by which a single-mode input state is split into a large number (eight) of output modes. We reconstruct the photon statistics of weak coherent input light from experimental data and show that there is a high probability of inferring the input photon number from a measurement of the number of detection events on a single run.},
}

@article{XMZLP20,
  title = {Secure quantum key distribution with realistic devices},
  author = {Xu, Feihu and Ma, Xiongfeng and Zhang, Qiang and Lo, Hoi-Kwong and Pan, Jian-Wei},
  journal = {Rev. Mod. Phys.},
  volume = {92},
  issue = {2},
  pages = {025002},
  numpages = {60},
  year = {2020},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.92.025002},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.92.025002}
}



@article{FJPF03,
  title = {Photon-number resolution using time-multiplexed single-photon detectors},
  author = {Fitch, M. J. and Jacobs, B. C. and Pittman, T. B. and Franson, J. D.},
  journal = {Phys. Rev. A},
  volume = {68},
  issue = {4},
  pages = {043814},
  numpages = {6},
  year = {2003},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.68.043814},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.68.043814}
}




@inproceedings{gavinsky2012quantum,
  title={Quantum money with classical verification},
  author={Gavinsky, Dmitry},
  booktitle={Computational Complexity (CCC), 2012 IEEE 27th Annual Conference on},
  pages={42--52},
  year={2012},
  organization={IEEE}
}
@inproceedings{aaronson2012quantum,
  title={Quantum money from hidden subspaces},
  author={Aaronson, Scott and Christiano, Paul},
  booktitle={Proceedings of the forty-fourth annual ACM symposium on Theory of computing},
  pages={41--60},
  year={2012},
  organization={ACM}
}


@article{kent2013no,
  title={A no-summoning theorem in relativistic quantum theory},
  author={Kent, Adrian},
  journal={Quantum Information Processing},
  pages={1--10},
  year={2013},
  publisher={Springer}
}

@article{kent2012quantum,
  title={Quantum tasks in {M}inkowski space},
  author={Kent, Adrian},
  journal={Classical and Quantum Gravity},
  volume={29},
  number={22},
  pages={224013},
  year={2012},
  publisher={IOP Publishing}
}

@article{hayden2016summoning,
  title={Summoning information in spacetime, or where and when can a qubit be?},
  author={Hayden, Patrick and May, Alex},
  journal={J. Phys. A: Math. Theor.},
  volume={49},
  number={17},
  pages={175304},
  year={2016},
  publisher={IOP Publishing}
}

@article{adlam2016quantum,
  title={Quantum paradox of choice: More freedom makes summoning a quantum state harder},
  author={Adlam, Emily and Kent, Adrian},
  journal={Physical Review A},
  volume={93},
  number={6},
  pages={062327},
  year={2016},
  publisher={APS}}


@article{vaidman2003instantaneous,
  title={Instantaneous measurement of nonlocal variables},
  author={Vaidman, Lev},
  journal={Physical Review Letters},
  volume={90},
  number={1},
  pages={010402},
  year={2003},
  publisher={APS}}


@article{buhrman2014position,
  title={Position-based quantum cryptography: Impossibility and constructions},
  author={Buhrman, Harry and Chandran, Nishanth and Fehr, Serge and Gelles, Ran and Goyal, Vipul and Ostrovsky, Rafail and Schaffner, Christian},
  journal={SIAM Journal on Computing},
  volume={43},
  number={1},
  pages={150--178},
  year={2014},
  publisher={SIAM}
}


@article{brassard1988minimum,
  title={Minimum disclosure proofs of knowledge},
  author={Brassard, Gilles and Chaum, David and Cr{\'e}peau, Claude},
  journal={Journal of Computer and System Sciences},
  volume={37},
  number={2},
  pages={156--189},
  year={1988},
  publisher={Elsevier}
}

@article{kentrel,
author={Adrian Kent}, 
title={Unconditionally secure bit commitment},
journal={Phys. Rev. Lett.},
volume= { 83},
pages={ 1447--1450},
year={1999}}

@article{kentrelfinite, 
author={Adrian Kent}, 
title={Secure Classical Bit Commitment using Fixed Capacity
Communication Channels}, 
journal={J. Cryptology},
volume= { 18},
year={2005},
pages={ 313-335}}

@article{kent2011unconditionally,
  title={Unconditionally secure bit commitment with flying qudits},
  author={Kent, Adrian},
  journal={New Journal of Physics},
  volume={13},
  number={11},
  pages={113015},
  year={2011},
  publisher={IOP Publishing}
}


@article{kent2012unconditionally,
  title={Unconditionally secure bit commitment by transmitting measurement outcomes},
  author={Kent, Adrian},
  journal={Physical Review Letters},
  volume={109},
  number={13},
  pages={130501},
  year={2012},
  publisher={APS}
}

@article{lunghi2013experimental,
  title={Experimental bit commitment based on quantum communication and special relativity},
  author={Lunghi, Tommaso and Kaniewski, J and Bussieres, F{\'e}lix and Houlmann, Rapha{\"e}l and Tomamichel, M and Kent, A and Gisin, Nicolas and Wehner, S and Zbinden, Hugo},
  journal={Physical Review Letters},
  volume={111},
  number={18},
  pages={180504},
  year={2013},
  publisher={APS}
}
	
@article{kent2014secure,
  title={Secure and Robust Transmission and Verification of Unknown Quantum States in {M}inkowski Space},
  author={Kent, Adrian and Massar, Serge and Silman, Jonathan},
  journal={Scientific Reports},
  volume={4},
  pages={3901},
  year={2014},
  publisher={Nature Publishing Group}
}

@article{AS10,
	doi = {10.1088/1367-2630/12/3/033027},
	url = {https://doi.org/10.1088/1367-2630/12/3/033027},
	year = 2010,
	month = {mar},
	publisher = {{IOP} Publishing},
	volume = {12},
	number = {3},
	pages = {033027},
	author = {N Aharon and J Silman},
	title = {Quantum dice rolling: a multi-outcome generalization of quantum coin flipping},
	journal = {New J. Phys.},
	abstract = {The problem of quantum dice rolling (DR)—a generalization of the problem of quantum coin flipping (CF) to more than two outcomes and parties—is studied in both its weak and strong variants. We prove by construction that quantum mechanics allows for (i) weak N-sided DR admitting arbitrarily small bias for any N and (ii) two-party strong N-sided DR saturating Kitaev's bound for any N. To derive (ii) we also prove by construction that quantum mechanics allows for (iii) strong imbalanced CF saturating Kitaev's bound for any degree of imbalance. Furthermore, as a corollary of (ii) we introduce a family of optimal 2m-party strong nm-sided DR protocols for any pair m and n.}
}

@inproceedings{pedersen1991non,
  title={Non-interactive and information-theoretic secure verifiable secret sharing},
  author={Pedersen, Torben Pryds},
  booktitle={Annual International Cryptology Conference},
  pages={129--140},
  year={1991},
  organization={Springer}
}

@inproceedings{chailloux2017relativistic,
  title={Relativistic (or 2-Prover 1-Round) Zero-Knowledge Protocol for {NP} Secure Against Quantum Adversaries},
  author={Chailloux, Andr{\'e} and Leverrier, Anthony},
  booktitle={Annual International Conference on the Theory and Applications of Cryptographic Techniques},
  pages={369--396},
  year={2017},
  organization={Springer}
}

@article{kent2018unconstrained,
title={Unconstrained Summoning},
author={Kent, Adrian},
journal={Phys. Rev. A},
volume={98},
page={062332},
year={2018}}

@article{ZYWCCGH15,
  title = {Measurement-device-independent quantum coin tossing},
  author = {Zhao, Liangyuan and Yin, Zhenqiang and Wang, Shuang and Chen, Wei and Chen, Hua and Guo, Guangcan and Han, Zhengfu},
  journal = {Phys. Rev. A},
  volume = {92},
  issue = {6},
  pages = {062327},
  numpages = {7},
  year = {2015},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.92.062327},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.92.062327}
}


@inproceedings{chaum1983blind,
  title={Blind signatures for untraceable payments},
  author={Chaum, David},
  booktitle={Advances in cryptology},
  pages={199--203},
  year={1983},
  organization={Springer}
}


@inproceedings{GK15,
  title={New constructions for quantum money},
  author={Georgiou, Marios and Kerenidis, Iordanis},
  booktitle={LIPIcs-Leibniz International Proceedings in Informatics},
  volume={44},
  year={2015},
  organization={Schloss Dagstuhl-Leibniz-Zentrum fuer Informatik},
  doi = {10.4230/LIPIcs.TQC.2015.92},
  url = {https://drops.dagstuhl.de/opus/volltexte/2015/5551/}
}

@inproceedings{chaum1988untraceable,
  title={Untraceable electronic cash},
  author={Chaum, David and Fiat, Amos and Naor, Moni},
  booktitle={Conference on the Theory and Application of Cryptography},
  pages={319--327},
  year={1988},
  organization={Springer}
}

@inproceedings{kumar2017traceability,
  title={A traceability analysis of Monero�s blockchain},
  author={Kumar, Amrit and Fischer, Cl{\'e}ment and Tople, Shruti and Saxena, Prateek},
  booktitle={European Symposium on Research in Computer Security},
  pages={153--173},
  year={2017},
  organization={Springer}
}

@inproceedings{aaronson2009quantum,
  title={Quantum copy-protection and quantum money},
  author={Aaronson, Scott},
  booktitle={Computational Complexity, 2009. CCC'09. 24th Annual IEEE Conference on},
  pages={229--242},
  year={2009},
  organization={IEEE}
}

@article{mosca2010quantum,
  title={Quantum coins},
  author={Mosca, Michele and Stebila, Douglas},
  journal={Error-Correcting Codes, Finite Geometries and Cryptography},
  volume={523},
  pages={35--47},
  year={2010},
  publisher={American Mathematical Soc.}
}


@MISC{Kentfuturepositioncommitment, 
   author       = "Kent, Adrian",
title = "Future Position Commitment",
   howpublished = "{International Patent Application No. }WO2017001850A1.", 
   year         =  "2018"
}

@MISC{Kentmethodandsystem, 
   author       = "Kent, Adrian",
title = "Cryptographic method and system",
   howpublished = "{UK Patent Application No. }GB1719870.6.", 
}


@article{PGK18,
  title = {Practical and unconditionally secure spacetime-constrained oblivious transfer},
  author = {Pital\'ua-Garc\'{\i}a, Dami\'an and Kerenidis, Iordanis},
  journal = {Phys. Rev. A},
  volume = {98},
  issue = {3},
  pages = {032327},
  numpages = {9},
  year = {2018},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.98.032327},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.98.032327}
}

@article{PG19,
  title = {One-out-of-$m$ spacetime-constrained oblivious transfer},
  author = {Pital\'ua-Garc\'{\i}a, Dami\'an},
  journal = {Phys. Rev. A},
  volume = {100},
  issue = {1},
  pages = {012302},
  numpages = {20},
  year = {2019},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.100.012302},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.100.012302}
}

@Book{Mitzenmacherbook,
 author    = "M. Mitzenmacher and E. Upfal",
 title     = "Probability and Computing: Randomized Algorithms and Probabilistic Analysis",
 publisher = "Cambridge University Press",
address= "Cambridge, UK",
 year      =  2005,
}

@Book{LandauLifshitzbook,
 author    = "L. D. Landau and E. M. Lifshitz",
 title     = "THE CLASSICAL THEORY OF FIELDS",
 publisher = "PERGAMON PRESS",
address= "Oxford, UK",
 year      =  1971,
 note = {Translated from the Russian by
M. HAMERMESH, University of Minnesota},
}


@article{flexibletokens,
  title = {Flexible quantum tokens in spacetime},
  author = {Kent, Adrian and Pital\'ua-Garc\'{\i}a, Dami\'an},
  journal = {Phys. Rev. A},
  volume = {101},
  issue = {2},
  pages = {022309},
  numpages = {7},
  year = {2020},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.101.022309},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.101.022309}
}


@unpublished{KLPGR21,
  title = {Practical quantum tokens without quantum memories and experimental tests},
  author = {A. Kent and D. Lowndes and D. Pital\'ua-Garc\'ia and J. Rarity},
year={2021},
eprint = {2104.11717},
archivePrefix = {arXiv},
SLACcitation = {%%CITATION=arXiv:2104.11717;%%},
}









@article{BCDKPG21,
  title = {Multiphoton and Side{-}Channel Attacks in Mistrustful Quantum Cryptography},
  author = {Bozzio, Mathieu and Cavaill\`es, Adrien and Diamanti, Eleni and Kent, Adrian and Pital\'ua-Garc\'{\i}a, Dami\'an},
  journal = {PRX Quantum},
  volume = {2},
  issue = {3},
  pages = {030338},
  numpages = {54},
  year = {2021},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PRXQuantum.2.030338}
}



@misc{conversations,
note = {Conversations with experimental
  colleagues Mathieu Bozzio, Siddarth K. Joshi, and David
  Lowndes}
  }

@misc{conversations2,
note = {Conversations with experimental
  colleagues Siddarth K. Joshi, and David
  Lowndes}
  }


@article{B83,
author = {Blum, Manuel},
title = {Coin Flipping by Telephone a Protocol for Solving Impossible Problems},
year = {1983},
issue_date = {Winter-Spring 1983},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {15},
number = {1},
issn = {0163-5700},
url = {https://doi.org/10.1145/1008908.1008911},
doi = {10.1145/1008908.1008911},
abstract = {Alice and Bob want to flip a coin by telephone. (They have just divorced, live in different cities, want to decide who gets the car.) Bob would not like to tell Alice HEADS and hear Alice (at the other end of the line) say "Here goes . . . I'm flipping the coin. . . . You lost!"Coin-flipping in the SPECIAL way done here has a serious purpose. Indeed, it should prove an INDISPENSABLE TOOL of the protocol designer. Whenever a protocol requires one of two adversaries, say Alice, to pick a sequence of bits at random, and whenever it serves Alice's interests best NOT to pick her sequence of bits at random, then coin-flipping (Bob flipping coins to Alice) as defined here achieves the desired goal:1. It GUARANTEES to Bob that Alice will pick her sequence of bits at random. Her bit is 1 if Bob flips heads to her, O otherwise.2. It GUARANTEES to Alice that Bob will not know WHAT sequence of bits he flipped to her.Coin-flipping has already proved useful in solving a number of problems once thought impossible: mental poker, certified mail, and exchange of secrets. It will certainly prove a useful tool in solving other problems as well.},
journal = {SIGACT News},
month = jan,
pages = {23–27},
numpages = {5}
}

@InProceedings{C88,
author="Cr{\'e}peau, Claude",
editor="Pomerance, Carl",
title="Equivalence Between Two Flavours of Oblivious Transfers",
booktitle="Advances in Cryptology --- CRYPTO '87",
year="1988",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="350--354",
abstract="The concept of oblivious transfer (O.T.) that was induced by Halpern and Rabin m] turned out to be a very useful tool in designing cryptographic protocols. The related notion of ``one-out-of-two oblivious transfer'' was proposed by Even, Goldreich and Lempel in [EGL] together with some applications. Some more applications of this protocol can be found in recent papers [BCR], [GMWj. So far, the two notions where believed to be closely related but not known to be equivalent. This paper presents a proof that these two notions are computationally equivalent.",
isbn="978-3-540-48184-3"
}




@article{ASMMDWA20,
  title = {Imperfect 1-Out-of-2 Quantum Oblivious Transfer: Bounds, a Protocol, and its Experimental Implementation},
  author = {Amiri, Ryan and St\'arek, Robert and Reichmuth, David and Puthoor, Ittoop V. and Mi\ifmmode \check{c}\else \v{c}\fi{}uda, Michal and Mi\ifmmode \check{s}\else \v{s}\fi{}ta, Jr., Ladislav and Du\ifmmode \check{s}\else \v{s}\fi{}ek, Miloslav and Wallden, Petros and Andersson, Erika},
  journal = {PRX Quantum},
  volume = {2},
  issue = {1},
  pages = {010335},
  numpages = {21},
  year = {2021},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PRXQuantum.2.010335},
  url = {https://link.aps.org/doi/10.1103/PRXQuantum.2.010335}
}







@article {LC99,
	author = {Lo, Hoi-Kwong and Chau, H. F.},
	title = {Unconditional Security of Quantum Key Distribution over Arbitrarily Long Distances},
	volume = {283},
	number = {5410},
	pages = {2050--2056},
	year = {1999},
	doi = {10.1126/science.283.5410.2050},
	publisher = {American Association for the Advancement of Science},
	abstract = {Quantum key distribution is widely thought to offer unconditional security in communication between two users. Unfortunately, a widely accepted proof of its security in the presence of source, device, and channel noises has been missing. This long-standing problem is solved here by showing that, given fault-tolerant quantum computers, quantum key distribution over an arbitrarily long distance of a realistic noisy channel can be made unconditionally secure. The proof is reduced from a noisy quantum scheme to a noiseless quantum scheme and then from a noiseless quantum scheme to a noiseless classical scheme, which can then be tackled by classical probability theory.},
	issn = {0036-8075},
	URL = {https://science.sciencemag.org/content/283/5410/2050},
	journal = {Science}
}

@article{DGHMR06,
	doi = {10.1088/1367-2630/8/10/249},
	url = {https://doi.org/10.1088/1367-2630/8/10/249},
	year = 2006,
	month = {oct},
	publisher = {{IOP} Publishing},
	volume = {8},
	number = {10},
	pages = {249--249},
	author = {J L Duligall and M S Godfrey and K A Harrison and W J Munro and J G Rarity},
	title = {Low cost and compact quantum key distribution},
	journal = {New J. Phys.},
	abstract = {We present the design of a novel free-space quantum cryptography system, complete with purpose-built software, that can operate in daylight conditions. The transmitter and receiver modules are built using inexpensive off-the-shelf components. Both modules are compact allowing the generation of renewed shared secrets on demand over a short range of a few metres. An analysis of the software is shown as well as results of error rates and therefore shared secret yields at varying background light levels. As the system is designed to eventually work in short-range consumer applications, we also present a use scenario where the consumer can regularly ‘top up’ a store of secrets for use in a variety of one-time-pad (OTP) and authentication protocols.}
}





@article{KPG20,
  title = {Flexible quantum tokens in spacetime},
  author = {Kent, Adrian and Pital\'ua-Garc\'{\i}a, Dami\'an},
  journal = {Phys. Rev. A},
  volume = {101},
  issue = {2},
  pages = {022309},
  numpages = {7},
  year = {2020},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.101.022309},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.101.022309}
}


@article{ACGKM16,
author = {D. Aharonov and A. Chailloux and M. Ganz and I. Kerenidis and
L. Magnin},
title = {A Simpler Proof of the Existence of Quantum Weak Coin Flipping with Arbitrarily Small Bias},
journal = {SIAM J. Comput.},
year = {2016},
volume= {45},
pages= {633--679},
url = {https://doi.org/10.1137/14096387X}
}

@article{BCKD20,
  title = {Quantum weak coin flipping with a single photon},
  author = {Bozzio, Mathieu and Chabaud, Ulysse and Kerenidis, Iordanis and Diamanti, Eleni},
  journal = {Phys. Rev. A},
  volume = {102},
  issue = {2},
  pages = {022414},
  numpages = {15},
  year = {2020},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.102.022414},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.102.022414}
}

@article{HS20,
	doi = {10.1088/1367-2630/ab6872},
	url = {https://doi.org/10.1088/1367-2630/ab6872},
	year = 2020,
	month = {feb},
	publisher = {{IOP} Publishing},
	volume = {22},
	number = {2},
	pages = {023007},
	author = {Karol Horodecki and Maciej Stankiewicz},
	title = {Semi-device-independent quantum money},
	journal = {New J. Phys.},
	abstract = {The seminal idea of quantum money, not forgeable due to laws of Quantum Mechanics, proposed by Stephen Wiesner, has laid the foundations for the Quantum Information Theory in the early ’70s. Recently, several other schemes for quantum currencies have been proposed, all, however, relying on the assumption that the quantum source device, acts according to its specification. This makes several known quantum money protocols vulnerable to the so-called hardware Trojan horse attacks. We, therefore, study the following problem: to what extent quantum money schemes can be made independent from the inner working of source and verification-devices used by the honest parties (bank and mint) in creating and processing the quantum money? Drawing inspirations from the semi-device-independent quantum key distribution protocol, we introduce the first scheme of quantum money with this assumption partially relaxed, along with the proof of its unforgeability. Finally, we formulate and discuss a quantum analog of the Oresme–Copernicus–Gresham’s law of economy, that may hold in the future.}
}

@article{AA17,
  title = {Quantum money with nearly optimal error tolerance},
  author = {Amiri, Ryan and Arrazola, Juan Miguel},
  journal = {Phys. Rev. A},
  volume = {95},
  issue = {6},
  pages = {062334},
  numpages = {12},
  year = {2017},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.95.062334},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.95.062334}
}


@article{BDG19,
  title = {Semi-device-independent quantum money with coherent states},
  author = {Bozzio, Mathieu and Diamanti, Eleni and Grosshans, Fr\'ed\'eric},
  journal = {Phys. Rev. A},
  volume = {99},
  issue = {2},
  pages = {022336},
  numpages = {9},
  year = {2019},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.99.022336},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.99.022336}
}


@Article{K19,
AUTHOR = {Kumar, Niraj},
TITLE = {Practically Feasible Robust Quantum Money with Classical Verification},
JOURNAL = {Cryptography},
VOLUME = {3},
YEAR = {2019},
NUMBER = {4},
PAGES = {26},
URL = {https://www.mdpi.com/2410-387X/3/4/26},
ISSN = {2410-387X},
ABSTRACT = {We introduce a private quantum money scheme with the note verification procedure based on sampling matching, a problem in a one-way communication complexity model. Our scheme involves a bank who produces and distributes quantum notes, noteholders who are untrusted, and trusted local verifiers of the bank to whom the holders send their notes in order to carry out transactions. The key aspects of our money scheme include: note verification procedure requiring a single round classical interaction between the local verifier and bank; fixed verification circuit that uses only passive linear optical components; re-usability of each note in our scheme which grows linearly with the size of note; and an unconditional security against any adversary trying to forge the banknote while tolerating the noise of up to 21.4%. We further describe a practical implementation technique of our money scheme using weak coherent states of light and the verification circuit involving a single 50/50 beam splitter and two single-photon threshold detectors. Previous best-known matching based money scheme proposal involves a verification circuit where the number of optical components increase proportional to the increase in desired noise tolerance (robustness). In contrast, we achieve any desired noise tolerance (up to a maximal threshold value) with only a fixed number of optical components. This considerable reduction of components in our scheme enables us to reach the robustness values that is not feasible for any existing money scheme with the current technology.},
DOI = {10.3390/cryptography3040026}
}






@article{WLZSZLDYZ19,
  title = {Efficient quantum memory for single-photon polarization qubits},
  author = {Y. Wang and J. Li and S. Zhang and K. Su and Y. Zhou and K. Liao and S. Du and H. Yan and S.-L. Zhu},
  journal = {Nat. Photon.},
  volume = {13},
  pages = {346--351},
  year = {2019},
  doi = {10.1038/s41566-019-0368-8},
  url = {https://doi.org/10.1038/s41566-019-0368-8}
}

@article{WMHSG20,
  title = {A quantum memory at telecom wavelengths},
  author = {A. Wallucks and I. Marinkovi\'{c} and B. Hensen and R. Stockill and S. Gr\"{o}blacher},
  journal = {Nat. Phys.},
  volume = {16},
  pages = {772--777},
  year = {2020},
  doi = {10.1038/s41567-020-0891-z},
  url = {https://doi.org/10.1038/s41567-020-0891-z}
}

@article{BBP17,
  title = {Experimental realization of quantum cheque using a five{-}qubit quantum computer},
  author = {B. K. Behera and A. Banerjee and P. K. Panigrahi},
  journal = {Quantum Inf. Process.},
  volume = {16},
  pages = {312},
  year = {2017},
  doi = {10.1007/s11128-017-1762-0},
  url = {https://doi.org/10.1007/s11128-017-1762-0}
}

@article{WUZALZDYK17,
  title = {Single{-}qubit quantum memory exceeding ten{-}minute coherence time},
  author = {Y. Wang and M. Um and J. Zhang and S. An and M. Lyu and J.-N. Zhang and L.-M. Duan and D. Yum and K. Kim},
  journal = {Nat. Photon.},
  volume = {11},
  pages = {646--650},
  year = {2017},
  doi = {10.1038/s41566-017-0007-1},
  url = {https://doi.org/10.1038/s41566-017-0007-1}
}


@article{WLQUZWYGZK21,
author = "P. Wang and C.-Y. Luan and M. Qiao and M. Um and J. Zhang and Y. Wang and X. Yuan and M. Gu and J. Zhang and K. Kim",
title= "Single ion qubit with estimated coherence time exceeding one hour",
year = "2021",
journal = "Nat. Commun.",
volume = "12",
pages = "233",
doi = "10.1038/s41467-020-20330-w",
}




@unpublished{YangLiu,
author="Y. Liu and Q. Zhang",
note="private communication",
}

@unpublished{Bussieres,
author="F. Bussi\`{e}res",
note="private communication",
}




%QUANTUM GRAVITY

@article{CST19,
	doi = {10.1088/1361-6382/aaf9ca},
	url = {https://doi.org/10.1088%2F1361-6382%2Faaf9ca},
	year = 2019,
	month = {jan},
	publisher = {{IOP} Publishing},
	volume = {36},
	number = {3},
	pages = {034001},
	author = {Daniel Carney and Philip C E Stamp and Jacob M Taylor},
	title = {Tabletop experiments for quantum gravity: a user's manual},
	journal = {Class. Quantum Grav.},
	abstract = {Recent advances in cooling, control, and measurement of mechanical systems in the quantum regime have opened the possibility of the first direct observation of quantum gravity, at scales achievable in experiments. This paper gives a broad overview of this idea, using some matter-wave and optomechanical systems to illustrate the predictions of a variety of models of low-energy quantum gravity. We first review the treatment of perturbatively quantized general relativity as an effective quantum field theory, and consider the particular challenges of observing quantum effects in this framework. We then move on to a variety of alternative models, such as those in which gravity is classical, emergent, or responsible for a breakdown of quantum mechanics.}
}

@article{K21.2,
  title = {Quantum state readout, collapses, probes, and signals},
  author = {Kent, Adrian},
  journal = {Phys. Rev. D},
  volume = {103},
  issue = {6},
  pages = {064061},
  numpages = {8},
  year = {2021},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.103.064061},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.103.064061}
}


@article{K21,
  title = {Testing quantum gravity near measurement events},
  author = {Kent, Adrian},
  journal = {Phys. Rev. D},
  volume = {103},
  issue = {6},
  pages = {064038},
  numpages = {6},
  year = {2021},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.103.064038},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.103.064038}
}


@article{TD16,
  title = {Sourcing semiclassical gravity from spontaneously localized quantum matter},
  author = {Tilloy, Antoine and Di\'osi, Lajos},
  journal = {Phys. Rev. D},
  volume = {93},
  issue = {2},
  pages = {024026},
  numpages = {12},
  year = {2016},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.93.024026},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.93.024026}
}


@article{C08,
	doi = {10.1088/0264-9381/25/15/154010},
	url = {https://doi.org/10.1088%2F0264-9381%2F25%2F15%2F154010},
	year = 2008,
	month = {jul},
	publisher = {{IOP} Publishing},
	volume = {25},
	number = {15},
	pages = {154010},
	author = {S Carlip},
	title = {Is quantum gravity necessary?},
	journal = {Class. Quantum Grav.},
	abstract = {In view of the enormous difficulties we seem to face in quantizing general relativity, we should perhaps consider the possibility that gravity is a fundamentally classical interaction. Theoretical arguments against such mixed classical–quantum models are strong, but not conclusive, and the question is ultimately one for experiment. I review some work in progress on the possibility of experimental tests, exploiting the nonlinearity of the classical–quantum coupling, which could help settle this question.}
}

@article{R63,
title = {On quantization of fields},
journal = {Nucl. Phys.},
volume = {40},
pages = {353-356},
year = {1963},
issn = {0029-5582},
doi = {10.1016/0029-5582(63)90279-7},
author = {L. Rosenfeld},
abstract = {Critical remarks on some formal and physical aspects of field quantization, with special application to the case of gravitation.}
}

@article{K78,
  title={Relativistic models of nonlinear quantum mechanics},
  author={Kibble, TWB},
  journal={Commun. Math. Phys.},
  volume={64},
  number={1},
  pages={73--82},
  year={1978},
doi={10.1007/BF01940762},
  publisher={Springer}
}

@article{KR80,
	doi = {10.1088/0305-4470/13/1/015},
	url = {https://doi.org/10.1088/0305-4470/13/1/015},
	year = 1980,
	month = {jan},
	publisher = {{IOP} Publishing},
	volume = {13},
	number = {1},
	pages = {141--148},
	author = {T W B Kibble and S Randjbar{-D}aemi},
	title = {Non-linear coupling of quantum theory and classical gravity},
	journal = {J. Phys. A: Math. Gen.},
	abstract = {Discusses the possibility that the non-linear evolution proposed earlier for a relativistic quantum field theory may be related to its coupling to a classical gravitational field. Formally, in the Schrodinger picture, it is shown how both the Schrodinger equation and Einstein's equations (with the expectation value of the energy-momentum tensor on the right) can be derived from a variational principle. This yields a non-linear quantum evolution. Other terms can be added to the action integral to incorporate explicit nonlinearities of the type discussed previously. The authors discuss briefly the possibility of giving a meaning to the resulting equation in a Heisenberg or interaction-like picture.}
}

@article{PG81,
  title = {Indirect Evidence for Quantum Gravity},
  author = {Page, Don N. and Geilker, C. D.},
  journal = {Phys. Rev. Lett.},
  volume = {47},
  issue = {14},
  pages = {979--982},
  numpages = {0},
  year = {1981},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.47.979},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.47.979}
}


@article{C01,
	doi = {10.1088/0034-4885/64/8/301},
	url = {https://doi.org/10.1088/0034-4885/64/8/301},
	year = 2001,
	month = {jul},
	publisher = {{IOP} Publishing},
	volume = {64},
	number = {8},
	pages = {885--942},
	author = {S Carlip},
	title = {Quantum gravity: a progress report},
	journal = {Rep. Prog. Phys},
	abstract = {The problem of reconciling general relativity and quantum theory has fascinated and bedeviled physicists for more than 70 years. Despite recent progress in string theory and loop quantum gravity, a complete solution remains out of reach. I review the status of the continuing effort to quantize gravity, emphasizing the underlying conceptual issues and the various attempts to come to grips with them.}
}

@article{M62,
  title={Les th{\'e}ories relativistes de la gravitation},
  author={M{\o}ller, Christian and others},
  journal={Colloques Internationaux CNRS},
  volume={91},
  number={1},
  year={1962},
  publisher={CNRS Paris}
}

@article{BUGLTCPW20,
  title={A strong no-go theorem on the {W}igner’s friend paradox},
  author={Bong, Kok-Wei and Utreras-Alarc{\'o}n, An{\'\i}bal and Ghafari, Farzad and Liang, Yeong-Cherng and Tischler, Nora and Cavalcanti, Eric G and Pryde, Geoff J and Wiseman, Howard M},
  journal={Nat. Phys.},
  volume={16},
  number={12},
  pages={1199--1205},
  year={2020},
doi={10.1038/s41567-020-0990-x},
  publisher={Nature Publishing Group}
}

@article{DPCDLB21,
  title={Underground test of gravity-related wave function collapse},
  author={Donadi, Sandro and Piscicchia, Kristian and Curceanu, Catalina and Di{\'o}si, Lajos and Laubenstein, Matthias and Bassi, Angelo},
  journal={Nat. Phys.},
  volume={17},
  number={1},
  pages={74--78},
  year={2021},
  publisher={Nature Publishing Group},
doi={10.1038/s41567-020-1008-4}
}

@article{P98,
  title={Quantum computation, entanglement and state reduction},
  author={Penrose, Roger},
  journal={Phil. Trans. R. Soc. A.},
  volume={356},
  number={1743},
  pages={1927--1939},
  year={1998},
  publisher={The Royal Society},
doi={10.1098/rsta.1998.0256}
}

@article{D84,
  title={Gravitation and quantum-mechanical localization of macro{-}objects},
  author={Di{\'o}si, L},
  journal={Phys. Lett. A},
  volume={105},
  number={4-5},
  pages={199--202},
  year={1984},
doi={10.1016/0375-9601(84)90397-9}
}

@article{GCB19,
	doi = {10.1038/s41467-018-08155-0},
	url = {https://doi.org/10.1038/s41467-018-08155-0},
	year = 2019,
	volume = {10},
	pages = {494},
	author = {F. Giacomini and E. Castro{-}Ruiz and {\v{C}}. Brukner},
	title = {Quantum mechanics and the covariance of physical laws in quantum reference frames},
	journal = {Nature Communications},
}

@article{WY03,
  title = {Quantum Key Distribution with High Loss: Toward Global Secure Communication},
  author = {Hwang, Won-Young},
  journal = {Phys. Rev. Lett.},
  volume = {91},
  issue = {5},
  pages = {057901},
  numpages = {4},
  year = {2003},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.91.057901},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.91.057901}
}

@article{WCSL10,
  title = {Implementation of two-party protocols in the noisy-storage model},
  author = {Wehner, Stephanie and Curty, Marcos and Schaffner, Christian and Lo, Hoi-Kwong},
  journal = {Phys. Rev. A},
  volume = {81},
  issue = {5},
  pages = {052336},
  numpages = {26},
  year = {2010},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.81.052336},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.81.052336}
}



@article{HIGM95,
  title = {Quantum cryptography with coherent states},
  author = {Huttner, B. and Imoto, N. and Gisin, N. and Mor, T.},
  journal = {Phys. Rev. A},
  volume = {51},
  issue = {3},
  pages = {1863--1869},
  numpages = {0},
  year = {1995},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.51.1863},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.51.1863}
}


@article{LLRZBLBZCFZP21,
	doi = {10.1038/s41567-020-01147-2},
		year = {2021},
	volume = {17},
	pages = {448–451},
	author = {W.-Z. Liu and M.-H. Li and S. Ragy and S.-R. Zhao and B. Bai and Y. Liu and P. J. Brown and J. Zhang and R. Colbeck and J. Fan and Q. Zhang  and J.-W. Pan },
	title = {Device{-}independent randomness expansion against quantum side information},
	journal = {Nature Phys.},
}

@article{VPR19,
	doi = {10.1088/1367-2630/ab0e3b},
		year = {2019},
	volume = {21},
	pages = {043057},
	author = {V. Vilasini and C. Portmann and L. del Rio},
	title = {Composable security in relativistic quantum cryptography},
	journal = {New J. Phys.},
}



@unpublished{PR21,
  title = {Security in Quantum Cryptography},
  author = {C. Portmann and R. Renner},
year={2021},
eprint = {2102.00021},
archivePrefix = {arXiv},
SLACcitation = {%%CITATION=arXiv:1308.5009;%%},
}

@article{G49,
  title = {An Example of a New Type of Cosmological Solutions of {E}instein's Field Equations of Gravitation},
  author = {G\"odel, Kurt},
  journal = {Rev. Mod. Phys.},
  volume = {21},
  issue = {3},
  pages = {447--450},
  numpages = {0},
  year = {1949},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.21.447},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.21.447}
}

@article{H19,
title = {A systematic approach to generalisations of {G}eneral {R}elativity and their cosmological implications},
journal = {Phys. Rep.},
volume = {796},
pages = {1-113},
year = {2019},
issn = {0370-1573},
doi = {https://doi.org/10.1016/j.physrep.2018.11.006},
url = {https://www.sciencedirect.com/science/article/pii/S0370157318303569},
author = {Lavinia Heisenberg},
keywords = {Modified gravity, Massive gravity, Scalar–tensor theories, Generalised Proca, Multi-Proca, Scalar–vector–tensor theories, Cosmology},
abstract = {A century ago, Einstein formulated his elegant and elaborate theory of General Relativity, which has so far withstood a multitude of empirical tests with remarkable success. Notwithstanding the triumphs of Einstein’s theory, the tenacious challenges of modern cosmology and of particle physics have motivated the exploration of further generalised theories of space–time. Even though Einstein’s interpretation of gravity in terms of the curvature of space–time is commonly adopted, the assignment of geometrical concepts to gravity is ambiguous because General Relativity allows three entirely different, but equivalent approaches of which Einstein’s interpretation is only one. From a field-theoretical perspective, however, the construction of a consistent theory for a Lorentz-invariant massless spin-2 particle uniquely leads to General Relativity. Keeping Lorentz invariance then implies that any modification of General Relativity will inevitably introduce additional propagating degrees of freedom into the gravity sector. Adopting this perspective, we will review the recent progress in constructing consistent field theories of gravity based on additional scalar, vector and tensor fields. Within this conceptual framework, we will discuss theories with Galileons, with Lagrange densities as constructed by Horndeski and beyond, extended to DHOST interactions, or containing generalised Proca fields and extensions thereof, or several Proca fields, as well as bigravity theories and scalar–vector–tensor theories. We will review the motivation of their inception, different formulations, and essential results obtained within these classes of theories together with their empirical viability.}
}






@incollection{EPS72,
  author      = "J. Ehlers and F. A. E. Pirani and A. Schild",
  title       = "The geometry of free fall and light propagation",
  editor      = "J. L. O{’}Reifeartaigh",
  booktitle   = "General Relativity, papers in honour of J. L. Synge",
  publisher   = "Clarendon Press",
  address     = "Oxford",
  year        = "1972",
  pages       = "63-84",
  note = "Republished in \cite{EPS72rep}"
}

@article{EPS72rep,
	doi = {10.1007/s10714-012-1353-4},
		year = {2012},
	volume = {44},
	pages = {1587--1609},
	author = {J. Ehlers and F. A. E. Pirani and A. Schild},
	title = {Republication of{:} {T}he geometry of free fall and light propagation},
	journal = {Gen. Relativ. Gravit.},
}

@article{S00,
	doi = {10.1023/A:1003797204134},
		year = {2000},
	volume = {30},
	pages = {1819--1847},
	author = {George Svetlichny },
	title = {The Space-Time Origin of Quantum Mechanics: Covering Law},
	journal = {Found. Phys.},
}

@article{MBPZTBP18,
  title={A coherent spin--photon interface in silicon},
  author={Mi, Xiao and Benito, M{\'o}nica and Putz, Stefan and Zajac, David M and Taylor, Jacob M and Burkard, Guido and Petta, Jason R},
  journal={Nature},
  volume={555},
  number={7698},
  pages={599--603},
  year={2018},
  publisher={Nature Publishing Group},
doi={10.1038/nature25769}
}

@article {SZKBSMBSV18,
	author = {Samkharadze, N. and Zheng, G. and Kalhor, N. and Brousse, D. and Sammak, A. and Mendes, U. C. and Blais, A. and Scappucci, G. and Vandersypen, L. M. K.},
	title = {Strong spin{-}photon coupling in silicon},
	volume = {359},
	number = {6380},
	pages = {1123--1127},
	year = {2018},
	doi = {10.1126/science.aar4054},
	publisher = {American Association for the Advancement of Science},
	abstract = {To help develop quantum circuits, much effort has been directed toward achieving the strong-coupling regime by using gate-defined semiconductor quantum dots. Potentially, the magnetic dipole, or spin, of a single electron for use as a qubit has advantages over charge-photon coupling owing to its longer lifetime. Samkharadze et al. hybridized the electron spin with the electron charge in a double silicon quantum dot. This approach yielded strong coupling between the single electron spin and a single microwave photon, providing a route to scalable quantum circuits with spin qubits.Science, this issue p. 1123Long coherence times of single spins in silicon quantum dots make these systems highly attractive for quantum computation, but how to scale up spin qubit systems remains an open question. As a first step to address this issue, we demonstrate the strong coupling of a single electron spin and a single microwave photon. The electron spin is trapped in a silicon double quantum dot, and the microwave photon is stored in an on-chip high-impedance superconducting resonator. The electric field component of the cavity photon couples directly to the charge dipole of the electron in the double dot, and indirectly to the electron spin, through a strong local magnetic field gradient from a nearby micromagnet. Our results provide a route to realizing large networks of quantum dot{\textendash}based spin qubit registers.},
	issn = {0036-8075},
	journal = {Science}
}

@article{KMBM20,
  title = {Quantum gravity witness via entanglement of masses: Casimir screening},
  author = {van de Kamp, Thomas W. and Marshman, Ryan J. and Bose, Sougato and Mazumdar, Anupam},
  journal = {Phys. Rev. A},
  volume = {102},
  issue = {6},
  pages = {062807},
  numpages = {12},
  year = {2020},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.102.062807},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.102.062807}
}

@article{CMT21,
  title = {Using an Atom Interferometer to Infer Gravitational Entanglement Generation},
  author = {Carney, Daniel and M\"uller, Holger and Taylor, Jacob M.},
  journal = {PRX Quantum},
  volume = {2},
  issue = {3},
  pages = {030330},
  numpages = {16},
  year = {2021},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PRXQuantum.2.030330},
  url = {https://link.aps.org/doi/10.1103/PRXQuantum.2.030330}
}

@article{HR18,
	doi = {10.1088/1751-8121/aaa734},
	url = {https://doi.org/10.1088/1751-8121/aaa734},
	year = 2018,
	month = {jan},
	publisher = {{IOP} Publishing},
	volume = {51},
	number = {8},
	pages = {085303},
	author = {Michael J W Hall and Marcel Reginatto},
	title = {On two recent proposals for witnessing nonclassical gravity},
	journal = {J. Phys. A: Math. Theor.},
	abstract = {Two very similar proposals have been made recently for witnessing nonclassical features of gravity, by Bose et al and by Marletto and Vedral. However, while these proposals are asserted to be very general, they are in fact based on a very strong claim: that quantum systems cannot become entangled via a classical intermediary. We point out that the support provided for this claim is only applicable to a very limited class of quantum-classical interaction models, corresponding to Koopman-type dynamics. We show that the claim is also valid for mean-field models, but that it is contradicted by explicit counterexamples based on the configuration-ensemble model. Thus, neither proposal provides a definitive test of nonclassical gravity.}
}


@article{HVNCRI21,
  title = {Non{-}Gaussianity as a Signature of a Quantum Theory of Gravity},
  author = {Howl, Richard and Vedral, Vlatko and Naik, Devang and Christodoulou, Marios and Rovelli, Carlo and Iyer, Aditya},
  journal = {PRX Quantum},
  volume = {2},
  issue = {1},
  pages = {010325},
  numpages = {32},
  year = {2021},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PRXQuantum.2.010325},
  url = {https://link.aps.org/doi/10.1103/PRXQuantum.2.010325}
}


@article{K06,
author = {Kiefer, C.},
title = {Quantum gravity: general introduction and recent developments},
journal = {Ann. Phys.},
volume = {15},
number = {1-2},
pages = {129-148},
keywords = {Quantum gravity, quantum cosmology, loop quantum gravity, quantum geometrodynamics, string theory},
doi = {https://doi.org/10.1002/andp.200510175},
abstract = {Abstract I briefly review the current status of quantum gravity. After giving some general motivations for the need of such a theory, I discuss the main approaches in quantizing general relativity: Covariant approaches (perturbation theory, effective theory, and path integrals) and canonical approaches (quantum geometrodynamics, loop quantum gravity). I then address quantum gravitational aspects of string theory. This is followed by a discussion of black holes and quantum cosmology. I end with some remarks on the observational status of quantum gravity.},
year = {2006}
}


@book{Oritibook,
place={Cambridge},
Editor={D. Oriti},
title={Approaches to Quantum Gravity: Toward a New Understanding of Space, Time and Matter},
DOI={10.1017/CBO9780511575549},
publisher={Cambridge University Press},
year={2009}}

@article{ANVKVGZ99,
  title={Wave--particle duality of {C}$_{60}$ molecules},
  author={Arndt, Markus and Nairz, Olaf and Vos-Andreae, Julian and Keller, Claudia and Van der Zouw, Gerbrand and Zeilinger, Anton},
  journal={Nature},
  volume={401},
  number={6754},
  pages={680--682},
  year={1999},
doi={10.1038/44348},
  publisher={Nature Publishing Group}
}

@article{HGHNA12,
  title = {Colloquium: Quantum interference of clusters and molecules},
  author = {Hornberger, Klaus and Gerlich, Stefan and Haslinger, Philipp and Nimmrichter, Stefan and Arndt, Markus},
  journal = {Rev. Mod. Phys.},
  volume = {84},
  issue = {1},
  pages = {157--173},
  numpages = {0},
  year = {2012},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.84.157},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.84.157}
}


@article{CSP09,
  title = {Optics and interferometry with atoms and molecules},
  author = {Cronin, Alexander D. and Schmiedmayer, J\"org and Pritchard, David E.},
  journal = {Rev. Mod. Phys.},
  volume = {81},
  issue = {3},
  pages = {1051--1129},
  numpages = {0},
  year = {2009},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.81.1051},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.81.1051}
}

@article{AH14,
  title={Testing the limits of quantum mechanical superpositions},
  author={Arndt, Markus and Hornberger, Klaus},
  journal={Nat. Phys.},
  volume={10},
  number={4},
  pages={271--277},
  year={2014},
doi={10.1038/nphys2863},
  publisher={Nature Publishing Group}
}

@article{EGAMT13,
  title={Matter--wave interference of particles selected from a molecular library with masses exceeding 10000 amu},
  author={Eibenberger, Sandra and Gerlich, Stefan and Arndt, Markus and Mayor, Marcel and T{\"u}xen, Jens},
  journal={ Phys. Chem. Chem. Phys.},
  volume={15},
  number={35},
  pages={14696--14700},
  year={2013},
doi={10.1039/C3CP51500A },
  publisher={Royal Society of Chemistry}
}

@article{FGZKPMGA19,
  title={Quantum superposition of molecules beyond 25 kDa},
  author={Fein, Yaakov Y and Geyer, Philipp and Zwick, Patrick and Kia{\l}ka, Filip and Pedalino, Sebastian and Mayor, Marcel and Gerlich, Stefan and Arndt, Markus},
  journal={Nat. Phys.},
  volume={15},
  number={12},
  pages={1242--1245},
  year={2019},
doi={10.1038/s41567-019-0663-9},
  publisher={Nature Publishing Group}
}

@article{GBCDBKPU21,
  title={Testing the foundation of quantum physics in space via Interferometric and non-interferometric experiments with mesoscopic nanoparticles},
  author={Gasbarri, Giulio and Belenchia, Alessio and Carlesso, Matteo and Donadi, Sandro and Bassi, Angelo and Kaltenbaek, Rainer and Paternostro, Mauro and Ulbricht, Hendrik},
  journal={Commun. Phys.},
  volume={4},
  number={1},
  pages={1--13},
  year={2021},
doi={10.1038/s42005-021-00656-7},
url={https://www.nature.com/articles/s42005-021-00656-7},
  publisher={Nature Publishing Group}
}

@article{F67,
  title = {Possibility of Faster{-}Than{-}Light Particles},
  author = {Feinberg, G.},
  journal = {Phys. Rev.},
  volume = {159},
  issue = {5},
  pages = {1089--1105},
  numpages = {0},
  year = {1967},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.159.1089},
  url = {https://link.aps.org/doi/10.1103/PhysRev.159.1089}
}



@article{MS13,
author = {Maldacena, J. and Susskind, L.},
title = {Cool horizons for entangled black holes},
journal = {Fortschr. Phys.},
volume = {61},
number = {9},
pages = {781-811},
doi = {https://doi.org/10.1002/prop.201300020},
abstract = {Abstract General relativity contains solutions in which two distant black holes are connected through the interior via a wormhole, or Einstein-Rosen bridge. These solutions can be interpreted as maximally entangled states of two black holes that form a complex EPR pair. We suggest that similar bridges might be present for more general entangled states. In the case of entangled black holes one can formulate versions of the AMPS(S) paradoxes and resolve them. This suggests possible resolutions of the firewall paradoxes for more general situations.},
year = {2013}
}




@unpublished{H05,
  title = {Probability theories with dynamic causal structure: a new framework for quantum gravity},
  author = {Hardy, Lucien},
year={2005},
eprint = {gr-qc/0509120},
archivePrefix = {arXiv},
SLACcitation = {%%CITATION=arXiv:1308.5009;%%},
}
